Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models

How to explore efficiently is a central problem in multi-armed bandits. In this paper, we introduce the metadata-based multi-task bandit problem, where the agent needs to solve a large number of related multi-armed bandit tasks and can leverage some task-specific features (i.e., metadata) to share knowledge across tasks. As a general framework, we propose to capture task relations through the lens of Bayesian hierarchical models, upon which a Thompson sampling algorithm is designed to efficiently learn task relations, share information, and minimize the cumulative regrets. Two concrete examples for Gaussian bandits and Bernoulli bandits are carefully analyzed. The Bayes regret for Gaussian bandits clearly demonstrates the benefits of information sharing with our algorithm. The proposed method is further supported by extensive experiments.

==> ARCHIVE/Archive_related_work.tex <==

Susan's intelligent polling \cite{tomkins2019intelligent}: 
    the cloest work. They also consider pooling information over $N$ (contextual) bandit tasks (patients), but use a mixed effect model and did not consider the similarity capture by $\vxi$. 
    Let the content of the $t$-th interaction of the $i$-th task be $\vc_{t,i}$:
    \begin{equation*}
        \begin{split}
            \vthe_i &= \vthe + \mu_i \\
            R_{t,i} &= \vthe_i^T \vc_{t, i} + \epsilon_{t,i} 
        \end{split}
    \end{equation*}


==> ARCHIVE/Real_Data.tex <==
\subsection{Real data}
% calibrated from a multi-task supervised learning task?
Due to the absence of open dataset containing  logged feedbacks from multiple MAB tasks, following the literature\citep{cella2020meta, gentile2014online, metapricing}, 
we convert a logged contextual bandit dataset for our experiment purpose. 

\begin{itemize}
    \item Each user is a task
    \item Clustering the news/movies to create several arms 
\end{itemize}


% \textbf{Setting.}
% We need to find a dataset on MAB problems with many tasks and some task-specific features (or CMAB whose context can also be used as feature, due to repeated nature). 
% continuous reward (not binary)

% For example, many products with static features and some binary decisions need to be made
% Ideally, we should have a logged bandit-feedback dataset of similar MAB tasks (experiments), without context, with discrete actions and continuous rewards. 
% The motivating example is where we have many products with their static features and we need to make some binary decision for each of them. 
% If no such a dataset is available, I am thinking of using snthetic dataset to study the asymptotic with both N and T, and use the Warfarin dataset to study large N small T (with small noise variance, T = 20 may be enough, as in the RI example; besides, Since the main improvement comes from information sharing among tasks, large N samll T is beneficial to us) 


==> ARCHIVE/dicussions_IP.tex <==
\subsection{Comparison with \citet{tomkins2019intelligent}}
Treat $ia$ as $i$, we can find that \citet{tomkins2019intelligent} can be understood as a random slope (random coefficient) model, while our model is a random intercept model. 
We may even consider the random intercept and slope model. 
However, their use cases are different. 
Besides, when the second term is generalized to nonlinear, the random coefficient model is difficult to formularize. 


\begin{align*}
    y_{ij} &= \alpha + \vx_{ij}^T\beta_i + \epsilon_{ij}\\
    y_{ij} &= \alpha_i + \vx_i^T\beta + \epsilon_{ij}\\
    y_{ij} &= \alpha_i + \vx_{ij}^T\beta_i + \epsilon_{ij}
\end{align*}




% \subsection{Meta contextual MAB}
% We compare our model with the model in \citet{tomkins2019intelligent}, which is representative of the literature on meta contextual MAB. 
% % For ease of comparison
% Let $S_{i.t}$ be the context for the $t$th interaction with the $i$th task. 
% Intelligent Pooling assumes
% % \begin{align}
% % \vthe_i &= \vthe + \delta_i, \forall i\\
% % R_{it} &= f(S_{it}, A_{it}; \vthe_i) + \epsilon_{it}, 
% % \end{align}
% % or equivalently, 
% \begin{equation}
% R_{it} = f(S_{it}, A_{it}; \vthe + \delta_i) + \epsilon_{it}.
% \end{equation}


% Let $\vx_i$ be the static features of task $i$. 
% Our model is 
% % \begin{align}
% % r_{i, a} &= g(\vx_i, a; \vthe) + \delta_{ia}, \forall i, a\\
% % R_{i, t} &= \sum_a \mathbb{I}(A_{it} = a)r_{ia} + \epsilon_{it}.
% % \end{align}
% % or equivalently, 
% \begin{equation}
% \begin{split}
%     R_{i, t} &= g(\vx_i, A_{it}; \vthe) + \sum_a \mathbb{I}(A_{it} = a) \delta_{ia}+ \epsilon_{it} %\\
%     % R_{i, t} &= f(\vx_{i(t)}, A_{it}; \vthe) + \sum_a \mathbb{I}(A_{it} = a) \delta_{ia}+ \epsilon_{it}.\\
%     % R_{i, t} &= f(\vx_{i(t)}, A_{it}; \vthe + \vthe_i) + \epsilon_{it}.
% \end{split}
% \end{equation}


% For the nonliner case, we need the following modifications
% \begin{equation}
% \begin{split}
%     R_{it} &= f(S_{it}, A_{it}; \vthe + \vthe_i) + \epsilon_{it}.\\
%     R_{it} &= f(\vxi, A_{it}; \vthe + \vthe_i) + \epsilon_{it}.\\
%     R_{it} &= f(\vxi, A_{it}; \vthe + \vthe_{ia}) + \epsilon_{it}. \\
%     R_{it} &= f(\vxi, A_{it}; \vthe) + f(\vxi, A_{it}; \vthe_{ia}) + \epsilon_{it}. \text{Not identifiable (not a valid model)}\\
%     R_{it} &= f(\vxi, A_{it}; \vthe) + \delta_{ia} + \epsilon_{it}.\\
% \end{split}
% \end{equation}
% Except for the first step, neither of them is a special case of the previous one. 


% \textbf{Connections.} When we remove $\delta_i$ from (6) and $\delta_{ia}$ from (9), and set $S_{it} = \vx_i$ for all $t$
% these two models coincide at the  contextual MAB method
% \begin{equation}\label{formula: CMAB}
%     R_{i, t} = f(S_{it}, A_{it}; \vthe) + \epsilon_{it}, \forall i
% \end{equation}
% Otherwise, neither one is a special case of the other. 
% The difference can also be seen through the following combination of both (multiple contexutal MAB tasks with task-specific faetures which capture the task similiarity). We add static feature-based task similarity model to (6) and extend our model to contextual MAB: 
% \begin{equation}\label{formular: CMTB}
%     \begin{split}
%         \vthe_i &= g(\vx_i; \beta) + \delta_{i},\\
% R_{i, t} &= f(S_{it}, A_{it}; \vthe_i) + \epsilon_{it}, 
%     \end{split}
% \end{equation}

% In short, Intelligent Pooling applies to multiple contextual MAB tasks but the task similarity has not been modeled; our model applies to multiple MAB tasks without contexts but with the task similarity carefully modeled. 
% Therefore, these two approaches are orthogonal. 
% % , and are applicable when different information is available. 
% When no context information is available, their method is not applicable (Naively set $\vx_i = S_{i,t}$ will lead to $r_{ia} = f(\vx_{i}, a; \vthe + \delta_i) = f(\vx_{i}, a; \vthe_i)$, whose meaning is not clear). 
% When there are huge heterogeneity, such as there are several clusters, their method is also not efficient. 

% \textbf{When f is nonlinear (above).} If the implications of two models are the same (or one is a special case of the other), then no matter which functional class we choose (linear, random forests, NN, GP), the connections should hold (which is not the case here)

% \textbf{When f is linear.} One may argue that, when f is a linear function, the two forms look similar. We take a close look. 
% Write $\vx_{ia} = \vphi(\vx_i, a)$. 
% Then by setting $S_{it} = \vx_i$, 
% Intelligent Pooling assumes
% \begin{equation*}
%     r_{ia} = \vx_{ia}^T (\vthe + \vthe_i) = \vx_{ia}^T \vthe +  \vx_{ia}^T \vthe_i, \vthe_i \sim N(0, \Cov)
% \end{equation*}
% % It is equal to $r_{ia} = \vx_{ia}^T \vthe +  \delta_i, \vthe_i \sim N(0, \vx_{ia}^T \Cov \vx_{ia})$. 
% Our model is
% \begin{equation*}
%     r_{ia} = \vx_{ia}^T\vthe + \delta_{ia}, \delta_{ia} \sim N(0, \sigma^2)
% \end{equation*}
% We need to take the following steps so that Intelligent Pooling can apply to our problem (equivalent to our model) (\textbf{for now, assume $\vxi$ contains continuous variables. When only categorical variables are present and we only consider the linear form, this two model coincidences. But actually a lot of models are the same under such a restrictive setting, since essentially we are considering a block design.}): 
% % There are still the following differences between Intelligent Pooling and  (our problem):
% \begin{enumerate}
%     \item modify $\vthe_i$ as $\vthe_{ia}$: this modification already implies that for tasks (products/patients) with the same features, the optimal action can vary.
%     \item one may tend to write $\vx_{ia}^T\vthe_{ia}$ as $\delta_{ia}$. Then we need to explain the meaning of $\vx_{ia}^T\vthe_{ia}, \; \vthe_{ia} \sim N(0, \Cov)$. 
%     % What does his 
%     One may argue this is sometimes used to handle heteroscedasticity, but why do we need such a dependency needs to be explained. 
%     \item Even if we ignore the two points above: recall that, so far, our discussions are only about models. 
%     The inference goal of IP, $\vthe_{ia}$, is not identifiable in our problem. Of course, we can modify their algorithm, and also the theory, and numerical studies. But now we have already modified a lot.
% \end{enumerate}

% Some other arguments: 
% \begin{enumerate}
%     \item In nonlinear cases, the above connections not feasible (1. $\delta_i$ is not meaningful any longer; 2. can be modified as a mean-zero random-effect function term $f_i$, but not identifiable)
%     \item \textbf{How to prove that their model can be applied to our problem:} one can consider the example in the next section, and remember our goal is $\{r_{ia}\}$. 
%     % If their model and method can be 
%     We are not clear how to adapt their model and method to such a problem. 
%     \item It might help to distinguish the following models (in the simplified regression setup. \textbf{$\vxi$ includes continuous variables}): 
% \end{enumerate}
%     \begin{align*}
% \text{(1)}\; y_{i} &= \vxi^T \vbeta + \epsilon_{i}; (\text{linear fixed effect model})\\
% \text{(2)}\; y_{ij} &= \vxi^T \vbeta + \epsilon_{ij} (\text{linear fixed effect model - why contextual bandit not appropriate})\\
% \text{(3)}\; y_{ij} &= \vx_{ij}^T (\vbeta + \vbeta_i) +  \epsilon_{ij}, \vbeta_i \sim N(0,\Cov) (\text{their model in their problem. Sometimes called \textbf{random coefficient model}})\\
% \text{(4)}\; y_{ij} &= \vxi^T (\vbeta + \vbeta_i) +  \epsilon_{ij}, \vbeta_i \sim N(0,\Cov) (\text{their model in our problem.})\\
% &\;\;\;\;\;\;\;\;\;(\text{Why their method fails: 1. meaning of $\vxi^T \vbeta_i$? 2. $\vbeta_i$ not identifiable})\\
% \text{(5)}\; y_{ij} &= \vxi^T \vbeta + \delta_i + \epsilon_{ij}, \delta_i \sim N(0,\sigma^2) (\text{our model in our problem. Not a special case of model 3 and 4. } )\\
% \text{(6)}\; y_{ij} &= \vxi^T \vbeta + \delta_i + \epsilon_{ij}, \delta_i \sim N(0,\sigma_i^2) (\text{one possible extension of our model. Not a special case of model 3 and 4.} )
%     \end{align*}

% % Covariance modelling and multilevel structures
% % A general form of linear mixed effect models (in our case. Focus on the regression function part) is: 
% % \begin{equation*}
% %     r_{ia} = \vx_{ia}^T \vthe + \mathbf{z}_{ia}^T \vbeta 
% % \end{equation*}

% % (to be examined: whether this is trivial )

% % Even if we ignore all those issues, another thing in the linear model is that (if we shift our attention from the models to the estimator/algorithm/method) , their inferential goal is theta_i (theta_i = theta + \mu_i, in their notations). But  is not identifiable in our problem. See the follows. 

% % Consider the \mu_i term, which links with \delta_ia through \delta_ia = x_ia^T \mu_i. Even if we have infinite data points and then we know the true value of delta_ia, the number of possible values for \mu_i is still infinite.

% % 

% % All our previous discussions are purely mathematical. The intuition/reason behind them is, these two papers are about different problems.

% % context is not the same with static-feature


% % \textbf{1. Why not consider the most general form \eqref{formular: CMTB}? }
% % Technically, we can. With Gaussian linear mixed effect model or GP for both $f$ and $g$, the derivation will be similar. 
% % The concerns are mainly about the theoretical challenges and the finite-sample performance (the current model is more like mixed effect regression models,  \eqref{formular: CMTB} is more like varing-coefficient regression models. For \eqref{formular: CMTB}, I am not aware of any similar works and existing theory in the bandit literature.) 

% % Besides, I would like to note that the contextual features (which depend on t) are not always available. 
% % % MAB is not just a simpler version of contextual MAB, since 
% % Simply treating the static features as the context and ignoring the heterogeneity lead to model \eqref{formula: CMAB}, which results in biases with the presense of $\delta_{ia}$. 





==> ARCHIVE/discussion_comparison_related.tex <==
\section{Comparison with Related Methods}
In this section, we discuss the relationship of our setup with several related lines of research in more details. 

\subsection{Contextual MAB}
Let us consider a standard CMAB formulation in the multi-task setup. 
For time $t = 1, 2, \dots$, the agent receives a task index $i(t)$ along with its feature $\vx_{i(t)}$, regards it as the context of this interaction, selects some action $a_t$, and then receives some random reward $R_t$. 
The agent relate this reward with the context-action pair by assuming a relationship $R_t = f(\vx_{i(t)}, a_t; \vthe) + \epsilon_t$, for some function $f$ with unknown parameter $\vthe$ and some mean-zero random error $\epsilon_t$. 
The underlying assumption is $\Mean(R_t | \vx_{i(t)} = j, a_t = a) = f(\vx_j, a; \vthe)$ for any task $j$ and action $a$. 
This is an assumption we have to impose when we only interact with each task for one time. 
However, under the multi-task setup, where we need to interact with each task for multiple times, the repeated measurements nature allows us to include a mixed effect term to allow personalization for each individual tasks, which lead to the a general form of our model: 
\begin{equation*}
    \Mean(R_t | \vx_{i(t)} = j, a_t = a) = f(\vx_j, a; \vthe) + \delta_{i,a}, \forall i \in [N], a \in [K]. 
\end{equation*}
When the number of interactions with one task $i$ is limited, the above formulation will be dominated by $f(\vx_j, a; \vthe)$ and hence is close to a contextual MAB settting; while when the number increases, it will be dominated by $\delta_{i,a}$ and hence is close to the single-task MAB setting. 
As such, our model allows judiciously sharing information among tasks and hence reduces the variance, esoterically in the early period, and also allows personalization to each individual task according to its own history records. 


% CMAB algorithms typically  
% $r_{t,a} = f_{\vthe}(\vx_t, a)$  where $\vx_t$ is the "context" for the $t$-th interaction, $a$ is some action, and $r_{t,a}$ is the expected reward of this interaction. 



==> ARCHIVE/layout_example.tex <==

\section{The layout example}
\begin{itemize}
    \item Tasks: $i = 1, \dots, N$ products. 
        \begin{enumerate}
        \item shoe1, shoe2, ..., phone1, phone2, ..., TV1, ...
            % \item Shoes: shoe1, shoe2, ...
            % \item Electronics: phone1, TV1, ...
        \end{enumerate}
    \item Arms: for each product, $a = 1, \dots, K$ display layouts
        \begin{enumerate}
            \item (Image-title, new-release, brand, price, why-recommended)
            \item (Image-title, brand, reviews, price, why-recommended)
        \end{enumerate}
    % E.g.: Category = (Shoes): Option = (Image-title, new-release, brand, price, why-recommended). Category = (Electronics): Option = (Image-title, brand, reviews, price, why-recommended).
    \item Reward: $r_{ia}$ under each display layouts  %the product have a CTR
    \item Features: baseline features $\vxi$ (category, price, etc.)
\end{itemize}

Methods:
\begin{itemize}
    \item CMAB: $r_{ia} = f(\vxi, a; \vthe)$. Fully determined by features (even if we find it is sub-optimal after interactions). 
    \item independent MAB: $\{r_{ia}\}$ are independent %i.i.d.
    % \item meta MAB: $r_{ia} \sim N(\mu_r, \sigma_r^2)$ 
    \item Ours: $r_{ia} = f(\vxi, a; \vthe) + \delta_{ia}$
\end{itemize}
IP can not apply to such a problem. 


==> ARCHIVE/meta_oracle.tex <==
\section{The Oracle-TS and its Bayes regret}\label{supp-sec:oracle}
As our oracle-TS, for each task $i$, we consider the  standard Thompson sampling algorithm for Gaussian bandits with prior distribution as $\vr_{i} \sim \mathcal{N}(\vPhi_{i}\vthe, \Cov)$.  
With such a "true" prior, its asymptotic optimality for this single task has been derived in \citet{agrawal2013further}. 
Its optimality can be straightforwardly extended to the multi-task setting, to yield a Bayes regret of order $O(N\sqrt{T}log(T))$. 

[to be updated w/ new notations]
We briefly review the standard Thompson sampling algorithm for a single task below. 
At a decision point for task $i$, suppose the accumulated interaction data with task $i$ is $\mathcal{D}_i = \{(A_{i,t}, R_{i,t})\}$. 
Let $\rho(\vr_i)$ be the corresponding posterior with the data $\mathcal{D}_i$ and the prior $r_{i,a} \sim \mathcal{N}(\vphi(\vxi, a)^T\vthe, \sigma_1^2)$ for every $a \in [K]$. 
$\rho(\vr_i)$ follows a multivariate normal distribution. 
Then, the oracle-TS will take the action $A_{i,t} = argmax_a \{\tilde{r}_{i,a}\}_{a=1}^K$, where $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T$ is randomly sampled from $\rho(\vr_i)$. 

%  for every $a \in [K]$

==> ARCHIVE_Method/LMM.tex <==
% For simplicity, we assume $\epsilon_{i,t} \sim \mathcal{N}(0, \sigma^2)$ throughout this paper. 
% to mitigate the bias 
% The term $\delta_{i,a}$ is introduced to accommodate task-specific heterogeneity that can not be captured by the features. 
\subsection{Bayesian linear mixed effect model}\label{sec:LMM}

% can be some basis expansions 
% or mannually designed.
% typical in the linear bandit literture. 
% a set of basis functions which are “rich” enough to approx- imate the underlying function
Let $\vphi(\cdot, \cdot) : \mathbb{R}^p \times [K] \rightarrow  \mathbb{R}^d$ be a known map from the feature-action space to a $d$-dimensional space, and let $\vPhi_{i} = (\vphi(\vx_i, 1)^T, \dots, \vphi(\vx_i, K)^T)$ be the $K \times d$ transformed feature matrix for task $i$. 
We focus on the case that $\Mean(\vr_i|\vx_i)$ is a linear function of $\vPhi_{i}$  and consider the following Bayesian linear mixed effect model:
% , stacked vertically over the $K$ arms. 
\begin{equation}\label{eqn:LMM}
\begin{split}
    \vr_i = \vPhi_{i}\vthe + \vdelta_i, 
    % r_{i,a} &= \vphi(\vx_i, a)^T \vthe + \delta_{i,a}, 
\end{split}
\end{equation}
% for every i \in [N] and a \in [K]. 
% better replace with \Cov_{\vdelta}. But \cov_{a, a'}
where $\vthe$ is an unknown vector, and $\vdelta_{i} \stackrel{i.i.d.}{\sim} \mathcal{N}(0, \Cov)$ for some 
% unknown 
covariance matrix $\Cov$. 
$\{\vx_i\}$, $\{\vdelta_i\}$, and $\{\epsilon_{it}\}$ are mutually independent. 
% where $\delta_{i,a} \stackrel{i.i.d.}{\sim} \mathcal{N}(0, \sigma_2^2)$ for an unknown parameter $\sigma_2$. 
In this model, the fixed effect term $\vPhi_{i}\vthe$ captures the task similarity through their features $\vx_i$, and the random effect term $\vdelta_i$ allows task heterogeneity. 
We assume the prior distribution $\vthe \sim \mathcal{N}(\vmu_\theta, \Cov_\theta)$ for some user-specified parameters $(\vmu_\theta, \Cov_\theta)$. 

% three types
% 1. x -> transform -> X
% 2. directly observe X
% 3. r_{i, a} = $\vx_i^T \vthe_{a}$
% 3. E(R_{i, t}| A_{i,t} = a) $\vx_i^T \vthe_{a}$


\begin{remark}
% , and results developed in this paper continue to hold. 
Additional structures can be imposed on $\Cov$ to derive a simper model. 
For example, one can require the arms of a task to have independent random effects by specifying $\Cov = \sigma_1^2 \vI$ for an unknown parameter $\sigma_1$, and one additional random effect term can be added at the task level by specifying $\Cov = \sigma_1^2 \vI + \sigma_2^2 \vJ$ with an additional unknown parameter $\sigma_2$. 
The induced models are popular choices in the literature on mixed effect models \citep{fitzmaurice2008primer}, and they are special cases of model \eqref{eqn:LMM}. 
\end{remark}

% The parameter $\Cov$, together with $\sigma^2$, can be learned from data via Empirical Bayes \citep{carlin2000bayes}  to adapt to the degree of heterogeneity and noise. 
% We will detail the procedure in Section \ref{sec:TS}. 



% Similar models have been widely considered in the literature on linear bandits \citep{chu2011contextual, tomkins2019intelligent}, although we utilize such a model to incorporate the task-specific features. 


\subsection{Thompson sampling for feature-based multi-task bandits}\label{sec:TS}
Thompson sampling is one of the most popular bandit framework \citep{agrawal2013further,russo2017tutorial,tomkins2020intelligentpooling}. 
The algorithm requires a prior over model parameters as the input, updates a posterior according to observed interactions, and samples an action to take according to its probability of being the optimal one. 
In this section, we develop a TS-type algorithm for the feature-based multi-task bandits problem with the objective of minimizing the Bayes regret. 


Suppose at a decision point,  
we have accumulated a dataset $\mathcal{D} = \{(A_{j}, R_{j}, i(j))\}_{j=1}^n$ of size $n$, where the data for all tasks have been combined and re-indexed. 
Here, $i(j)$ is the task index for the $j$-th tuple in $\mathcal{D}$, $A_{j}$ is the implemented action and $R_{j}$ is the observed reward. 
Suppose we are going to make decision for the $i$-th task at this time point. 
To adapt the TS algorithm, we need to derive the posterior of $\vr_i$ 
% , update the hyper-parameters, 
and sample an action to take. 
The full TS algorithm is summarized in Algorithm \ref{alg:TS}, with the key components detailed below. 
% should we talk about the action to take?
\input{Algorithm/alg_TS}

% The posterior will then be used to sample an action according to its probability of being the optimal one, in a Thompson sampling manner, as detailed in Algorithm \ref{alg:TS}. 
% posteriors for the expected rewards of arms in this task have analytic expressions. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% with calendar time $t_0$, _{t_0}
% $\mathcal{D} = \{(A_{i,t}, R_{i,t}, i)\}$ of size $n$
\textbf{Posterior updating.}
Given the model assumptions, the posteriors of $\vr_i$ have analytic expressions. 
We begin by introducing some notations. 
% model \eqref{eqn:R} and \eqref{eqn:LMM} together
The Bayesian linear mixed effect model \eqref{eqn:LMM} induces a kernel function $\mathcal{K}$, such that for any two tuples $O = (a, r, i)$ and $O' = (a', r', i')$, we have 
\begin{equation*}
    \mathcal{K}(O, O') = \vphi^T(\vx_i, a) \Cov_{\vthe} \vphi(\vx_{i'}, a') 
    + \Cov_{a, a'} \mathbb{I}(i = i'),
    % + \sigma_2^2 \mathbb{I}(i = i', a = a'),
\end{equation*}
where $\Cov_{a, a'}$ is the $(a,a')$-th entry of $\Cov$. 
Besides, let $\mK$ be a $n \times n$ kernel matrix of the pairwise kernel values for tuples in $\mathcal{D}$. 
Set $\vR = (R_1, \dots, R_n)^T$ be a $n$-dimensional vector of the observed rewards. 
% and $\vmu = (\mu_{A_1}(\vx_{i(1)}), \dots, \mu_{A_n}(\vx_{i(n)}))^T$. 
% $\vR$ be a $n$-dimensional vector with the $j$-th entry be the observed reward of the $j$-th tuple in $\mathcal{D}$, and 
Define $\vPhi$ as a $n \times d$ feature matrix with the $j$-th row be the feature vector $\vphi^T(\vx_{i(j)}, A_{j})$. %of the $j$-th tuple in $\mathcal{D}$. 
% For the $i$-th task, let $\vr_i = (r_{i1}, \dots, r_{iK})^T$. 
% $\mathcal{D} = \bigcup_{i,a} \mathcal{D}_{i,a}$, where $\mathcal{D}_{i,a}$ is empty if action $a$ has not been taken for task $i$ yet, and $\mathcal{D}_{i,a} = \{(A_{i,t}, R_{i,t}, i) : A_{i,t} = a\}$ otherwise. 
% Let $\vone_d$, $\vzero_d$, and $\vI_d$ be a d-dimensional vector of all ones, a d-dimensional vector of all zeros, and an identity matrix of dimension $d \times d$, respectively. 
% When the subscript is omitted, the appropriate dimension can be inferred from the context. 
Finally, for every $i \in [N]$, define a $K \times n$ matrix $\boldsymbol{M}_i$, such that the $(a, j)$-th entry of $\boldsymbol{M}_i$ is 
$\Cov_{A_j, a} * \I(i(j) = i)$. 
% $\sigma_2^2 * \I(i(j) = i, A_j = a)$. 
% is $\sigma^2$, if for the $j$-th tuple in $\mathcal{D}$, the task index is $i$ and the action we took is $a$. 
% The other entries of $\boldsymbol{M}_i$ are all zero. 
The posterior of $\vr_i$ conditional on the accumulated data follows a multivariate normal distribution $\rho(\vr_i)$, with mean and covariance as follows: 
\begin{equation}\label{eqn:post}
    \begin{split}
        \mathbb{E}(\vr_i|\mathcal{D}) &= \vPhi_{i} \vmu_{\vthe} + (\vPhi_i\Cov_{\vthe}\vPhi^T + \boldsymbol{M}_i) (\mK + \sigma^2 \vI)^{-1} (\vR - \vPhi \vmu_{\vthe}),  \\
        cov(\vr_i | \mathcal{D}) &= (\vPhi_{i} \Cov_{\vthe} \vPhi_{i}^T + \Cov) - (\vPhi_i\Cov_{\vthe}\vPhi^T + \boldsymbol{M}_i) (\mK + \sigma^2 \vI)^{-1} (\vPhi_i\Cov_{\vthe}\vPhi^T + \boldsymbol{M}_i)^T. 
    \end{split}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Action selection.} 
The posterior is used to sample an action in the TS manner. 
Specifically, 
we first sample a reward vector $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T \sim \rho(\vr_i)$, and then take the action $ \argmax_{a \in [K]} \tilde{r}_{i,a}$.  
% A_j = 
%  according to its probability of being the optimal one, 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \label{eqn:post}
% variance -> 0
% Interpretation: 
% $\mathbb{E}(r_{i,a}|\mathcal{D})$ is composed of two parts: $
% \vphi(\vx_i, a)^T\vmu_{\vthe} + (\vphi(\vx_i, a)^T\Cov_{\vthe}\vPhi^T)(\mK + \sigma^2 \vI)^{-1}(\vR - \vPhi \vmu_{\vthe})$
% and 
% $\boldsymbol{M}_i(\mK + \sigma^2 \vI)^{-1}(\vR - \vPhi \vmu_{\vthe})$. 
% Informally speaking, the first term is to estimate the fixed effect term $\vphi(\vx_i, a)^T \vthe$ and the second term is to estimate the random effect term $\delta_{i,a}$. 
% When there are no data points of taking action $a$ in task $i$ is $0$, the second term is $0$ and our estimation of $r_{i,a}$ depends on the information pooled from the other tasks; 
% While when the number of data points of taking action $a$ in task $i$ is large or when $\sigma_2$ is large, then second term will dominate, which implies we would like to rely more on the rewards generated by taking action $a$ in task $i$ itself. 


% \hl{prior; other task through X; its own experiment data; hyper-parameters}
% better prior 
% will still rely on the task-specific feedback to mitigate the potention bias. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% \textbf{Remark.} 
\begin{remark}
The linear assumption in \eqref{eqn:LMM} allows efficient computation and the model is less prone to over-fitting. 
% when the number of tasks $N$ is not large. 
% bias variance
Nevertheless, the idea of utilizing task-specific features in multi-task bandits via a mixed effect model is generally applicable. % and not limited to the linear form
One can replace $\vPhi_{i}\vthe$ in \eqref{eqn:LMM} with $f(\vx_i; \vthe)$ for some non-parametric function $f(\cdot)$, and proceed in a similar way. 
 As an example, a mixed-effect Gaussian process model and the corresponding TS algorithm are derived in Appendix \ref{sec:GP}. % provided
\end{remark}
% Can theory be extended? the linear. As long as the regression model converge. 
% The other has no explicit form
% Which also allows explicit
% really? except for GP, other can be derive?

At each decision point, the computation will be dominated by the calculation of the matrix inverse and the determinant for $(\mK + \sigma^2 \vI)$, which suffers from a cubic complexity $O(n^3)$ as well-known in the Gaussian process literature. 
In Appendix \ref{sec:implementation}, we introduce an efficient implementation, which utilizes the block structure induced by the mixed effect model via using the well-known Woodbury matrix identity \citep{rasmussen2003gaussian}. 

% To alleviate the computational burden, we
% Step \eqref{eqn:post} and \eqref{eqn:Hyper-parameter} are both closely related with the kernel function and the matrix inverse. 


==> Additional_Related_Work.tex <==
\section{Additional Related Work}\label{sec:appendix_additional_related_work}
In this section, we compare this paper with additional related works. 
To begin with, we note that there are several terms used in the literature for problems concerned with multiple tasks, which is often a source of confusion. 
Based on  \cite{hospedales2020meta}, 
\textit{meta learning} assumes tasks are drawn from a distribution and aims to maximize the average performance over this task distribution (\textit{meta-objective}); 
\textit{transfer learning} uses data from finished tasks to improve the performance on a new task, and typically focuses on the single-task objective, although the viewpoint of meta learning can be applied to achieve this goal (as in the sequential setting of our work); 
\textit{multi-task learning} aims to jointly learn a few tasks, where typically the number of tasks is fixed and the meta-objective is not adopted, although the viewpoint of meta learning can be applied in these problems as well (as in the concurrent setting of our work). 
There are often some overlaps between these concepts. 
In this work, we adopt the task distribution viewpoint as well as the meta-objective \cite{hospedales2020meta}, which are naturally related with our hierarchical Bayesian framework, allows us to model heterogeneity, and enables knowledge sharing via constructing informative priors. 
We refer to our problem as multi-task bandits to focus on the fact that there are multiple tasks, since our methodology is applicable to the sequential setting (transfer learning), the concurrent setting (multi-task learning), and even more complex settings. 
% Continual learning (CL) Continual or lifelong learning

% Low-rank bandits. is an extention
According to the taxonomy developed in \cite{zhang2017survey}, multi-task algorithms can be classified into the feature learning approach, low-rank approach, task clustering approach, task relation learning approach, and decomposition approach. 
In the bandit literature, \cite{yang2021impact} considers that one interacts with multiple linear bandit
tasks concurrently and the coefficient vectors of these tasks share the same low-dimensional space, and hence belongs to the feature learning approach; 
\cite{kveton2017stochastic} studies finding the maximum entry of a low-rank matrix in a bandit manner and \cite{jun2019bilinear} assumes the coefficient matrix of a bilinear bandit problem is low-rank, and hence they belong to the low-rank approach; 
clustering of bandits \citep{gentile2014online, li2016collaborative} and latent bandits \citep{hong2020latent, hong2020non} assume there is a perfect clustered structure, and hence they belong  to the task clustering approach. 
In contrast to these papers, our work belongs to the relation learning approach, which aims to learn the task relations from data by assuming some probabilistic model or applying some penalty function. 
Our approach provides nice interpretability and is flexible with arguably less strict assumptions.  
In particular, to the best of our knowledge, this is the \textit{first} work that can leverage the task-specific metadata in multi-task bandits, which is an important information source that none of the existing methods can utilize. 
Although we focus on MAB in the main text, the idea of utilizing metadata is generally applicable. 
We discuss its extensions to linear bandits and clustering of bandits in Appendix \ref{sec:extension_contextual}. 


Besides, similar with meta MAB, there are also several works on meta linear bandits. 
Meta linear bandits studies the problem where the coefficients of multiple linear bandit tasks are close \citep{multilinear} or are drawn from one prior distribution \citep{metapricing, tomkins2019intelligent, cella2020meta}. 
% IP in the appendix. % random coeffcient model % share some similar technical tools 
Therefore, these works focus on a different problem from ours and they also did not model the task relations with metadata. 
In addition, \cite{ortega2019meta} proposes a sequential strategy for meta bandits, but as noted in \cite{hsu2019empirical}, no efficient algorithm has been proposed. 
Lastly, we note that there are two papers \cite{deshmukh2017multi, krause2011contextual} applying multi-task learning to share information across multiple arms of a single task, and hence they have a totally different focus from ours. 

% metadata and BHM is main.
% : transfer RL survey. 
% In the main text, we focus on the literature on bandits. 
% at a high level, 
Our bandit problem is certainly related to Reinforcement Learning (RL). 
In recent years, there is a surge of interest in multi-task RL, transfer RL, and meta RL. 
See \cite{zhu2020transfer} and \cite{vithayathil2020survey} for some recent surveys. 
Among the existing works, 
\cite{wilson2007multi, lazaric2010bayesian, grant2018recasting} consider applying Bayesian hierarchical model to multi-task/meta RL. 
However, none of these works can utilize the metadata, which is an important and ubiquitous information source. 
In the concurrent work \cite{sodhani2021multi}, the authors, for the first time, consider using metadata in multi-task reinforcement learning to infer the appropriate state representation for each task. 
They consider a finite set of state encoders, design a special-purpose neural network, and train the whole pipeline end-to-end. 
In contrast, 
we study MAB, allow infinite number of task instances, aim to learn the average reward of each task instead of state representation,  design a unified Bayesian Hierarchical model framework for this problem, and establish theoretical guarantees. 
Therefore, although both work consider similar types of side information (i.e., metadata), the problem and methodology are fundamentally different. 


Finally, we would like to further compare our setup with CMAB, and discuss the limitations of adopting CMAB in our problem. 
In the standard contextual MAB setup, we assume $\Mean(R_{i,t}|S_{i,t} = s, A_{i,t} = a) = g(s, a;\gamma)$ for some function $g$, where $S_{i,t}$ is the context. 
Therefore, it already allows the randomness of $R_{i,t}$. 
In our setup,  by regarding the metadata as "contexts" and neglecting the task identities, the relationship is equal to $\Mean(R_{i,t}|\vx_{i} = \vx, A_{i,t} = a) = g(\vx, a;\gamma)$, where we note that the expectation is taken over all tasks with metadata $\vx$. 
This implies that for all tasks with the same metadata, the decision rule will be always the same, no matter what their action-reward history is. 
Instead, our setup adds another layer to allow variations of $\vr_i$ conditional on $\vx_i$. 
In another word, we utilize the predictive power of $\vx_i$ but does not assume $\vr_i$ can be fully determined by it. 
% by neglecting the task identities and regarding the metadata as "contexts". % static metadata
% and hence it is reasonable to assume $\vr_i = f(\vx_i)$
% Recall that $\vr_i$ is the expected reward vector for all arms

% warm-starting bandit / offline data: the same bandit task
% collaborative filtering: metaTS

% ,  assumes such a clustered structure has been learned from logged data. 
% Multi-task Linear Bandits: sequential, epsilon


==> Additional_Results.tex <==
\section{Additional Experiment Results}\label{sec:appendix_addi_numerical_results}

\subsection{Robustness to model misspecifications}\label{sec:appendix_robustness}
To allow efficient information sharing, we make a model assumption that $\vr_i | \vx_i, \vthe \sim f(\vr_i | \vx_i, \vthe), \forall i \in [N]$. 
When this model is correctly specified, we have shown superior theoretical and numerical performance of {\name}. 
However, we acknowledge that all models can be misspecifed. 
Intuitively, the model is used to pool information to provide an informative prior. 
As long as the learned prior is not significantly worse than a manually specified one, the performance would be comparable; and when the prior contains more information, we can attain a lower regret. 

We empirically investigate the robustness of {\name} in this section. 
We focus on the Gaussian bandits case under the concurrent setting. 
Findings under the other settings are largely the same and hence omitted. 
Specifically, 
instead of generating data according to $\vr_i = \vPhi_{i}\vthe + \vdelta_i$, we consider the data generation process $\vr_i = (1 - \lambda) cos(c\vPhi_{i}\vthe)/c + \lambda \vPhi_{i}\vthe  + \vdelta_i$, where $cos$ applies the cosine function to each entry, 
c is a normalization constant such that the entries of $\vPhi_{i}\vthe$ are all in $[-\pi/2,\pi/2]$, 
and $\lambda \in [0,1]$ controls the degree of misspecification. 
When $\lambda = 1$, we are considering the LMM; while when $\lambda = 0$, the metadata  provides few  information through such a linear form. 

In results reported in Figure \ref{fig:simu_Gaussian_robustness_concurrent}, we observe that {\name} is fairly robust to model misspecifications. 
When $\lambda = 1/2$ or $3/4$, that is, when there exists mild or moderate misspecification, {\name} still yields much lower regrets than individual-TS and meta-TS. 
When $\lambda = 1/4$, the performance of {\name} becomes comparable with individual-TS and meta-TS. 
Only when $\lambda = 0$, that is, the metadata are useless through a linear form, {\name} shows slightly higher regret in the initial period due to the additionally introduced variance. 
As expected, linear-TS and OSFA both severely suffer from the bias. 
Notably, in all cases, {\name} always yields the desired sublinear Bayes regret in $T$, as expected. 
Therefore, it shows that, even when the model is severely misspecified, the cost would be acceptable. 



\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/mis_cos_0.75_0.25_concurrent.png}
         \caption{$\lambda = 3/4$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/mis_cos_0.5_0.5_concurrent.png}
         \caption{$\lambda = 1/2$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/mis_cos_0.25_0.75_concurrent.png}
         \caption{$\lambda = 1/4$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/mis_cos_0_1_concurrent.png}
         \caption{$\lambda = 0$}
     \end{subfigure}
     \\
\caption{
Average Bayes regret for Gaussian bandits with misspecified hierarchical models. 
A smaller value of $\lambda$ implies a more severe misspecification. 
The regrets of OSFA are an order of magnitude higher and hence hidden. 
}
% The yellow line (TR, m = 2) and green line (TR, m = 3) are largely overlapped
\label{fig:simu_Gaussian_robustness_concurrent}
\end{figure}


% \begin{figure}[t]
%      \centering
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/mis_cos_0_1_episodic.png}
%          \caption{$\lambda = 0$}
%      \end{subfigure}
%      \\
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/mis_cos_0.25_0.75_episodic.png}
%          \caption{$\lambda = 1/4$}
%      \end{subfigure}
%      \\
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/mis_cos_0.5_0.5_episodic.png}
%          \caption{$\lambda = 1/2$}
%      \end{subfigure}
%      \\
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/mis_cos_0.75_0.25_episodic.png}
%          \caption{$\lambda = 3/4$}
%      \end{subfigure}
%      \\
% \caption{
% Average Bayes regret for Gaussian bandits with misspecified hierarchical models. 
% A smaller value of $\lambda$ implies a more serious misspecification. 
% The regrets of OSFA are an order of magnitude higher and hence hidden in the upper subplots. 
% }
% % The yellow line (TR, m = 2) and green line (TR, m = 3) are largely overlapped
% \label{fig:simu_Gaussian_robustness_concurrent}
% \end{figure}


\subsection{Multi-task regrets}\label{sec:appendix_figure_MTR}
In the main text, we report the Bayes regret of different algorithms. 
Although the multi-task regrets for those figures can also be derived according to its definition, we choose to explicitly report them again in this section, in order to make the comparison more clearly. 

Specifically, the multi-task regrets for Gaussian bandits and Bernoulli bandits are presented in Figure \ref{fig:simu_Gaussian_multi-task}  and \ref{fig:simu_Binary_multi-task}, respectively. 
In the sequential setting, we can see the multi-task regrets of {\name} converge to zero, while meta-TS and individual-TS have a constant regret, and linear-TS as well as OSFA suffer from the bias. 


\begin{figure}[h]
     \centering
 \begin{subfigure}[b]{\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Figures/Gaussian_all_6_MTR.png}
    %  \caption{Episodic, $\sigma_3 = 5$}
    %  \label{fig:y equals x}
 \end{subfigure}
\caption{
Gaussian bandits: 
the solid lines denote the average multi-task regret with the shared areas indicating the standard errors.  
The regrets of OSFA are much higher in some subplots and hence hidden.
}
% an order of magnitude
% The yellow line (TR, m = 2) and green line (TR, m = 3) are largely overlapped
\label{fig:simu_Gaussian_multi-task}
\end{figure}
\begin{figure}[h]
 \centering
 \begin{subfigure}[b]{\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Figures/binary_all_6_MTR.png}
    %  \caption{Episodic, $\sigma_3 = 5$}
    %  \label{fig:y equals x}
 \end{subfigure}
\caption{
Bernoulli bandits: 
the solid lines denote the average multi-task regret with the shared areas indicating the standard errors.  
A larger value of $\psi$ implies a larger variation of $\vr_i$ condition on $\vx_i$. 
}
\vspace{-0.3cm}
\label{fig:simu_Binary_multi-task}
\end{figure}



\subsection{Trends with experiment hyper-parameters}\label{sec:appendix_more}
In this section, we report additional results under other combinations of $(K, d, T, N)$, to show that our conclusions in the main text are representative, and study the trend of the performance of {\name}. 
We focus on the Gaussian bandits case under the concurrent setting. 
To save computational cost, we set the base combination of hyper-parameters as $\sigma_1^2 = 0.5$, $K = 8$, $d = 15$, $N = 100$, and $T = 100$, and run $50$ random seeds for each. 

In Figure \ref{fig:simu_Gaussian_trend}, we vary the value of $K$, $d$, $N$, $\sigma$ individually. 
Overall, {\name} consistently demonstrates lower regrets and shows robustness. 
Our findings can be summarized as follows. 
\begin{itemize}
    % we also share information across arms... it is like cheating...
    \item As $K$ increases, the learning problem for all algorithm becomes more difficult. {\name} still demonstrates better performance, and even when $T = 100$, its advantage is still fairly clear.
    \item As $d$ increases, the learning problem for {\name} becomes more difficult, while it still shows much better performance. 
    \item As $\sigma$ increases, overall the learning problem for all algorithm becomes more difficult. {\name} still demonstrates better performance, and even when $T = 100$, its advantage is still fairly clear.
    \item As $N$ increases, {\name} can learn the task distribution more easily and its performance converges to that of oracle-TS more quickly. 
\end{itemize}

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/trend_K0.5.png}
        %  \caption{$\lambda = 3/4$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/trend_d0.5.png}
        %  \caption{$\lambda = 1/4$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/trend_sigma0.5.png}
        %  \caption{$\lambda = 0$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/trend_N0.5.png}
        %  \caption{$\lambda = 1/2$}
     \end{subfigure}
     \\
\caption{
Trends of the average Bayes regret for Gaussian bandits with different parameters. 
% under different settings. . 
}
% The yellow line (TR, m = 2) and green line (TR, m = 3) are largely overlapped
\label{fig:simu_Gaussian_trend}
\end{figure}


==> Algorithm/TS_faster_binary.tex <==
\begin{algorithm}[!h]
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
\SetAlgoLined
\Input{
$\prob(\vthe)$, $\phi$, updating frequency $l$
% Prior parameters $\vmu_\theta$, $\Cov_\theta$, $\Cov$ and $\sigma^2$
% , initial values 
}

% \textbf{Initialization.} 
Set $\mH = \{\}$ and $\prob(\vthe| \mH) = \prob(\vthe)$

\For{decision point $j = 0, \dots$,}{ 
% \For{all decision point (i,t)}{ 
\If{$j = k * l$ for some constant $k$}{
Apply approximate posterior inference methods (such as Gibbs sampling or variational inference) to sample one $\Tilde{\vthe}$ from  $\prob(\vthe| \mH)$\\
}


Retrieve the task index $i$\\
Sample a reward vector $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T$ 
from 
$c * f_{Beta}(\vr_i|\vx_i, \Tilde{\vthe}) \prob(\mH_i|\vr_i) $, where $c$ is a normalization factor. 
% , where $f(\vr_i|\vx_i, \Tilde{\vthe})$ is the Beta distribution specified by the first equation of \eqref{eqn:BBLM}, $\prob(\mH_i|\vr_i)$ is the likelihood over $\mH_i$ 
% for the Bernoulli distribution specified by the second equation of \eqref{eqn:BBLM}, 
% and $c$ is a normalization factor
\\ 
Take action $A_j = argmax_{a \in [K]} \; \tilde{r}_{i,a}$\\ %$A_{i,t}$
Receive reward $R_j$\\ % R_{i,t}
Update the dataset as $\mH \leftarrow \mH \cup \{(A_{j}, R_{j}, \vx_i, i)\}$
% \\
% Update the hyper-parameter  $\sigma$ and  $\Cov$  according to 
% \eqref{eqn:Hyper-parameter}
\\
}
 \caption{Efficient 
 Implementation of {\name} for  Bernoulli Bandits}\label{alg:TS_faster_binary}
\end{algorithm}


==> Algorithm/alg_TS_faster_general.tex <==
\begin{algorithm}[!h]
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
\SetAlgoLined
\Input{
$\prob(\vthe)$, $\phi$, updating frequency $l$
% Prior parameters $\vmu_\theta$, $\Cov_\theta$, $\Cov$ and $\sigma^2$
% , initial values 
}

% \textbf{Initialization.} 
Set $\mH = \{\}$ and $\prob(\vthe| \mH) = \prob(\vthe)$

\For{decision point $j = 0, \dots$,}{ 
% \For{all decision point (i,t)}{ 
\If{$mod(j, l) = 0$}{
Update $\prob(\vthe| \mH)$ (possibly via approximate posterior inference methods, such as Gibbs sampling or variational inference)

Sample one $\Tilde{\vthe}$ from  $\prob(\vthe| \mH)$\\
}


Retrieve the task index $i$\\
Sample a reward vector $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T$ 
from 
$c * f(\vr_i|\vx_i, \Tilde{\vthe}) \prob(\mH_i|\vr_i) $, where $c$ is a normalization factor. 
% , where $f(\vr_i|\vx_i, \Tilde{\vthe})$ is the Beta distribution specified by the first equation of \eqref{eqn:BBLM}, $\prob(\mH_i|\vr_i)$ is the likelihood over $\mH_i$ 
% for the Bernoulli distribution specified by the second equation of \eqref{eqn:BBLM}, 
% and $c$ is a normalization factor
\\ 
Take action $A_j = argmax_{a \in [K]} \; \tilde{r}_{i,a}$\\ %$A_{i,t}$
Receive reward $R_j$\\ % R_{i,t}
Update the dataset as $\mH \leftarrow \mH \cup \{(A_{j}, R_{j}, \vx_i, i)\}$
% \\
% Update the hyper-parameter  $\sigma$ and  $\Cov$  according to 
% \eqref{eqn:Hyper-parameter}
\\
}
 \caption{Computationally Efficient Variant of {\name} under General Settings}\label{alg:TS_faster_general}
\end{algorithm}


==> Algorithm/alg_modified_MTS.tex <==
\begin{algorithm}[!h]
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
\SetAlgoLined
\Input{
$\prob(\vthe)$ and known parameters for the hierarchical model
% Prior parameters $\vmu_\theta$, $\Cov_\theta$, $\Cov$ and $\sigma^2$
% , initial values 
}

% \textbf{Initialization.} 
Set $\mH = \{\}$ and $\prob(\vthe| \mH) = \prob(\vthe)$

Set $count(i) = 0, \forall i \in [N]$

\For{each decision point $j$}{
Retrieve the task index $i$\\

\uIf{count(i) < K}{
    count(i) = count(i) + 1

    Take action $A_j = count(i)$ \tcp*{Alignment period}
}
\Else{ 
Sample a reward vector $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T$ 
from 
$c * \prob(\mH_i|\vr_i)  f(\vr_i|\vx_i, \Tilde{\vthe}_i)$, where $c$ is a normalization factor. \tcp*{TS with prior $f(\vr_i|\vx_i, \Tilde{\vthe}_i)$}

Take action $A_j = argmax_{a \in [K]} \; \tilde{r}_{i,a}$
}


Receive reward $R_j$\\ % R_{i,t}
Update the dataset as $\mH \leftarrow \mH \cup \{(A_{j}, R_{j}, \vx_i, i)\}$

\uIf{count(i) = K}{ 
Sample one $\Tilde{\vthe}$ from  $\prob(\vthe| \mH)$, and denote it as $\Tilde{\vthe}_i$ \tcp*{Fixed down the prior for task $i$}
}

% $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T \sim \prob(\vr_i | \mH)$ \\ 

% Interact with task $i$ for $T_i$ rounds with $TS\big(f(\vr_i|\vx_i, \Tilde{\vthe})\big)$, and update $\mH$ with observed action-reward pairs\\


% Update the posterior $\prob(\vthe | \mH)$, according to the hierarchical model\\


}

 \caption{The Modified {\name}}\label{alg:modified_MTS}
\end{algorithm}


==> Details_Experiment.tex <==
\section{More on the Experiment Details}\label{sec:appendix_Experiment_Details}
In this section, we report additional details of our epperiments and implementations. 
Recall that we use $\vI$ to denote identity matrix, the  dimension of which can be inferred from the context. 

\subsection{Hyperparameters}
Since all baselines that we consider are TS-type algorithms, we need to specify (i) the priors and (ii) the variance terms which are assumed to be known. 
For fair comparisons, we apply the law of total expectation and the law of total variance to derive these quantities. 
Roughly speaking, for meta-TS, we marginalize out $(\vx, \vr)$ conditional on $\vthe$; 
for individual-TS and OSFA, we additionally marginalize out $\vthe$; 
For linear-TS or GLM-TS, we use the same prior of $\vthe$ as {\name}, and marginalize $\vr_i$ conditional on $\vx_i$ to set the variance of the stochastic reward variable. 
When the marginal distribution does not belong to a standard distribution family, we use the Gaussian distribution as an approximation. 


\paragraph{Gaussian bandits.}
According to our data generation model, based on the law of total expectation and the law of total variance, it is easy to verify that 
\begin{align*}
    cov \big( \vr_i \big | \vthe, \vx_i)
    &= \Cov = \sigma_1^2 \vI\\
    %%%%%%%%%%%%%%%%%%%%%%%%
    \Mean \big( \vr_i \big | \vthe)  &= \vthe_{1:K},\\ 
    %%%%%%%%%%%%%%%%%%%%%%%%
    cov \big( \vr_i \big | \vthe)
    &= \Mean\big(
    cov\big(\vr_i | \vx_i \big)
    \big | \vthe)
    +
    cov\big(
    \Mean\big(\vr_i | \vx_i \big)
    \big | \vthe)\\
    % &= \sigma_1^2 \vI + ||\vthe||^2 \vI, 
    &= \sigma_1^2 \vI + ||\vthe_{(K+1):d}||^2 \vI
    = (\sigma_1^2 + ||\vthe_{(K+1):d}||^2) \vI, \\
    %%%%%%%%%%%%%%%%%%%%%%%%
    \Mean \big( \vr_i \big) &= \vzero\\
    %%%%%%%%%%%%%%%%%%%%%%%%
    cov \big( \vr_i \big)
    &= \Mean\big(
    cov\big(\vr_i  | \vthe \big)
    \big)
    +
    cov\big(
    \Mean\big(\vr_i | \vthe \big)
    \big)\\
    &= \big(\sigma_1^2 + \Mean(||\vthe_{(K+1):d}||^2)\big) \vI + d^{-1} \vI\\
    &= \big(\sigma_1^2 + \Mean(||\vthe_{(K+1):d}||^2) + d^{-1}\big) \vI,
\end{align*}
where $\vthe_{1:K}$ is the first $K$ entries of $\vthe$, and $\vthe_{(K+1):d}$ is the remaining entries. 
Therefore, for OSFA and individual-TS, we use  $\normal\big(\vzero, 
\big(\sigma_1^2 + \Mean(||\vthe_{(K+1):d}||^2) + d^{-1}\big) \vI 
\big)$ as the prior; 
for meta-TS, we use $\normal\big(\vmu, (\sigma_1^2 + ||\vthe_{(K+1):d}||^2) \vI \big)$ as the \textit{unknown} prior, with $\vmu$ as an unknown parameter
, and use 
$ \Mean \big( \vr_i \big | \vthe) =  \vthe_{1:K} \sim \normal(\vzero, d^{-1}\vI)$ as the hyper-prior for $\vmu$; 
for linear-TS, we use $\normal(0, d^{-1}\vI)$ as the prior for the regression coefficients $\vthe$ and $\sigma_1^2 + \sigma^2$ as the variance term of the stochastic reward variable. 

\paragraph{Bernoulli bandits.}
According to our data generation model, based on the law of total expectation and the law of total variance, 
recall the discussion on the parameterization of Beta distributions in Appendix \ref{sec: beta_parameterization}
it is easy to verify that 
\begin{align*}
    \Mean \big( \vr_i \big | \vthe)  &= (\Mean(logistic(\vphi(\vx_1, a)^T \vthe)|\vthe), \dots, \Mean(logistic(\vphi(\vx_K, a)^T \vthe)|\vthe))^T \\
    %%%%%%%%%%%%%%%%%%%%%%%%
    cov \big( \vr_i \big | \vthe)
    &= \Mean\big(
    cov\big(\vr_i | \vx_i \big)
    \big | \vthe)
    +
    cov\big(
    \Mean\big(\vr_i | \vx_i \big)
    \big | \vthe)\\
    %&= c_b \vI + c_b' \vI\\
    &= diag(c_{b,1}, \dots, c_{b,K}) + diag(c'_{b,1}, \dots, c'_{b,K})\\
    %%%%%%%%%%%%%%%%%%%%%%%%
    \Mean \big( \vr_i \big) &= \frac{1}{2} * \vone\\
    %%%%%%%%%%%%%%%%%%%%%%%%
    cov \big( \vr_i \big)
    &= \Mean\big(
    cov\big(\vr_i  | \vthe \big)
    \big)
    +
    cov\big(
    \Mean\big(\vr_i | \vthe \big)
    \big), 
    % \\
    % &= \big(\sigma_1^2 + \Mean(||\vthe_{(K+1):d}||^2)\big) \vI + d^{-1} \vI\\
    % &= \big(\sigma_1^2 + \Mean(||\vthe_{(K+1):d}||^2) + d^{-1}\big) \vI
\end{align*}
where $c_{b,i} = \frac{\psi}{1 + \psi} \Mean_{\vx}(logistic(\vphi(\vx_i, a)^T \vthe) (1 - logistic(\vphi(\vx_i, a)^T \vthe))|\vthe)$, 
and $c_{b,i}' = var_{\vx}(logistic(\vphi(\vx_i, a)^T \vthe)|\vthe)$. 
We obtain these two quantities as well as $\Mean \big( \vr_i \big | \vthe)$ and 
$cov \big( \vr_i \big)$ 
via Monte carlo simulation, since there is no explicit form. 

Define $\psi(\mu, \sigma^2_2) = [\mu(1-\mu) / \sigma^2_2 - 1]^{-1}$.
% Let $\mu = 1 / 2$ and $\psi = 1 / (1 / (c_b + c_b') - 1)$. 
For OSFA and individual-TS, we use  $Beta\big(1 / 2, \psi(1/2, cov \big( \vr_i \big))\big)$ as the prior for each arm; 
for meta-TS, following the implementations in \cite{kveton2021meta}, we randomly pick a set of Beta distributions as candidates, with $Beta\big( \Mean \big( \vr_i \big | \vthe), \psi(\Mean \big( \vr_i \big | \vthe), cov \big( \vr_i|\vx_i \big)) \big)$ as one of them, and maintain a Categorical distribution over them, with the uniform one as the initial prior; 
Finally, for GLB-TS, we choose the TS algorithm proposed in \cite{kveton2020randomized}, and set the exploration parameter $\alpha = 1$ as in \cite{kveton2020randomized}. 
% use $\normal(0, d^{-1}\vI)$ as the prior for the regression coefficients (no variance term for the stochastic reward variable is needed). 
% as the hyper-prior



% In this section, we present results with $N = 40$ and $T_1 = \dots = T_N = T = 50$. 
% We consider two kinds of task sequence:
% (i) the episodic setting, where we begin to interact with the $(i + 1)$-th task only after we finish the $i$-th task, % the $T$ interactions with
% and (ii) the concurrent setting, where we interact with every task for their $t$-th time simultaneously, and then interact for the $(t + 1)$-th time. % with them
% We set $K = 10$, $p = 10$, $\sigma = 1$, and $\Cov = \sigma_3^2 \vI$ for some hyper-parameter $\sigma_3$. Here, $\sigma_3^2$ controls the magnitude of the random effect term, which indicates how useful the task-specific metadata are. 
% % some efforts here. 
% The metadata $\{\vx_i\}$ are randomly generated from the standard multivariate normal distribution and the coefficient vector $\vthe$ is sampled from $\mathcal{N}(0, d^{-1}\vI)$. 
% To set the prior for the four competing TS algorithms, we integrate out $(\vx,\vr)$ to specify the mean part and apply the law of total variance to specify the variance part. 


% $\vr_i \sim \normal(\vzero, )$
% Before all random seeds, we use the same $\vthe$ sampled from $\mathcal{N}(0, d^{-1}\vI)$. 

% \begin{equation}
%     \begin{split}
%             r_{i,a} &\sim Beta\big(logistic(\vphi(\vx_i, a)^T \vthe), \psi \big), \forall a \in [K],\\
%     % \vr_i &\sim Beta(logistic(\vPhi_i\vthe), \psi)\\
%     R_{i,t} &\sim Bernoulli \big(\sum_a \I(A_{i, t} = a) r_{i, a} \big), 
%     \end{split}
% \end{equation}

\subsection{Implementation Details}

\paragraph{Implementation of Meta-TS under the concurrent setting.}
The original meta-TS proposed in \cite{kveton2021meta} can only be applied to the episodic setting and does not fit in the concurrent setting. 
Based on their models, we derived the posterior and adapt meta-TS to the concurrent setting, as follows. 
For Gaussian bandits, meta-TS aims to learn the unknown parameter $\vmu_m = \Mean(\vr_i)$, and assumes 
$\vr_i \sim \normal \big(\vmu_m, \sigma^2_m \vI \big)$ for some known $\sigma^2_m$. 
See the last subsection for details. 
Therefore, given a dataset  $\mH = \{(A_{j}, R_{j}, \vx_{j}, i(j))\}$, the posterior of $\vmu_m$ can be derived as follows. 
The entries of $\vmu_m$ are independent. 
Let $\Bar{R}_{i,a}$ denote the mean observed reward for taking action $a$ in task $i$, and $n_{i,a}$ be the count. 
Then we have $\Bar{R}_{i,a} \sim \normal\big( \mu_{m,a}, \sigma_1^2 + \sigma^2 / n_{i,a} \big)$. 
Note the prior for $\mu_{m,a}$ is $\normal(0, d^{-1})$. 
Let $\sigma_{i,a} = \sqrt{\sigma_1^2 + \sigma^2 / n_{i,a}}$. 
We have 
\begin{align*}
    \prob \Big[ \mu_{m,a}  |\mH \Big] \sim \normal 
    \Big(\frac{\sum_i \Bar{R}_{i,a} / \sigma_{i,a}^2 }{\sum_i \sigma_{i,a}^{-2} + d}
    , (\sum_i \sigma_{i,a}^{-2} + d)^{-1}
    \Big), \forall a \in [K]
\end{align*}
Then, at each decision point, we sample one $\Tilde{\vmu}_m$, and treat $\vr_i \sim \normal \big(\Tilde{\vmu}_m, \sigma^2_m \vI \big)$ as the prior to proceed with a standard single-task Gaussian TS algorithm. 
We similarly modified meta-TS for the Bernoulli bandits. 
% \begin{align*}
%     \prob \Big[ \vmu_m  |\mH \Big]
%     &= \frac{\prob(\vmu_m) \prob(\mH|\vmu_m)}{\int_{\vmu_m} \prob(\vmu_m)
%     }\\
%     &= \frac{\prob(\vmu_m) 
%     \prod_i \prob(\vr_i|\vmu_m) \prob(\mH_i|\vr_i)
%     }{\int_{\vmu_m} 
%     \prob(\vmu_m) 
%     \prod_i \prob(\vr_i|\vmu_m) \prob(\mH_i|\vr_i)
%     }
% \end{align*}



\paragraph{Implementation of {\name}.}
For Bernoulli bandits, we use the Python package \textsf{PyMC3} and adopt a popular MCMC algorithm , NUTS \cite{hoffman2014no}. 
The acceptance rate is set as $0.85$, and the number of samples per time is set as $2000$. 
% The No-U-Turn Sampler
For the computationally efficient variant of {\name}, 
in both Gaussian bandits and Bernoulli bandits, 
we sample a new $\vthe$ at the end of interactions with a task under the sequential setting, and at the end of a round under the concurrent setting. 


==> Extension_Contextual.tex <==
\subsection{Extension to contextual bandits}\label{sec:extension_contextual}
In this section, we discuss several possible directions to extend the metadata-based multi-task bandit framework to contextual bandits. 
We consider the following formulation of contextual bandits (the other formulations can be similarly derived). 
For each task $i \in [N]$, at each decision point $t$, 
the agent choose an arm $A_{i,t} \in \mathcal{R}^p$, and then receive a stochastic reward $R_{i,t} \sim f(A_{i,t};\vbeta_i)$, where $\vbeta_i$ is a length-$d$ vector of unknown parameters associated with task $i$. 
Here, $A_{i,t}$ is a feature vector which is a function of the context and the pulled arm. 
In addition, each task has a $p$-dimensional feature vector $\vx_i$ (i.e., metadata). 
% observe a feature $S_{i,t}$, 

A straightforward extension of the methodology presented in the main text is to consider that $\vbeta_i$ is sampled from some conditional distribution on $\vx_i$. Specifically, for some conditional distribution function $g$, we consider the following hierarchical model: 
\begin{equation}\label{eqn:extension_contextual}
    \begin{split}
    \vthe &\sim \prob(\vthe),\\
    \vbeta_i &\sim g(\vx_i; \vthe),\\
    R_{i,t} &\sim f(A_{i,t}; \vbeta_i). 
    \end{split}
\end{equation}
As a concrete example, we consider the linear Gaussian case. Let  $\mThe = (\vthe_1, \dots, \vthe_d)$ be a $p \times d$ coefficeint matrix and $\Cov_{\vbeta}$ be some covariance matrix, we consider
\begin{align*}
    \vthe_j &\sim \normal(\vmu_{\vthe}, \Cov_{\vthe}), \forall j \in [d] \\
    \vbeta_i &\sim  \mThe^T \vx_i + \normal(\vzero, \Cov_{\vbeta}), \forall i \in [N]\\
    R_{i,t} &\sim A_{i,t}^T\vbeta_i + \normal(0,\sigma^2).
\end{align*}
% Let $\boldsymbol{A}_i = (A_{i,1}, \dots, A_{i,T_i})^T$, $\vR_i = (R_{i,1}, \dots, R_{i,T_i})^T$, $\vR = (\vR_1^T, \dots, \vR_N^T)^T$, and $\boldsymbol{Z} = (\boldsymbol{A}_1 \vx_1; \dots, \boldsymbol{A}_N \vx_N)$, we have 
% \begin{align*}
%     \vR| \{R_{i,t}\}, \{A_{i,t}\} \sim \normal\Big(\boldsymbol{Z}\vmu_{\vthe},
%     (\boldsymbol{Z}\vmu_{\vthe})  \Cov_{\vthe} (\boldsymbol{Z}\vmu_{\vthe})^T + diag(\boldsymbol{A}_1 \Cov_{\vbeta} \boldsymbol{A}_1^T, \dots, \boldsymbol{A}_N \Cov_{\vbeta} \boldsymbol{A}_N^T)
%     \Big), 
% \end{align*}
% with which we can then get the posterior of $\vthe$, denoted as $\prob(\vthe|\mH)$. 
The posterior of $\mThe$ can be similarly developed as in the main text using the property of Gaussian bilinear model. 
With a sample $\Tilde{\mThe}$ from $\prob(\mThe|\mH)$, 
we can interact with each task $i$ using a single-task TS with $\normal( \Tilde{\mThe}^T\vx_i, \Cov_{\vbeta})$ as the prior for $\vbeta_i$. 

% Since there are several types of formulation of contextual bandits
% We first recall the definition of contextual MAB in the multi-task setup:
% for each task $i \in [N]$, at each decision point $t$, 
% the agent observe a context $S_{i,t}$, choose an arm $A_{i,t} \in [K]$, and then receive a stochastic reward $R_{i,t} \sim f(S_{i,t}, A_{i,t};\vthe_i)$, where $\vthe_i$ is some unknown parameters associated with task $i$. 



% Second, our work can be extended to contextual bandits, 
% based on the idea of clustering of bandits \citep{gentile2014online, li2016collaborative} when the set of task instances is finite, or the idea of when the set is infinite. 

One possible concern about model \eqref{eqn:extension_contextual} is that, when the number of tasks is not large, a simpler model might be preferred. In that case, we can consider that $\vbeta_i$ is a deterministic function of $\vx_i$. 
\begin{align*}
    \vthe &\sim \prob(\vthe)\\
    \vbeta_i &= g(\vx_i; \vthe)\\
    R_{i,t} &\sim f(A_{i,t}; \vbeta_i).
\end{align*} 
In reinforcement learning, this formulation shares similar forms with contextual Markov decision process \cite{modi2018markov, modi2020no}. 
Now, the linear Gaussian case can be written as 
\begin{align*}
    \vthe_j &\sim \normal(\vmu_{\vthe}, \Cov_{\vthe}), \forall j \in [d] \\
    R_{i,t} &\sim A_{i,t}^T \mThe^T\vx_i + \normal(0,\sigma^2).
\end{align*}
Such a model can utilize the data from all tasks, while avoiding a naive pooling which assumes the coefficient vector of all tasks are the same. 
Indeed, this is a kind of varying-coefficient models in statistics \cite{fan2008statistical}. 
Low-rank assumption can also be considered in this bilinear problem. 

Finally, as another direction to derive a simpler model, we may consider the idea of clustering of bandits \citep{gentile2014online, li2016collaborative}, by assuming there is a set of $M$ task instances, and each task are drawn independently from them. 
The metadata contain information about the probability that one task belong to each cluster, through a function $g$. 
\begin{align*}
    \vthe &\sim \prob(\vthe),\\
    \vbeta_j &\sim \prob(\vbeta), \forall j \in [M]\\
    k_i &\sim g(\vx_i; \vthe), \forall i \in [N] \\
    \vbeta_i &= \sum_j \vI(k_i = j) \vbeta'_k, \forall i \in [N]\\
    R_{i,t} &\sim f(A_{i,t}; \vbeta_i), \forall i \in [N], \forall t \in [T_i]. 
\end{align*} 
Under appropriate model assumptions, the posterior can be obtained using approximate posterior inference tools. 

These three models are all built under our metadata-based multi-task bandit framework, and the corresponding multi-task TS algorithms can be similarly developed. 
The key idea is to leverage the metadata to describe the relations between bandit tasks, while allowing heterogeneity. 
% hierarchical Bayes
The choice between them reflects the bias-variance trade-off.



==> Extension_GP.tex <==
\section{Details and Extensions of the Method}\label{sec:appendix_Hierarchical}
% More on the Hierarchical Models

\subsection{Mean-precision parameterization of the Beta distribution}\label{sec: beta_parameterization}

We note that a Beta distribution has different parameterizations. 
In the most common parameterization, a Beta random variable $u \sim Beta(\alpha_1, \alpha_2)$ is specified by two shape parameters $\alpha_1$ and $\alpha_2$. 
We have 
\begin{equation*}
    \mu = \Mean(u) = \frac{\alpha_1}{\alpha_1 + \alpha_2}, \quad 
    var(u) = \mu (1 - \mu)\psi / (1 + \psi), 
\end{equation*}
where $\psi = 1 /(\alpha_1 +\alpha_2 )$ is the so-called precision parameter.
Alternatively, this Beta random variable can be fully specified by $(\mu, \psi)$. 
Given $(\mu, \psi)$, we have $\alpha_1 = \mu / \psi$ and $\alpha_2 = (1 - \mu) / \psi$. 
Given $(\mu, var(u))$, we have $\psi = [\mu(1-\mu) / var(u) - 1]^{-1}$. 

In BBLM, we adopt this mean-precision parameterization, with  $\Mean(r_{i,a}) = logistic(\vphi^T(\vx_i, a) \vthe)$ and the precision of $r_{i,a}$ equal to $\psi$, for any $i$ and $a$. 

% pi / phi_beta, (1 - pi) / phi_beta

% \begin{equation*}
%     \begin{split}
%             r_{i,a} &\sim Beta\big(logistic(\vphi^T(\vx_i, a) \vthe), \psi \big), \forall a \in [K],\\
%     % \vr_i &\sim Beta(logistic(\vPhi_i\vthe), \psi)\\
%     R_{i,t} &\sim Bernoulli \big(\sum_a \I(A_{i, t} = a) r_{i, a} \big), 
%     \end{split}
% \end{equation*}

\subsection{Extension to Mixed-Effect Gaussian Process for Gaussian Bandits}\label{sec:GP}
In this section, we introduce an extension of the method developed in Section \ref{sec:LMM} to the Gaussian process setting. 
In such a setup, the function $f(\vx) = \Mean(\vr_i|\vx_i = \vx)$ is a continuous function sampled from a Gaussian process. 
Specifically, for each action $a \in [K]$, we have a specified mean function $\mu_a : \mR^p \rightarrow \mR$ and a kernel function $\mathcal{K}_a : \mR^p \times \mR^p \rightarrow \mR$. 
Let $\mathcal{GP}(\mu_a, \mathcal{K}_a)$ denote the corresponding Gaussian process. 
We consider the following mixed-effect Gaussian process model: 
% for the associated Gaussian process
% \begin{equation}
% \begin{split}
%     f_a &\sim \mathcal{GP}(\mu_a, \mathcal{K}_a), \forall a \in [K]; \\
%     % \delta_{i,a} &\sim \mathcal{N}(0, \sigma_1^2), \forall i \in [N], a \in [K]\\ 
%     % r_{i,a} &= f_a(\vx_i) + \delta_{i,a}, \\
%     r_{i,a} &\sim \mathcal{N}(f_a(\vx_i), \Cov^2), \forall i \in [N], a \in [K]; \\
%     %\stackrel{i.i.d.}
%     % \delta_{i,a} &\sim \mathcal{N}(0, \Cov^2)\\
%     R_{i, t} &= \sum_a \mathbb{I}(A_{it} = a)r_{ia} + \epsilon_{it}.
% \end{split}
% \end{equation}

\begin{equation}\label{eqn:GP}
\begin{split}
    f_a &\sim \mathcal{GP}(\mu_a, \mathcal{K}_a), \forall a \in [K]; \\
    % \delta_{i,a} &\sim \mathcal{N}(0, \sigma_1^2), \forall i \in [N], a \in [K]\\ 
    % r_{i,a} &= f_a(\vx_i) + \delta_{i,a}, \\
    \vdelta_i &\sim \mathcal{N}(0, \Cov) , \forall i \in [N];\\ 
    \vr_{i} &= \vf(\vx_i) + \vdelta_i, \forall i \in [N], 
    % \\
    % %\stackrel{i.i.d.}
    % % \delta_{i,a} &\sim \mathcal{N}(0, \Cov^2)\\
    % R_{i, t} &= \sum_a \mathbb{I}(A_{it} = a)r_{i,a} + \epsilon_{it}.
\end{split}
\end{equation}
where $\vf(\vx) = (f_1(\vx), \dots, f_K(\vx))^T$. 
% The model can be straightforwardly extended to allow the K GPs to be correlated. 

To design the corresponding TS algorithm, we essentially need to derive the corresponding posterior for $\{\vr_i\}$. 
We begin by introducing some notations. 
The model \eqref{eqn:GP} induces a kernel function $\mathcal{K}$, such that for any two tuples $O = (a, r, \vx, i)$ and $O' = (a', r', \vx', i')$, we have 
\begin{equation*}
    \mathcal{K}(O, O') = \sum_a \mathcal{K}_a(\vx, \vx') \mathbb{I}(a = a') +  \Cov_{a, a'} \mathbb{I}(i = i'). 
\end{equation*}
% We sort the dataset  $\mathcal{H}$ as $\{(A_j, R_j, i(j))\}$, where $A_j, R_j$, and $i(j)$ is the action, reward, and task index for the $j$-th tuple in $\mathcal{H}$. 
Let $\mK$ be an $n \times n$ kernel matrix of the pairwise kernel values for tuples in $\mathcal{H}$. 
Set $\vR = (R_1, \dots, R_n)^T$ be an $n$-dimensional vector of the observed rewards and $\vmu = 
(\mu_{A_1}(\vx_{i(1)}), \dots, \mu_{A_n}(\vx_{i(n)}))^T$. 
Finally, we use $\vI$ to denote an identity matrix, the  dimension of which can be inferred from the context. 


% and $\vPhi$ be a $n \times d$ feature matrix with the $j$-th row be the feature vector $\vphi^T(\vx_{i}, A_{i,t})$ of the $j$-th tuple in $\mathcal{H}$. 



% For the $i$-th task, let $\vr_i = (r_{i,1}, \dots, r_{i, K})^T$. 
% \textbf{Posterior  updating.}
Define a $K \times n$ matrix $\boldsymbol{M}_i$, such that the $(a, j)$-th entry of $\boldsymbol{M}_i$ is 
$\mathcal{K}_a(\vx_i, \vx_{i(j)}) \mathbb{I}(a = A_j) + \Cov_{A_j, a} * \I(i(j) = i)$, and define a $K \times K$ diagonal matrix $\mK_i$ with the $a$-th diagonal entry be $\mathcal{K}_a(\vxi, \vxi)$. 
Let $\vmu_i = (\mu_{1}(\vx_{i}), \dots, \mu_{K}(\vx_{i}))^T$. 
The posterior of $\vr_i$ conditional on the accumulated data follows a multivariate normal distribution, with mean and covariance given by: 
\begin{equation}\label{eqn:post_GP}
    \begin{split}
        \mathbb{E}(\vr_i|\mathcal{H}) &= \vmu_i + \boldsymbol{M}_i (\mK + \sigma_1^2 \vI)^{-1} (\vR - \vmu),  \\
        cov(\vr_i | \mathcal{H}) &= (\mK_i + \Cov) - \boldsymbol{M}_i (\mK + \sigma_1^2 \vI)^{-1} \boldsymbol{M}_i^T. 
    \end{split}
\end{equation}
The posterior will then be used to sample an action according to its probability of being the optimal one, in a Thompson sampling manner, as detailed in Algorithm \ref{alg:TS}. 
% Therefore, the MTTS algorithm  
% $A_{i,t}$

% The hyper-parameter updating step can be solved as the MLE of the following regression problem: 
% \begin{equation*}
%     \vR \sim \mathcal{N}(\vmu, \mK(\Cov, \gamma) + \sigma_1^2 \vI), 
% \end{equation*}
% where $\gamma$ is the bandwidth of the kernel function. 
% Q: the other hyper-parameters?

\subsection{Adaptive hyper-parameter updating with empirical bayes}\label{sec:appendix_hyper_updating_EB}
Following the literature \cite{kveton2021meta, agrawal2013thompson}, 
we assume the variance components as known for the two examples in Section \ref{sec:method}. 
In practice, we can apply empirical Bayes to update these hyperparameters adaptively. 
We take the LMM as an example. 
As discussed in Section \ref{sec:LMM}, our model requires four hyperparametes: $\vmu_{\vthe}$, $\Cov_{\vthe}$, $\sigma$, and $\Cov$. 
Among them, $\vmu_{\vthe}$ and  $\Cov_{\vthe}$, the prior parameters of $\vthe$, can be specified as any appropriate values according to domain knowledge, and will not affect our algorithm as well as its regret bound. 
For $\sigma$ and $\Cov$, similar with the approach commonly adopted in the literature on Gaussian process \citep{tomkins2019intelligent, rasmussen2003gaussian}, 
they can be learned from the data. 
Specifically, we can specify them as the maximizer of the marginal likelihood with respect to $(\sigma, \Cov)$, marginalized over $\vthe$ and $\{\vdelta_i\}_{i \in [N]}$. 
% $\{\delta_{i,a}\}_{i \in [N], a \in [K]}$. 
The log marginal likelihood can be derived as 
\begin{equation}\label{eqn:Hyper-parameter}
\begin{split}
l(\sigma, \Cov|\mathcal{D}) 
= -\frac{1}{2} \Big[ (\vR - \vPhi \vmu_{\vthe})^T (\mK(\Cov) + \sigma^2 \vI)^{-1}(\vR - \vPhi \vmu_{\vthe}) + log|\mK(\Cov) + \sigma^2 \vI|
+ N log(2\pi)  \Big], 
\end{split}
\end{equation}
where $\mK(\Cov)$ indicates the dependency of $\mK$ on $\Cov$. 
Note that $\Cov$ controls the degree of heterogeneity conditional on the metadata. % among tasks
Such an Empirical Bayes \citep{carlin2000bayes} approach makes sure our method is  adaptive to the prediction power of the metadata. 


\input{Extension_Contextual}

==> Figures/Figures_Gaussian.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square4_p_raw10_orderconcurrent.png}
         \caption{Concurrent, $\sigma_3 = 5$}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square1_p_raw10_orderconcurrent.png}
         \caption{Concurrent, $\sigma_3 = 1$}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square0.25_p_raw10_orderconcurrent.png}
         \caption{Concurrent, $\sigma_3 = 0.2$}
         \label{fig:five over x}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square4_p_raw10_orderepisodic.png}
         \caption{Episodic, $\sigma_3 = 5$}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square1_p_raw10_orderepisodic.png}
         \caption{Episodic, $\sigma_3 = 1$}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square0.25_p_raw10_orderepisodic.png}
         \caption{Episodic, $\sigma_3 = 0.2$}
         \label{fig:five over x}
     \end{subfigure}
\caption{
The average regret and its $95\%$ confidence interval, aggregated over 100 random seeds. 
The regret of OSFA is at least an order of magnitude higher than that of the others and hence not reported. 
}
\label{fig:simu_Gaussian}
\end{figure}


\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/one_cluster.png}
         \caption{Episodic, $\sigma_3 = 5$}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/one_cluster.png}
         \caption{Episodic, $\sigma_3 = 1$}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/one_cluster.png}
         \caption{Episodic, $\sigma_3 = 0.2$}
         \label{fig:five over x}
     \end{subfigure}
\caption{
\textbf{Placeholder for Binary}
}
\label{fig:simu_Binary}
\end{figure}


==> LMM_implemetation.tex <==
% \section{More details about the experiments}
% \section{Implementation}
\section{Implementation}\label{sec:appendix_Implementation}
In this section, we discuss efficient ways to implement {\name}, and analyze its computational complexity. 
We use $\vI$ to denote identity matrix, the dimension of which can be inferred from the context. 
% and $\vJ$ to denote an all-one matrix

\subsection{Efficient Implementation for Gaussian bandits with LMM}\label{sec:appendix_implementation_gaussian}

At each decision point, the computation will be dominated by the calculation of the matrix inverse for $(\mK + \sigma^2 \vI)$, which suffers from a cubic complexity $O(n^3)$ as well-known in the Gaussian process literature \cite{shi2012mixed}. 
% Step \eqref{eqn:post} and \eqref{eqn:Hyper-parameter} are both closely related with the kernel function and the matrix inverse. 
To alleviate the computational burden, we utilize the block structure induced by the mixed effect model via using the well-known Woodbury matrix identity \citep{rasmussen2003gaussian}, which is reviewed as follows. 
\begin{lemma}[Woodbury matrix identity] For any matrix $W$ and any invertible matrices $Z$, $U$, and $V$ with appropriate dimensions, the following relationship holds:
\begin{equation*}
    (\mZ + \mU\mW\mV^T)^{-1} = \mZ^{-1} - \mZ^{-1}\mU(\mW^{-1} + \mV^T\mZ^{-1}\mU)^{-1}\mV^T\mZ^{-1}
\end{equation*}
% Similarly, for the matrix determinant, we have $|\mZ+\mU \mW \mV^T| = |\mZ||\mW||\mW^{-1} + \mV^T\mZ^{-1}\mU|$.
\end{lemma}



% , and each entry of $\vJ_{i}$ is the corresponding entry of $\Cov$. 
% Specifically, we have $\vJ = diag(\vJ_{11}, \dots, \vJ_{1K}, \vJ_{21}, \dots, \vJ_{NK})$, where 
% $\vJ_{i,a}$ is an all-ones matrix whose dimension equal to the $\#\{(A_j, R_j, i(j)) \in \mathcal{D}: A_j = a, i(j) = i\}$. 
We start by writting $\mK = \vPhi \Cov_{\vthe} \vPhi^T + \vJ$. 
Without loss of generality, we can rearrange the tuples in $\mathcal{D}$ so that $\vJ$ becomes a block diagonal matrix as $\vJ = diag(\vJ_{1}, \dots, \vJ_{N})$, where $\vJ_{i}$ is the submatrix for task $i$. 
% or even (i,a) when \Sigma_delta is diagonal
The dimension of $\vJ_{i}$ equals to $\#\{(A_j, R_j, \vx_{i(j)}, i(j)) \in \mathcal{D}: i(j) = i\}$ and it is a pairwise kernel matrix 
induced by the kernel $\Tilde{\mathcal{K}}(O, O') = \Cov_{a, a'}$. 
Therefore, we have
\begin{align*}
    (\mK + \sigma^2 \vI)^{-1} 
    &= (\vPhi \Cov_{\vthe} \vPhi^T + (\vJ + \sigma^2 \vI) )^{-1}\\
    &= (\vJ + \sigma^2 \vI)^{-1} \Big[
    \vI - \vPhi (\Cov_{\vthe}^{-1} + \vPhi^T  (\vJ + \sigma^2 \vI)^{-1} \vPhi)^{-1} \vPhi^T (\vJ + \sigma^2 \vI)^{-1} \Big], 
\end{align*}
the computation cost of which will be dominated by $(\vJ + \sigma^2 \vI)^{-1}$, which yields a block diagonal structure and hence the matrix inverse can be more efficiently computed. 
Suppose we already have 
$t_0$ interactions with each of $N$ tasks. 
The computational cost is reduced from 
$O(N^3t_0^3)$ to $O(Nt_0^3)$. 
In addition, when $\Cov$ is diagonal, we can further apply the Woodbury matrix identity to compute $(\vJ_{i} + \sigma^2 \vI)^{-1}$. 
\newcommand{\JsigmaInv}{(\vJ + \sigma^2 \vI)^{-1}}

Furthermore, 
to make the computation more efficient, we define $\Cov_{in} = (\Cov_{\vthe}^{-1} + \vPhi^T  \JsigmaInv \vPhi)^{-1}
, \vJ_{\vPhi} = \JsigmaInv \vPhi
, \Tilde{\vR}= (\vR - \vPhi \vmu_{\vthe})
, \vJ_{\vR} = \JsigmaInv \Tilde{\vR}$. 
Next, we define 
\begin{align*}
\vJ_{\vPhi,\vR} &= \vPhi^T \JsigmaInv \Tilde{\vR}\\
\vJ_{\vPhi, \vPhi} &= \vPhi^T \JsigmaInv \vPhi\\
\vJ_{\vPhi, \vM, i} &= \vM_i \JsigmaInv \vPhi\\
\vJ_{\vR, \vM, i} &= \vM_i \JsigmaInv \Tilde{\vR}\\
\vJ_{\vM, i} &= \vM_i \JsigmaInv \vM_i^T. 
\end{align*}
For these components, we can efficiently utilize the block structure to only update the corresponding part. 
Finally, we have 
\begin{equation*}
    \begin{split}
        \mathbb{E}(\vr_i|\mathcal{D}) 
        % &= \vPhi_{i} \vmu_{\vthe} + (\vPhi_i\Cov_{\vthe}\vPhi^T + \vM_i) \JsigmaInv \Big[\vI -  \vPhi \Cov_{in} \vPhi^T \JsigmaInv\Big] \Tilde{\vR}  \\
        % &= \vPhi_{i} \vmu_{\vthe} + (\vPhi_i\Cov_{\vthe}\vPhi^T + \vM_i) \JsigmaInv \Big[\Tilde{\vR} -  \vPhi \Cov_{in} \vJ_{\vPhi,\vR} \Big]  \\
        &= \vPhi_{i} \vmu_{\vthe} 
        + \vPhi_i\Cov_{\vthe}\vJ_{\vPhi,\vR}
        + \vJ_{\vR, \vM, i}
        - \vPhi_i\Cov_{\vthe} \vJ_{\vPhi, \vPhi} \Cov_{in} \vJ_{\vPhi,\vR}
        - \vJ_{\vPhi, \vM, i} \Cov_{in} \vJ_{\vPhi,\vR},  \\
        cov(\vr_i | \mathcal{D}) 
        % &= (\vPhi_{i} \Cov_{\vthe} \vPhi_{i}^T + \Cov) - (\vPhi_i\Cov_{\vthe}\vPhi^T + \vM_i) \JsigmaInv \Big[\vI - \vPhi \Cov_{in} \vJ_{\vPhi}^T \Big] (\vPhi_i\Cov_{\vthe}\vPhi^T + \vM_i)^T\\
        &= (\vPhi_{i} \Cov_{\vthe} \vPhi_{i}^T + \Cov) 
        - \vJ_{\vM, i} 
        - (\vPhi_{i} \Cov_{\vthe}) \vJ_{\vPhi, \vPhi}  (\vPhi_{i} \Cov_{\vthe})^T
        % - \vPhi_{i} \Cov_{\vthe} \vJ_{\vPhi, \vPhi} 
        - \vPhi_{i} \Cov_{\vthe} \vJ_{\vPhi, \vM, i}^T
        - (\vPhi_{i} \Cov_{\vthe} \vJ_{\vPhi, \vM, i}^T)^T\\
        &\quad +  (\vPhi_i\Cov_{\vthe}\vJ_{\vPhi, \vPhi} + \vJ_{\vPhi, \vM, i})  \Cov_{in} 
         (\vPhi_i\Cov_{\vthe} \vJ_{\vPhi, \vPhi} + \vJ_{\vPhi, \vM, i})^T\\
    \end{split}
\end{equation*}

% The hyper-parameter updating step can be solved as the MLE of the following regression problem: 
% \begin{equation*}
%     \vR \sim \mathcal{N}(\vPhi \vmu_{\vthe}, \mK(\Cov) + \sigma^2 \vI)
% \end{equation*}
% % which can be solved by GP regression softwares. Refer to \citet{tomkins2019intelligent} for more details. 
% Similar trick can apply to the hyper-parameter updating step. 
% To compute $|\mK(\Cov) + \sigma^2 \vI|$, we have
% \begin{align*}
%     |\mK(\Cov) + \sigma^2 \vI| 
%     &= |(\vPhi \Cov_{\vthe} \vPhi^T + (\vJ + \sigma^2 \vI) )| \\
%     &= |( \vJ + \sigma^2 \vI)| * |\Cov_{\vthe}|  * |(\Cov_{\vthe})^{-1} + \vPhi^T (\vJ + \sigma^2 \vI)^{-1} \vPhi|. 
% \end{align*}
% Again, the block diagonal structure can be utilized to largely reduce the computation cost. 

% We might need to use GPytorch for implementation. 
% The code \footnote{https://github.com/StatisticalReinforcementLearningLab/intelligent\_pooling} for \citet{tomkins2019intelligent} might be a good example. 
% We may need to take a look at \citet{tomkins2020intelligentpooling} to learn more about the implementation tricks. 
% If the scalability is an issue, we may need to consider some approximate solution. 

% Efficient

\paragraph{Alternative implementation.}
For the $\vthe$-centered sampling scheme (e.g., Algorithm \ref{alg:TS_faster_general}), note that 
\begin{align*}
    &\vthe | \mH \sim \mathcal{N}\Big(\Tilde{\Cov}(\vPhi^T \mV^{-1}\vR + \Cov_{\vthe}^{-1}\vmu_{\vthe}), \Tilde{\Cov}\Big),\\
    &\Tilde{\Cov} = (\vPhi^T \mV^{-1} \vPhi + \Cov_{\vthe}^{-1})^{-1}, \mV = \sigma^2 \vI_n + \vJ, %\Cov_{\delta}, 
\end{align*}
where the dominating step is still to compute $\mV^{-1}$, and similar tricks can be applied. 
As a special case, consider $\Cov = \sigma_1^2 \vI$. 
We rearrange $\vJ$ as $diag(\vJ_{1,1}, \dots, \vJ_{1,K}, \dots, \vJ_{N,1}, \dots, \vJ_{N,K})$, where $\vJ_{i,a} = \sigma_1^2 \vone \vone^T$, and apply similar rearrangement to $\vPhi$ and $\vR$. 
Hence we have $\mV^{-1} = (\sigma^2 \vI_n + \vJ)^{-1} = diag((\sigma^2  \vI + \vJ_{1,1})^{-1}, \dots, (\sigma^2  \vI + \vJ_{N,K})^{-1})$. 
According to the Woodbury matrix identity, we have $(\sigma^2 \vI +  \vJ_{i,a})^{-1} = \sigma^{-2}\vI - \sigma^{-4}(\sigma_1^{-2} + n_{i,a} \sigma^{-2})^{-1}\vone\vone^T$, where $n_{i,a}$ is the count that action $a$ is implemented for task $i$. 

After we sample one $\Tilde{\vthe}$, the prior of $\vr_i$ can then be updated as $\normal(\vPhi_i \Tilde{\vthe}, \Cov)$. 
Its posterior then follows from the standard normal-normal conjugate relationship. 

% \input{incremental_LMM}

\subsection{Computationally Efficient Variant of {\name} under General Settings}\label{sec:appendix_TS_general}

In Section \ref{sec:general_framework}, we discuss how to ease the computation when directly sampling from $\prob(\vr_i|\vx_i)$ is computationally heavy, and present the variant under the sequential setting. 
We present the variant under the general settings in Algorithm \ref{alg:TS_faster_general}. 
Specifically, it requires an updating frequency $l$ as a hyper-parameter, and will sample a new $\vthe$ once we have $l$ new data points. 
$\prob(\vthe|\mH)$ can be computed via various approximate posterior inference tools. 
% Here, $\prob(\vthe|\mH)$ can be updated incrementally, and various approximate posterior inference tools can be used to compute it. 

\input{Algorithm/alg_TS_faster_general}

\subsection{Implementation for Bernoulli bandits with BBLM}\label{sec:appendix_implementation_Bernoulli}
In this section, we discuss our implementation of {\name} for Bernoulli bandits, under the BBLM introduced in \eqref{eqn:BBLM}. 
It follows Algorithm \ref{alg:TS_faster_general}. 

% introduce an computationally efficient variant
% We require an updating frequency $l$ as a hyper-parameter, and will sample a new $\vthe$ once we have $l$ new data points. 
Still, the dominating step is to sample from $\prob(\vthe| \mH)$. 
Fortunately, the model yields a nice hierarchical structure, where 
the first term essentially requires us to fit a Beta-logistic regression, and the second term is the likelihood of a simple binomial distribution, with a beta conjugate in our case. 
Specifically, 
note that $f(\vr_i|\vx_i, \vthe) = \prod_{a=1}^K f'_{Beta}(r_{i,a}|\vphi(\vx_i, a), \vthe)$, where $f'_{Beta}(r_{i,a}|\vphi(\vx_i, a), \vthe)$ is the density function of $Beta\big(logistic(\vphi(\vx_i, a)^T \vthe), \psi \big)$. 
Also note that, the likelihood for the Bernoulli distribution of task $i$ over $\mH_i$, as specified by the second equation of \eqref{eqn:BBLM}, is $\prob(\mH_i|\vr_i) = \prod_{a=1}^K r_{i,a}^{n_{i,a}}$, where $n_{i,a}$ is the number of times that action $a$ is selected for task $i$ in $\mH_i$. 
Both parts are computationally tractable. 
In our experiments, we use the MCMC algorithm implemented by the \textsf{Python} package \textsf{PYMC3} \cite{salvatier2016probabilistic} to compute the approximate posterior. 
% The full algorithm is described in Algorithm \ref{alg:TS_faster_binary}. 
% \input{Algorithm/TS_faster_binary}


\input{computational_complexity}

==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/1_Abstract.tex <==
\begin{abstract}
\vspace{-.1cm}
How to explore efficiently is a central problem in multi-armed bandits. 
In this paper, we introduce the metadata-based multi-task bandit problem, where the agent needs to solve a large number of related multi-armed bandit tasks and can leverage some task-specific features (i.e., metadata) to share knowledge across tasks. 
As a general framework, we propose to capture task relations through the lens of Bayesian hierarchical models, upon which a Thompson sampling algorithm is designed to efficiently learn task relations, share information, and minimize the cumulative regrets. 
Two concrete examples for Gaussian bandits and Bernoulli bandits are carefully analyzed. 
The Bayes regret for Gaussian bandits clearly demonstrates the benefits of information sharing with our algorithm. 
The proposed method is further supported by extensive experiments. 
\end{abstract}

% general


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/1_Intro.tex <==
\vspace{-.3cm}
\section{Introduction}\label{sec:Introduction}
\vspace{-.1cm}
The multi-armed bandit (MAB) is a popular framework for sequential decision making problems, where the agent will sequentially choose among a few arms and receive a random reward for the arm  \citep{lattimore2020bandit}. 
Since the mean rewards for the arms are not known \textit{a priori} and must be learned through partial feedbacks, the agent is faced with the well-known exploration-exploitation trade-off. 
% with the goal to maximize the cumulative reward.
MAB is receiving increasing attention and has been widely applied to areas such as clinical trials \citep{durand2018contextual}, finance \citep{shen2015portfolio}, recommendation systems \citep{zhou2017large}, among others. 


% there would be several candidate layouts, while the optimal layout may differ from page to page; 
% , while the best option is also not consistent; 
% price or inventory decision  % selling strategy
% , and there is typically large variance among individuals. 
% , especially when the allowed round of interactions is limited, as in
% pool information for each individual
% race, age, gender. Needs to be personalized to each patient according to its response history
% precision medicine? previous interaction and feedback? not sure...
% in web page design, the company needs to choose the optimal layout for each page from several options; 
How to explore efficiently is a central problem in MAB. 
% In the era of big data, i
In many modern applications, we usually have a large number of separate but related MAB tasks. 
For example, in e-commerce, the company needs to find the optimal display mode for each of many products, and in medical applications,  % clinical trials
each patient needs to individually undergo a series of treatment periods to find the personalized optimal treatment. % dose or
These tasks typically share similar problem structures, but may have different reward distributions. % improve the efficiency and
Intuitively, appropriate information sharing can largely speed up our learning process and reduce the regret, while a naive pooling may cause a linear regret due to the bias. 
% which is known as \textit{negative transfer} \cite{zheng2019metadata, sodhani2021multi}. 
% inductive bias
% we are learning the task relations. 

% judiciously
% while avoiding the potential bias induced by a naive pooling?
% , since a poor pooling will again result in either bias or additional regret due to information loss.  of this problem
% and emphasize

% One limitation of existing MTRL methods is the inability to leverage side information (or metadata), like the description of a task, to learn generalizable skills and transfer com- mon knowledge across tasks. Such metadata is often avail- able in real-world tasks but is not leveraged in the typical MTRL setting. This

% characterize  some
% in the literature; to be reviewed in
% In this work, we propose to additionally leverage 
% intrinsic information valuable
% additionally focus on the usefulness of \textit{task-specific features} (a.k.a. \textit{metadata}), which contains some \textit{static} meta information of each task. 
% In this work, we additionally focus on the usefulness of \textit{task-specific features} (a.k.a. \textit{metadata}), which contains some \textit{static} meta information of each task. 
This paper is concerned with the following question: \textit{given a large number of MAB tasks, how do we efficiently share information among them?} 
The central task is to capture task relations in a principled way \cite{zheng2019metadata}. 
While a few approaches have been proposed (see Section \ref{sec:Related Work}), most of them only utilize the action-reward pairs observed for each task. 
To our knowledge, none of the existing works can leverage another valuable information source, i.e.,  the \textit{metadata} of each task, which contains some \textit{static} task-specific features. 
Such metadata is commonly available in real applications \cite{you2016metadata, zheng2019metadata, sodhani2021multi}, such as the demographic features of each customer or patient, or basic information of each web page or product. 
Although the metadata can hardly be directly utilized in a single MAB task, 
it usually contains intrinsic information about each task, and hence can guide us to learn task relations and efficiently share knowledge in the multi-task setup. 
% is important in the multi-task setup. 
% and also task relations
% , and can guide us to efficiently learn task relations and share knowledge in the multi-task setup. 
Specifically, suppose task $i$ has a feature vector $\vx_i$ (i.e., metadata) and its expected reward vector for all arms is $\vr_i$. 
We consider a general formulation that $\vr_i$ is sampled from the conditional distribution $\prob(\vr_i|\vx_i)$. 
When $\prob(\vr_i|\vx_i)$ is informative, 
% allow efficient information sharing, is known and
the metadata, being appropriately utilized, can guide our exploration and hence reduce the regret. 
Several specific cases of $\prob(\vr_i|\vx_i)$ are illustrated in Figure \ref{fig:demo}. 
% our setting
% of a bandit algorithm
% We focus on two important information sources: \textit{task-specific features}, which contains some \textit{static} information of each task and can characterize the task relations, and \textit{task-specific history}, which contains past action-reward pairs from each task. 
% Instead of imposing a restrictive model $\vr_i = f(\vx_i)$ for a deterministic function $f$, 

% To further illustrate the motivations, 
 % certain confidence
 
\input{Figures/demo}

As one of our motivating examples, consider that a company needs to learn about the personal preference of many users over several options (e.g., message templates), via sequential interactions with each user. 
Suppose some user features (e.g., gender, age, geography) are informative in predicting the preference.  Then, even before any interactions with a specific user, we can predict her preference with high probability, based on her features and our experience with other users. 
Such knowledge can be concisely encoded as $\prob(\vr_i|\vx_i)$. 
However, $\vr_i$ typically can not be fully determined by $\vx_i$. 
Given the possible heterogeneity of $\vr_i$ conditional on $\vx_i$, the true reward distribution (and optimal arm) of this specific user still needs to be learned and confirmed via interactions with herself. 
Therefore, we must carefully utilize these features in a multi-task algorithm. %bandit
Indeed, we conjecture this is one way how humans adapt to tasks effectively, by constructing a rough first impression according to features, and then adjusting the impression gradually in the following interactions. 

% [\textit] previous
% For example, in clinical trials, two patients may exhibit similar demographic features and the initial treatment plan would be similar; while after several visitation, their responses might be quite different, which drives the necessity to adopt different strategy. 


% and can efficiently guide exploration and reduce the regret. 
% and the empirical performance of TS with a mis-specified prior 
% importance of prior; carefully 
% the performance of TS has been found  

% while minimizing the cumulative regrets; Towards this end, 
% the logic of this paragraph in the introduction. 
% 1. which end?
% 2. logic of this paragraph?
% Thompson sampling (TS) algorithm
To judiciously share information and minimize cumulative regrets, we design a multi-task bandit algorithm. % to share knowledge. 
Recall that, when $\prob(\vr_i|\vx_i)$ is known \textit{a priori}, a Thompson sampling (TS) algorithm \citep{russo2017tutorial} with $\prob(\vr_i|\vx_i)$ as the prior of $\vr_i$ for each task $i$ is known to be (nearly) optimal in Bayes regret, 
for a wide range of problems \citep{lattimore2020bandit}. 
However, such knowledge typically is absent, and 
many concerns have been raised regarding that TS is 
sensitive to the prior \citep{liu2016prior, honda2014optimality, metapricing,hamidi2020worst}. 
In this work, we aim to aggregate data from all tasks to construct an informative prior for each task. 
Specifically, we propose to characterize the task relations via a Bayesian hierarchical model, 
upon which the Multi-Task TS ({\name}) algorithm is designed to continuously learn $\prob(\vr_i|\vx_i)$ by aggregating data. 
% from all tasks. 
With such a design, {\name} yields a similar low regret to the oracle TS algorithm which knows $\prob(\vr_i|\vx_i)$ \textit{a priori}. 
In particular, the metadata $\vx_i$ allows us to efficiently capture task relations and share information. 
The benefits can be seen clearly from our experiments and analysis. 
% regret posit; hypothesize
% information-sharing structure between tasks

% , and hence judiciously share information among tasks to guide exploration. 
% , via an informative prior.   [??]

% address the multi-task problem through the lens of Bayesian hierarchical models. 

% efficient exploration applications
\textbf{Contribution.} \,
Our contributions can be summarized as follows. 
First of all, motivated by the usefulness of the commonly available metadata, we introduce and formalize the metadata-based multi-task MAB problem. 
The related notion of regret (multi-task regret) is defined, which serves as an appropriate metric for this problem. 
Second, we propose to address this problem with a unified hierarchical Bayesian framework, which characterizes the task relations in a principled way. % information-sharing structure between tasks
We design a TS-type algorithm, named {\name}, to continuously learn the task distribution while minimizing the cumulative regrets. % reward distributions MAB tasks
The framework is general to accommodate various reward distributions and sequences of interactions, and interpretable as one can study how the information from other tasks affects one specific task and how its metadata determines its prior. 
% it is clear how data from other tasks are utilized to facilitate one specific task. 
Two concrete examples for Gaussian bandits and Bernoulli bandits are carefully analyzed, and efficient implementations are discussed. 
Our formulation and framework open a door to connect the multi-task bandit problem with the rich literature on Bayesian hierarchical models. 
Third, we theoretically demonstrate the benefits of metadata-based information sharing, by deriving the regret bounds for {\name} and several baselines under a Gaussian bandit setting. 
Specifically, the average multi-task regret of {\name} decreases as the number of tasks grows, while the other baselines suffer a linear regret. 
Lastly, systematic simulation experiments are conducted to investigate the performance of {\name} under different conditions, which provides meaningful insights. 
% and demonstrates its superior performance. 
% since they fail to efficiently share knowledge


% As a multi-task algorithm, {\name} yields desired interpretability, as one can study how the information from other tasks affects one specific task, via investigating how its metadata determines its prior. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Outline
% We will first introduce the general framework in Section \ref{sec:general_framework}, and then  discuss two concrete and representative examples: 
% Bayesian linear mixed effect model for Gaussian bandits in Section \ref{sec:general_framework}, 
% and Beta-Binomial logistic model for Bernoulli bandits in Section \ref{sec:general_framework}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The advantage of our method over the CMAB approache and the meta bandit approach can be more clearly seen from the motivating example presented in Figure \ref{fig:demo}, 
% where we show the expected rewards for individual tasks (dots) and their expectation conditional on one feature (solid lines). 
% It can be seen that the feature is informative to predict the advantage of one arm over another, while there still exists huge heterogeneity even conditional on this feature. 
% In such a case, a meta bandit method would average the rewards over different feature values to construct a prior distribution for the new task, and hence loses information contained in this feature;  while a CMAB approach will simply rely on the solid line in Figure \ref{fig:demo} and make sub-optimal decisions for tasks whose best arm is not consistent with the general trend. 
% % for each arm
% % some tasks due to the bias. 
% % more explanation
% % huge variance? a bandit that will not converging? 
% Our method provides a more flexible solution:  
% it utilizes task-level features to share information, provides personalized recommendation for each individual task, and is adaptive to the degree of task relations. 
% % feature; heterogeneity
% % Middle ground between CMAB and ind. MABs. Use context (features) to share while also respect their heterogeneity. [*personalized CMAB*]
% % \hl{not one between them!}
% % bridges these two approach and

% % Contribution: a middle ground between the independent-task setting and the fully-polled setting. Compared with the former, more stable and with lower variance; compared with the latter, more flexible and with less bias. 


% In addition, in terms of the Bayes regret, we obtain a rate of order $O(N\sqrt{T}logT)$. 
% Although the linear dependency on $N$ is unavoidable under the problem setting that these tasks still yield some variance even conditional on their features, 
% in our numerical experiments, 
% we will show that the finite-sample performance of our method 
% improves significantly over the other competing methods. 
% will be much smaller than that of learning each task independently. 


% Naively treating these tasks as independent will ignore their common structure and lose useful information, while directly polling them. 
% In this work, we aim to utilize the task specific feature $\vx_i$. 
% Although these $N$ tasks are independent, we can assume they share some relations, captured by $\vx_i$. 
% personalized contextual bandit???


% \textbf{A concrete example (to be discussed).}
% One of our motivating example is the layout optimization tasks faced by many tech companies. 
% In such a task, there are usually several candidate layouts (arms), and 
% we need to find the optimal layout for each product so as to maximize some business metrics (rewards). 
% However, the optimal layout will vary among different products (tasks). 
% The product-specific features (features) (fixed effect), such as its category and average selling price, can partially guide us to find the best option, however there is typically still non-negligible heterogeneity (random effect) and we should figure out the product-specific optimal layout via exploration. 
% In this example, purely relying on the product-specific features may lead to sub-optimal decisions due to the bias and also does not utilize the experiment opportunities for each individual product, 
% while treating each task as independent will lose useful information can be shared among tasks. 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth, height=0.4\textwidth]{Figures/faceout.png}
%     \caption{1}
%     \label{fig:demo}
% \end{figure}


% However, in the multi-task setup where we need to interact with the same task for multiple times,  such an approach ignores the repeated measurement nature, which enables personalization to each individual task according to its own reward records. 
% Our approach can be regarded as adding a random effect term to address this issue. 

% The fact that we will interact with each task for multiple times allows us to further model the task heterogeneity conditional on these baseline features. 
% The above observations motivate us to propose a Bayesian linear mixed effect model in this multi-task setup. 
% , which allows sharing information among tasks , and also allows personalization to each individual task. 


% From a statistical perspective, the model of meta bandits can be regarded as a \textit{random effect model}, which assumes a hierarchical structure and regards the task-specific effects as random samples. 
% In contrast, the model in CMAB is a \textit{fixed effect model} \citep{baltagi2008econometric}, where the task-specific effects are fully captured by their features through a regression model.  
% To allow metadata-based information sharing while avoiding the potential bias induced by  purely relying on these features, 
% it is natural to consider combining these two approaches via a mixed effect model. 
% A \textit{mixed effect model} contains both a fixed effect term that captures the relations and a  random effect term that captures the heterogeneity, and it has been widely studied in the analysis of longitudinal data \citep{fitzmaurice2008primer}. 
% A review of related concepts is provided in Appendix \ref{sec:review-LMM}. 

% \begin{align*}
%     &\vr_i \sim \mathcal{P}_{\vr} & &\vr_i = f(\vx_i) & &\vr_i \sim \mathcal{P}_{\vr|\vx = \vx_i} \\
%       & \text{meta MAB} & & \text{contextual MAB} & & \text{Ours}
% \end{align*}

% The interactions with these tasks may happen concurrently or sequentially.


    % Specifically, we 
% Specifically, suppose there are $N$ tasks and the number of interactions per task is $T$, we 
% prove that our algorithm yields a multi-task regret of order 
% yields a Bayes regret of order $O(N\sqrt{T}logT)$. In contrast, naively applying the contextual MAB algorithms will suffer from a regret of  order $O(NT)$ due to the incurred bias. 
% In addition, the multi-task regret of our algorithm scales   sublinearly with $N$, the number of tasks.  
% In contrast, simply averaging information over tasks or applying the meta MAB algorithms will lead to a linear multi-task regret. 
% of order $O(N\sqrt{T}logT)$. 
% The regret for other baselines are also analyzed and compared. 
% at order $O(\sqrt{NT} logT)$,

% The multi-task regret of an algorithm is defined as its regret  compared to an oracle algorithm which knows the task distribution conditional on the task features, and it serves as an appropriate metric for this problem. 


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/2_Related_work.tex <==
\section{Related Work}\label{sec:Related Work}
\vspace{-.2cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% as displayed in Figure XX.  can be viewed  of
First of all, our setup subsumes the meta MAB problem \citep{hsu2019empirical, boutilier2020differentiable, kveton2021meta, kveton2021metalearning} as a special case, where $\vx_i$ degenerates to a constant. 
Meta MAB assumes the tasks arrive \textit{sequentially} and are drawn from one \textit{metadata-agnostic} distribution. 
Among these works, meta TS \cite{kveton2021meta} is the most related one, which assumes the mean reward vectors $\{\vr_i\}$ are i.i.d. sampled from some distribution $f(\vr;\vthe)$, and pool data to learn $\vthe$. 
% with unknown parameters $\vthe$. 
% improve the  performance for a new task, via either learning $\vthe$ \cite{kveton2021meta},  
%  with task-specific features
The other works either pool data from accomplished tasks to optimize algorithm hyper-parameters \cite{hsu2019empirical} or directly optimize the policy via policy gradient \cite{boutilier2020differentiable, kveton2021metalearning}. 
Compared with meta MAB, our setting is more general as we allow incorporating metadata to learn and capture  task relations, and also allow the interactions with different tasks to arrive in arbitrary orders. 
The former is particularly important when there exists significant heterogeneity among tasks (e.g., setting (c) in Figure \ref{fig:demo}), where a naive pooling may lose most information; 
the latter allows broader applications. 
The results developed in this paper are equally applicable to meta MAB. 
% the visitation of patients
% While to choose 
% Medical study
% - applications: current for layout and products, sequential for patients, random for customers.


% A detailed comparisons of the related literature can be found in Appendix XX. 
In addition to meta MAB, 
there are several other topics concerned with multiple bandit tasks. 
We review the most related papers in this section, and provide a comprehensive comparison with additional related works and concepts in Appendix \ref{sec:appendix_additional_related_work}. 
First of all, there is a large number of works on multi-agent bandits  \citep{kar2011bandit, cesa2016delay, wang2020optimal, dubey2020cooperative} studying that multiple agents interact with the same task concurrently. 
In contrast, we consider there is inter-task heterogeneity. 
Given such heterogeneity, certain approaches to capture task relations are then required: 
when there exist useful network structures between tasks, \cite{cesa2013gang} and \cite{vaswani2017horde} propose to utilize this knowledge to capture task relations; 
\cite{azar2013sequential} assumes there is a \textit{finite} number of task instances, considers the tasks arrive sequentially, and aims to transfer knowledge about this set of instances; 
\cite{wang2021multitask} assumes there exist pairwise upper bounds on the difference in reward distributions; 
clustering of bandits \citep{gentile2014online, li2016collaborative} and latent bandits \citep{hong2020latent, hong2020non} assume there is a perfect clustered structure, that tasks in the same cluster share the same reward distribution. % commonly available; capture task relations by
In contrast to all these setups, to our knowledge, this is the first work that can utilize metadata, an important information source that is commonly available. 
Besides, our modelling-based approach provides nice interpretability and is flexible to accommodate  arbitrary order of interactions. 
% built on the unified hierarchical Bayes framework, our approach is more flexible to accommodate various MAB tasks and arbitrary orders of interactions. 
Lastly, we learn task relations from data automatically, with arguably fewer structural assumptions. 
% , and the modelling-based approach also provides nice interpretability. 

% which exists in many real-world applications and typically contains useful information. 
% Bayesian hierarchical models provide a valuable view-point for meta-learning, by providing a modeling rather than an algorithmic framework for understanding the meta- learning process. In

% Transfer Learning in Bandits with Latent Continuity:
% Lipschitz constant: unknown.
% We are going to estimate it in a meta way.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the presence of task-specific features, 
another approach to pool information is to adapt contextual MAB (CMAB)  algorithms \citep{lu2010contextual, zhou2015survey, reeve2018k, arya2020randomized, srinivas2009gaussian, kveton2020randomized, li2017provably}, 
by neglecting the task identities and regarding the metadata as "contexts". % static features
Specifically, one can assume a \textit{deterministic} relationship $\vr_i = f(\vx_i;\vthe)$ for some function $f$, and then apply CMAB algorithms to learn $\vthe$. 
However, such a solution heavily relies on the \textit{realizability} assumption \cite{foster2020adapting},  
that $\vr_i = f(\vx_i;\vthe)$ holds exactly with no variation or error. 
When this assumption is violated, a linear regret is generally unavoidable. 
This limitation attracts increasing attention \cite{foster2020adapting,krishnamurthy2021tractable,krishnamurthy2021adapting}.  
In our setup, the agent will interact with each task multiple times and the metadata is fixed, which naturally enables us to relax this restrictive assumption by regarding $\vr_i$ as a random variable  sampled from $\prob(\vr_i|\vx_i)$. 
% the conditional distribution
% even conditional on $\vx_i$. 
% allowing  variations of $\vr_i$ conditional on $\vx_i$. 
To our knowledge, this is the first work that can handle the realizability issue via utilizing the repeated-measurement structure. 
% via Bayesian hierarchical models. 
% among a specified class; deterministic
% for some $f$
%  (e.g. a linear function)
% feature transformation? f() relationship? correct?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% essentially ignores the identity of each task. 
% , and hence is a fully-pooled setting. 
% To see the difference and drawbacks, suppose we have two tasks $i$ and $j$ with $\vx_i = \vx_j$, then in CB, the two tasks must have the same reward distribution; while our model allows them to have different distribution and utilize their own experiment data, hence is more suitable for this RI project and personalized medicine. 
% no focus on the multi-task



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Finally, there exists a rich literature on multi-task supervised learning (see \cite{zhang2017survey} for a survey), where hierarchical models \citep{luo2018mixed, shi2012mixed, wang2012nonparametric} are a popular choice, \cite{raina2006constructing, anderer2019adaptive, nabi2020bayesian} studied aggregating historical data to construct informative priors, and \cite{zheng2019metadata} considered leveraging  metadata to cluster tasks. 
% you2016metadata
Besides, this work is certainly related to single-task bandits. 
In particular, Thompson sampling is one of the most popular approaches with superior  performance \citep{agrawal2013further,russo2017tutorial,tomkins2020intelligentpooling,kveton2021meta,agrawal2013thompson,dumitrascu2018pg}. 
Its popularity is partially due to its flexibility to incorporate prior knowledge \cite{chapelle2011empirical}. 
We provide a data-driven approach to construct such a prior. 
Our work naturally builds on these two areas to provide an efficient solution to the metadata-based multi-task MAB problem. 
% the hierarchical models and TS
%  and bridges
% leverage commonly available context attributes in nowadays systems, i.e., the metadata.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Instead, in real applications, there are usually some task-specific features available, which can partially characterize the task relations and could help us predict the expected rewards. % for each individual task. 
% For example, products belonging to the same category or having similar average price may prefer similar layouts, and the optimal doses for patients of similar demographic features usually are closer. % with higher probability
% The existing meta bandits approaches fail to utilize these task-specific features to capture task relations. 
% , and when there are huge inter-task heterogeneity, such as when there are several task clusters, these methods will be less efficient. 




==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/3_Setup.tex <==
% Here, $r_{i, a}$ is the expected reward of taking action $a \in [K]$ for task $i \in [N]$
\vspace{-.2cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Metadata-based Multi-task MAB}\label{sec:setup}
\vspace{-.2cm}
In this section, we introduce a general framework for the metadata-based multi-task MAB problem. 
For any positive integer $M$, we denote the set $\{1, 2, \dots, M\}$ by $[M]$. 
Let $\mathbb{I}$ be the indicator function. 
Suppose we have a large number of $K$-armed bandit tasks with the same set of actions, denoted as $[K] = \{1, \dots, K\}$. 
Each task instance $i$ is specified by a tuple $(\vr_i, \vx_i)$, 
where $\vr_i = (r_{i,1}, \dots, r_{i,K})^T$ is the vector of mean rewards for the $K$ arms and $\vx_i$ is a $p$-dimensional vector of task-specific features (i.e., metadata). 
The metadata can include categorical and continuous variables, and even  outputs from pre-trained language or computer vision models \cite{devlin2018bert, li2019visualbert}. 
We assume these task instances are i.i.d. sampled from some unknown \textit{task distribution} $\mathcal{P}_{\vr, \vx}$, which induces a conditional distribution $\prob(\vr_i|\vx_i)$. 
We will interact with each task repeatedly. 
For each task $i$, at its $t$-th decision point, we choose one arm $A_{i,t} \in [K]$, and then receive a random reward $R_{i,t}$ according to $R_{i,t} = \sum_{a=1}^K \I(A_{i,t} = a) r_{i,a} + \epsilon_{i,t}$, where $\epsilon_{i,t}$ is a mean-zero error term.  

% metadata-based 
% emphasize
We call this setup \textit{multi-task MAB} to focus on the fact that there is more than one MAB task. 
New tasks may appear and interactions with different tasks may happen in arbitrary orders. 
When the tasks arrive in a sequential manner (i.e., task $i + 1$ begins only when task $i$ is  finished), our setup is an instance of \textit{meta learning} \cite{kveton2021meta, hsu2019empirical, baxter2000model, thrun1998lifelong}, which we refer to as the \textit{sequential} setting in this paper. 

Suppose until a time point, we have interacted with $N$ tasks, and for each task $i \in [N]$, we have made $T_i$ decisions. 
% Let the best arm for task $i$ be $a_i^* = \argmax_{a \in [K]} r_{i,a}$. 
The performance of a bandit algorithm can be measured by its 
\textit{Bayes regret}, % defined as 
\begin{equation*}%\label{def:BR}
  BR(N, \{T_i\}) =  \mathbb{E}_{\vx, \vr, \epsilon} 
        \sum\nolimits_{i \in [N]}  \sum\nolimits_{t \in [T_i]}
%   \sum_{i = 1}^N\sum_{t = 1}^{T_i} 
    ( 
    % r_{i, a_i^*} 
    max_{a \in [K]} \, r_{i,a}
    - r_{i,A_{i,t}}), 
\end{equation*}
%  max_{a \in [K]} \, r_{i,a}
% \vthe, the problem instance $\vthe$, 
% $(\vx, \vr)$ the prior over 
where the expectation is taken with respect to the task instances $\{(\vr_i, \vx_i)\}$, the random errors, the order of interactions, and the randomness due to the algorithm. 
Here, the metadata $\{\vx_i\}$ and the order of interactions enter the definition because they might affect the decisions of a multi-task algorithm. % feature-dependent 
When the algorithm does not share information across tasks, the definition reduces to the standard single-task Bayes regret \citep{lattimore2020bandit} accumulated over $N$ tasks. 
The Bayes regret is particularly suitable for multi-task bandits, under the task distribution view \cite{zhang2017survey, kveton2021meta}. 
% is naturally related to the task distribution view of multi-task bandits. 
% naturally related to
% We note that, although the Bayes regret is often regarded as 
% in the single-task setting, 
% it is appropaite when we consider a large number of tasks. 

% why BR? because of multi-task? natural! 
Given the existence of inter-task heterogeneity, the Bayes regret of any bandit algorithms will unavoidably scale linearly with $N$. 
We next introduce a new metric, refer to as the \textit{multi-task regret}, which allows us to clearly see the benefits of multi-task learning and can serve as an appropriate metric for multi-task bandit algorithms. 

To begin with, we first review Thompson sampling (TS), which is one of the most popular bandit algorithm framework  \citep{agrawal2013further,russo2017tutorial,tomkins2020intelligentpooling}. 
For each task $i$, the standard single-task TS algorithm requires a prior $Q(\vr_i)$ as the input, maintains a posterior of $\vr_i$, and samples an action according to its posterior probability of being the optimal one. 
% Not necessary in the main text (Alg 2)
We denote  $TS(Q(\vr))$ as a TS algorithm with some distribution $Q(\vr)$ as the prior. 
Most Bayes regret guarantees for TS require the specified prior is equal to the true distribution of $\vr$ \cite{russo2017tutorial,lattimore2020bandit}. 
When this condition is satisfied, it is well-known that this TS algorithm is (nearly) optimal for a wide range of problems \citep{russo2017tutorial,lattimore2020bandit}. 
% See Appendix \ref{supp-sec:oracle} for more details. 
In our setup, this assumption means that, for each task $i$, we will apply 
% TS with $\prob(\vr_i|\vx_i)$ as the prior. 
$TS\big(\prob(\vr_i|\vx_i)\big)$. 
It is natural to set such an (nearly) optimal algorithm as our skyline, which we refer to as \textit{oracle-TS}. 
% Not truly optimal. Just a skyline we choose 
% Theorem 2 is somewhat surprising in the context of that suggests
% that a  can result in very poor for prior-dependent Thompson Sampling
% (see, e.g., Honda and Takemura 2014, Liu and Li 2015, Hamidi and Bayati 2020). 

% the best a multi-task algorihtm can achieve in our setup
% empirical performance good. 
However, it is arguably a strong assumption that the agent can know $\prob(\vr_i|\vx_i)$ \textit{a priori}, and a growing literature finds that TS with a mis-specified prior can yield a poor regret due to over-exploration \citep{chapelle2011empirical, liu2016prior, honda2014optimality, russo2017tutorial,hamidi2020worst}. 
% The following arguments and definition is not that natural
% Therefore, it would be desired if a metadata-based multi-task MAB algorithm is able to aggregate data from tasks to learn $\prob(\vr_i|\vx_i)$, so as to yield similar regrets with oracle-TS. 
Therefore, a well-designed metadata-based multi-task MAB algorithm should be able to aggregate data to learn the task distribution pattern (i.e., $\prob(\vr_i|\vx_i)$), so as to yield similar low regrets with oracle-TS. 
Motivated by these discussions, 
we define the \textit{multi-task regret} of an algorithm as the difference between its Bayes regret and the Bayes regret of oracle-TS, which can be equivalently written as 
% the \textit{multi-task regret} relative to oracle-TS is defined as
% \vspace{-.2cm}
\begin{equation*}
      MTR(N, \{T_i\}) =  \mathbb{E}_{\vx, \vr, \epsilon} 
    %   \sum_{i = 1}^N \sum_{t = 1}^{T_i}
      \sum\nolimits_{i \in [N]}  \sum\nolimits_{t \in [T_i]}
      ( r_{i, A^\mathcal{O}_{i,t}} - r_{i, A_{i,t}}), 
    % \mathcal{O}(i)
\end{equation*}
where $A^\mathcal{O}_{i,t}$ is the action that oracle-TS takes, and the expectation is additionally taken over its randomness. 
This regret reflects the price of not knowing the prior \textit{a priori}, and measures the performance of a multi-task algorithm in learning the task distribution pattern while maintaining a low regret. 
% By definition, the multi-task regret of an algorithm is equal to its Bayes regret minus the Bayes regret of  oracle-TS.
A similar concept is defined in \cite{metapricing} for meta learning in dynamic pricing. %feature-agnostic

% For sub-gaussian. Or all? The results?

% The  multi-task regret provides an appropriate metric for the metadata-based multi-task MAB problem. 
% Similar concepts have been discussed in \cite{metapricing} and \cite{kveton2021meta} under the feature-agnostic meta bandits setting. 

% However, these tasks typically share some structural similarity, which can be partially captured by the $p$-dimensional task-specific feature vector $\vx_i$. 

% Q: is this the lower bound for any algorithms? 
% We are the first to establish? We can 



==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/4_1_General_framework.tex <==
% We will first introduce the general framework in Section \ref{sec:general_framework}, and then  discuss two concrete and representative examples. 
\subsection{General framework}\label{sec:general_framework}
% In this work, we propose to address the metadata-based multi-task MAB problem through the lens of Bayesian hierarchical models. 
To address the metadata-based multi-task MAB problem, 
in this section, 
we introduce a general hierarchical Bayesian framework to characterize the information-sharing structure among tasks, and design a TS algorithm that can continuously learn $\prob(\vr|\vx)$ and yield a low regret. 
For ease of exposition, we assume discrete probability spaces. 
Our discussion is equally applicable to continuous settings. 
Two representative examples are given in the following subsections. 
% concrete and -type
% multi-task
% (i.e., as if we know  $\prob(\vr_i|\vx_i)$ \textit{a priori}). 
% attain low regret compare to oracle-TS. 
% allow efficiently information sharing 
% does not need to know to minimize the Bayes regret. 
% for the setup introduced in Section XX, and then 
% [Some introduction about Bayesian hierarchical model]

% \begin{equation}\label{eqn:hierachical_model}
%   \begin{alignedat}{2}
% &\text{(Prior)} \quad
% \quad\quad\quad    \vthe &&\sim \prob(\vthe), \\
% &\text{(Inter-task)} \quad
% \;    \vr_i | \vx_i, \vthe &&\sim f(\vr_i | \vx_i, \vthe),  \\
% &\text{(Intra-task)} \quad
% \;    R_{i,t} &&= r_{i, A_{i,t}} + \epsilon_{i,t}. 
%     % \end{split}
%       \end{alignedat}
% \end{equation}

% to describe the distribution of the mean vector conditional on the features , 
% to describe the distribution of 
% where $\prob(\vr_i | \vx_i, \vthe)$ is 
To learn $\prob(\vr|\vx)$, we make a model assumption that $\vr_i$ is sampled from $f(\vr_i | \vx_i, \vthe)$, for a model $f$ parameterized by the unknown parameter $\vthe$. 
For example, in Gaussian bandits, $f(\vr_i | \vx_i, \vthe)$ can be the conditional density function of a linear model with Gaussian errors (see Section \ref{sec:LMM}). 
% or by a Beta-logistic model in Bernoulli bandits (See Section \ref{sec:binary}). 
We denote the prior of $\vthe$ as $\prob(\vthe)$. 
Therefore, our full model is the following Bayesian hierarchical model: 
\begin{equation}\label{eqn:hierachical_model}
  \begin{alignedat}{2}
&\text{(Prior)} \quad
\quad\quad\quad    \vthe &&\sim \prob(\vthe), \\
&\text{(Inter-task)} \quad
\;    \vr_i | \vx_i, \vthe &&\sim f(\vr_i | \vx_i, \vthe), \forall i \in [N],  \\
&\text{(Intra-task)} \quad
\;    R_{i,t} &&= \sum\nolimits_{a \in [K]} \I(A_{i,t} = a) r_{i,a} + \epsilon_{i,t}, \forall i \in [N], t \in [T_i]. 
    % \end{split}
      \end{alignedat}
\end{equation}
We note that $\prob(\vthe)$ is specified by the users, and our regret analysis is a worst-case frequentist regret bound with respect to $\vthe$. 
Besides, the inter-task layer clearly subsumes the meta MAB model $\vr_i|\vthe \sim f(\vr_i|\vthe)$ and the CMAB model $\vr_i = f(\vx_i;\vthe)$ as two special cases. 
% A review of related statistical concepts is provided in Appendix \ref{sec:review-LMM}. 
% . Our model can be regarded as a bridge of them to address the XXx problem, under the Bayesian setting. in Section \ref{sec:Theory} 

% If it is random, would be trivial?
% of size $n$

Suppose until a decision point,  
we have accumulated a dataset $\mH = \{(A_{j}, R_{j}, \vx_{j}, i(j))\}_{j=1}^n$, where the data for all tasks have been combined and re-indexed. 
Here, $i(j)$ is the task index for the $j$th tuple in $\mH$, $\vx_{j} = \vx_{i(j)}$ is its metadata, 
$A_{j}$ is the implemented action and $R_{j}$ is the observed reward. 
Suppose we need to make a decision for task $i$ at this time point. 
To adapt the TS algorithm, one needs to compute the posterior of $\vr_i$ as $\prob(\vr_i|\mH)$ according to the specified hierarchical model, sample a reward vector, and then act greedily to it. 
Based on this framework, we designed the Multi-Task Thompson Sampling ({\name}) algorithm, which is summarized as Algorithm \ref{alg:TS}. 

\input{Algorithm/alg_TS}

% The posterior will then be used to sample an action according to its probability of being the optimal one, in a Thompson sampling manner, as detailed in Algorithm \ref{alg:TS}. 
% posteriors for the expected rewards of arms in this task have analytic expressions. 


Algorithm \ref{alg:TS} is natural and general. 
Once a hierarchical model is specified, the remaining step to adapt {\name} is to compute the posterior $\prob(\vr_i | \mH)$. 
We will discuss two concrete examples in the following sections. 
Before we proceed, 
we remark that the posterior can be written as 
% one equivalent form of 
\begin{equation}\label{alternative_form}
    \prob(\vr_i | \mH) 
    % \\
    % &= \int_{\vthe} \prob(\vthe| \mH)  \prob(\vr_i|\vthe, \mH) d\vthe 
    % \propto  \prob(\mH_i|\vr_i)  \int_{\vthe} \prob(\vthe| \mH)  \prob(\vr_i|\vthe) d\vthe      \\
    = \int_{\vthe} \prob(\vthe| \mH)  f(\vr_i|\vthe,  \mH) d\vthe 
    \propto  \prob(\mH_i|\vr_i)  \int_{\vthe} \prob(\vthe| \mH)  f(\vr_i|\vx_i, \vthe) d\vthe, 
\end{equation}
where $\mH_i$ is the subset of $\mH$ that contains the history of task $i$. 
Note that $\prob(\mH_i|\vr_i)$ is the likelihood for task $i$ alone. 
Therefore, 
\eqref{alternative_form} provides a nice interpretation: 
up to a normalization constant, 
$\int_{\vthe} \prob(\vthe| \mH)  f(\vr_i|\vx_i, \vthe) d\vthe$ can be regarded as a prior for task $i$, and this prior will be continuously updated by pooling data based on the hierarchical model. 
Specifically, data from all tasks are utilized to infer $\vthe$ via $\prob(\vthe|\mH)$, which is then used to infer $\prob(\vr_i|\vx_i)$ through $f(\vr_i|\vx_i, \vthe)$. 
% stated in the introduction
% task-specific features
This is consistent with our motivations, that we would like to utilize the metadata $\{\vx_i\}$ to guide exploration (via the prior), while also using the task-specific history $\mH_i$ (via the likelihood $\prob(\mH_i|\vr_i)$). 
As a multi-task algorithm, {\name} yields desired interpretability, as one can study how the information from other tasks affects one specific task, via investigating how its metadata determines its prior. 
% The learned f function also provides some insights.
% but sampled. The main issue. 
% modelling-based approach
% task relations

% features affects the prior
% ; 
% {\name} also partially avoids the privacy concern by summarizing data into a vector $\vthe$, instead of sharing raw data. 
% Finally, we note that {\name} summarizes information into a vector $\vthe$ and hence partially avoids the privacy concern in multi-task learning.

% of an MAB algorithm
% combine (i) task-specific features, which allows us to learn $\prob(\vr_i|\vx_i)$ to guide exploration (via prior), and (ii) the task-specific history, which is utilized via the likelihood $\prob(\mH_i|\vr_i)$. 

% more
In addition, the relationship \eqref{alternative_form} suggests a computationally efficient variant of Algorithm \ref{alg:TS}. % way to implement
We note two facts: 
(i) it is typically more demanding to compute $\prob(\vthe| \mH)$ than $\prob(\mH_i|\vr_i) f(\vr_i|\vx_i,\vthe)$, since the former involves a regression problem and usually has no explicit form, while the latter usually has analytic solutions by choosing conjugate priors; 
(ii) according to \eqref{alternative_form}, to sample $\vr_i$ from $\prob(\vr_i | \mH)$, it is equivalent to first sample one $\Tilde{\vthe}$ from  $\prob(\vthe| \mH)$, and then 
sample $\vr_i$ with probability proportional to  $\prob(\mH_i|\vr_i) f(\vr_i|\vx_i, \Tilde{\vthe})$.
Therefore, when it is computationally heavy to sample $\prob(\vr_i | \mH)$ every time, we can instead sample $\Tilde{\vthe}$ from  $\prob(\vthe| \mH)$ at a lower frequency, and 
apply $TS\big(f(\vr_i|\vx_i, \Tilde{\vthe})\big)$ to task $i$ before sampling the next value of $\vthe$. 
% Here, $\prob(\vthe| \mH)$ can be updated incrementally. 
This variant can be regarded as updating the inter-task data pooling module in a batch mode, and it shows desired regret in our analysis and negligible costs in our experiments. 
Under the sequential setting, this variant is described in Algorithm \ref{alg:TS_faster}, and the general form is given in Appendix \ref{sec:appendix_TS_general}. 
See Section \ref{sec:binary} for a concrete example. 

% so no need to sample, actually

% $\prob(\vr_i|\Tilde{\vthe}, \vx_i)$ as the prior for $\vr_i$ to proceed with a standard single-task TS algorithm. 

% yu2020graphical


\input{Algorithm/alg_TS_faster}



==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/4_2LMM.tex <==
% can be some basis expansions or mannually designed.; a set of basis functions which are “rich” enough to approximate the underlying function

\subsection{Gaussian bandits with Bayesian linear mixed  models}\label{sec:LMM}
In this section, we focus on Gaussian bandits, where the error term $\epsilon_{i,t}$ follows $\mathcal{N}(0, \sigma^2)$ for a known parameter $\sigma$. 
We will first introduce a linear mixed model to characterize the information-sharing structure, 
and then derive the corresponding posterior. 
We use $\vI_m$ to denote an $m \times m$ identity matrix.  
Let $\vphi(\cdot, \cdot) : \mathbb{R}^p \times [K] \rightarrow  \mathbb{R}^d$ be a known map from the metadata-action pair to a $d$-dimensional transformed feature vector, and let $\vPhi_{i} = (\vphi(\vx_i, 1), \dots, \vphi(\vx_i, K))^T$. 
% be the $K \times d$ transformed feature matrix for task $i$. 
We focus on the case that $\Mean(\vr_i|\vx_i)$ is linear in $\vPhi_{i}$  and consider the following linear mixed model (LMM):
\begin{equation}\label{eqn:LMM}
\begin{split}
% Q: full model here?
%     R_{i,t} &\sim \mathcal{N} \big(\sum_a \I(A_{i, t} = a) r_{i, a},  \sigma^2\big), \forall a \in [K], 
    \vr_i = \vPhi_{i}\vthe + \vdelta_i, \;\; \forall i \in [N]
\end{split}
\end{equation}
where $\vthe$ is an unknown vector, and $\vdelta_{i} \stackrel{i.i.d.}{\sim} \mathcal{N}(\vzero, \Cov)$ for some known covariance matrix $\Cov$. 
% $\{\vx_i\}$, $\{\vdelta_i\}$, and $\{\epsilon_{i,t}\}$ are mutually independent. \hl{should be earlier}
In this model, the \textit{fixed effect} term $\vPhi_{i}\vthe$ captures the task relations through their metadata, and the \textit{random effect} term $\vdelta_i$ allows inter-task heterogeneity that can not be captured by the metadata. 
We adopt the prior distribution $\vthe \sim \mathcal{N}(\vmu_\theta, \Cov_\theta)$ with hyper-parameters $\vmu_\theta$ and $\Cov_\theta$. 


% \begin{remark}
% Additional structures can be imposed on $\Cov$ to derive special cases. 
% For example, one can require the arms of a task to have independent random effects by specifying $\Cov = \sigma_1^2 \vI$ for some $\sigma_1$. 
% % , and one additional random effect term can be added at the task level by specifying $\Cov = \sigma_1^2 \vI + \sigma_2^2 \vJ$ for some $\sigma_2$. 
% % The induced models are popular choices in the literature on mixed effect models \citep{fitzmaurice2008primer}. %, and they are  of model \eqref{eqn:LMM}. 
% % model \eqref{eqn:LMM} subsumes
% Besides, the corresponding linear CMAB model $\vr_i = \vPhi_{i}\vthe$ and meta MAB model $\vr_i = \vmu + \vdelta_i$ for some unknown vector $\vmu$ can be regarded as the so-called \textit{fixed effect} model and \textit{random effect} model in the literature \cite{fitzmaurice2008primer}. 
% \end{remark}


The posterior of $\vr_i$ under LMM has an analytic expression. 
We begin by introducing some notations. 
Recall that the history is $\mH = \{(A_{j}, R_{j}, \vx_{j}, i(j))\}_{j=1}^n$ of size $n$. 
Denote $\vR = (R_1, \dots, R_n)^T$ 
and 
$\vPhi = (\vphi(\vx_{1}, A_{1}), \dots, \vphi(\vx_{n}, A_{n}))^T$. 
Let $\Sigma_{a, a'}$ be the $(a,a')$-th entry of $\Cov$. 
The LMM induces an $n \times n$ kernel matrix $\mK$, the $(l,m)$-th entry of which is 
$\vphi^T(\vx_l, A_l) \Cov_{\vthe} \vphi(\vx_m, A_m) + \Sigma_{A_l, A_m} \mathbb{I}(i = i')$. 
Finally, define a $K \times n$ matrix $\boldsymbol{M}_i$, such that the $(a, j)$-th entry of $\boldsymbol{M}_i$ is 
$\I(i(j) = i) \Cov_{A_j, a}$. 
The posterior of $\vr_i$ follows a multivariate normal distribution, with mean and covariance as 
\begin{equation*}%\label{eqn:post}
    \begin{split}
        \mathbb{E}(\vr_i|\mathcal{H}) &= \vPhi_{i} \vmu_{\vthe} + (\vPhi_i\Cov_{\vthe}\vPhi^T + \boldsymbol{M}_i) (\mK + \sigma^2 \vI_n)^{-1} (\vR - \vPhi \vmu_{\vthe}),  \\
        cov(\vr_i | \mathcal{H}) &= (\vPhi_{i} \Cov_{\vthe} \vPhi_{i}^T + \Cov) - (\vPhi_i\Cov_{\vthe}\vPhi^T + \boldsymbol{M}_i) (\mK + \sigma^2 \vI_n)^{-1} (\vPhi_i\Cov_{\vthe}\vPhi^T + \boldsymbol{M}_i)^T. 
    \end{split}
\end{equation*}
% with the derived posterior, 
At each decision point, we can then follow Algorithm \ref{alg:TS} to act. 
The computation is dominated by the matrix inverse of $(\mK {+} \sigma^2 \vI_n)$. 
% , which yields a cubic complexity $O(n^3)$. 
In Appendix \ref{sec:appendix_implementation_gaussian}, we introduce an efficient implementation via using the Woodbury matrix identity \citep{rasmussen2003gaussian} and the block structure induced by the LMM. 
% posterior of \vthe derived in Appendix \label{sec:appendix_implementation_gaussian}. 
% Not easy to report the order. 

\begin{remark}
The idea of addressing metadata-based multi-task MAB problems via mixed effect models is generally applicable. % more
One can replace the linear form of \eqref{eqn:LMM} with other functional forms and proceed similarly. 
As an example, a mixed-effect Gaussian process model and the corresponding {\name} algorithm are derived in Appendix \ref{sec:GP}. 
\end{remark}
% for Gaussian bandits

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \label{eqn:post}
% variance -> 0
% Interpretation: 
% $\mathbb{E}(r_{i,a}|\mathcal{H})$ is composed of two parts: $
% \vphi(\vx_i, a)^T\vmu_{\vthe} + (\vphi(\vx_i, a)^T\Cov_{\vthe}\vPhi^T)(\mK + \sigma^2 \vI)^{-1}(\vR - \vPhi \vmu_{\vthe})$
% and 
% $\boldsymbol{M}_i(\mK + \sigma^2 \vI)^{-1}(\vR - \vPhi \vmu_{\vthe})$. 
% Informally speaking, the first term is to estimate the fixed effect term $\vphi(\vx_i, a)^T \vthe$ and the second term is to estimate the random effect term $\delta_{i,a}$. 
% When there are no data points of taking action $a$ in task $i$ is $0$, the second term is $0$ and our estimation of $r_{i,a}$ depends on the information pooled from the other tasks; 
% While when the number of data points of taking action $a$ in task $i$ is large or when $\sigma_2$ is large, then second term will dominate, which implies we would like to rely more on the rewards generated by taking action $a$ in task $i$ itself. 


% \hl{prior; other task through X; its own experiment data; hyper-parameters}
% better prior 
% will still rely on the task-specific feedback to mitigate the potention bias. 

% For the $i$-th task, let $\vr_i = (r_{i1}, \dots, r_{iK})^T$. 
% $\mathcal{H} = \bigcup_{i,a} \mathcal{H}_{i,a}$, where $\mathcal{H}_{i,a}$ is empty if action $a$ has not been taken for task $i$ yet, and $\mathcal{H}_{i,a} = \{(A_{i,t}, R_{i,t}, i) : A_{i,t} = a\}$ otherwise. 
% Let $\vone_d$, $\vzero_d$, and $\vI_d$ be a d-dimensional vector of all ones, a d-dimensional vector of all zeros, and an identity matrix of dimension $d \times d$, respectively. 
% When the subscript is omitted, the appropriate dimension can be inferred from the context. 



==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/4_3_GLMM.tex <==
\subsection{Bernoulli bandits with Beta-Bernoulli logistic models}\label{sec:binary}
The Bernoulli bandits, where the reward is a binary random variable, is another popular MAB problem. 
As a concrete example, 
we consider the Beta-Bernoulli logistic model (BBLM) to characterize the information-sharing structure. 
Recall $r_{i,a}$ is the expected reward of the $a$th arm of task $i$. 
In BBLM, $r_{i,a}$ follows a Beta distribution with  
$\Mean(r_{i,a}|\vx_i)$ being a logistic function of $\vphi^T(\vx_i, a)  \vthe$. 
We assume the prior $\vthe \sim \mathcal{N}(\vmu_\theta, \Cov_\theta)$ as well. 
% Specifically, t
The BBLM is then defined as 
\begin{equation}\label{eqn:BBLM}
    \begin{split}
            r_{i,a} &\sim \text{Beta}\big(logistic(\vphi^T(\vx_i, a) \vthe), \psi \big), \; \forall a \in [K], i \in [N]\\
    % \vr_i &\sim Beta(logistic(\vPhi_i\vthe), \psi)\\
    R_{i,t} &\sim \text{Bernoulli} \big(\sum\nolimits_{a \in [K]} \I(A_{i, t} = a) r_{i, a} \big)  \; ,\forall t \in [T_i], i \in [N], 
    \end{split}
\end{equation}
where  $logistic(x) \equiv 1 / (1 + exp^{-1}(x))$, $\psi$ is a known parameter, and  $\text{Beta}(\mu, \psi)$ denotes a Beta distribution with mean $\mu$ and precision $\psi$. 
In regression analysis, the BBLM is popular for binary responses when there exist multiple levels in the data structure \cite{forcina1988regression, najera2018comparison}. 

% particular % Not challenge
One challenge to adapting Algorithm \ref{alg:TS} to Bernoulli bandits is that the posterior does not have an explicit form. 
This is also a common challenge to generalized linear bandits  \citep{li2017provably, kveton2020randomized}. 
In model \eqref{eqn:BBLM}, the main challenge comes from the Beta logistic model part. 
We can hence follow the algorithm suggested by 
\eqref{alternative_form} to sample $\vthe$ at a lower frequency.  
%  typically can be efficiently computed
The nice hierarchical structure of model \eqref{eqn:BBLM} allows efficient computation of the posterior of $\vthe$ via approximate posterior inference algorithms, such as Gibbs sampler \cite{johnson2010gibbs} or variational inference \cite{blei2017variational}.  
For example, with Gibbs sampler, the algorithm will alternate between the first layer of \eqref{eqn:BBLM}, which involves a Beta regression, and its second layer, which yields a Beta-Binomial conjugate form. 
Both parts are computationally tractable. 
We defer the details to Appendix \ref{sec:appendix_implementation_Bernoulli} to save space. 
Finally, we note that, similar models and computation techniques can be developed for other reward variable distributions with a conjugate prior. 

% , we will use Gibbs sampling for the Bernoulli bandits. 
% Some theoretical supports can be found in \citet{kveton2020randomized}. 
% dumitrascu2018pg


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/5_Theory.tex <==
\vspace{-.25cm}
\section{Regret Analysis}\label{sec:Theory}
\vspace{-.2cm}
% \subsection{Regret bound}\label{sec:regret_bound}
In this section, we present the regret bound for {\name} under the linear mixed model introduced in Section \ref{sec:LMM}. 
We will focus on a simplified version of Algorithm \ref{alg:TS}, due to the technical challenge to analyze the behaviour of TS with a misspecified prior. 
Indeed, to analyze {\name}, we need a tight bound on the difference in Bayes regret between TS with a misspecified prior and TS with the correct prior.  
To the best of our knowledge, it is still an open and challenging problem in the literature \cite{metapricing,kveton2021meta}.
% even the difference in prior is minor
% show the benefits of information sharing
% Specifically

We consider two modifications (see Appendix \ref{sec:main_proof} for a formal description): 
% Emphasize this challenge in a more clear way. Even though we can know our estimation of P(r|x)
(i) we introduce an "alignment period" for each task, by 
pulling each arm once in its first $K$ interactions, 
and (ii) instead of continuously updating the prior as in \eqref{alternative_form}, 
we fix down a prior for each task after its alignment period, with the prior learned from data generated during all finished alignment periods. 
These two modifications are considered so that we can apply our "prior alignment" proof technique, which is inspired by \cite{metapricing} and allows us to bound the multi-task regret. 
We note similar modifications are imposed in the literature as well, due to similar technical challenges \cite{metapricing,kveton2021meta}. 
% (see, e.g., Remark 8 in \cite{metapricing} or Section $4$ in \cite{kveton2021meta}). 
% (see Section \ref{sec: proof_sketch}).  
The former modification causes an additional $O(NK)$ regret, and the latter essentially utilizes less information in constructing the priors  than Algorithm \ref{alg:TS} and is imposed to simplify the analysis. % purely
Even though, the modified version suffices to show the benefits of information sharing. 
Besides, the second modification is consistent with Algorithm \ref{alg:TS_faster} and hence we provide certain guarantees to this variant. % computationally efficient
Finally, the vanilla {\name} (Algorithm \ref{alg:TS}) shows desired sublinear regrets in experiments. 
% the modified version + NK?


For a matrix $\vA$, we denote its operator norm and minimum singular value by $||\vA||$ and  $\sigma_{min}({\vA})$, respectively. 
For a vector $\vv$, we define $||\vv||$ to be its $\ell_2$ norm. 
$\TO$ is the big-$O$ notation that hides logarithmic terms. 
We make the following regularity assumptions. 

\begin{assumption}\label{asmp:cov_x}
$\sigma_{min}\big( \Mean(\vPhi_i^T\vPhi_i) \big) \ge Kc_1$ and
$max_{i \in [N]} ||\vPhi_i^T\vPhi_i|| \le KC_1$ for some positive constants $c_1$ and $C_1$. 
\end{assumption}

\begin{assumption}\label{asmp:linear_magnitute}
$max_{a \in [K]} ||\vphi(\vx_i, a)|| \le C_2$ and $\norm{\vthe} \le C_3$ for some positive constants $C_2$ and $C_3$. 
\end{assumption}
%  $max_{a \in [K], i \in [N]} \Mean[r_{i,a}|\vx_i]$ is bounded
\begin{assumption}\label{asmp:cov_others}
$\norm{\vmu_{\vthe}}$, $\norm{\Cov_{\vthe}}$ and $\norm{\Cov}$ are bounded.  
\end{assumption}
\vspace{-.1cm}
These regularity conditions are standard in the literature on Bayesian bandits \cite{russo2014learning,lattimore2020bandit}, 
linear bandits \cite{agrawal2013thompson, cella2020meta} and feature-based structured bandits \cite{ou2018multinomial, li2018online}. 
Under these conditions, we can derive the following regret bound for the modified {\name}. 
For simplicity, we assume $T_1 = \dots = T_N = T$. 
% More general form will involve the order of interactions and can be established following our proof on a case-by-case basis. 
% over $N$ tasks with $T$ interactions per task
\begin{theorem}\label{thm:meta_ours}
Under Assumptions $1 - 3$, 
when $d = o(N)$ and $K < min(N,T)$, 
the multi-task regret of the modified {\name} under the LMM is bounded as 
\vspace{-.05cm}
\begin{align*}
     MTR(N, \{T_i\}) 
    &= O\big( \sqrt{Nlog(NT)}(\sqrt{d} {+} \sqrt{log(NT)} \big)  \sqrt{TK logT} 
    {+} log^2(NT) \sqrt{(T{-}K)KlogT}
    {+} NK \big)\\
    &= \TO\big(  \sqrt{Nd} \sqrt{TK} + NK\big).
    \alignlable{eqn:MTR_results}
\end{align*}
\end{theorem}
\vspace{-.2cm}
We remark this is a worst-case frequentist regret bound with respect to $\vthe$. 
% One can simply replace $T$ in the condition with $min(T_i)$, and prove a regret with $T$ replaced by $max(T_i)$. 
To save space, the proof of Theorem \ref{thm:meta_ours} is deferred to Appendix \ref{sec:main_proof}. 
Note that the single-task Bayes regret of oracle-TS is $O(\sqrt{TKlogT})$ based on the literature (e.g., \cite{lattimore2020bandit}). 
The Bayes regret of the modified {\name} then follows from the definition of multi-task regret. 

\begin{corollary}
Under the same conditions as Theorem \ref{thm:meta_ours}, 
the Bayes regret of the modified {\name} can be bounded as 
$BR(N, \{T_i\}) = \TO \big(  \sqrt{Nd} \sqrt{TK} + NK + N\sqrt{TK}\big).$
% over $N$ tasks with $T$ interactions per task is bounded as 
% \begin{equation*}
%      BR(N, \{T_i\}) = \TO \big(  \sqrt{N} \sqrt{dTK} + NK + N\sqrt{TK}\big).
% \end{equation*}
\end{corollary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Discussion}\label{sec:theory_discussion}
\vspace{-.15cm}
\textbf{Discussions.} \;
% \paragraph{Discussions.}
For comparison purposes,
we informally summarize the regret bounds of several baselines in Table \ref{tab:regret}. 
To save space, the formal statements and their proofs are deferred to  Appendix \ref{sec:proof_lemmas}. 
We consider the following algorithms: 
(i) One TS policy for all tasks, referred to as \textit{one-size-fit-all (OSFA)}; 
(ii) An individual TS policy for each task, referred to as \textit{individual-TS}; 
(iii) TS for linear bandits \cite{agrawal2013thompson},  referred to as \textit{linear-TS}; 
(iv)  Meta-Thompson sampling (meta-TS) proposed in \cite{kveton2021meta}.
Specifically, meta-TS, under the Gaussian bandits setting, assumes $\vr_i \sim \normal(\vmu, \Cov)$ for some unknown vector $\vmu$, and it pools data to learn $\vmu$.
To recap, OSFA ignores the inter-task heterogeneity and linear-TS assumes $\vr_i$ is fully determined by the metadata, while individual-TS does not share information and meta-TS fails to utilize the metadata to efficiently share information. 
% ignores the heterogeneity that can not be captured
% through the assumed functional form


In the MTR bound for {\name} \eqref{eqn:MTR_results}, 
the first term is sublinear in $N$, which implies {\name} is continuously learning about $\prob(\vr_i|\vx_i)$ and will behave closer to oracle-TS as $N$ increases. 
The $\TO(NK)$ term is due to the imposed $K$ alignment rounds in our analysis. 
In contrast to {\name}, 
the multi-task regrets of these baseline algorithms unavoidably scale linearly in $N$, since they fail to utilize knowledge about $\prob(\vr_i|\vx_i)$, which can efficiently guide the exploration. 
The regret rates suggest that {\name} is particularly valuable in task-rich settings ($N \gg d$). 
We note that, although their difference in multi-task regret is of the same order as the Bayes regret of oracle-TS, which implies the Bayes regret of {\name}, meta-TS, and individual-TS will be of the same order, the hidden multiplicative factors can differ a lot.  
We observe a substantial gap in the experiments. 
Finally, OSFA and linear-TS even suffer a linear regret in $T$, due to the bias caused by ignoring the heterogeneity. 
In contrast, {\name} yields a desired sublinear Bayes regret in $T$. %since it can account for the heterogeneity. 
Finally, \cite{kveton2021meta} adopts a recursive approach to obtain a $\TO(\sqrt{N}KT^2 {+} N\sqrt{KT})$ Bayes regret bound for meta-TS. 
Our bound clearly demonstrates the usefulness of the prior alignment proof technique, which can be applied to meta-TS as well. 

% is tighter and
% Finally, under the meta MAB setting, we can similarly prove a regret bound for meta-TS as XX, which improves the regret bound in XX. This improvement is due to the novel prior alignment technique. 

% when LMM degenerates to XXX!!! under their setting!! and the bound of {\name} degenerates to XXX!
% Besides, when $\vx_i \equiv 1$, that is, under the degenerate case, the multi-task regret for metaTS with a similar modifications is derived as $\TO(KT^2\sqrt{N} + KN + T)$  in \cite{kveton2021meta}, while ours is $\TO(  \sqrt{N}K \sqrt{T} + NK)$. 
% This improvement demonstrates the usefulness of the prior alignment technique. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{table_rate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Proof sketch}\label{sec: proof_sketch}
% \begin{enumerate}
%     \item Bayes regret of the oracle-TS is $\TO(N\sqrt{KT})$: adapt from existing results
%     \item multi-task regret of the modified oracle-TS is $\TO(NK)$: use that standard proof framework
%     \item Bound the difference between the modified oracle-TS and the modified TS
%     \begin{enumerate}
%         \item the estimated prior is close to the true prior: concentration inequality for $\hat{\Mean} [\vr_i| \vx_i]$ (The analysis of LMM in IP) +  posterior concentration (analysis in metaTS)
%         % theta, then for 
%         \item the induced multi-task regret cause by the misspecified prior is small ("prior alignment" technique): after the K pulls, w.h.p., the posterior now is the same. The remaining probability is negligible. Similar with the meta pricing paper. 
%     \end{enumerate}
% \end{enumerate}


% To save space, the full proof of Theorem \ref{thm:meta_ours} is deferred to Appendix \ref{sec:main_proof}. 
% We outline the proof as the following steps. 
% (i) we first apply the property of Gaussian linear mixed model to prove that the sampled prior mean for the $i$-th task will concentrate around its  true prior $\Mean(\vr_i | \vx_i)$, as roughly the order of $\TO(\sqrt{dK} i^{-1/2})$ with high probability; 
% (ii) when the sampled prior is close to the true prior, we apply the "prior alignment" technique to bound the meta regret accumulated over the $i$-th task  by $\TO(\sqrt{dK} i^{-1/2} \sqrt{(T-K)K})$, which can be summed over the $N$ tasks to yield a bound $\TO(\sqrt{dK} \sqrt{N} \sqrt{(T-K)K})$; 
% (iii) we bound the meta regret in the forced exploration period by $O(NK)$. 
% (iv) we bound the other terms by d\sqrt{(T-K)KlogT}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% a general bound: valid for any schedule. As long as the regression part and the reward part satisfies some concentration inequality, then it can hold. 
% linear + Gaussian random effect: as long as the estimated prior is close.
% Gaussian errors: otherwise, difficult to apply the transformation? [can still? one-to-one mapping?]



==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/6_Simulation.tex <==
\vspace{-.1cm}
% \subsection{Synthetic data} 
In this section, we conduct simulation experiments to support our theoretical results and study the empirical performance of {\name}. % under different conditions
We use model \eqref{eqn:LMM} and \eqref{eqn:BBLM} as our data generation model for Gaussian bandits and Bernoulli bandits, respectively. 
In the main text, we present results with $N = 200$, $T = 200$, $K = 8$ and $d = 15$. 
We set $\vphi(\vx_i, a) = (\vone_a^T, \Tilde{\vphi}_{i,a}^T)^T$, where $\vone_a$ is a length-$K$ indicator vector taking value $1$ at the $a$-th entry, and $\Tilde{\vphi}_{i,a}$ is sampled from $\normal(\vzero, \vI_{d-K})$. 
The coefficient vector $\vthe$ is sampled from $\mathcal{N}(\vzero, d^{-1}\vI_d)$. 
% $U[-1, 1]$ . 
For Gaussian bandits, 
we set $\sigma = 1$ and $\Cov = \sigma_1^2 \vI_K$, for different values of $\sigma_1$. 
For Bernoulli bandits, we vary the precision $\psi$. 
A higher value of $\sigma_1$ or $\psi$ implies a larger inter-task heterogeneity conditional on the metadata. 
We consider two representative types of task sequence:
(i) the \textit{sequential} setting, where the $(i + 1)$-th task begins after we finish the $i$-th task, 
and (ii) the \textit{concurrent} setting, where we interact with all tasks for the $t$-th time simultaneously. 

% is a hyper-parameter which 

For Gaussian bandits, 
we compare {\name} with the four algorithms discussed in Section \ref{sec:Theory}: OSFA, individual-TS, linear-TS, and meta-TS. 
Besides, we also investigate the performance of the computationally efficient variant of {\name} 
in Algorithm \ref{alg:TS_faster}, referred to as {\name}-approx. 
For Bernoulli bandits, we replace linear-TS with a TS algorithm for generalized linear bandits \cite{kveton2020randomized}, which is referred to as GLB-TS. 
The other baselines are also replaced with their Bernoulli variants. 
% conjugate priors
To set the priors for these TS algorithms, we 
apply the law of total expectation (variance) to 
integrate out $(\vx,\vr)$ to specify the mean (variance) term. 
See Appendix \ref{sec:appendix_Experiment_Details} for more details about the implementations. 
% settings and
% each seed, sample one $\vthe$
% N^{-1} BR(N, \{T\})
% , under the two task sequence settings and with different values of $\sigma_1$, 
% \ref{fig:simu_Gaussian} and \ref{fig:simu_Binary}, respectively. 

\textbf{Results.} \;
Results aggregated over $100$ random seeds are presented in Figure \ref{fig:simu}. 
% Results for Gaussian bandits and Bernoulli bandits 
% are presented in Figure \ref{fig:simu}. 
% All results are aggregated over $100$ random seeds. 
% Under the concurrent (sequential) setting, the average Bayes regrets per interaction (task) are displayed, which shows the trend with $T$ ($N$).
Under the concurrent setting, the average Bayes regrets per interaction are displayed, which shows the trend with $T$; 
under the sequential setting, the average Bayes regrets per task are displayed, which shows the trend with $N$. 
Such a choice allows us to see the regret rates derived in Section \ref{sec:Theory} more clearly. 
Recall that the multi-task regret of an algorithm can be calculated as the difference between the Bayes regret of itself and oracle-TS. 
For ease of comparison, we also report the multi-task regrets in Appendix \ref{sec:appendix_figure_MTR}. 
% For each seed, we sample a new $\vthe$. 

% and its Bayes regret becomes; closer
Overall, {\name} performs favorably compared with the other baselines. 
Our findings can be summarized as follows. 
First, in the sequential setting, the Bayes regret of {\name} approaches that of oracle-TS, which shows that {\name} yields a sublinear multi-task regret in $N$. 
This implies {\name} is learning  $\prob(\vr|\vx)$ and will eventually behave similarly to oracle-TS. 
In contrast, there exists a consistent and significant performance gap between oracle-TS and the other baselines. 
This demonstrates the benefit of metadata-based information sharing. 
% No need for that modifications
Second, in the concurrent setting, {\name} shows a sublinear Bayes regret in $T$. 
This implies {\name} is learning the best arm for each task. 
% similar
Although individual-TS and meta-TS also yield sublinear trends, their cumulative regrets can be significantly higher. 
For example, in Gaussian bandits, the cumulative regret of {\name} is only $53.3\%$ of the regret for individual-TS when $\sigma_1^2 = 0.25$, and $68.2\%$ when $\sigma_1^2 = 0.5$. 
This demonstrates that, with information sharing and the guidance of metadata, {\name} can explore more efficiently. 
The benefit is particularly important when the horizon $T$ is not long, and {\name} enables a jump-start for each task. 
Third, the trend with $\sigma_1^2$ and $\psi$ is clear: 
when the metadata is less useful ($\sigma_1^2 = 1$ or $\psi = 0.2$), the performance of meta-TS and individual-TS becomes closer to {\name}, while linear-TS (GLB-TS) and OSFA suffer from the bias; 
when the metadata is highly informative, the advantage of {\name} over meta-TS and individual-TS becomes much more significant, and the performance of linear-TS (GLB-TS) becomes relatively better. 
Overall, {\name} shows robustness. 
Lastly, {\name}-approx yields similar performance with the vanilla {\name}, except  when $N$ is still small. 
% version of
% almost the same
% that its regret is slightly higher

Additional results under other settings are reported in Appendix \ref{sec:appendix_more}, where {\name} consistently performs favorably, and shows reasonable trends with hyperparameters such as $N$, $K$, and $d$. 
% We observe that when $d$ increases, the multi-task regret of {\name} also grows, due to the fact that it is more challenging to learn $\prob(\vr|\vx)$. 
% We observe that the benefits of meta-learning are preserved as the number of arms K or dimensions d increase. 
% How- ever, as expected, they diminish when the prior variance σ02 approaches the meta-prior variance σq2.
Finally, recall that, to share information, we made a model assumption that $\vr_i | \vx_i, \vthe \sim f(\vr_i | \vx_i, \vthe)$. 
When this model is correctly specified, {\name} has shown superior theoretical and numerical performance. 
Intuitively, this model is designed to pool information to provide an informative prior. 
As long as the learned prior provides reasonable information relative to a manually specified one, the performance of {\name} is expected to be better or at least comparable. 
We empirically investigate the impact of model misspecication to {\name} in Appendix \ref{sec:appendix_robustness}, where {\name} demonstrates great robustness. 
% However, we acknowledge that all models can be misspecifed. 
% is not significantly worse than
% inductive bias



% computation only 1/T
% in the initial period 

% In Appendix E, we report additional experimental results. We observe that the benefits of meta-learning are preserved as the number of arms K or dimensions d increase. How- ever, as expected, they diminish when the prior variance σ02 approaches the meta-prior variance σq2. In this case, there is little benefit from adapting to prior P∗, and all algorithms perform similarly.

\input{Figures/Figures}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% as the number of arms K or dimensions d increase. 





==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/7_Discussion.tex <==
\vspace{-.25cm}
\section{Discussion}\label{sec:discussion}
\vspace{-.2cm}
In this paper, we study the metadata-based multi-task MAB problem, where we can utilize the metadata to capture and learn task relations, so as to judiciously share knowledge. % task-specific features of each task
We formalize this problem under a general framework and define the notion of regret. % corresponding
We propose to address this problem with Bayesian hierarchical models and design a TS-type algorithm, {\name}, to share information and minimize regrets. 
Two concrete examples are analyzed and efficient implementations are discussed. 
The derived regret rates and experiment results both support the usefulness of {\name}. 

The proposed framework can be extended in several aspects. 
First, the variance components are assumed known for the two examples in Section \ref{sec:method}. % as in the literature metaTS and linear bandits
In practice, we can apply empirical Bayes to update these hyperparameters adaptively. See Appendix \ref{sec:appendix_hyper_updating_EB} for  details. 
% , so as to adapt to the degree of heterogeneity and noise. 
% or latent bandits \citep{hong2020latent, hong2020non}  
Second, our work can be extended to contextual bandits, 
based on the idea of clustering of bandits \citep{gentile2014online, li2016collaborative} when the set of task instances is finite, or the idea of contextual Markov decision process \cite{modi2018markov} when the set is infinite. % , modi2020no
See Appendix \ref{sec:extension_contextual} for details. 
Third, while our analysis for {\name} can be directly extended to other functional forms, the prior alignment technique does utilize some properties of Gaussian distributions. 
A novel analysis of TS with mis-specified priors would be of independent interest. 
% Analysis for more general settings requires an in-depth analysis of TS with mis-specified priors, which needs some novel tools and is important in its own right.  
% On a Case by case basis
% n in-depth
% our analysis of {\name} is under the Gaussian assumption. 
% Third, we consider the task-specific features as static in this paper. 
% While one has to consider CMAB when the features will change quickly, the extension of this work to piecewisely stationary environments is straightforward. 

% continuously
% When the features are (nearly) , we can divide a task into multiple ones 

% The data of other users (tasks) can be stored in $\vthe$ and hence largely avoid the issue of privacy. 
% can be stored in vthe; thus not applicable. 

% Broader Impact
% We develop bandit-style exploration algorithms that can be easily trained on historical data. This
% fundamentally alters the current prevalent approach to bandit algorithm design, which is by theory.
% Bandit algorithms are often deployed in user-facing domains. However, we do not propose any new
% domain. So our impact on users should be limited to those that already exist. Beyond this, we are not
% aware of any societal consequences of our work, such as on welfare, fairness, or privacy.


%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
% Our model and algorithm can be straightforwardly extended to other functional form and distribution assumptions, with appropriate modification of the posterior derivations. 
%%%%%%%%%%%%%%%%%%%%%%%%
% 1. Extension to contextual bandits
% varying-coef
% closely related with Susan's???
% many types, additive or multiplicative 
% \begin{equation*}
%     \begin{split}
%         \vthe(\vx) &\sim \mathcal{GP}(\mu(\vx), \mathcal{K}(\vx, \vx')) \\
%         \vthe_i &\sim \vthe(\vxi) + \mathbf{e}_{i}, \forall i = 1, \dots, N \\
%         R_{i,t} &= \boldsymbol{\phi}(c_{i,t}, A_{i,t})^T\vthe_i
%         + \epsilon_{i,t}
%     \end{split}
% \end{equation*}

%%%%%%%%%%%%%%%%%%%%%%%%


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/ARCHIVE/Archive_related_work.tex <==

Susan's intelligent polling \cite{tomkins2019intelligent}: 
    the cloest work. They also consider pooling information over $N$ (contextual) bandit tasks (patients), but use a mixed effect model and did not consider the similarity capture by $\vxi$. 
    Let the content of the $t$-th interaction of the $i$-th task be $\vc_{t,i}$:
    \begin{equation*}
        \begin{split}
            \vthe_i &= \vthe + \mu_i \\
            R_{t,i} &= \vthe_i^T \vc_{t, i} + \epsilon_{t,i} 
        \end{split}
    \end{equation*}


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/ARCHIVE/Real_Data.tex <==
\subsection{Real data}
% calibrated from a multi-task supervised learning task?
Due to the absence of open dataset containing  logged feedbacks from multiple MAB tasks, following the literature\citep{cella2020meta, gentile2014online, metapricing}, 
we convert a logged contextual bandit dataset for our experiment purpose. 

\begin{itemize}
    \item Each user is a task
    \item Clustering the news/movies to create several arms 
\end{itemize}


% \textbf{Setting.}
% We need to find a dataset on MAB problems with many tasks and some task-specific features (or CMAB whose context can also be used as feature, due to repeated nature). 
% continuous reward (not binary)

% For example, many products with static features and some binary decisions need to be made
% Ideally, we should have a logged bandit-feedback dataset of similar MAB tasks (experiments), without context, with discrete actions and continuous rewards. 
% The motivating example is where we have many products with their static features and we need to make some binary decision for each of them. 
% If no such a dataset is available, I am thinking of using snthetic dataset to study the asymptotic with both N and T, and use the Warfarin dataset to study large N small T (with small noise variance, T = 20 may be enough, as in the RI example; besides, Since the main improvement comes from information sharing among tasks, large N samll T is beneficial to us) 


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/ARCHIVE/dicussions_IP.tex <==
\subsection{Comparison with \citet{tomkins2019intelligent}}
Treat $ia$ as $i$, we can find that \citet{tomkins2019intelligent} can be understood as a random slope (random coefficient) model, while our model is a random intercept model. 
We may even consider the random intercept and slope model. 
However, their use cases are different. 
Besides, when the second term is generalized to nonlinear, the random coefficient model is difficult to formularize. 


\begin{align*}
    y_{ij} &= \alpha + \vx_{ij}^T\beta_i + \epsilon_{ij}\\
    y_{ij} &= \alpha_i + \vx_i^T\beta + \epsilon_{ij}\\
    y_{ij} &= \alpha_i + \vx_{ij}^T\beta_i + \epsilon_{ij}
\end{align*}




% \subsection{Meta contextual MAB}
% We compare our model with the model in \citet{tomkins2019intelligent}, which is representative of the literature on meta contextual MAB. 
% % For ease of comparison
% Let $S_{i.t}$ be the context for the $t$th interaction with the $i$th task. 
% Intelligent Pooling assumes
% % \begin{align}
% % \vthe_i &= \vthe + \delta_i, \forall i\\
% % R_{it} &= f(S_{it}, A_{it}; \vthe_i) + \epsilon_{it}, 
% % \end{align}
% % or equivalently, 
% \begin{equation}
% R_{it} = f(S_{it}, A_{it}; \vthe + \delta_i) + \epsilon_{it}.
% \end{equation}


% Let $\vx_i$ be the static features of task $i$. 
% Our model is 
% % \begin{align}
% % r_{i, a} &= g(\vx_i, a; \vthe) + \delta_{ia}, \forall i, a\\
% % R_{i, t} &= \sum_a \mathbb{I}(A_{it} = a)r_{ia} + \epsilon_{it}.
% % \end{align}
% % or equivalently, 
% \begin{equation}
% \begin{split}
%     R_{i, t} &= g(\vx_i, A_{it}; \vthe) + \sum_a \mathbb{I}(A_{it} = a) \delta_{ia}+ \epsilon_{it} %\\
%     % R_{i, t} &= f(\vx_{i(t)}, A_{it}; \vthe) + \sum_a \mathbb{I}(A_{it} = a) \delta_{ia}+ \epsilon_{it}.\\
%     % R_{i, t} &= f(\vx_{i(t)}, A_{it}; \vthe + \vthe_i) + \epsilon_{it}.
% \end{split}
% \end{equation}


% For the nonliner case, we need the following modifications
% \begin{equation}
% \begin{split}
%     R_{it} &= f(S_{it}, A_{it}; \vthe + \vthe_i) + \epsilon_{it}.\\
%     R_{it} &= f(\vxi, A_{it}; \vthe + \vthe_i) + \epsilon_{it}.\\
%     R_{it} &= f(\vxi, A_{it}; \vthe + \vthe_{ia}) + \epsilon_{it}. \\
%     R_{it} &= f(\vxi, A_{it}; \vthe) + f(\vxi, A_{it}; \vthe_{ia}) + \epsilon_{it}. \text{Not identifiable (not a valid model)}\\
%     R_{it} &= f(\vxi, A_{it}; \vthe) + \delta_{ia} + \epsilon_{it}.\\
% \end{split}
% \end{equation}
% Except for the first step, neither of them is a special case of the previous one. 


% \textbf{Connections.} When we remove $\delta_i$ from (6) and $\delta_{ia}$ from (9), and set $S_{it} = \vx_i$ for all $t$
% these two models coincide at the  contextual MAB method
% \begin{equation}\label{formula: CMAB}
%     R_{i, t} = f(S_{it}, A_{it}; \vthe) + \epsilon_{it}, \forall i
% \end{equation}
% Otherwise, neither one is a special case of the other. 
% The difference can also be seen through the following combination of both (multiple contexutal MAB tasks with task-specific faetures which capture the task similiarity). We add static feature-based task similarity model to (6) and extend our model to contextual MAB: 
% \begin{equation}\label{formular: CMTB}
%     \begin{split}
%         \vthe_i &= g(\vx_i; \beta) + \delta_{i},\\
% R_{i, t} &= f(S_{it}, A_{it}; \vthe_i) + \epsilon_{it}, 
%     \end{split}
% \end{equation}

% In short, Intelligent Pooling applies to multiple contextual MAB tasks but the task similarity has not been modeled; our model applies to multiple MAB tasks without contexts but with the task similarity carefully modeled. 
% Therefore, these two approaches are orthogonal. 
% % , and are applicable when different information is available. 
% When no context information is available, their method is not applicable (Naively set $\vx_i = S_{i,t}$ will lead to $r_{ia} = f(\vx_{i}, a; \vthe + \delta_i) = f(\vx_{i}, a; \vthe_i)$, whose meaning is not clear). 
% When there are huge heterogeneity, such as there are several clusters, their method is also not efficient. 

% \textbf{When f is nonlinear (above).} If the implications of two models are the same (or one is a special case of the other), then no matter which functional class we choose (linear, random forests, NN, GP), the connections should hold (which is not the case here)

% \textbf{When f is linear.} One may argue that, when f is a linear function, the two forms look similar. We take a close look. 
% Write $\vx_{ia} = \vphi(\vx_i, a)$. 
% Then by setting $S_{it} = \vx_i$, 
% Intelligent Pooling assumes
% \begin{equation*}
%     r_{ia} = \vx_{ia}^T (\vthe + \vthe_i) = \vx_{ia}^T \vthe +  \vx_{ia}^T \vthe_i, \vthe_i \sim N(0, \Cov)
% \end{equation*}
% % It is equal to $r_{ia} = \vx_{ia}^T \vthe +  \delta_i, \vthe_i \sim N(0, \vx_{ia}^T \Cov \vx_{ia})$. 
% Our model is
% \begin{equation*}
%     r_{ia} = \vx_{ia}^T\vthe + \delta_{ia}, \delta_{ia} \sim N(0, \sigma^2)
% \end{equation*}
% We need to take the following steps so that Intelligent Pooling can apply to our problem (equivalent to our model) (\textbf{for now, assume $\vxi$ contains continuous variables. When only categorical variables are present and we only consider the linear form, this two model coincidences. But actually a lot of models are the same under such a restrictive setting, since essentially we are considering a block design.}): 
% % There are still the following differences between Intelligent Pooling and  (our problem):
% \begin{enumerate}
%     \item modify $\vthe_i$ as $\vthe_{ia}$: this modification already implies that for tasks (products/patients) with the same features, the optimal action can vary.
%     \item one may tend to write $\vx_{ia}^T\vthe_{ia}$ as $\delta_{ia}$. Then we need to explain the meaning of $\vx_{ia}^T\vthe_{ia}, \; \vthe_{ia} \sim N(0, \Cov)$. 
%     % What does his 
%     One may argue this is sometimes used to handle heteroscedasticity, but why do we need such a dependency needs to be explained. 
%     \item Even if we ignore the two points above: recall that, so far, our discussions are only about models. 
%     The inference goal of IP, $\vthe_{ia}$, is not identifiable in our problem. Of course, we can modify their algorithm, and also the theory, and numerical studies. But now we have already modified a lot.
% \end{enumerate}

% Some other arguments: 
% \begin{enumerate}
%     \item In nonlinear cases, the above connections not feasible (1. $\delta_i$ is not meaningful any longer; 2. can be modified as a mean-zero random-effect function term $f_i$, but not identifiable)
%     \item \textbf{How to prove that their model can be applied to our problem:} one can consider the example in the next section, and remember our goal is $\{r_{ia}\}$. 
%     % If their model and method can be 
%     We are not clear how to adapt their model and method to such a problem. 
%     \item It might help to distinguish the following models (in the simplified regression setup. \textbf{$\vxi$ includes continuous variables}): 
% \end{enumerate}
%     \begin{align*}
% \text{(1)}\; y_{i} &= \vxi^T \vbeta + \epsilon_{i}; (\text{linear fixed effect model})\\
% \text{(2)}\; y_{ij} &= \vxi^T \vbeta + \epsilon_{ij} (\text{linear fixed effect model - why contextual bandit not appropriate})\\
% \text{(3)}\; y_{ij} &= \vx_{ij}^T (\vbeta + \vbeta_i) +  \epsilon_{ij}, \vbeta_i \sim N(0,\Cov) (\text{their model in their problem. Sometimes called \textbf{random coefficient model}})\\
% \text{(4)}\; y_{ij} &= \vxi^T (\vbeta + \vbeta_i) +  \epsilon_{ij}, \vbeta_i \sim N(0,\Cov) (\text{their model in our problem.})\\
% &\;\;\;\;\;\;\;\;\;(\text{Why their method fails: 1. meaning of $\vxi^T \vbeta_i$? 2. $\vbeta_i$ not identifiable})\\
% \text{(5)}\; y_{ij} &= \vxi^T \vbeta + \delta_i + \epsilon_{ij}, \delta_i \sim N(0,\sigma^2) (\text{our model in our problem. Not a special case of model 3 and 4. } )\\
% \text{(6)}\; y_{ij} &= \vxi^T \vbeta + \delta_i + \epsilon_{ij}, \delta_i \sim N(0,\sigma_i^2) (\text{one possible extension of our model. Not a special case of model 3 and 4.} )
%     \end{align*}

% % Covariance modelling and multilevel structures
% % A general form of linear mixed effect models (in our case. Focus on the regression function part) is: 
% % \begin{equation*}
% %     r_{ia} = \vx_{ia}^T \vthe + \mathbf{z}_{ia}^T \vbeta 
% % \end{equation*}

% % (to be examined: whether this is trivial )

% % Even if we ignore all those issues, another thing in the linear model is that (if we shift our attention from the models to the estimator/algorithm/method) , their inferential goal is theta_i (theta_i = theta + \mu_i, in their notations). But  is not identifiable in our problem. See the follows. 

% % Consider the \mu_i term, which links with \delta_ia through \delta_ia = x_ia^T \mu_i. Even if we have infinite data points and then we know the true value of delta_ia, the number of possible values for \mu_i is still infinite.

% % 

% % All our previous discussions are purely mathematical. The intuition/reason behind them is, these two papers are about different problems.

% % context is not the same with static-feature


% % \textbf{1. Why not consider the most general form \eqref{formular: CMTB}? }
% % Technically, we can. With Gaussian linear mixed effect model or GP for both $f$ and $g$, the derivation will be similar. 
% % The concerns are mainly about the theoretical challenges and the finite-sample performance (the current model is more like mixed effect regression models,  \eqref{formular: CMTB} is more like varing-coefficient regression models. For \eqref{formular: CMTB}, I am not aware of any similar works and existing theory in the bandit literature.) 

% % Besides, I would like to note that the contextual features (which depend on t) are not always available. 
% % % MAB is not just a simpler version of contextual MAB, since 
% % Simply treating the static features as the context and ignoring the heterogeneity lead to model \eqref{formula: CMAB}, which results in biases with the presense of $\delta_{ia}$. 





==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/ARCHIVE/discussion_comparison_related.tex <==
\section{Comparison with Related Methods}
In this section, we discuss the relationship of our setup with several related lines of research in more details. 

\subsection{Contextual MAB}
Let us consider a standard CMAB formulation in the multi-task setup. 
For time $t = 1, 2, \dots$, the agent receives a task index $i(t)$ along with its feature $\vx_{i(t)}$, regards it as the context of this interaction, selects some action $a_t$, and then receives some random reward $R_t$. 
The agent relate this reward with the context-action pair by assuming a relationship $R_t = f(\vx_{i(t)}, a_t; \vthe) + \epsilon_t$, for some function $f$ with unknown parameter $\vthe$ and some mean-zero random error $\epsilon_t$. 
The underlying assumption is $\Mean(R_t | \vx_{i(t)} = j, a_t = a) = f(\vx_j, a; \vthe)$ for any task $j$ and action $a$. 
This is an assumption we have to impose when we only interact with each task for one time. 
However, under the multi-task setup, where we need to interact with each task for multiple times, the repeated measurements nature allows us to include a mixed effect term to allow personalization for each individual tasks, which lead to the a general form of our model: 
\begin{equation*}
    \Mean(R_t | \vx_{i(t)} = j, a_t = a) = f(\vx_j, a; \vthe) + \delta_{i,a}, \forall i \in [N], a \in [K]. 
\end{equation*}
When the number of interactions with one task $i$ is limited, the above formulation will be dominated by $f(\vx_j, a; \vthe)$ and hence is close to a contextual MAB settting; while when the number increases, it will be dominated by $\delta_{i,a}$ and hence is close to the single-task MAB setting. 
As such, our model allows judiciously sharing information among tasks and hence reduces the variance, esoterically in the early period, and also allows personalization to each individual task according to its own history records. 


% CMAB algorithms typically  
% $r_{t,a} = f_{\vthe}(\vx_t, a)$  where $\vx_t$ is the "context" for the $t$-th interaction, $a$ is some action, and $r_{t,a}$ is the expected reward of this interaction. 



==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/ARCHIVE/layout_example.tex <==

\section{The layout example}
\begin{itemize}
    \item Tasks: $i = 1, \dots, N$ products. 
        \begin{enumerate}
        \item shoe1, shoe2, ..., phone1, phone2, ..., TV1, ...
            % \item Shoes: shoe1, shoe2, ...
            % \item Electronics: phone1, TV1, ...
        \end{enumerate}
    \item Arms: for each product, $a = 1, \dots, K$ display layouts
        \begin{enumerate}
            \item (Image-title, new-release, brand, price, why-recommended)
            \item (Image-title, brand, reviews, price, why-recommended)
        \end{enumerate}
    % E.g.: Category = (Shoes): Option = (Image-title, new-release, brand, price, why-recommended). Category = (Electronics): Option = (Image-title, brand, reviews, price, why-recommended).
    \item Reward: $r_{ia}$ under each display layouts  %the product have a CTR
    \item Features: baseline features $\vxi$ (category, price, etc.)
\end{itemize}

Methods:
\begin{itemize}
    \item CMAB: $r_{ia} = f(\vxi, a; \vthe)$. Fully determined by features (even if we find it is sub-optimal after interactions). 
    \item independent MAB: $\{r_{ia}\}$ are independent %i.i.d.
    % \item meta MAB: $r_{ia} \sim N(\mu_r, \sigma_r^2)$ 
    \item Ours: $r_{ia} = f(\vxi, a; \vthe) + \delta_{ia}$
\end{itemize}
IP can not apply to such a problem. 


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/ARCHIVE/meta_oracle.tex <==
\section{The Oracle-TS and its Bayes regret}\label{supp-sec:oracle}
As our oracle-TS, for each task $i$, we consider the  standard Thompson sampling algorithm for Gaussian bandits with prior distribution as $\vr_{i} \sim \mathcal{N}(\vPhi_{i}\vthe, \Cov)$.  
With such a "true" prior, its asymptotic optimality for this single task has been derived in \citet{agrawal2013further}. 
Its optimality can be straightforwardly extended to the multi-task setting, to yield a Bayes regret of order $O(N\sqrt{T}log(T))$. 

[to be updated w/ new notations]
We briefly review the standard Thompson sampling algorithm for a single task below. 
At a decision point for task $i$, suppose the accumulated interaction data with task $i$ is $\mathcal{D}_i = \{(A_{i,t}, R_{i,t})\}$. 
Let $\rho(\vr_i)$ be the corresponding posterior with the data $\mathcal{D}_i$ and the prior $r_{i,a} \sim \mathcal{N}(\vphi(\vxi, a)^T\vthe, \sigma_1^2)$ for every $a \in [K]$. 
$\rho(\vr_i)$ follows a multivariate normal distribution. 
Then, the oracle-TS will take the action $A_{i,t} = argmax_a \{\tilde{r}_{i,a}\}_{a=1}^K$, where $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T$ is randomly sampled from $\rho(\vr_i)$. 

%  for every $a \in [K]$

==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/ARCHIVE_Method/LMM.tex <==
% For simplicity, we assume $\epsilon_{i,t} \sim \mathcal{N}(0, \sigma^2)$ throughout this paper. 
% to mitigate the bias 
% The term $\delta_{i,a}$ is introduced to accommodate task-specific heterogeneity that can not be captured by the features. 
\subsection{Bayesian linear mixed effect model}\label{sec:LMM}

% can be some basis expansions 
% or mannually designed.
% typical in the linear bandit literture. 
% a set of basis functions which are “rich” enough to approx- imate the underlying function
Let $\vphi(\cdot, \cdot) : \mathbb{R}^p \times [K] \rightarrow  \mathbb{R}^d$ be a known map from the feature-action space to a $d$-dimensional space, and let $\vPhi_{i} = (\vphi(\vx_i, 1)^T, \dots, \vphi(\vx_i, K)^T)$ be the $K \times d$ transformed feature matrix for task $i$. 
We focus on the case that $\Mean(\vr_i|\vx_i)$ is a linear function of $\vPhi_{i}$  and consider the following Bayesian linear mixed effect model:
% , stacked vertically over the $K$ arms. 
\begin{equation}\label{eqn:LMM}
\begin{split}
    \vr_i = \vPhi_{i}\vthe + \vdelta_i, 
    % r_{i,a} &= \vphi(\vx_i, a)^T \vthe + \delta_{i,a}, 
\end{split}
\end{equation}
% for every i \in [N] and a \in [K]. 
% better replace with \Cov_{\vdelta}. But \cov_{a, a'}
where $\vthe$ is an unknown vector, and $\vdelta_{i} \stackrel{i.i.d.}{\sim} \mathcal{N}(0, \Cov)$ for some 
% unknown 
covariance matrix $\Cov$. 
$\{\vx_i\}$, $\{\vdelta_i\}$, and $\{\epsilon_{it}\}$ are mutually independent. 
% where $\delta_{i,a} \stackrel{i.i.d.}{\sim} \mathcal{N}(0, \sigma_2^2)$ for an unknown parameter $\sigma_2$. 
In this model, the fixed effect term $\vPhi_{i}\vthe$ captures the task similarity through their features $\vx_i$, and the random effect term $\vdelta_i$ allows task heterogeneity. 
We assume the prior distribution $\vthe \sim \mathcal{N}(\vmu_\theta, \Cov_\theta)$ for some user-specified parameters $(\vmu_\theta, \Cov_\theta)$. 

% three types
% 1. x -> transform -> X
% 2. directly observe X
% 3. r_{i, a} = $\vx_i^T \vthe_{a}$
% 3. E(R_{i, t}| A_{i,t} = a) $\vx_i^T \vthe_{a}$


\begin{remark}
% , and results developed in this paper continue to hold. 
Additional structures can be imposed on $\Cov$ to derive a simper model. 
For example, one can require the arms of a task to have independent random effects by specifying $\Cov = \sigma_1^2 \vI$ for an unknown parameter $\sigma_1$, and one additional random effect term can be added at the task level by specifying $\Cov = \sigma_1^2 \vI + \sigma_2^2 \vJ$ with an additional unknown parameter $\sigma_2$. 
The induced models are popular choices in the literature on mixed effect models \citep{fitzmaurice2008primer}, and they are special cases of model \eqref{eqn:LMM}. 
\end{remark}

% The parameter $\Cov$, together with $\sigma^2$, can be learned from data via Empirical Bayes \citep{carlin2000bayes}  to adapt to the degree of heterogeneity and noise. 
% We will detail the procedure in Section \ref{sec:TS}. 



% Similar models have been widely considered in the literature on linear bandits \citep{chu2011contextual, tomkins2019intelligent}, although we utilize such a model to incorporate the task-specific features. 


\subsection{Thompson sampling for feature-based multi-task bandits}\label{sec:TS}
Thompson sampling is one of the most popular bandit framework \citep{agrawal2013further,russo2017tutorial,tomkins2020intelligentpooling}. 
The algorithm requires a prior over model parameters as the input, updates a posterior according to observed interactions, and samples an action to take according to its probability of being the optimal one. 
In this section, we develop a TS-type algorithm for the feature-based multi-task bandits problem with the objective of minimizing the Bayes regret. 


Suppose at a decision point,  
we have accumulated a dataset $\mathcal{D} = \{(A_{j}, R_{j}, i(j))\}_{j=1}^n$ of size $n$, where the data for all tasks have been combined and re-indexed. 
Here, $i(j)$ is the task index for the $j$-th tuple in $\mathcal{D}$, $A_{j}$ is the implemented action and $R_{j}$ is the observed reward. 
Suppose we are going to make decision for the $i$-th task at this time point. 
To adapt the TS algorithm, we need to derive the posterior of $\vr_i$ 
% , update the hyper-parameters, 
and sample an action to take. 
The full TS algorithm is summarized in Algorithm \ref{alg:TS}, with the key components detailed below. 
% should we talk about the action to take?
\input{Algorithm/alg_TS}

% The posterior will then be used to sample an action according to its probability of being the optimal one, in a Thompson sampling manner, as detailed in Algorithm \ref{alg:TS}. 
% posteriors for the expected rewards of arms in this task have analytic expressions. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% with calendar time $t_0$, _{t_0}
% $\mathcal{D} = \{(A_{i,t}, R_{i,t}, i)\}$ of size $n$
\textbf{Posterior updating.}
Given the model assumptions, the posteriors of $\vr_i$ have analytic expressions. 
We begin by introducing some notations. 
% model \eqref{eqn:R} and \eqref{eqn:LMM} together
The Bayesian linear mixed effect model \eqref{eqn:LMM} induces a kernel function $\mathcal{K}$, such that for any two tuples $O = (a, r, i)$ and $O' = (a', r', i')$, we have 
\begin{equation*}
    \mathcal{K}(O, O') = \vphi^T(\vx_i, a) \Cov_{\vthe} \vphi(\vx_{i'}, a') 
    + \Cov_{a, a'} \mathbb{I}(i = i'),
    % + \sigma_2^2 \mathbb{I}(i = i', a = a'),
\end{equation*}
where $\Cov_{a, a'}$ is the $(a,a')$-th entry of $\Cov$. 
Besides, let $\mK$ be a $n \times n$ kernel matrix of the pairwise kernel values for tuples in $\mathcal{D}$. 
Set $\vR = (R_1, \dots, R_n)^T$ be a $n$-dimensional vector of the observed rewards. 
% and $\vmu = (\mu_{A_1}(\vx_{i(1)}), \dots, \mu_{A_n}(\vx_{i(n)}))^T$. 
% $\vR$ be a $n$-dimensional vector with the $j$-th entry be the observed reward of the $j$-th tuple in $\mathcal{D}$, and 
Define $\vPhi$ as a $n \times d$ feature matrix with the $j$-th row be the feature vector $\vphi^T(\vx_{i(j)}, A_{j})$. %of the $j$-th tuple in $\mathcal{D}$. 
% For the $i$-th task, let $\vr_i = (r_{i1}, \dots, r_{iK})^T$. 
% $\mathcal{D} = \bigcup_{i,a} \mathcal{D}_{i,a}$, where $\mathcal{D}_{i,a}$ is empty if action $a$ has not been taken for task $i$ yet, and $\mathcal{D}_{i,a} = \{(A_{i,t}, R_{i,t}, i) : A_{i,t} = a\}$ otherwise. 
% Let $\vone_d$, $\vzero_d$, and $\vI_d$ be a d-dimensional vector of all ones, a d-dimensional vector of all zeros, and an identity matrix of dimension $d \times d$, respectively. 
% When the subscript is omitted, the appropriate dimension can be inferred from the context. 
Finally, for every $i \in [N]$, define a $K \times n$ matrix $\boldsymbol{M}_i$, such that the $(a, j)$-th entry of $\boldsymbol{M}_i$ is 
$\Cov_{A_j, a} * \I(i(j) = i)$. 
% $\sigma_2^2 * \I(i(j) = i, A_j = a)$. 
% is $\sigma^2$, if for the $j$-th tuple in $\mathcal{D}$, the task index is $i$ and the action we took is $a$. 
% The other entries of $\boldsymbol{M}_i$ are all zero. 
The posterior of $\vr_i$ conditional on the accumulated data follows a multivariate normal distribution $\rho(\vr_i)$, with mean and covariance as follows: 
\begin{equation}\label{eqn:post}
    \begin{split}
        \mathbb{E}(\vr_i|\mathcal{D}) &= \vPhi_{i} \vmu_{\vthe} + (\vPhi_i\Cov_{\vthe}\vPhi^T + \boldsymbol{M}_i) (\mK + \sigma^2 \vI)^{-1} (\vR - \vPhi \vmu_{\vthe}),  \\
        cov(\vr_i | \mathcal{D}) &= (\vPhi_{i} \Cov_{\vthe} \vPhi_{i}^T + \Cov) - (\vPhi_i\Cov_{\vthe}\vPhi^T + \boldsymbol{M}_i) (\mK + \sigma^2 \vI)^{-1} (\vPhi_i\Cov_{\vthe}\vPhi^T + \boldsymbol{M}_i)^T. 
    \end{split}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Action selection.} 
The posterior is used to sample an action in the TS manner. 
Specifically, 
we first sample a reward vector $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T \sim \rho(\vr_i)$, and then take the action $ \argmax_{a \in [K]} \tilde{r}_{i,a}$.  
% A_j = 
%  according to its probability of being the optimal one, 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \label{eqn:post}
% variance -> 0
% Interpretation: 
% $\mathbb{E}(r_{i,a}|\mathcal{D})$ is composed of two parts: $
% \vphi(\vx_i, a)^T\vmu_{\vthe} + (\vphi(\vx_i, a)^T\Cov_{\vthe}\vPhi^T)(\mK + \sigma^2 \vI)^{-1}(\vR - \vPhi \vmu_{\vthe})$
% and 
% $\boldsymbol{M}_i(\mK + \sigma^2 \vI)^{-1}(\vR - \vPhi \vmu_{\vthe})$. 
% Informally speaking, the first term is to estimate the fixed effect term $\vphi(\vx_i, a)^T \vthe$ and the second term is to estimate the random effect term $\delta_{i,a}$. 
% When there are no data points of taking action $a$ in task $i$ is $0$, the second term is $0$ and our estimation of $r_{i,a}$ depends on the information pooled from the other tasks; 
% While when the number of data points of taking action $a$ in task $i$ is large or when $\sigma_2$ is large, then second term will dominate, which implies we would like to rely more on the rewards generated by taking action $a$ in task $i$ itself. 


% \hl{prior; other task through X; its own experiment data; hyper-parameters}
% better prior 
% will still rely on the task-specific feedback to mitigate the potention bias. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% \textbf{Remark.} 
\begin{remark}
The linear assumption in \eqref{eqn:LMM} allows efficient computation and the model is less prone to over-fitting. 
% when the number of tasks $N$ is not large. 
% bias variance
Nevertheless, the idea of utilizing task-specific features in multi-task bandits via a mixed effect model is generally applicable. % and not limited to the linear form
One can replace $\vPhi_{i}\vthe$ in \eqref{eqn:LMM} with $f(\vx_i; \vthe)$ for some non-parametric function $f(\cdot)$, and proceed in a similar way. 
 As an example, a mixed-effect Gaussian process model and the corresponding TS algorithm are derived in Appendix \ref{sec:GP}. % provided
\end{remark}
% Can theory be extended? the linear. As long as the regression model converge. 
% The other has no explicit form
% Which also allows explicit
% really? except for GP, other can be derive?

At each decision point, the computation will be dominated by the calculation of the matrix inverse and the determinant for $(\mK + \sigma^2 \vI)$, which suffers from a cubic complexity $O(n^3)$ as well-known in the Gaussian process literature. 
In Appendix \ref{sec:implementation}, we introduce an efficient implementation, which utilizes the block structure induced by the mixed effect model via using the well-known Woodbury matrix identity \citep{rasmussen2003gaussian}. 

% To alleviate the computational burden, we
% Step \eqref{eqn:post} and \eqref{eqn:Hyper-parameter} are both closely related with the kernel function and the matrix inverse. 


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Additional_Related_Work.tex <==
\section{Additional Related Work}\label{sec:appendix_additional_related_work}
In this section, we compare this paper with additional related works. 
To begin with, we note that there are several terms used in the literature for problems concerned with multiple tasks, which is often a source of confusion. 
Based on  \cite{hospedales2020meta}, 
\textit{meta learning} assumes tasks are drawn from a distribution and aims to maximize the average performance over this task distribution (\textit{meta-objective}); 
\textit{transfer learning} uses data from finished tasks to improve the performance on a new task, and typically focuses on the single-task objective, although the viewpoint of meta learning can be applied to achieve this goal (as in the sequential setting of our work); 
\textit{multi-task learning} aims to jointly learn a few tasks, where typically the number of tasks is fixed and the meta-objective is not adopted, although the viewpoint of meta learning can be applied in these problems as well (as in the concurrent setting of our work). 
There are often some overlaps between these concepts. 
In this work, we adopt the task distribution viewpoint as well as the meta-objective \cite{hospedales2020meta}, which are naturally related with our hierarchical Bayesian framework, allows us to model heterogeneity, and enables knowledge sharing via constructing informative priors. 
We refer to our problem as multi-task bandits to focus on the fact that there are multiple tasks, since our methodology is applicable to the sequential setting (transfer learning), the concurrent setting (multi-task learning), and even more complex settings. 
% Continual learning (CL) Continual or lifelong learning

% Low-rank bandits. is an extention
According to the taxonomy developed in \cite{zhang2017survey}, multi-task algorithms can be classified into the feature learning approach, low-rank approach, task clustering approach, task relation learning approach, and decomposition approach. 
In the bandit literature, \cite{yang2021impact} considers that one interacts with multiple linear bandit
tasks concurrently and the coefficient vectors of these tasks share the same low-dimensional space, and hence belongs to the feature learning approach; 
\cite{kveton2017stochastic} studies finding the maximum entry of a low-rank matrix in a bandit manner and \cite{jun2019bilinear} assumes the coefficient matrix of a bilinear bandit problem is low-rank, and hence they belong to the low-rank approach; 
clustering of bandits \citep{gentile2014online, li2016collaborative} and latent bandits \citep{hong2020latent, hong2020non} assume there is a perfect clustered structure, and hence they belong  to the task clustering approach. 
In contrast to these papers, our work belongs to the relation learning approach, which aims to learn the task relations from data by assuming some probabilistic model or applying some penalty function. 
Our approach provides nice interpretability and is flexible with arguably less strict assumptions.  
In particular, to the best of our knowledge, this is the \textit{first} work that can leverage the task-specific metadata in multi-task bandits, which is an important information source that none of the existing methods can utilize. 
Although we focus on MAB in the main text, the idea of utilizing metadata is generally applicable. 
We discuss its extensions to linear bandits and clustering of bandits in Appendix \ref{sec:extension_contextual}. 


Besides, similar with meta MAB, there are also several works on meta linear bandits. 
Meta linear bandits studies the problem where the coefficients of multiple linear bandit tasks are close \citep{multilinear} or are drawn from one prior distribution \citep{metapricing, tomkins2019intelligent, cella2020meta}. 
% IP in the appendix. % random coeffcient model % share some similar technical tools 
Therefore, these works focus on a different problem from ours and they also did not model the task relations with metadata. 
In addition, \cite{ortega2019meta} proposes a sequential strategy for meta bandits, but as noted in \cite{hsu2019empirical}, no efficient algorithm has been proposed. 
Lastly, we note that there are two papers \cite{deshmukh2017multi, krause2011contextual} applying multi-task learning to share information across multiple arms of a single task, and hence they have a totally different focus from ours. 

% metadata and BHM is main.
% : transfer RL survey. 
% In the main text, we focus on the literature on bandits. 
% at a high level, 
Our bandit problem is certainly related to Reinforcement Learning (RL). 
In recent years, there is a surge of interest in multi-task RL, transfer RL, and meta RL. 
See \cite{zhu2020transfer} and \cite{vithayathil2020survey} for some recent surveys. 
Among the existing works, 
\cite{wilson2007multi, lazaric2010bayesian, grant2018recasting} consider applying Bayesian hierarchical model to multi-task/meta RL. 
However, none of these works can utilize the metadata, which is an important and ubiquitous information source. 
In the concurrent work \cite{sodhani2021multi}, the authors, for the first time, consider using metadata in multi-task reinforcement learning to infer the appropriate state representation for each task. 
They consider a finite set of state encoders, design a special-purpose neural network, and train the whole pipeline end-to-end. 
In contrast, 
we study MAB, allow infinite number of task instances, aim to learn the average reward of each task instead of state representation,  design a unified Bayesian Hierarchical model framework for this problem, and establish theoretical guarantees. 
Therefore, although both work consider similar types of side information (i.e., metadata), the problem and methodology are fundamentally different. 


Finally, we would like to further compare our setup with CMAB, and discuss the limitations of adopting CMAB in our problem. 
In the standard contextual MAB setup, we assume $\Mean(R_{i,t}|S_{i,t} = s, A_{i,t} = a) = g(s, a;\gamma)$ for some function $g$, where $S_{i,t}$ is the context. 
Therefore, it already allows the randomness of $R_{i,t}$. 
In our setup,  by regarding the metadata as "contexts" and neglecting the task identities, the relationship is equal to $\Mean(R_{i,t}|\vx_{i} = \vx, A_{i,t} = a) = g(\vx, a;\gamma)$, where we note that the expectation is taken over all tasks with metadata $\vx$. 
This implies that for all tasks with the same metadata, the decision rule will be always the same, no matter what their action-reward history is. 
Instead, our setup adds another layer to allow variations of $\vr_i$ conditional on $\vx_i$. 
In another word, we utilize the predictive power of $\vx_i$ but does not assume $\vr_i$ can be fully determined by it. 
% by neglecting the task identities and regarding the metadata as "contexts". % static metadata
% and hence it is reasonable to assume $\vr_i = f(\vx_i)$
% Recall that $\vr_i$ is the expected reward vector for all arms

% warm-starting bandit / offline data: the same bandit task
% collaborative filtering: metaTS

% ,  assumes such a clustered structure has been learned from logged data. 
% Multi-task Linear Bandits: sequential, epsilon


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Additional_Results.tex <==
\section{Additional Experiment Results}\label{sec:appendix_addi_numerical_results}

\subsection{Robustness to model misspecifications}\label{sec:appendix_robustness}
To allow efficient information sharing, we make a model assumption that $\vr_i | \vx_i, \vthe \sim f(\vr_i | \vx_i, \vthe), \forall i \in [N]$. 
When this model is correctly specified, we have shown superior theoretical and numerical performance of {\name}. 
However, we acknowledge that all models can be misspecifed. 
Intuitively, the model is used to pool information to provide an informative prior. 
As long as the learned prior is not significantly worse than a manually specified one, the performance would be comparable; and when the prior contains more information, we can attain a lower regret. 

We empirically investigate the robustness of {\name} in this section. 
We focus on the Gaussian bandits case under the concurrent setting. 
Findings under the other settings are largely the same and hence omitted. 
Specifically, 
instead of generating data according to $\vr_i = \vPhi_{i}\vthe + \vdelta_i$, we consider the data generation process $\vr_i = (1 - \lambda) cos(c\vPhi_{i}\vthe)/c + \lambda \vPhi_{i}\vthe  + \vdelta_i$, where $cos$ applies the cosine function to each entry, 
c is a normalization constant such that the entries of $\vPhi_{i}\vthe$ are all in $[-\pi/2,\pi/2]$, 
and $\lambda \in [0,1]$ controls the degree of misspecification. 
When $\lambda = 1$, we are considering the LMM; while when $\lambda = 0$, the metadata  provides few  information through such a linear form. 

In results reported in Figure \ref{fig:simu_Gaussian_robustness_concurrent}, we observe that {\name} is fairly robust to model misspecifications. 
When $\lambda = 1/2$ or $3/4$, that is, when there exists mild or moderate misspecification, {\name} still yields much lower regrets than individual-TS and meta-TS. 
When $\lambda = 1/4$, the performance of {\name} becomes comparable with individual-TS and meta-TS. 
Only when $\lambda = 0$, that is, the metadata are useless through a linear form, {\name} shows slightly higher regret in the initial period due to the additionally introduced variance. 
As expected, linear-TS and OSFA both severely suffer from the bias. 
Notably, in all cases, {\name} always yields the desired sublinear Bayes regret in $T$, as expected. 
Therefore, it shows that, even when the model is severely misspecified, the cost would be acceptable. 



\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/mis_cos_0.75_0.25_concurrent.png}
         \caption{$\lambda = 3/4$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/mis_cos_0.5_0.5_concurrent.png}
         \caption{$\lambda = 1/2$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/mis_cos_0.25_0.75_concurrent.png}
         \caption{$\lambda = 1/4$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/mis_cos_0_1_concurrent.png}
         \caption{$\lambda = 0$}
     \end{subfigure}
     \\
\caption{
Average Bayes regret for Gaussian bandits with misspecified hierarchical models. 
A smaller value of $\lambda$ implies a more severe misspecification. 
The regrets of OSFA are an order of magnitude higher and hence hidden. 
}
% The yellow line (TR, m = 2) and green line (TR, m = 3) are largely overlapped
\label{fig:simu_Gaussian_robustness_concurrent}
\end{figure}


% \begin{figure}[t]
%      \centering
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/mis_cos_0_1_episodic.png}
%          \caption{$\lambda = 0$}
%      \end{subfigure}
%      \\
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/mis_cos_0.25_0.75_episodic.png}
%          \caption{$\lambda = 1/4$}
%      \end{subfigure}
%      \\
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/mis_cos_0.5_0.5_episodic.png}
%          \caption{$\lambda = 1/2$}
%      \end{subfigure}
%      \\
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/mis_cos_0.75_0.25_episodic.png}
%          \caption{$\lambda = 3/4$}
%      \end{subfigure}
%      \\
% \caption{
% Average Bayes regret for Gaussian bandits with misspecified hierarchical models. 
% A smaller value of $\lambda$ implies a more serious misspecification. 
% The regrets of OSFA are an order of magnitude higher and hence hidden in the upper subplots. 
% }
% % The yellow line (TR, m = 2) and green line (TR, m = 3) are largely overlapped
% \label{fig:simu_Gaussian_robustness_concurrent}
% \end{figure}


\subsection{Multi-task regrets}\label{sec:appendix_figure_MTR}
In the main text, we report the Bayes regret of different algorithms. 
Although the multi-task regrets for those figures can also be derived according to its definition, we choose to explicitly report them again in this section, in order to make the comparison more clearly. 

Specifically, the multi-task regrets for Gaussian bandits and Bernoulli bandits are presented in Figure \ref{fig:simu_Gaussian_multi-task}  and \ref{fig:simu_Binary_multi-task}, respectively. 
In the sequential setting, we can see the multi-task regrets of {\name} converge to zero, while meta-TS and individual-TS have a constant regret, and linear-TS as well as OSFA suffer from the bias. 


\begin{figure}[h]
     \centering
 \begin{subfigure}[b]{\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Figures/Gaussian_all_6_MTR.png}
    %  \caption{Episodic, $\sigma_3 = 5$}
    %  \label{fig:y equals x}
 \end{subfigure}
\caption{
Gaussian bandits: 
the solid lines denote the average multi-task regret with the shared areas indicating the standard errors.  
The regrets of OSFA are much higher in some subplots and hence hidden.
}
% an order of magnitude
% The yellow line (TR, m = 2) and green line (TR, m = 3) are largely overlapped
\label{fig:simu_Gaussian_multi-task}
\end{figure}
\begin{figure}[h]
 \centering
 \begin{subfigure}[b]{\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Figures/binary_all_6_MTR.png}
    %  \caption{Episodic, $\sigma_3 = 5$}
    %  \label{fig:y equals x}
 \end{subfigure}
\caption{
Bernoulli bandits: 
the solid lines denote the average multi-task regret with the shared areas indicating the standard errors.  
A larger value of $\psi$ implies a larger variation of $\vr_i$ condition on $\vx_i$. 
}
\vspace{-0.3cm}
\label{fig:simu_Binary_multi-task}
\end{figure}



\subsection{Trends with experiment hyper-parameters}\label{sec:appendix_more}
In this section, we report additional results under other combinations of $(K, d, T, N)$, to show that our conclusions in the main text are representative, and study the trend of the performance of {\name}. 
We focus on the Gaussian bandits case under the concurrent setting. 
To save computational cost, we set the base combination of hyper-parameters as $\sigma_1^2 = 0.5$, $K = 8$, $d = 15$, $N = 100$, and $T = 100$, and run $50$ random seeds for each. 

In Figure \ref{fig:simu_Gaussian_trend}, we vary the value of $K$, $d$, $N$, $\sigma$ individually. 
Overall, {\name} consistently demonstrates lower regrets and shows robustness. 
Our findings can be summarized as follows. 
\begin{itemize}
    % we also share information across arms... it is like cheating...
    \item As $K$ increases, the learning problem for all algorithm becomes more difficult. {\name} still demonstrates better performance, and even when $T = 100$, its advantage is still fairly clear.
    \item As $d$ increases, the learning problem for {\name} becomes more difficult, while it still shows much better performance. 
    \item As $\sigma$ increases, overall the learning problem for all algorithm becomes more difficult. {\name} still demonstrates better performance, and even when $T = 100$, its advantage is still fairly clear.
    \item As $N$ increases, {\name} can learn the task distribution more easily and its performance converges to that of oracle-TS more quickly. 
\end{itemize}

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/trend_K0.5.png}
        %  \caption{$\lambda = 3/4$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/trend_d0.5.png}
        %  \caption{$\lambda = 1/4$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/trend_sigma0.5.png}
        %  \caption{$\lambda = 0$}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/trend_N0.5.png}
        %  \caption{$\lambda = 1/2$}
     \end{subfigure}
     \\
\caption{
Trends of the average Bayes regret for Gaussian bandits with different parameters. 
% under different settings. . 
}
% The yellow line (TR, m = 2) and green line (TR, m = 3) are largely overlapped
\label{fig:simu_Gaussian_trend}
\end{figure}


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Algorithm/TS_faster_binary.tex <==
\begin{algorithm}[!h]
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
\SetAlgoLined
\Input{
$\prob(\vthe)$, $\phi$, updating frequency $l$
% Prior parameters $\vmu_\theta$, $\Cov_\theta$, $\Cov$ and $\sigma^2$
% , initial values 
}

% \textbf{Initialization.} 
Set $\mH = \{\}$ and $\prob(\vthe| \mH) = \prob(\vthe)$

\For{decision point $j = 0, \dots$,}{ 
% \For{all decision point (i,t)}{ 
\If{$j = k * l$ for some constant $k$}{
Apply approximate posterior inference methods (such as Gibbs sampling or variational inference) to sample one $\Tilde{\vthe}$ from  $\prob(\vthe| \mH)$\\
}


Retrieve the task index $i$\\
Sample a reward vector $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T$ 
from 
$c * f_{Beta}(\vr_i|\vx_i, \Tilde{\vthe}) \prob(\mH_i|\vr_i) $, where $c$ is a normalization factor. 
% , where $f(\vr_i|\vx_i, \Tilde{\vthe})$ is the Beta distribution specified by the first equation of \eqref{eqn:BBLM}, $\prob(\mH_i|\vr_i)$ is the likelihood over $\mH_i$ 
% for the Bernoulli distribution specified by the second equation of \eqref{eqn:BBLM}, 
% and $c$ is a normalization factor
\\ 
Take action $A_j = argmax_{a \in [K]} \; \tilde{r}_{i,a}$\\ %$A_{i,t}$
Receive reward $R_j$\\ % R_{i,t}
Update the dataset as $\mH \leftarrow \mH \cup \{(A_{j}, R_{j}, \vx_i, i)\}$
% \\
% Update the hyper-parameter  $\sigma$ and  $\Cov$  according to 
% \eqref{eqn:Hyper-parameter}
\\
}
 \caption{Efficient 
 Implementation of {\name} for  Bernoulli Bandits}\label{alg:TS_faster_binary}
\end{algorithm}


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Algorithm/alg_TS.tex <==


\begin{algorithm}[!t]
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
\SetAlgoLined
\Input{
Prior $\prob(\vthe)$ and known parameters of the hierarchical model
% a specified hierarchical model, 
% Prior parameters $\vmu_\theta$, $\Cov_\theta$, $\Cov$ and $\sigma^2$
% , initial values 
}

% \textbf{Initialization.} 
Set $\mH = \{\}$

\For{every decision point j}{ 
% \For{all decision point (i,t)}{ 
Retrieve the task index $i$\\
Compute the posterior for $\vr_{i}$ as $\prob(\vr_i | \mH)$, according to the  hierarchical model \eqref{eqn:hierachical_model}
(see Section \ref{sec:LMM} and \ref{sec:binary} for examples)\\
% a normal distribution $\rho(\vr_{i})$, the parameters of which are computed according to \eqref{eqn:post}\\ 
Sample a reward vector $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T \sim \prob(\vr_i | \mH)$ \\ 
Take action $A_j = argmax_{a \in [K]} \; \tilde{r}_{i,a}$\\ %$A_{i,t}$
Receive reward $R_j$\\ % R_{i,t}
Update the dataset as $\mH \leftarrow \mH \cup \{(A_{j}, R_{j}, \vx_i, i)\}$
% \\
% Update the hyper-parameter  $\sigma$ and  $\Cov$  according to 
% \eqref{eqn:Hyper-parameter}
\\
}
% Thompson Sampling for Feature-based Multi-Task Bandits
 \caption{{\name}: Multi-task Thompson Sampling}\label{alg:TS}
\end{algorithm}




==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Algorithm/alg_TS_faster.tex <==
\begin{algorithm}[!t]
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
\SetAlgoLined
\Input{
Prior $\prob(\vthe)$ and known parameters of the hierarchical model
% Prior parameters $\vmu_\theta$, $\Cov_\theta$, $\Cov$ and $\sigma^2$
% , initial values 
}

% \textbf{Initialization.} 
Set $\mH = \{\}$ and $\prob(\vthe| \mH) = \prob(\vthe)$

\For{task $i \in [N]$}{

Sample one $\Tilde{\vthe}$ from the current posterior $\prob(\vthe| \mH)$
% $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T \sim \prob(\vr_i | \mH)$ \\ 

Apply $TS\big(f(\vr_i|\vx_i, \Tilde{\vthe})\big)$ to task $i$ for $T_i$ rounds, and collect observed data as $\mH_i$
% update $\mH$ with observed action-reward pairs\\

Update  $\mH =  \mH \cup \mH_i$

% the hierarchical model
Update the posterior of $\vthe$ according to the  hierarchical model \eqref{eqn:hierachical_model}
% , with $\prob(\vthe | \mH)$ as the prior and $\mH_i$ as the data



}

\caption{Computationally Efficient Variant of {\name} under the Sequential Setting}\label{alg:TS_faster}
\end{algorithm}


% \For{$t \in [T]$}{

% % a normal distribution $\rho(\vr_{i})$, the parameters of which are computed according to \eqref{eqn:post}\\ 
% Take action $A_j = argmax_a \{\tilde{r}_{i,a}\}_{a=1}^K$\\ %$A_{i,t}$
% Receive reward $R_j$\\ % R_{i,t}
% Update the dataset as $\mH \leftarrow \mH \cup \{(A_{j}, R_{j}, \vx_i, i)\}$


% }


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Algorithm/alg_TS_faster_general.tex <==
\begin{algorithm}[!h]
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
\SetAlgoLined
\Input{
$\prob(\vthe)$, $\phi$, updating frequency $l$
% Prior parameters $\vmu_\theta$, $\Cov_\theta$, $\Cov$ and $\sigma^2$
% , initial values 
}

% \textbf{Initialization.} 
Set $\mH = \{\}$ and $\prob(\vthe| \mH) = \prob(\vthe)$

\For{decision point $j = 0, \dots$,}{ 
% \For{all decision point (i,t)}{ 
\If{$mod(j, l) = 0$}{
Update $\prob(\vthe| \mH)$ (possibly via approximate posterior inference methods, such as Gibbs sampling or variational inference)

Sample one $\Tilde{\vthe}$ from  $\prob(\vthe| \mH)$\\
}


Retrieve the task index $i$\\
Sample a reward vector $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T$ 
from 
$c * f(\vr_i|\vx_i, \Tilde{\vthe}) \prob(\mH_i|\vr_i) $, where $c$ is a normalization factor. 
% , where $f(\vr_i|\vx_i, \Tilde{\vthe})$ is the Beta distribution specified by the first equation of \eqref{eqn:BBLM}, $\prob(\mH_i|\vr_i)$ is the likelihood over $\mH_i$ 
% for the Bernoulli distribution specified by the second equation of \eqref{eqn:BBLM}, 
% and $c$ is a normalization factor
\\ 
Take action $A_j = argmax_{a \in [K]} \; \tilde{r}_{i,a}$\\ %$A_{i,t}$
Receive reward $R_j$\\ % R_{i,t}
Update the dataset as $\mH \leftarrow \mH \cup \{(A_{j}, R_{j}, \vx_i, i)\}$
% \\
% Update the hyper-parameter  $\sigma$ and  $\Cov$  according to 
% \eqref{eqn:Hyper-parameter}
\\
}
 \caption{Computationally Efficient Variant of {\name} under General Settings}\label{alg:TS_faster_general}
\end{algorithm}


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Algorithm/alg_modified_MTS.tex <==
\begin{algorithm}[!h]
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{output}
\SetAlgoLined
\Input{
$\prob(\vthe)$ and known parameters for the hierarchical model
% Prior parameters $\vmu_\theta$, $\Cov_\theta$, $\Cov$ and $\sigma^2$
% , initial values 
}

% \textbf{Initialization.} 
Set $\mH = \{\}$ and $\prob(\vthe| \mH) = \prob(\vthe)$

Set $count(i) = 0, \forall i \in [N]$

\For{each decision point $j$}{
Retrieve the task index $i$\\

\uIf{count(i) < K}{
    count(i) = count(i) + 1

    Take action $A_j = count(i)$ \tcp*{Alignment period}
}
\Else{ 
Sample a reward vector $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T$ 
from 
$c * \prob(\mH_i|\vr_i)  f(\vr_i|\vx_i, \Tilde{\vthe}_i)$, where $c$ is a normalization factor. \tcp*{TS with prior $f(\vr_i|\vx_i, \Tilde{\vthe}_i)$}

Take action $A_j = argmax_{a \in [K]} \; \tilde{r}_{i,a}$
}


Receive reward $R_j$\\ % R_{i,t}
Update the dataset as $\mH \leftarrow \mH \cup \{(A_{j}, R_{j}, \vx_i, i)\}$

\uIf{count(i) = K}{ 
Sample one $\Tilde{\vthe}$ from  $\prob(\vthe| \mH)$, and denote it as $\Tilde{\vthe}_i$ \tcp*{Fixed down the prior for task $i$}
}

% $(\tilde{r}_{i,1}, \dots, \tilde{r}_{i,K})^T \sim \prob(\vr_i | \mH)$ \\ 

% Interact with task $i$ for $T_i$ rounds with $TS\big(f(\vr_i|\vx_i, \Tilde{\vthe})\big)$, and update $\mH$ with observed action-reward pairs\\


% Update the posterior $\prob(\vthe | \mH)$, according to the hierarchical model\\


}

 \caption{The Modified {\name}}\label{alg:modified_MTS}
\end{algorithm}


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Details_Experiment.tex <==
\section{More on the Experiment Details}\label{sec:appendix_Experiment_Details}
In this section, we report additional details of our epperiments and implementations. 
Recall that we use $\vI$ to denote identity matrix, the  dimension of which can be inferred from the context. 

\subsection{Hyperparameters}
Since all baselines that we consider are TS-type algorithms, we need to specify (i) the priors and (ii) the variance terms which are assumed to be known. 
For fair comparisons, we apply the law of total expectation and the law of total variance to derive these quantities. 
Roughly speaking, for meta-TS, we marginalize out $(\vx, \vr)$ conditional on $\vthe$; 
for individual-TS and OSFA, we additionally marginalize out $\vthe$; 
For linear-TS or GLM-TS, we use the same prior of $\vthe$ as {\name}, and marginalize $\vr_i$ conditional on $\vx_i$ to set the variance of the stochastic reward variable. 
When the marginal distribution does not belong to a standard distribution family, we use the Gaussian distribution as an approximation. 


\paragraph{Gaussian bandits.}
According to our data generation model, based on the law of total expectation and the law of total variance, it is easy to verify that 
\begin{align*}
    cov \big( \vr_i \big | \vthe, \vx_i)
    &= \Cov = \sigma_1^2 \vI\\
    %%%%%%%%%%%%%%%%%%%%%%%%
    \Mean \big( \vr_i \big | \vthe)  &= \vthe_{1:K},\\ 
    %%%%%%%%%%%%%%%%%%%%%%%%
    cov \big( \vr_i \big | \vthe)
    &= \Mean\big(
    cov\big(\vr_i | \vx_i \big)
    \big | \vthe)
    +
    cov\big(
    \Mean\big(\vr_i | \vx_i \big)
    \big | \vthe)\\
    % &= \sigma_1^2 \vI + ||\vthe||^2 \vI, 
    &= \sigma_1^2 \vI + ||\vthe_{(K+1):d}||^2 \vI
    = (\sigma_1^2 + ||\vthe_{(K+1):d}||^2) \vI, \\
    %%%%%%%%%%%%%%%%%%%%%%%%
    \Mean \big( \vr_i \big) &= \vzero\\
    %%%%%%%%%%%%%%%%%%%%%%%%
    cov \big( \vr_i \big)
    &= \Mean\big(
    cov\big(\vr_i  | \vthe \big)
    \big)
    +
    cov\big(
    \Mean\big(\vr_i | \vthe \big)
    \big)\\
    &= \big(\sigma_1^2 + \Mean(||\vthe_{(K+1):d}||^2)\big) \vI + d^{-1} \vI\\
    &= \big(\sigma_1^2 + \Mean(||\vthe_{(K+1):d}||^2) + d^{-1}\big) \vI,
\end{align*}
where $\vthe_{1:K}$ is the first $K$ entries of $\vthe$, and $\vthe_{(K+1):d}$ is the remaining entries. 
Therefore, for OSFA and individual-TS, we use  $\normal\big(\vzero, 
\big(\sigma_1^2 + \Mean(||\vthe_{(K+1):d}||^2) + d^{-1}\big) \vI 
\big)$ as the prior; 
for meta-TS, we use $\normal\big(\vmu, (\sigma_1^2 + ||\vthe_{(K+1):d}||^2) \vI \big)$ as the \textit{unknown} prior, with $\vmu$ as an unknown parameter
, and use 
$ \Mean \big( \vr_i \big | \vthe) =  \vthe_{1:K} \sim \normal(\vzero, d^{-1}\vI)$ as the hyper-prior for $\vmu$; 
for linear-TS, we use $\normal(0, d^{-1}\vI)$ as the prior for the regression coefficients $\vthe$ and $\sigma_1^2 + \sigma^2$ as the variance term of the stochastic reward variable. 

\paragraph{Bernoulli bandits.}
According to our data generation model, based on the law of total expectation and the law of total variance, 
recall the discussion on the parameterization of Beta distributions in Appendix \ref{sec: beta_parameterization}
it is easy to verify that 
\begin{align*}
    \Mean \big( \vr_i \big | \vthe)  &= (\Mean(logistic(\vphi(\vx_1, a)^T \vthe)|\vthe), \dots, \Mean(logistic(\vphi(\vx_K, a)^T \vthe)|\vthe))^T \\
    %%%%%%%%%%%%%%%%%%%%%%%%
    cov \big( \vr_i \big | \vthe)
    &= \Mean\big(
    cov\big(\vr_i | \vx_i \big)
    \big | \vthe)
    +
    cov\big(
    \Mean\big(\vr_i | \vx_i \big)
    \big | \vthe)\\
    %&= c_b \vI + c_b' \vI\\
    &= diag(c_{b,1}, \dots, c_{b,K}) + diag(c'_{b,1}, \dots, c'_{b,K})\\
    %%%%%%%%%%%%%%%%%%%%%%%%
    \Mean \big( \vr_i \big) &= \frac{1}{2} * \vone\\
    %%%%%%%%%%%%%%%%%%%%%%%%
    cov \big( \vr_i \big)
    &= \Mean\big(
    cov\big(\vr_i  | \vthe \big)
    \big)
    +
    cov\big(
    \Mean\big(\vr_i | \vthe \big)
    \big), 
    % \\
    % &= \big(\sigma_1^2 + \Mean(||\vthe_{(K+1):d}||^2)\big) \vI + d^{-1} \vI\\
    % &= \big(\sigma_1^2 + \Mean(||\vthe_{(K+1):d}||^2) + d^{-1}\big) \vI
\end{align*}
where $c_{b,i} = \frac{\psi}{1 + \psi} \Mean_{\vx}(logistic(\vphi(\vx_i, a)^T \vthe) (1 - logistic(\vphi(\vx_i, a)^T \vthe))|\vthe)$, 
and $c_{b,i}' = var_{\vx}(logistic(\vphi(\vx_i, a)^T \vthe)|\vthe)$. 
We obtain these two quantities as well as $\Mean \big( \vr_i \big | \vthe)$ and 
$cov \big( \vr_i \big)$ 
via Monte carlo simulation, since there is no explicit form. 

Define $\psi(\mu, \sigma^2_2) = [\mu(1-\mu) / \sigma^2_2 - 1]^{-1}$.
% Let $\mu = 1 / 2$ and $\psi = 1 / (1 / (c_b + c_b') - 1)$. 
For OSFA and individual-TS, we use  $Beta\big(1 / 2, \psi(1/2, cov \big( \vr_i \big))\big)$ as the prior for each arm; 
for meta-TS, following the implementations in \cite{kveton2021meta}, we randomly pick a set of Beta distributions as candidates, with $Beta\big( \Mean \big( \vr_i \big | \vthe), \psi(\Mean \big( \vr_i \big | \vthe), cov \big( \vr_i|\vx_i \big)) \big)$ as one of them, and maintain a Categorical distribution over them, with the uniform one as the initial prior; 
Finally, for GLB-TS, we choose the TS algorithm proposed in \cite{kveton2020randomized}, and set the exploration parameter $\alpha = 1$ as in \cite{kveton2020randomized}. 
% use $\normal(0, d^{-1}\vI)$ as the prior for the regression coefficients (no variance term for the stochastic reward variable is needed). 
% as the hyper-prior



% In this section, we present results with $N = 40$ and $T_1 = \dots = T_N = T = 50$. 
% We consider two kinds of task sequence:
% (i) the episodic setting, where we begin to interact with the $(i + 1)$-th task only after we finish the $i$-th task, % the $T$ interactions with
% and (ii) the concurrent setting, where we interact with every task for their $t$-th time simultaneously, and then interact for the $(t + 1)$-th time. % with them
% We set $K = 10$, $p = 10$, $\sigma = 1$, and $\Cov = \sigma_3^2 \vI$ for some hyper-parameter $\sigma_3$. Here, $\sigma_3^2$ controls the magnitude of the random effect term, which indicates how useful the task-specific metadata are. 
% % some efforts here. 
% The metadata $\{\vx_i\}$ are randomly generated from the standard multivariate normal distribution and the coefficient vector $\vthe$ is sampled from $\mathcal{N}(0, d^{-1}\vI)$. 
% To set the prior for the four competing TS algorithms, we integrate out $(\vx,\vr)$ to specify the mean part and apply the law of total variance to specify the variance part. 


% $\vr_i \sim \normal(\vzero, )$
% Before all random seeds, we use the same $\vthe$ sampled from $\mathcal{N}(0, d^{-1}\vI)$. 

% \begin{equation}
%     \begin{split}
%             r_{i,a} &\sim Beta\big(logistic(\vphi(\vx_i, a)^T \vthe), \psi \big), \forall a \in [K],\\
%     % \vr_i &\sim Beta(logistic(\vPhi_i\vthe), \psi)\\
%     R_{i,t} &\sim Bernoulli \big(\sum_a \I(A_{i, t} = a) r_{i, a} \big), 
%     \end{split}
% \end{equation}

\subsection{Implementation Details}

\paragraph{Implementation of Meta-TS under the concurrent setting.}
The original meta-TS proposed in \cite{kveton2021meta} can only be applied to the episodic setting and does not fit in the concurrent setting. 
Based on their models, we derived the posterior and adapt meta-TS to the concurrent setting, as follows. 
For Gaussian bandits, meta-TS aims to learn the unknown parameter $\vmu_m = \Mean(\vr_i)$, and assumes 
$\vr_i \sim \normal \big(\vmu_m, \sigma^2_m \vI \big)$ for some known $\sigma^2_m$. 
See the last subsection for details. 
Therefore, given a dataset  $\mH = \{(A_{j}, R_{j}, \vx_{j}, i(j))\}$, the posterior of $\vmu_m$ can be derived as follows. 
The entries of $\vmu_m$ are independent. 
Let $\Bar{R}_{i,a}$ denote the mean observed reward for taking action $a$ in task $i$, and $n_{i,a}$ be the count. 
Then we have $\Bar{R}_{i,a} \sim \normal\big( \mu_{m,a}, \sigma_1^2 + \sigma^2 / n_{i,a} \big)$. 
Note the prior for $\mu_{m,a}$ is $\normal(0, d^{-1})$. 
Let $\sigma_{i,a} = \sqrt{\sigma_1^2 + \sigma^2 / n_{i,a}}$. 
We have 
\begin{align*}
    \prob \Big[ \mu_{m,a}  |\mH \Big] \sim \normal 
    \Big(\frac{\sum_i \Bar{R}_{i,a} / \sigma_{i,a}^2 }{\sum_i \sigma_{i,a}^{-2} + d}
    , (\sum_i \sigma_{i,a}^{-2} + d)^{-1}
    \Big), \forall a \in [K]
\end{align*}
Then, at each decision point, we sample one $\Tilde{\vmu}_m$, and treat $\vr_i \sim \normal \big(\Tilde{\vmu}_m, \sigma^2_m \vI \big)$ as the prior to proceed with a standard single-task Gaussian TS algorithm. 
We similarly modified meta-TS for the Bernoulli bandits. 
% \begin{align*}
%     \prob \Big[ \vmu_m  |\mH \Big]
%     &= \frac{\prob(\vmu_m) \prob(\mH|\vmu_m)}{\int_{\vmu_m} \prob(\vmu_m)
%     }\\
%     &= \frac{\prob(\vmu_m) 
%     \prod_i \prob(\vr_i|\vmu_m) \prob(\mH_i|\vr_i)
%     }{\int_{\vmu_m} 
%     \prob(\vmu_m) 
%     \prod_i \prob(\vr_i|\vmu_m) \prob(\mH_i|\vr_i)
%     }
% \end{align*}



\paragraph{Implementation of {\name}.}
For Bernoulli bandits, we use the Python package \textsf{PyMC3} and adopt a popular MCMC algorithm , NUTS \cite{hoffman2014no}. 
The acceptance rate is set as $0.85$, and the number of samples per time is set as $2000$. 
% The No-U-Turn Sampler
For the computationally efficient variant of {\name}, 
in both Gaussian bandits and Bernoulli bandits, 
we sample a new $\vthe$ at the end of interactions with a task under the sequential setting, and at the end of a round under the concurrent setting. 


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Extension_Contextual.tex <==
\subsection{Extension to contextual bandits}\label{sec:extension_contextual}
In this section, we discuss several possible directions to extend the metadata-based multi-task bandit framework to contextual bandits. 
We consider the following formulation of contextual bandits (the other formulations can be similarly derived). 
For each task $i \in [N]$, at each decision point $t$, 
the agent choose an arm $A_{i,t} \in \mathcal{R}^p$, and then receive a stochastic reward $R_{i,t} \sim f(A_{i,t};\vbeta_i)$, where $\vbeta_i$ is a length-$d$ vector of unknown parameters associated with task $i$. 
Here, $A_{i,t}$ is a feature vector which is a function of the context and the pulled arm. 
In addition, each task has a $p$-dimensional feature vector $\vx_i$ (i.e., metadata). 
% observe a feature $S_{i,t}$, 

A straightforward extension of the methodology presented in the main text is to consider that $\vbeta_i$ is sampled from some conditional distribution on $\vx_i$. Specifically, for some conditional distribution function $g$, we consider the following hierarchical model: 
\begin{equation}\label{eqn:extension_contextual}
    \begin{split}
    \vthe &\sim \prob(\vthe),\\
    \vbeta_i &\sim g(\vx_i; \vthe),\\
    R_{i,t} &\sim f(A_{i,t}; \vbeta_i). 
    \end{split}
\end{equation}
As a concrete example, we consider the linear Gaussian case. Let  $\mThe = (\vthe_1, \dots, \vthe_d)$ be a $p \times d$ coefficeint matrix and $\Cov_{\vbeta}$ be some covariance matrix, we consider
\begin{align*}
    \vthe_j &\sim \normal(\vmu_{\vthe}, \Cov_{\vthe}), \forall j \in [d] \\
    \vbeta_i &\sim  \mThe^T \vx_i + \normal(\vzero, \Cov_{\vbeta}), \forall i \in [N]\\
    R_{i,t} &\sim A_{i,t}^T\vbeta_i + \normal(0,\sigma^2).
\end{align*}
% Let $\boldsymbol{A}_i = (A_{i,1}, \dots, A_{i,T_i})^T$, $\vR_i = (R_{i,1}, \dots, R_{i,T_i})^T$, $\vR = (\vR_1^T, \dots, \vR_N^T)^T$, and $\boldsymbol{Z} = (\boldsymbol{A}_1 \vx_1; \dots, \boldsymbol{A}_N \vx_N)$, we have 
% \begin{align*}
%     \vR| \{R_{i,t}\}, \{A_{i,t}\} \sim \normal\Big(\boldsymbol{Z}\vmu_{\vthe},
%     (\boldsymbol{Z}\vmu_{\vthe})  \Cov_{\vthe} (\boldsymbol{Z}\vmu_{\vthe})^T + diag(\boldsymbol{A}_1 \Cov_{\vbeta} \boldsymbol{A}_1^T, \dots, \boldsymbol{A}_N \Cov_{\vbeta} \boldsymbol{A}_N^T)
%     \Big), 
% \end{align*}
% with which we can then get the posterior of $\vthe$, denoted as $\prob(\vthe|\mH)$. 
The posterior of $\mThe$ can be similarly developed as in the main text using the property of Gaussian bilinear model. 
With a sample $\Tilde{\mThe}$ from $\prob(\mThe|\mH)$, 
we can interact with each task $i$ using a single-task TS with $\normal( \Tilde{\mThe}^T\vx_i, \Cov_{\vbeta})$ as the prior for $\vbeta_i$. 

% Since there are several types of formulation of contextual bandits
% We first recall the definition of contextual MAB in the multi-task setup:
% for each task $i \in [N]$, at each decision point $t$, 
% the agent observe a context $S_{i,t}$, choose an arm $A_{i,t} \in [K]$, and then receive a stochastic reward $R_{i,t} \sim f(S_{i,t}, A_{i,t};\vthe_i)$, where $\vthe_i$ is some unknown parameters associated with task $i$. 



% Second, our work can be extended to contextual bandits, 
% based on the idea of clustering of bandits \citep{gentile2014online, li2016collaborative} when the set of task instances is finite, or the idea of when the set is infinite. 

One possible concern about model \eqref{eqn:extension_contextual} is that, when the number of tasks is not large, a simpler model might be preferred. In that case, we can consider that $\vbeta_i$ is a deterministic function of $\vx_i$. 
\begin{align*}
    \vthe &\sim \prob(\vthe)\\
    \vbeta_i &= g(\vx_i; \vthe)\\
    R_{i,t} &\sim f(A_{i,t}; \vbeta_i).
\end{align*} 
In reinforcement learning, this formulation shares similar forms with contextual Markov decision process \cite{modi2018markov, modi2020no}. 
Now, the linear Gaussian case can be written as 
\begin{align*}
    \vthe_j &\sim \normal(\vmu_{\vthe}, \Cov_{\vthe}), \forall j \in [d] \\
    R_{i,t} &\sim A_{i,t}^T \mThe^T\vx_i + \normal(0,\sigma^2).
\end{align*}
Such a model can utilize the data from all tasks, while avoiding a naive pooling which assumes the coefficient vector of all tasks are the same. 
Indeed, this is a kind of varying-coefficient models in statistics \cite{fan2008statistical}. 
Low-rank assumption can also be considered in this bilinear problem. 

Finally, as another direction to derive a simpler model, we may consider the idea of clustering of bandits \citep{gentile2014online, li2016collaborative}, by assuming there is a set of $M$ task instances, and each task are drawn independently from them. 
The metadata contain information about the probability that one task belong to each cluster, through a function $g$. 
\begin{align*}
    \vthe &\sim \prob(\vthe),\\
    \vbeta_j &\sim \prob(\vbeta), \forall j \in [M]\\
    k_i &\sim g(\vx_i; \vthe), \forall i \in [N] \\
    \vbeta_i &= \sum_j \vI(k_i = j) \vbeta'_k, \forall i \in [N]\\
    R_{i,t} &\sim f(A_{i,t}; \vbeta_i), \forall i \in [N], \forall t \in [T_i]. 
\end{align*} 
Under appropriate model assumptions, the posterior can be obtained using approximate posterior inference tools. 

These three models are all built under our metadata-based multi-task bandit framework, and the corresponding multi-task TS algorithms can be similarly developed. 
The key idea is to leverage the metadata to describe the relations between bandit tasks, while allowing heterogeneity. 
% hierarchical Bayes
The choice between them reflects the bias-variance trade-off.



==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Extension_GP.tex <==
\section{Details and Extensions of the Method}\label{sec:appendix_Hierarchical}
% More on the Hierarchical Models

\subsection{Mean-precision parameterization of the Beta distribution}\label{sec: beta_parameterization}

We note that a Beta distribution has different parameterizations. 
In the most common parameterization, a Beta random variable $u \sim Beta(\alpha_1, \alpha_2)$ is specified by two shape parameters $\alpha_1$ and $\alpha_2$. 
We have 
\begin{equation*}
    \mu = \Mean(u) = \frac{\alpha_1}{\alpha_1 + \alpha_2}, \quad 
    var(u) = \mu (1 - \mu)\psi / (1 + \psi), 
\end{equation*}
where $\psi = 1 /(\alpha_1 +\alpha_2 )$ is the so-called precision parameter.
Alternatively, this Beta random variable can be fully specified by $(\mu, \psi)$. 
Given $(\mu, \psi)$, we have $\alpha_1 = \mu / \psi$ and $\alpha_2 = (1 - \mu) / \psi$. 
Given $(\mu, var(u))$, we have $\psi = [\mu(1-\mu) / var(u) - 1]^{-1}$. 

In BBLM, we adopt this mean-precision parameterization, with  $\Mean(r_{i,a}) = logistic(\vphi^T(\vx_i, a) \vthe)$ and the precision of $r_{i,a}$ equal to $\psi$, for any $i$ and $a$. 

% pi / phi_beta, (1 - pi) / phi_beta

% \begin{equation*}
%     \begin{split}
%             r_{i,a} &\sim Beta\big(logistic(\vphi^T(\vx_i, a) \vthe), \psi \big), \forall a \in [K],\\
%     % \vr_i &\sim Beta(logistic(\vPhi_i\vthe), \psi)\\
%     R_{i,t} &\sim Bernoulli \big(\sum_a \I(A_{i, t} = a) r_{i, a} \big), 
%     \end{split}
% \end{equation*}

\subsection{Extension to Mixed-Effect Gaussian Process for Gaussian Bandits}\label{sec:GP}
In this section, we introduce an extension of the method developed in Section \ref{sec:LMM} to the Gaussian process setting. 
In such a setup, the function $f(\vx) = \Mean(\vr_i|\vx_i = \vx)$ is a continuous function sampled from a Gaussian process. 
Specifically, for each action $a \in [K]$, we have a specified mean function $\mu_a : \mR^p \rightarrow \mR$ and a kernel function $\mathcal{K}_a : \mR^p \times \mR^p \rightarrow \mR$. 
Let $\mathcal{GP}(\mu_a, \mathcal{K}_a)$ denote the corresponding Gaussian process. 
We consider the following mixed-effect Gaussian process model: 
% for the associated Gaussian process
% \begin{equation}
% \begin{split}
%     f_a &\sim \mathcal{GP}(\mu_a, \mathcal{K}_a), \forall a \in [K]; \\
%     % \delta_{i,a} &\sim \mathcal{N}(0, \sigma_1^2), \forall i \in [N], a \in [K]\\ 
%     % r_{i,a} &= f_a(\vx_i) + \delta_{i,a}, \\
%     r_{i,a} &\sim \mathcal{N}(f_a(\vx_i), \Cov^2), \forall i \in [N], a \in [K]; \\
%     %\stackrel{i.i.d.}
%     % \delta_{i,a} &\sim \mathcal{N}(0, \Cov^2)\\
%     R_{i, t} &= \sum_a \mathbb{I}(A_{it} = a)r_{ia} + \epsilon_{it}.
% \end{split}
% \end{equation}

\begin{equation}\label{eqn:GP}
\begin{split}
    f_a &\sim \mathcal{GP}(\mu_a, \mathcal{K}_a), \forall a \in [K]; \\
    % \delta_{i,a} &\sim \mathcal{N}(0, \sigma_1^2), \forall i \in [N], a \in [K]\\ 
    % r_{i,a} &= f_a(\vx_i) + \delta_{i,a}, \\
    \vdelta_i &\sim \mathcal{N}(0, \Cov) , \forall i \in [N];\\ 
    \vr_{i} &= \vf(\vx_i) + \vdelta_i, \forall i \in [N], 
    % \\
    % %\stackrel{i.i.d.}
    % % \delta_{i,a} &\sim \mathcal{N}(0, \Cov^2)\\
    % R_{i, t} &= \sum_a \mathbb{I}(A_{it} = a)r_{i,a} + \epsilon_{it}.
\end{split}
\end{equation}
where $\vf(\vx) = (f_1(\vx), \dots, f_K(\vx))^T$. 
% The model can be straightforwardly extended to allow the K GPs to be correlated. 

To design the corresponding TS algorithm, we essentially need to derive the corresponding posterior for $\{\vr_i\}$. 
We begin by introducing some notations. 
The model \eqref{eqn:GP} induces a kernel function $\mathcal{K}$, such that for any two tuples $O = (a, r, \vx, i)$ and $O' = (a', r', \vx', i')$, we have 
\begin{equation*}
    \mathcal{K}(O, O') = \sum_a \mathcal{K}_a(\vx, \vx') \mathbb{I}(a = a') +  \Cov_{a, a'} \mathbb{I}(i = i'). 
\end{equation*}
% We sort the dataset  $\mathcal{H}$ as $\{(A_j, R_j, i(j))\}$, where $A_j, R_j$, and $i(j)$ is the action, reward, and task index for the $j$-th tuple in $\mathcal{H}$. 
Let $\mK$ be an $n \times n$ kernel matrix of the pairwise kernel values for tuples in $\mathcal{H}$. 
Set $\vR = (R_1, \dots, R_n)^T$ be an $n$-dimensional vector of the observed rewards and $\vmu = 
(\mu_{A_1}(\vx_{i(1)}), \dots, \mu_{A_n}(\vx_{i(n)}))^T$. 
Finally, we use $\vI$ to denote an identity matrix, the  dimension of which can be inferred from the context. 


% and $\vPhi$ be a $n \times d$ feature matrix with the $j$-th row be the feature vector $\vphi^T(\vx_{i}, A_{i,t})$ of the $j$-th tuple in $\mathcal{H}$. 



% For the $i$-th task, let $\vr_i = (r_{i,1}, \dots, r_{i, K})^T$. 
% \textbf{Posterior  updating.}
Define a $K \times n$ matrix $\boldsymbol{M}_i$, such that the $(a, j)$-th entry of $\boldsymbol{M}_i$ is 
$\mathcal{K}_a(\vx_i, \vx_{i(j)}) \mathbb{I}(a = A_j) + \Cov_{A_j, a} * \I(i(j) = i)$, and define a $K \times K$ diagonal matrix $\mK_i$ with the $a$-th diagonal entry be $\mathcal{K}_a(\vxi, \vxi)$. 
Let $\vmu_i = (\mu_{1}(\vx_{i}), \dots, \mu_{K}(\vx_{i}))^T$. 
The posterior of $\vr_i$ conditional on the accumulated data follows a multivariate normal distribution, with mean and covariance given by: 
\begin{equation}\label{eqn:post_GP}
    \begin{split}
        \mathbb{E}(\vr_i|\mathcal{H}) &= \vmu_i + \boldsymbol{M}_i (\mK + \sigma_1^2 \vI)^{-1} (\vR - \vmu),  \\
        cov(\vr_i | \mathcal{H}) &= (\mK_i + \Cov) - \boldsymbol{M}_i (\mK + \sigma_1^2 \vI)^{-1} \boldsymbol{M}_i^T. 
    \end{split}
\end{equation}
The posterior will then be used to sample an action according to its probability of being the optimal one, in a Thompson sampling manner, as detailed in Algorithm \ref{alg:TS}. 
% Therefore, the MTTS algorithm  
% $A_{i,t}$

% The hyper-parameter updating step can be solved as the MLE of the following regression problem: 
% \begin{equation*}
%     \vR \sim \mathcal{N}(\vmu, \mK(\Cov, \gamma) + \sigma_1^2 \vI), 
% \end{equation*}
% where $\gamma$ is the bandwidth of the kernel function. 
% Q: the other hyper-parameters?

\subsection{Adaptive hyper-parameter updating with empirical bayes}\label{sec:appendix_hyper_updating_EB}
Following the literature \cite{kveton2021meta, agrawal2013thompson}, 
we assume the variance components as known for the two examples in Section \ref{sec:method}. 
In practice, we can apply empirical Bayes to update these hyperparameters adaptively. 
We take the LMM as an example. 
As discussed in Section \ref{sec:LMM}, our model requires four hyperparametes: $\vmu_{\vthe}$, $\Cov_{\vthe}$, $\sigma$, and $\Cov$. 
Among them, $\vmu_{\vthe}$ and  $\Cov_{\vthe}$, the prior parameters of $\vthe$, can be specified as any appropriate values according to domain knowledge, and will not affect our algorithm as well as its regret bound. 
For $\sigma$ and $\Cov$, similar with the approach commonly adopted in the literature on Gaussian process \citep{tomkins2019intelligent, rasmussen2003gaussian}, 
they can be learned from the data. 
Specifically, we can specify them as the maximizer of the marginal likelihood with respect to $(\sigma, \Cov)$, marginalized over $\vthe$ and $\{\vdelta_i\}_{i \in [N]}$. 
% $\{\delta_{i,a}\}_{i \in [N], a \in [K]}$. 
The log marginal likelihood can be derived as 
\begin{equation}\label{eqn:Hyper-parameter}
\begin{split}
l(\sigma, \Cov|\mathcal{D}) 
= -\frac{1}{2} \Big[ (\vR - \vPhi \vmu_{\vthe})^T (\mK(\Cov) + \sigma^2 \vI)^{-1}(\vR - \vPhi \vmu_{\vthe}) + log|\mK(\Cov) + \sigma^2 \vI|
+ N log(2\pi)  \Big], 
\end{split}
\end{equation}
where $\mK(\Cov)$ indicates the dependency of $\mK$ on $\Cov$. 
Note that $\Cov$ controls the degree of heterogeneity conditional on the metadata. % among tasks
Such an Empirical Bayes \citep{carlin2000bayes} approach makes sure our method is  adaptive to the prediction power of the metadata. 


\input{Extension_Contextual}

==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Figures/Figures.tex <==
\begin{figure}[t]
     \centering
 \begin{subfigure}[b]{\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Figures/Gaussian_all_6.png}
           \vspace{-.5cm}
     \caption{Gaussian bandits. 
The regrets of OSFA are much higher in some subplots and hence hidden.}
\label{fig:simu_Gaussian}
 \end{subfigure}
 \begin{subfigure}[b]{\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Figures/binary_all_6.png}
      \vspace{-.5cm}
     \caption{Bernoulli bandits. A larger value of $\psi$ implies a larger variation of $\vr_i$ condition on $\vx_i$. 
}
\label{fig:simu_Binary}
 \end{subfigure}
 \vspace{-.5cm}
\caption{
Average Bayes regret for various methods. Shared areas indicate the standard errors of the averages.}
% \vspace{-.3cm}
% an order of magnitude
% The yellow line (TR, m = 2) and green line (TR, m = 3) are largely overlapped
\label{fig:simu}
\end{figure}

% Gaussian bandits: 
% the solid lines denote the average Bayes regret with the shared areas indicating the standard errors of the averages.  
% The regrets of OSFA are much higher in some subplots and hence hidden.

% \begin{figure}[t]
%  \centering
%  \begin{subfigure}[b]{\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{Figures/binary_all_6.png}
%     %  \caption{Episodic, $\sigma_3 = 5$}
%     %  \label{fig:y equals x}
%  \end{subfigure}
%  \vspace{-.2cm}
% \caption{
% Bernoulli bandits: 
% the solid lines denote the average Bayes regret with the shared areas indicating the standard errors of the averages.  
% A larger value of $\phi$ implies a larger variation of $\vr_i$ condition on $\vx_i$. 
% }
% \vspace{-0.3cm}
% \label{fig:simu_Binary}
% \end{figure}



% \begin{figure}[t]
%      \centering
%      \begin{subfigure}[b]{0.9\textwidth}
%          \centering
%          \includegraphics[width=0.93\textwidth]{Figures/0_sequential.png}
%         %  \caption{Episodic, $\sigma_3 = 5$}
%         %  \label{fig:y equals x}
%      \end{subfigure}
%      \\
%      \begin{subfigure}[b]{0.9\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/0_concurrent.png}
%         %  \caption{Episodic, $\sigma_3 = 5$}
%         %  \label{fig:y equals x}
%      \end{subfigure}
% \caption{
% Gaussian bandits: 
% the solid lines denote the average Bayes regret with the shared areas indicating the standard errors.  
% The regrets of OSFA are much higher in the upper subplots and hence hidden.
% }
% % an order of magnitude
% % The yellow line (TR, m = 2) and green line (TR, m = 3) are largely overlapped
% \label{fig:simu_Gaussian}
% \end{figure}

% \begin{figure}[t]
%  \centering
%  \begin{subfigure}[b]{\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{Figures/binary_all.png}
%     %  \caption{Episodic, $\sigma_3 = 5$}
%     %  \label{fig:y equals x}
%  \end{subfigure}
% \caption{
% Bernoulli bandits: 
% the solid lines denote the average Bayes regret with the shared areas indicating the standard errors.  
% A larger value of $\phi$ implies a larger variation of $\vr_i$ condition on $\vx_i$. 
% }
% \vspace{-0.6cm}
% \label{fig:simu_Binary}
% \end{figure}


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Figures/Figures_Gaussian.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square4_p_raw10_orderconcurrent.png}
         \caption{Concurrent, $\sigma_3 = 5$}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square1_p_raw10_orderconcurrent.png}
         \caption{Concurrent, $\sigma_3 = 1$}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square0.25_p_raw10_orderconcurrent.png}
         \caption{Concurrent, $\sigma_3 = 0.2$}
         \label{fig:five over x}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square4_p_raw10_orderepisodic.png}
         \caption{Episodic, $\sigma_3 = 5$}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square1_p_raw10_orderepisodic.png}
         \caption{Episodic, $\sigma_3 = 1$}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/sigma1_square0.25_p_raw10_orderepisodic.png}
         \caption{Episodic, $\sigma_3 = 0.2$}
         \label{fig:five over x}
     \end{subfigure}
\caption{
The average regret and its $95\%$ confidence interval, aggregated over 100 random seeds. 
The regret of OSFA is at least an order of magnitude higher than that of the others and hence not reported. 
}
\label{fig:simu_Gaussian}
\end{figure}


\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/one_cluster.png}
         \caption{Episodic, $\sigma_3 = 5$}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/one_cluster.png}
         \caption{Episodic, $\sigma_3 = 1$}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/one_cluster.png}
         \caption{Episodic, $\sigma_3 = 0.2$}
         \label{fig:five over x}
     \end{subfigure}
\caption{
\textbf{Placeholder for Binary}
}
\label{fig:simu_Binary}
\end{figure}


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Figures/demo.tex <==


\begin{figure}[!t]
\centering
% \includegraphics[width=.8\textwidth]{figures/diag_with_cost.png}
\begin{subfigure}{.3\textwidth}
  \centering
    \vspace{.2cm}
  \includegraphics[width=0.82\linewidth]{Figures/one_cluster.png}
  \vspace{-.15cm}
  \caption{The meta MAB setting \cite{kveton2021meta, hsu2019empirical, baxter2000model}, where $\vx_i$ is a constant. % degenerates to
  }
\end{subfigure}%
\hspace{.3cm}
\begin{subfigure}{.3\textwidth}
  \vspace{.2cm}
  \centering
  \includegraphics[width=0.82\linewidth]{Figures/clustering.png}
  \vspace{-.15cm}
  \caption{
  There exists several task clusters, where $\vx_i$ is categorical. 
  }
\end{subfigure}%
% \vspace{-.2cm}
\hspace{.3cm}
\begin{subfigure}{.3\textwidth}
    \vspace{-.1cm}
  \centering
  \includegraphics[width=0.86\linewidth]{Figures/continuous.png}
  \vspace{-.15cm}
  \caption{
   $\vx_1$ is a continuous variable.  
  }
\end{subfigure}%
\vspace{-.1cm}
\caption{
Illustrations of the task distribution $\prob(\vr_i|\vx_i)$. 
% the feature-based multi-task MAB problem. 
In the first two subplots, each dot represents a task and the two axes  denote the expected rewards for two arms. 
In the last subplot, we have three arms, each dot represents one arm of a task, the x-axis denotes  one continuous feature $x_1$, and the y-axis denotes the expected reward. 
In the last two settings, the metadata is informative and can guide the exploration to reduce regrets, while there is still inter-task heterogeneity that can not be captured. % by the metadata
}
\label{fig:demo}
\end{figure}

% feature-dependent
% Several specific cases of the multi-task bandits problem
    % \includegraphics[width=0.5\textwidth, height=0.4\textwidth]{Figures/demo.png}
    % \caption{An example for illustration. The x-axis denotes the value of a task-specific feature, the y-axis denotes the expected reward, and the three curves represent three arms. 
    % The solid line indicates the average expected reward for tasks of a specific value, while the true expect reward for different tasks may spread around the mean curve, as indicated by the points. [. 
    % After we get real data, we can replace this plot with our example.]}

% \setlength{\textfloatsep}{20.0pt plus 2.0pt minus 4.0pt}% Remove \textfloatsep


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/LMM_implemetation.tex <==
% \section{More details about the experiments}
% \section{Implementation}
\section{Implementation}\label{sec:appendix_Implementation}
In this section, we discuss efficient ways to implement {\name}, and analyze its computational complexity. 
We use $\vI$ to denote identity matrix, the dimension of which can be inferred from the context. 
% and $\vJ$ to denote an all-one matrix

\subsection{Efficient Implementation for Gaussian bandits with LMM}\label{sec:appendix_implementation_gaussian}

At each decision point, the computation will be dominated by the calculation of the matrix inverse for $(\mK + \sigma^2 \vI)$, which suffers from a cubic complexity $O(n^3)$ as well-known in the Gaussian process literature \cite{shi2012mixed}. 
% Step \eqref{eqn:post} and \eqref{eqn:Hyper-parameter} are both closely related with the kernel function and the matrix inverse. 
To alleviate the computational burden, we utilize the block structure induced by the mixed effect model via using the well-known Woodbury matrix identity \citep{rasmussen2003gaussian}, which is reviewed as follows. 
\begin{lemma}[Woodbury matrix identity] For any matrix $W$ and any invertible matrices $Z$, $U$, and $V$ with appropriate dimensions, the following relationship holds:
\begin{equation*}
    (\mZ + \mU\mW\mV^T)^{-1} = \mZ^{-1} - \mZ^{-1}\mU(\mW^{-1} + \mV^T\mZ^{-1}\mU)^{-1}\mV^T\mZ^{-1}
\end{equation*}
% Similarly, for the matrix determinant, we have $|\mZ+\mU \mW \mV^T| = |\mZ||\mW||\mW^{-1} + \mV^T\mZ^{-1}\mU|$.
\end{lemma}



% , and each entry of $\vJ_{i}$ is the corresponding entry of $\Cov$. 
% Specifically, we have $\vJ = diag(\vJ_{11}, \dots, \vJ_{1K}, \vJ_{21}, \dots, \vJ_{NK})$, where 
% $\vJ_{i,a}$ is an all-ones matrix whose dimension equal to the $\#\{(A_j, R_j, i(j)) \in \mathcal{D}: A_j = a, i(j) = i\}$. 
We start by writting $\mK = \vPhi \Cov_{\vthe} \vPhi^T + \vJ$. 
Without loss of generality, we can rearrange the tuples in $\mathcal{D}$ so that $\vJ$ becomes a block diagonal matrix as $\vJ = diag(\vJ_{1}, \dots, \vJ_{N})$, where $\vJ_{i}$ is the submatrix for task $i$. 
% or even (i,a) when \Sigma_delta is diagonal
The dimension of $\vJ_{i}$ equals to $\#\{(A_j, R_j, \vx_{i(j)}, i(j)) \in \mathcal{D}: i(j) = i\}$ and it is a pairwise kernel matrix 
induced by the kernel $\Tilde{\mathcal{K}}(O, O') = \Cov_{a, a'}$. 
Therefore, we have
\begin{align*}
    (\mK + \sigma^2 \vI)^{-1} 
    &= (\vPhi \Cov_{\vthe} \vPhi^T + (\vJ + \sigma^2 \vI) )^{-1}\\
    &= (\vJ + \sigma^2 \vI)^{-1} \Big[
    \vI - \vPhi (\Cov_{\vthe}^{-1} + \vPhi^T  (\vJ + \sigma^2 \vI)^{-1} \vPhi)^{-1} \vPhi^T (\vJ + \sigma^2 \vI)^{-1} \Big], 
\end{align*}
the computation cost of which will be dominated by $(\vJ + \sigma^2 \vI)^{-1}$, which yields a block diagonal structure and hence the matrix inverse can be more efficiently computed. 
Suppose we already have 
$t_0$ interactions with each of $N$ tasks. 
The computational cost is reduced from 
$O(N^3t_0^3)$ to $O(Nt_0^3)$. 
In addition, when $\Cov$ is diagonal, we can further apply the Woodbury matrix identity to compute $(\vJ_{i} + \sigma^2 \vI)^{-1}$. 
\newcommand{\JsigmaInv}{(\vJ + \sigma^2 \vI)^{-1}}

Furthermore, 
to make the computation more efficient, we define $\Cov_{in} = (\Cov_{\vthe}^{-1} + \vPhi^T  \JsigmaInv \vPhi)^{-1}
, \vJ_{\vPhi} = \JsigmaInv \vPhi
, \Tilde{\vR}= (\vR - \vPhi \vmu_{\vthe})
, \vJ_{\vR} = \JsigmaInv \Tilde{\vR}$. 
Next, we define 
\begin{align*}
\vJ_{\vPhi,\vR} &= \vPhi^T \JsigmaInv \Tilde{\vR}\\
\vJ_{\vPhi, \vPhi} &= \vPhi^T \JsigmaInv \vPhi\\
\vJ_{\vPhi, \vM, i} &= \vM_i \JsigmaInv \vPhi\\
\vJ_{\vR, \vM, i} &= \vM_i \JsigmaInv \Tilde{\vR}\\
\vJ_{\vM, i} &= \vM_i \JsigmaInv \vM_i^T. 
\end{align*}
For these components, we can efficiently utilize the block structure to only update the corresponding part. 
Finally, we have 
\begin{equation*}
    \begin{split}
        \mathbb{E}(\vr_i|\mathcal{D}) 
        % &= \vPhi_{i} \vmu_{\vthe} + (\vPhi_i\Cov_{\vthe}\vPhi^T + \vM_i) \JsigmaInv \Big[\vI -  \vPhi \Cov_{in} \vPhi^T \JsigmaInv\Big] \Tilde{\vR}  \\
        % &= \vPhi_{i} \vmu_{\vthe} + (\vPhi_i\Cov_{\vthe}\vPhi^T + \vM_i) \JsigmaInv \Big[\Tilde{\vR} -  \vPhi \Cov_{in} \vJ_{\vPhi,\vR} \Big]  \\
        &= \vPhi_{i} \vmu_{\vthe} 
        + \vPhi_i\Cov_{\vthe}\vJ_{\vPhi,\vR}
        + \vJ_{\vR, \vM, i}
        - \vPhi_i\Cov_{\vthe} \vJ_{\vPhi, \vPhi} \Cov_{in} \vJ_{\vPhi,\vR}
        - \vJ_{\vPhi, \vM, i} \Cov_{in} \vJ_{\vPhi,\vR},  \\
        cov(\vr_i | \mathcal{D}) 
        % &= (\vPhi_{i} \Cov_{\vthe} \vPhi_{i}^T + \Cov) - (\vPhi_i\Cov_{\vthe}\vPhi^T + \vM_i) \JsigmaInv \Big[\vI - \vPhi \Cov_{in} \vJ_{\vPhi}^T \Big] (\vPhi_i\Cov_{\vthe}\vPhi^T + \vM_i)^T\\
        &= (\vPhi_{i} \Cov_{\vthe} \vPhi_{i}^T + \Cov) 
        - \vJ_{\vM, i} 
        - (\vPhi_{i} \Cov_{\vthe}) \vJ_{\vPhi, \vPhi}  (\vPhi_{i} \Cov_{\vthe})^T
        % - \vPhi_{i} \Cov_{\vthe} \vJ_{\vPhi, \vPhi} 
        - \vPhi_{i} \Cov_{\vthe} \vJ_{\vPhi, \vM, i}^T
        - (\vPhi_{i} \Cov_{\vthe} \vJ_{\vPhi, \vM, i}^T)^T\\
        &\quad +  (\vPhi_i\Cov_{\vthe}\vJ_{\vPhi, \vPhi} + \vJ_{\vPhi, \vM, i})  \Cov_{in} 
         (\vPhi_i\Cov_{\vthe} \vJ_{\vPhi, \vPhi} + \vJ_{\vPhi, \vM, i})^T\\
    \end{split}
\end{equation*}

% The hyper-parameter updating step can be solved as the MLE of the following regression problem: 
% \begin{equation*}
%     \vR \sim \mathcal{N}(\vPhi \vmu_{\vthe}, \mK(\Cov) + \sigma^2 \vI)
% \end{equation*}
% % which can be solved by GP regression softwares. Refer to \citet{tomkins2019intelligent} for more details. 
% Similar trick can apply to the hyper-parameter updating step. 
% To compute $|\mK(\Cov) + \sigma^2 \vI|$, we have
% \begin{align*}
%     |\mK(\Cov) + \sigma^2 \vI| 
%     &= |(\vPhi \Cov_{\vthe} \vPhi^T + (\vJ + \sigma^2 \vI) )| \\
%     &= |( \vJ + \sigma^2 \vI)| * |\Cov_{\vthe}|  * |(\Cov_{\vthe})^{-1} + \vPhi^T (\vJ + \sigma^2 \vI)^{-1} \vPhi|. 
% \end{align*}
% Again, the block diagonal structure can be utilized to largely reduce the computation cost. 

% We might need to use GPytorch for implementation. 
% The code \footnote{https://github.com/StatisticalReinforcementLearningLab/intelligent\_pooling} for \citet{tomkins2019intelligent} might be a good example. 
% We may need to take a look at \citet{tomkins2020intelligentpooling} to learn more about the implementation tricks. 
% If the scalability is an issue, we may need to consider some approximate solution. 

% Efficient

\paragraph{Alternative implementation.}
For the $\vthe$-centered sampling scheme (e.g., Algorithm \ref{alg:TS_faster_general}), note that 
\begin{align*}
    &\vthe | \mH \sim \mathcal{N}\Big(\Tilde{\Cov}(\vPhi^T \mV^{-1}\vR + \Cov_{\vthe}^{-1}\vmu_{\vthe}), \Tilde{\Cov}\Big),\\
    &\Tilde{\Cov} = (\vPhi^T \mV^{-1} \vPhi + \Cov_{\vthe}^{-1})^{-1}, \mV = \sigma^2 \vI_n + \vJ, %\Cov_{\delta}, 
\end{align*}
where the dominating step is still to compute $\mV^{-1}$, and similar tricks can be applied. 
As a special case, consider $\Cov = \sigma_1^2 \vI$. 
We rearrange $\vJ$ as $diag(\vJ_{1,1}, \dots, \vJ_{1,K}, \dots, \vJ_{N,1}, \dots, \vJ_{N,K})$, where $\vJ_{i,a} = \sigma_1^2 \vone \vone^T$, and apply similar rearrangement to $\vPhi$ and $\vR$. 
Hence we have $\mV^{-1} = (\sigma^2 \vI_n + \vJ)^{-1} = diag((\sigma^2  \vI + \vJ_{1,1})^{-1}, \dots, (\sigma^2  \vI + \vJ_{N,K})^{-1})$. 
According to the Woodbury matrix identity, we have $(\sigma^2 \vI +  \vJ_{i,a})^{-1} = \sigma^{-2}\vI - \sigma^{-4}(\sigma_1^{-2} + n_{i,a} \sigma^{-2})^{-1}\vone\vone^T$, where $n_{i,a}$ is the count that action $a$ is implemented for task $i$. 

After we sample one $\Tilde{\vthe}$, the prior of $\vr_i$ can then be updated as $\normal(\vPhi_i \Tilde{\vthe}, \Cov)$. 
Its posterior then follows from the standard normal-normal conjugate relationship. 

% \input{incremental_LMM}

\subsection{Computationally Efficient Variant of {\name} under General Settings}\label{sec:appendix_TS_general}

In Section \ref{sec:general_framework}, we discuss how to ease the computation when directly sampling from $\prob(\vr_i|\vx_i)$ is computationally heavy, and present the variant under the sequential setting. 
We present the variant under the general settings in Algorithm \ref{alg:TS_faster_general}. 
Specifically, it requires an updating frequency $l$ as a hyper-parameter, and will sample a new $\vthe$ once we have $l$ new data points. 
$\prob(\vthe|\mH)$ can be computed via various approximate posterior inference tools. 
% Here, $\prob(\vthe|\mH)$ can be updated incrementally, and various approximate posterior inference tools can be used to compute it. 

\input{Algorithm/alg_TS_faster_general}

\subsection{Implementation for Bernoulli bandits with BBLM}\label{sec:appendix_implementation_Bernoulli}
In this section, we discuss our implementation of {\name} for Bernoulli bandits, under the BBLM introduced in \eqref{eqn:BBLM}. 
It follows Algorithm \ref{alg:TS_faster_general}. 

% introduce an computationally efficient variant
% We require an updating frequency $l$ as a hyper-parameter, and will sample a new $\vthe$ once we have $l$ new data points. 
Still, the dominating step is to sample from $\prob(\vthe| \mH)$. 
Fortunately, the model yields a nice hierarchical structure, where 
the first term essentially requires us to fit a Beta-logistic regression, and the second term is the likelihood of a simple binomial distribution, with a beta conjugate in our case. 
Specifically, 
note that $f(\vr_i|\vx_i, \vthe) = \prod_{a=1}^K f'_{Beta}(r_{i,a}|\vphi(\vx_i, a), \vthe)$, where $f'_{Beta}(r_{i,a}|\vphi(\vx_i, a), \vthe)$ is the density function of $Beta\big(logistic(\vphi(\vx_i, a)^T \vthe), \psi \big)$. 
Also note that, the likelihood for the Bernoulli distribution of task $i$ over $\mH_i$, as specified by the second equation of \eqref{eqn:BBLM}, is $\prob(\mH_i|\vr_i) = \prod_{a=1}^K r_{i,a}^{n_{i,a}}$, where $n_{i,a}$ is the number of times that action $a$ is selected for task $i$ in $\mH_i$. 
Both parts are computationally tractable. 
In our experiments, we use the MCMC algorithm implemented by the \textsf{Python} package \textsf{PYMC3} \cite{salvatier2016probabilistic} to compute the approximate posterior. 
% The full algorithm is described in Algorithm \ref{alg:TS_faster_binary}. 
% \input{Algorithm/TS_faster_binary}


\input{computational_complexity}

==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Mis/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec:Experiments} about the potential model misspecification and Section \ref{sec:discussion} for possible extensions. }
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{
    We are not aware of any particular negative societal consequences of this work, 
    since we have not proposed any new use cases than existing bandit algorithms.}
    % In the main text, we discussed the privacy issue. 
    % Except for this point, 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section \ref{sec:Theory}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix \ref{sec:main_proof}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{In the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{sec:Experiments} and Appendix \ref{sec:appendix_Experiment_Details}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{In all figures.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix \ref{sec:Computational_complexity}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Mis/new_commands.tex <==
\newcommand{\lam}{\lambda}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vbeta}{\boldsymbol{\beta}}
\newcommand{\vlam}{\boldsymbol{\lam}}
\newcommand{\vrho}{\boldsymbol{\rho}}
\newcommand{\vM}{\boldsymbol{M}}

\newcommand{\hRI}{\widehat{RI}}
\newcommand{\vthe}{\boldsymbol{\theta}}
\newcommand{\mThe}{\boldsymbol{\Theta}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mO}{\mathcal{O}}

\newcommand{\TO}{\tilde{O}}

\newcommand{\indep}{\perp \!\!\! \perp}
% \newcommand{\Y}[1]{Y^*(#1)}
\newcommand{\Yz}{Y^*(0)}
\newcommand{\Yzi}{Y_i^*(0)}

\newcommand{\Yo}{Y^*(1)}
\newcommand{\Yoi}{Y_i^*(1)}

\newcommand{\mC}{\mathcal{C}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mJ}{\mathcal{J}}

\newcommand{\mE}{\mathbb{E}} 
\newcommand{\vxi}{\mathbf{x}_i} 
\newcommand{\vxj}{\mathbf{x}_j} 
\newcommand{\vc}{\mathbf{c}}
\newcommand{\veps}{\boldsymbol{\epsilon}}
\newcommand{\vdelta}{\boldsymbol{\delta}}


\newcommand{\dopt}{d^{opt}} 

\newcommand{\vA}{\boldsymbol{A}}
\newcommand{\vJ}{\boldsymbol{J}}


\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\neigh}{\mathcal{N}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\vvarphi}{\boldsymbol{\varphi}}

\newcommand{\vpi}{\boldsymbol{\pi}}
\newcommand{\vS}{\boldsymbol{S}}
\usepackage{soul}
\usepackage{xcolor}
\newcommand{\tH}{\tilde{H}}
\newcommand{\Mean}{{\mathbb{E}}}
\newcommand{\Var}{{\mathbb{VAR}}}
% \newcommand{\Cov}{{\mathbb{COV}}}
\newcommand{\Cov}{\boldsymbol{\Sigma}}

\newcommand{\prob}{\mathbb{P}}

\newcommand{\vphi}{\boldsymbol{\phi}}
\newcommand{\vPhi}{\boldsymbol{\Phi}}
\newcommand{\vR}{\boldsymbol{R}}
\newcommand{\vr}{\boldsymbol{r}}
\newcommand{\vone}{\boldsymbol{1}}
\newcommand{\vzero}{\boldsymbol{0}}
\newcommand{\vI}{\boldsymbol{I}}
\newcommand{\vmu}{\boldsymbol{\mu}}

\newcommand{\mX}{\boldsymbol{X}}
\newcommand{\mK}{\boldsymbol{K}}
\newcommand{\mZ}{\boldsymbol{Z}}
\newcommand{\mU}{\boldsymbol{U}}
\newcommand{\mW}{\boldsymbol{W}}
\newcommand{\mV}{\boldsymbol{V}}

\newcommand{\vv}{\boldsymbol{v}}

\newcommand{\TSnormal}[1]{TS(\mathcal{N}(#1, \Cov))}

\usepackage{amsthm}
\newtheorem{thm}{Theorem}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
% \newtheorem*{remark}{Remark}
\newtheorem{remark}{Remark}

\DeclarePairedDelimiter\norm{\lVert}{\rVert}

\newcommand{\alignlable}[1]{\stepcounter{equation}\tag{\theequation}\label{#1}
}
%%%%%%%%%%%%
\newlength{\leftstackrelawd}
\newlength{\leftstackrelbwd}
\def\eqstack#1#2{\settowidth{\leftstackrelawd}%
{${{}^{#1}}$}\settowidth{\leftstackrelbwd}{$#2$}%
\addtolength{\leftstackrelawd}{-\leftstackrelbwd}%
\leavevmode\ifthenelse{\lengthtest{\leftstackrelawd>0pt}}%
{\kern-.5\leftstackrelawd}{}\mathrel{\mathop{#2}\limits^{#1}}}


% \newcommand{\ourname}{{MTS}}
\def\name{MTTS}

==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Mis/packages.tex <==
\usepackage[utf8]{inputenc}
% \usepackage[left=1.02in, right=1.02in, top=1.1in, bottom=1.05in]{geometry}
\usepackage{array}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{setspace}
\usepackage{textcomp}
\usepackage{enumitem}
\usepackage{datetime2}
\usepackage{multirow}
\usepackage[font=small,labelfont=bf]{caption}
\DeclareMathOperator*{\argmin}{arg\!min}
\DeclareMathOperator*{\argmax}{arg\!max}
\usepackage{subcaption}

\usepackage{xcolor}
\usepackage{mathtools}

\usepackage{stackrel}

\usepackage{lineno}
\linenumbers



% \doublespacing
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Proof.tex <==
\section{Main Proof}\label{sec:main_proof}
For ease of notations, 
without loss of generality, 
we first consider the sequential setting, and we assume the tasks arrive according to their indexes, i.e., the $i$th task will arrive earlier than the $(i+1)$th. 
Otherwise, we can always re-index these tasks. 
Since in our proof, all analysis for the regret in task $i$ only uses the data generated by task $i$ itself and the data generated in the alignment periods of task $1, \dots, i - 1$, it is easy to verify that our proof continues to hold in other settings. 
% [more complex notations can be formalized after the proof is finished]. 

We first clarify some notations. 
We vertically stack the feature matrix for all tasks to define $\vPhi_{1:N} = (\vPhi_1; \dots; \vPhi_N)$, 
and we  can similarly define $\vdelta_{1:N} = (\vdelta_1^T, \dots, \vdelta_N^T)^T$. 
At the end of the alignment period of task $i$, we define the following notations: 
% the value of $\vPhi$  as
first, we define $\vPhi^e_{1:i} = (\vPhi_1; \dots; \vPhi_i)$, 
and we can similarly define $\vdelta^e_{1:i}$ and $\vR^e_{1:i}$; 
% Next, we define $\vvarphi^e_i$ as a matrix of dimension $(iT - T + K) \times (NK)$, where the $j$th row is an indicator vector with value $1$ at the entry $(i(j) - 1)T + A_j$; 
moreover, we denote $\mV^e_{1:i} = (\sigma^2 + 1) \vI$ of dimension $iK \times iK$. 
% $\Cov_{\vR}^{e,i} = \vPhi \vPhi^T + \vvarphi \vvarphi^T + \sigma^2 \vI$; 
finally, let $\mH^e_{1:i}$ be the history of all alignment periods so far. 
To simplify the notations, when the context is clear, we may drop the subscript $1:i$ and superscript   $e$. 
Recall that we use $\vI$ to denote identity matrix, the  dimension of which can be inferred from the context. 


The modified {\name} algorithm is summarized in Algorithm \ref{alg:modified_MTS}, and formally described as follows. 
For any $i \in [N]$, 
during our first $K$ interactions with task $i$, 
we pull the $K$ arms in a round robin. 
After this period, we sample a value $\vr^e_i$ from  the posterior $\vr | \mH^e_{1:i}$ , and then we use $\mathcal{N}(\vr^e_i, \Cov)$ as the prior of $\vr_i$ to continue interact with task $i$ as a standard single-task TS algorithm. 
In another word, we run $\TSnormal{\vr^e_i}$ with the following $T - K$ interactions. 
Note that this sampling is equivalent to first sample a value $\vthe^e_i \sim \vthe|\mH^e_{1:i}$, and then define $\vr^e_i = \vPhi_i\vthe^e_i$. 
Besides, as discussed in \eqref{alternative_form}, this procedure is equivalent to only use the data generated in the alignment periods to estimate the prior.  
Finally, we define a modified oracle-TS which also has the alignment period. The main part of our proof will focus on derive the regret to the modified oracle-TS, since its regret to the vanilla oracle-TS can be easily bounded. 

\input{Algorithm/alg_modified_MTS}


We begin by stating several lemmas, which will be used in our main proof. 
The proof of these lemmas are deferred to Appendix \ref{sec:proof_lemmas}. 
Without loss of generality, throughout the proof, we assume $\Cov_{\vthe} = \vI$, $\vmu_{\vthe} = \vzero$, and $\Cov = \vI$ to simplify the notations.  
It is easy to check that, under the boundedness assumption \ref{asmp:cov_others}, for general values of these terms, the regret bound still hold. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We first establish the concentration of $\vthe^e_i$ around $\vthe$. 
It mainly utilizes the property of Bayesian LMM.
%$\hat{\vthe}^e_i$. 
% at the end of its alignment period, 
\begin{lemma}[Concentration of $\vthe^e_i$]\label{lemma:concentration_sampled_theta}
For any task $i \in [N]$, 
% let $\vthe^e_i \sim \prob[\vthe|\mH^e_{1:i}]$. 
for any $\xi \in (0, 1)$, we have 
\begin{align*}
    \prob \Big(||\vthe^e_i - \vthe|| 
    \ge 
     [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(2 \sqrt{d} + 2\sqrt{2} \sqrt{-log \xi}\big) 
     + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}\Big) 
    \le 2\xi + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
\end{align*}
\end{lemma}
% \hat{\vthe}^e_i

% \subsection{Proof of Theorem \ref{thm:meta_ours}}
% \begin{proof}
% 1
% \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% , which together with Lemma \ref{lemma:concentration_hat_theta} can control the concentration of the sampled value of $\vthe$. 

Based on Lemma \ref{lemma:concentration_sampled_theta}, we are now ready to prove that the estimated task-specific prior mean will be close to the true prior mean with high probability. 
For any task $i \in [N]$, let $\vr^e_i = \vPhi_i\vthe^e_i$ be the sampled prior mean. 
Recall that $\Mean(\vr_i | \vx_i) = \vPhi_i\vthe$ is the true prior mean for a task with metadata $\vx_i$. We have the following result. 
\begin{lemma}[Concentration of $\vr^e_i$]\label{lemma:concentration_sampled_prior}
For any task $i \in [N]$, 
we have 
\begin{eqnarray}\label{eqn:concentration_sampled_prior}
\begin{split}
    \prob \Big(||\vr^e_i - \vPhi_i\vthe|| \ge 
 2\sqrt{2} C_2 \sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2} 
 + C_3[i c_1'K + 1]^{-1}\Big) 
    \le \frac{2}{NT} + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
\end{split}
\end{eqnarray}
where $c_1' = c_1 \frac{(\sigma^2+1)^{-1}}{2}$. 
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To derive the multi-task regret of the modified {\name}, 
we aim to use a "prior alignment" proof technique inspired by \cite{metapricing}. 
Specifically, one central challenge to the analysis is that, no existing method can well characterize the behaviour of a TS algorithm when the input prior is different with the true task distribution, even when the difference is negligible \cite{kveton2021meta, metapricing, liu2016prior}. 
Therefore, 
even though with Lemma \ref{eqn:concentration_sampled_prior}, we can establish that the learned prior will be more and more close to the ground truth as the number of tasks increases, 
and it is intuitive to believe that the multi-task regret per task will decay, 
it is challenging to formally prove such a regret bound following standard regret analysis approaches. 

The key idea of the "prior alignment" proof technique is that, 
suppose after some interactions with a task $i$, the posterior of $\vr_i$ for the modified {\name} is equal to the posterior for the modified oracle-TS, then their behaviour in the following interactions with this task will be exactly the same (in the probabilistic sense), and hence the multi-task regret in the following interactions with this task will be exactly zero. 
Suppose such an event happens with high probability, and this probability approaches $1$ as $i$ grows, we can then  derive a bound for the multi-task regret. 
This idea forms the skeleton of our proof. 



Towards this end, we begin by defining the realized random errors for the modified {\name} in the alignment period for the $i$th task as 
$\veps^e_i = (\epsilon_{i,1}, \dots, \epsilon_{i,K})^T$, where $\epsilon_{i,a}$ is the realized error when we pull arm $a$ in the $a$th interaction with task $i$. 
We can similarly define $\veps^*_i$ for the modified oracle-TS algorithm. 
Note that both algorithms take the same actions in the alignment period, and we also have $\veps^e_i \sim \veps^*_i \sim \mathcal{N}(\vzero, \sigma^2 \vI)$. 
We first note the following lemma, which establishes the difference between the posterior with $\mathcal{N}(\vr^e_i, \Cov)$ as the prior and the posterior with $\mathcal{N}( \vPhi_i\vthe, \Cov)$ as the prior, after observing $\vR^e_i$. 

\begin{lemma}[Posterior Difference]\label{lemma:post_relationship}
For any task $i \in [N]$, let  
$\mathcal{N}(\Tilde{\vr}^e_i, \Tilde{\Cov}^e_i)$ and $\mathcal{N}(\Tilde{\vr}^*_i, \Tilde{\Cov}^*_i)$ be the posterior after observing $\vR^e_i$, with $\mathcal{N}(\vr^e_i, \Cov)$  and $\mathcal{N}( \vPhi_i\vthe, \Cov)$ as the prior,  respectively. 
We have 
\begin{align*}
    \Tilde{\vr}^e_i - \Tilde{\vr}^*_i &= (\Cov^{-1} + \sigma^{-2} \vI)^{-1} \big[\Cov^{-1} (\vr^e_i - \vPhi_i\vthe) + \sigma^{-2} (\veps^e_i - \veps^*_i) \big]; \\
    \Tilde{\Cov}^e_i &= \Tilde{\Cov}^*_i. 
\end{align*}
\end{lemma}
A direct implication of this lemma is that, suppose when $\vr^e_i$ is close to $\vPhi_i\vthe$, 
the right-hand side of the first equation is equal to $0$ with high probability. 
Then, the multi-task regret of the modified {\name} in the following interactions with task $i$ will be exactly $0$, since the posterior after the alignment period is the same. 
% The multi-task regret when the condition does not hold can be simply bounded by 
% $(T - K) max(\vPhi_i\vthe) \le (T-K) C_2C_3$, 
% \hl{can introduce a condition to control as smaller. But needed?}
% while the probability of this event will approach $0$ when $i \rightarrow \infty$. 
% Specifically, for the first part, we have the following result. 

Given Lemma \ref{lemma:post_relationship}, we are now ready to apply the "prior alignment" technique to derive a regret bound for each task. 
For every $i \in [N]$, we denote the stochastic cumulative rewards in the last $T - K$ interactions starting from a posterior $\Tilde{\vr}$ as $R_i(T-K; \Tilde{\vr})$. Denote the cumulative rewards following the optimal action by $R^*_i(T-K)$. % of the modified oracle-TS
We denote the Bayes regret of $\TSnormal{\Tilde{\vr}^e_i}$ in the last $T - K$ interactions with task $i$ by
% a TS algorithm starting from the posterior $\Tilde{\vr}^e_i$
% _{\vr_i, \Tilde{\vr}^e_i, \veps^e_i}
% \sum_{t = K + 1}^{T} \big(  \big)
\begin{align*}
    BR_i(T-K; \Tilde{\vr}^e_i) = 
    \Mean \Big[R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \Big]. 
    % ( r_{i, a_i^*} - r_{i,A_{i,t}}). 
\end{align*}
We can similarly define $BR_i(T-K; \Tilde{\vr}^*_i)$. 
Our proof relies on the following bound, which controls the Bayes regret of a TS algorithm in the last $T - K$ interactions starting from a different prior. 
% let the posteriors be 
% $\mathcal{N}(\Tilde{\vr}^e_i, \Tilde{\Cov}^e_i)$ and $\mathcal{N}(\Tilde{\vr}^*_i, \Tilde{\Cov}^*_i)$, respectively. 
\begin{lemma}\label{lemma:regret_wrong_prior}
For any task $i \in [N]$
% , for $c_3 = 4\sigma \sqrt{K} + 2\sigma \sqrt{log(NT)}$, 
% with $C_6'$ as an universal constant, 
% |\mJ_{\vr}\Big
we have 
\begin{equation}\label{eqn:bound_J_r}
    \begin{split}
    &\Mean_{\veps^e_i}  
    \Big[
    R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \Big]\\
    &\le     
        exp\big(
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
\sigma
\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}
+ \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
\big)BR_i(T-K; \Tilde{\vr}^*_i)
+ \frac{2C_2C_3}{N}
        % + (T-K)C_2C_3  exp\{-(\frac{c_3 - 4\sigma \sqrt{K}}{ 2\sigma})^2\}
        % \Big]. 
%     &\Mean_{\veps^e_i|}  
%     \Big[
%     R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) | \mJ_{\vr} \Big]\\
%     &\le     
%         exp\big(
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
% + \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
% \big)BR_i(T-K; \Tilde{\vr}^*_i)
%         + (T-K)C_2C_3  exp\{-(\frac{c_3 - 4\sigma \sqrt{K}}{ 2\sigma})^2\}
%         % \Big]. 
    \end{split}
\end{equation}
\end{lemma}

% \begin{proposition}[Bayes regret of the oracle-TS]
% 1
% \end{proposition}
% We aim to establish that, 
% conditional on $\mJ_{\vr}$, 
% with high probability, for $\veps^e_i$, we can find the corresponding $\veps^*_i(\veps^e_i)$, and hence make sure the multi-task regret in the following steps is zero. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We are now ready to combine these results and present our main proof. 

\begin{proof}[Proof of Theorem \ref{thm:meta_ours}]
We first define the event that the estimated task-specific prior mean is close to the true one as 
\begin{align*}
    \mJ_{\vr} \equiv \Big\{||\vr^e_i - \vPhi_i\vthe|| \le 
 2\sqrt{2} C_2 \sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2} 
 + C_3[i c_1'K + 1]^{-1}
 , \forall i \in [N] \Big\}. 
    % | \mH^e_{1:i}
\end{align*}
For simplicity, 
we denote 
$c_4(i) \equiv  2\sqrt{2} C_2 \sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2} 
 + C_3[i c_1'K + 1]^{-1}$.
We note that $c_4(i)$ is a shorthand instead of a constant. 


% If not, we can bounded the regret by the maximum times $1 / \sqrt{i}$. 
% Recall our results in Lemma \ref{lemma:concentration_sampled_prior}: 
% \begin{eqnarray*}
% \begin{split}
%     \prob \Big(||\vr^e_i - \vPhi_i\vthe|| \ge 
%     \sqrt{K} c_1K \big(
%      [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} 
%      &\big(8 \sqrt{d} + 4 \sqrt{-log \xi}\big) \\
%      &+ \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
%      \big)
%     | \mH^e_{1:i}\Big) 
%     \le 2\xi + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
% \end{split}
% \end{eqnarray*}
% \hl{choose: the 2nd term can be control and the conclusion for the first part can hold.}


% \begin{equation}\label{def:BR}
%   BR(N, \{T_i\}) =  \mathbb{E}_{\vx, \vr, \epsilon} \sum_{i = 1}^N
%     \sum_{t = K + 1}^{T} ( r_{i, a_i^*} - r_{i,A_{i,t}}), 
% \end{equation}


% \begin{equation}
%       MTR(N, \{T_i\}; \mathcal{O}) =  \mathbb{E}_{\vx, \vr, \epsilon} \sum_{i = 1}^N 
%     \sum_{t = K + 1}^{T} ( r_{i, A^\mathcal{O}_{i,t}} - r_{i, A_{i,t}}), 
%     % \mathcal{O}(i)
% \end{equation}

% \textbf{Regret bound when $\mJ_{\vr}$ holds.}
We first focus on bounding the regret when $\mJ_{\vr}$ holds. 
% Recall that $c_3 = 4\sigma \sqrt{K} + 2\sigma \sqrt{log(NT)}$.
% Conditional on the event that the prior is close, 
% we can apply the prior alignment technique. 
Define
\begin{equation*}
    \mathcal{S} =  \Big\{i \in [N]: 
    2c_4(i)\sqrt{log(NT)} \le 1/2, \frac{\sigma}{2}c_4(i) \le 2\sqrt{log(NT)} \Big\}. 
    % , \;\;
    % \frac{\sigma^2}{2} c_4(i)^2 \le 1/2, \frac{\sigma^2}{2} c_4(i) \le c_3\}. 
\end{equation*}
% Since $d = o(N)$, $l$ is well defined and 
We first focus on the case that $\mathcal{S}$ is not empty. 
% The case that $\mathcal{S}$ is empty will be discussed at the end. 
Define $l = min(\mathcal{S})$. 
We have $l = O(d log(NT)  + log^2(NT))$ and $\mathcal{S} = \{i \in [N]: i \ge l\}$. 
It also implies $\frac{\sigma^2}{2}c_4(i)^2 \le 2\sigma c_4(i)\sqrt{log(NT)}$ for $i \ge l$. 

% agrawal2013further
% \norm{\vr^e_i - \vPhi_i\vthe}

% Besides, conditional on $\mJ_{\vr}$, we have $\norm{ (\vr^e_i - \vPhi_i\vthe)} \le c_4(i)$, which implies $\frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2 \le c_3 \norm{\vr^e_i - \vPhi_i\vthe}$. 
% \hl{some conditions required here. 2nd inequality}
    % &BR_i(T-K; \Tilde{\vr}^e_i) 
    % &\Mean_{\veps^e_i}  \sum_{t = K + 1}^{T} 
    % \Big[
    % (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i)) |\mJ_{\vr}\Big]\\

Therefore, 
for any $i \ge l$, % setting $\lambda = c_3$ in
by Lemma \ref{lemma:regret_wrong_prior}, we have
\begin{equation}\label{eqn:bound_J_r_large_i}
    \begin{split}
    &\Mean \Big[R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) | \Tilde{\vr}^e_i, \vPhi_i, \mathcal{J}_{\vr} \Big] \\
&\le     
exp\big(
\sigma
\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
+ \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
\big)BR_i(T-K; \Tilde{\vr}^*_i)
+ 2\frac{C_2 C_3}{N} \\
&\le     
exp\big(
% c_3 c_4(i)
c_4(i)\sigma\sqrt{2log(NT)}
+ \frac{\sigma^2}{2}c_4(i)^2
\big) BR_i(T-K; \Tilde{\vr}^*_i)
+ 2\frac{C_2 C_3}{N} \\
&\le 
\big(1 + 
8\sigma c_4(i)\sqrt{log(NT)}
\big)BR_i(T-K; \Tilde{\vr}^*_i)
        + 2\frac{C_2 C_3}{N} , 
\end{split}
\end{equation}
where the 
second inequality follows from the fact that $\norm{\vr^e_i - \vPhi_i\vthe} \le c_4(i)$ conditional on $\mJ_{\vr}$, and the last inequality is due to Lemma \ref{lemma:e_1_2a}. 
% (T-K)C_2C_3  exp\{-(\frac{c_3 - 4\sigma \sqrt{K}}{ 2\sigma})^2\}

% where the first term is due to $exp\big(
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
% + \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
% \big) \le exp\big(
% c_3 c_4(i)
% + \frac{\sigma^2}{2}c_4(i)^2
% \big)$

% better to refer to lemma 6, should be 
% $<=1+2(c3c4(i)+1/2)=2+2c3c4(i);
% c3c4(i)<=1/2 -> 1+4c3c4(i)<=2+2c3c4(i)$
% is it a problem?

% For any number $a \in [0,1]$, it holds that $exp(a) \le 1 + 2a$. 

% russo2014learning
For $i < l$, similar with Lemma 11 in \cite{metapricing}, we note that the Bayes regret for each task can be derived from the prior-independent regret bound for Gaussian bandits in the literature (e.g., \citep{bubeck2014prior}) as % agrawal2013further
\begin{align}\label{eqn:bound_J_r_small_i}
   \Mean \Big[R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) | \Tilde{\vr}^e_i, \vPhi_i, \mathcal{J}_{\vr} \Big] \le C_5 \sqrt{(T-K)KlogT}, 
\end{align}
where $C_5$ is a positive constant. 

% Recall the event 
% \begin{align*}
%     \mJ_{\vr} \equiv \{||\vr^e_i - \vPhi_i\vthe|| \ge 
%     \sqrt{K} c_1K \big(
%      [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} 
%      \big(8 \sqrt{d} + 4 \sqrt{-log \xi}\big) 
%      + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
%      \big) 
%      , \forall i \in [N]\}, 
%     % | \mH^e_{1:i}
% \end{align*}


% Combining \eqref{eqn:first_part_full}, \eqref{eqn:first_part_coef}, and \eqref{eqn:bound_part2}, we can obtain 
% \begin{equation}\label{eqn:bound_J_r}
%     \begin{split}
%     &\Mean_{\veps^e_i}  \sum_{t = K + 1}^{T} 
%     \Big[
%     (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i)) |\mJ_{\vr}\Big]\\
%     &\le     
%         (1 + 4c_3 c_4(i)) 
%         BR_i(T-K; \Tilde{\vr}^*_i) 
%         + (T-K) C_2C_3 exp\{-[(c_3 - 4\sigma \sqrt{K}) /  2\sigma]^2\}
%     \end{split}
% \end{equation}

% similar with the derivations for \eqref{eqn:bound_part2}, we can simply bound the multi-task regret for one task by 
% $(T-K) C_2C_3$. 
% Besides, 
% \textbf{Regret bound when $\neg \mJ_{\vr}$ holds.}
When $\neg \mJ_{\vr}$ holds, for $i \in [N]$, we define 
\begin{align*}
    \mJ_{\vr, i} \equiv \Big\{||\vr^e_i - \vPhi_i\vthe|| <
 2\sqrt{2} C_2 \sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2} 
 + C_3 [i c_1'K + 1]^{-1}\Big\}. 
    % | \mH^e_{1:i}
\end{align*}
From Lemma \ref{lemma:concentration_sampled_prior}, we know 
$\prob[\neg \mJ_{\vr, i}] \le 2\frac{1}{NT}+ d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}$. 
% we can apply a union bound over $i \in [N]$ to \eqref{eqn:concentration_sampled_prior} in to yield 
Then, by similar arguments with \eqref{eqn:bound_J_r_small_i}, we have 
\begin{equation}\label{eqn:bound_not_J_r}
    \begin{split}
    %     &\Mean \Big[\sum_{i=1}^N \big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \big) | \Tilde{\vr}^e_i, \vPhi_i, \neg \mathcal{J}_{\vr} \Big] \times
    % \prob[\mJ_{\vr}] \\
        &\sum_{i=1}^N \Mean \Big[ \big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \big) | \Tilde{\vr}^e_i, \vPhi_i, \neg \mathcal{J}_{\vr} \Big] \times
    \prob[\neg \mJ_{\vr}] \\
        &\le \sum_{i=1}^N \Mean \Big[ \big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \big) | \Tilde{\vr}^e_i, \vPhi_i, \neg \mathcal{J}_{\vr} \Big] \times
    \prob[\neg \mJ_{\vr, i}] \\
&\le \sum_{i=1}^N C_5 \sqrt{(T-K)KlogT} \times \prob[\neg \mJ_{\vr, i}]\\
&\le  C_5' d \sqrt{(T-K)KlogT}, 
    \end{split}
\end{equation}
where $C_5'$ is an universal constant. 


% \begin{align}
%     \Mean_{\veps^e_i}  \sum_{t = K + 1}^{T} 
%     \Big[
%     (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i)) |\neg \mJ_{\vr}\Big] \times
%     \prob[\neg \mJ_{\vr}] 
%         \le N(T-K) C_2C_3 [2\frac{1}{NT}+ d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}]. 
% \end{align}



% \textbf{Putting everything together.}
Finally, we note the following relationship
\begin{equation}\label{eqn:decomposition}
    \begin{split}
    &\Mean_{\veps^e_i}  
    \Big(R_i(T-K; \Tilde{\vr}^*_i) - R_i(T-K; \Tilde{\vr}^e_i)\Big)\\
    &=
    \Mean_{\veps^e_i}  
    \Big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i)\Big)
    - \Mean_{\veps^e_i}  
    \Big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^*_i)\Big)
    \\
    &=
    \Mean_{\veps^e_i}  
    \Big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) |\mJ_{\vr}\Big) \times
    \prob[\mJ_{\vr}] \\
    &+
    \Mean_{\veps^e_i}  
    \Big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) |\neg \mJ_{\vr} \Big) \times
    \prob[\neg \mJ_{\vr}] 
    - BR_i(T-K; \Tilde{\vr}^*_i) %\\
    % &\le
    % 4c_3 c_4(i)
    % BR_i(T-K; \Tilde{\vr}^*_i) 
    % + (T-K) C_2C_3 exp\{-[(c_3 - 4\sigma \sqrt{K}) /  2\sigma]^2\}\\
    % &+
    % N(T-K) C_2C_3 [2\frac{1}{NT}+ d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}] \alignlable{eqn:bound_each_i}.
    \end{split}
\end{equation}



% \eqref{eqn:bound_J_r} and  \eqref{eqn:bound_not_J_r} together imply a bound on the multi-task regret as 
Denote the Bayes regret of the modified oracle-TS as $BR'(N, \{T_i\})$. 
Based on \eqref{eqn:bound_J_r_large_i}, \eqref{eqn:bound_J_r_small_i}, and \eqref{eqn:bound_not_J_r}, we sum \eqref{eqn:decomposition} from $i = 1$ to $N$ to yield the regret of the modified {\name} to the modified oracle-TS as 
\begin{align*}
    %&MTR(N, \{T_i\}; \mO')\\
    &BR(N, \{T_i\}) - BR'(N, \{T_i\})\\
    % =  \mathbb{E}_{\vx, \vr, \epsilon} \sum_{i = 1}^N 
    % \sum_{t = K + 1}^{T} ( r_{i, A^\mathcal{O}_{i,t}} - r_{i, A_{i,t}}), 
    &\le \sum_{i=l}^N \Big[
        8\sigma c_4(i)\sqrt{log(NT)}  BR_i(T-K; \Tilde{\vr}^*_i)
        + 2\frac{C_2 C_3}{N} 
    \Big]\\
    &\;\; + C_5 l \sqrt{(T-K)KlogT} + C_5'd \sqrt{(T-K)KlogT}\\
    &\le \sum_{i=l}^N C_4'\Big[
        \sqrt{log(NT)} (\sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2} 
        + C_3[i c_1'K + 1]^{-1}
        ) BR_i(T-K; \Tilde{\vr}^*_i)\\
    &\;\; 
    % (T-K)C_2C_3  exp\{-log(NT)\}
    \Big]+ O(1)
     + C_6 (l+d) \sqrt{(T-K)KlogT} \\
    &\le \sum_{i=l}^N C_4'\Big[
        \sqrt{log(NT)} (\sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2}
        + C_3[i c_1'K + 1]^{-1}
        ) BR_i(T-K; \Tilde{\vr}^*_i)\Big] + O(1)\\
    &+ C'_6 (d log(NT) + log^2(NT)) \sqrt{(T-K)KlogT}  \\
    &= O(\sqrt{log(NT)} (\sqrt{d} + \sqrt{log(NT)} \big) \sqrt{N} \sqrt{(T-K)K logT}
    + (log(NT) d + log^2(NT)) \sqrt{(T-K)KlogT}), 
\end{align*}
where $C_4'$, $C_6$, and $C'_6$ some universal constants, 
the last inequality is due to $l = O(dlog(NT)  + log^2(NT))$, 
and the last equality is due to $BR_i(T-K; \Tilde{\vr}^*_i) = O(\sqrt{(T-K)K logT})$ according to Proposition 2 in \cite{russo2014learning}. 
In the last equality, we also utilize the fact that $\sum_{i=l}^{N}1/\sqrt{i} = O(\sqrt{N})$, and $\sum_{i=l}^{N}1/{i} = O(log(N))$. 
% results on 
% Gaussian bandits in the literature \cite{russo2014learning}. 
%  $l = O(N)$, 
Recall that, until now,  we consider the case that $\mathcal{S}$ is not empty. 
When $\mathcal{S}$ is empty, we have $N = O(log^2(NT))$, and then 
we can follow the arguments of \eqref{eqn:bound_J_r_small_i} to bound the regret when $\mJ_{\vr}$  holds as 
$O(log^2(NT)\sqrt{(T-K)KlogT})$, and we can similarly obtain the above bound. 


Finally, we bound the regret of the modified oracle-TS  to the vanilla oracle-TS. 
%  can be bounded by $O(NK)$
We denote the action that the modified oracle-TS takes at the $t$-th interaction with task $i$ as $A^{\Tilde{\mathcal{O}}}_{i,t}$. 
This multi-task regret of the modified oracle-TS is then equal to 
\begin{align*}
\mathbb{E}_{\vx, \vr, \epsilon} 
\sum_{t = 1}^{T} ( 
r_{i,A^{\mathcal{O}}_{i,t}} - 
r_{i, A^{\Tilde{\mathcal{O}}}_{i,t}}
)
&= \mathbb{E}_{\vx, \vr, \epsilon} 
\Big[
\big(
\sum_{t = 1}^{K} r_{i, A^{\mathcal{O}}_{i,t}} - 
\sum_{t = 1}^{K} r_{i, A^{\Tilde{\mathcal{O}}}_{i,t}}
\big)
+ 
\big(
\sum_{t = T - K + 1}^{T} r_{i, A^{\mathcal{O}}_{i,t}} - 
\sum_{t = T - K + 1}^{T} r_{i, A^{\Tilde{\mathcal{O}}}_{i,t}}
\big)
\Big]\\
&= O(K). 
\end{align*}
Here, for the first term, 
We note the regret from $K$ interactions with task $i$ is always bounded by 
$K max(\vr_i)$, the expectation of which over the task distribution is bounded by $KC_2C_3$. 
The second part is bounded by $0$, since the two algorithms share the same prior and the modified oracle-TS essentially have $K$ more data points with no confounding variables \cite{ye2020combining}. 

% For each $i$, the multi-task regret of the modified oracle-TS in the alignment period can be bounded by $KC_2C_3$. 
% For the remaining $T-K$ interactions, we note that $\vr_i | \vPhi_i \sim \normal(\vPhi_i\vthe, \Cov)$ and $\vR^e_i |\vr_i \sim \normal(\vr_i, \sigma^2 \vI)$. 
% Denote the corresponding density function as $h_1(\vr_i|\vPhi_i)$ and $h_2(\vR^e_i|\vr_i)$, respectively. 
% Write $h_3(\vr_i| \vR^e_i, \vPhi_i)$ as the posterior of $\vr_i$ after observing $\vR^e_i$. 
% Therefore, 
% conditional on $\vPhi_i$, 
% we can simply regard the behaviour of the modified oracle-TS in the remaining $T-K$ interactions as an vanilla oracle-TS algorithm with prior $\int h_3(\vr_i| \vR^e_i, \vPhi_i) h_2(\vR^e_i|\vr'_i) h_1(\vr'_i|\vPhi_i) d \vr'_i d \vR^e_i$, and hence bound 

Putting everything together, 
we conclude with  
\begin{align*}
    &MTR(N, \{T_i\})\\
    &= BR(N, \{T_i\}) - BR'(N, \{T_i\}) + N \times O(K)\\
    &= O(\sqrt{log(NT)} (\sqrt{d} + \sqrt{log(NT)} \big) \sqrt{N} \sqrt{(T-K)K logT}
    + (log(NT) d + log^2(NT)) \sqrt{(T-K)KlogT} + NK)\\
    &= O(\sqrt{log(NT)} (\sqrt{d} + \sqrt{log(NT)} \big) \sqrt{N} \sqrt{TK logT} 
    + log^2(NT) \sqrt{(T-K)KlogT}
    + NK)\\
    &= \TO(  \sqrt{N} \sqrt{dTK} + NK).
\end{align*}



\end{proof}



==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/Proof_lemmas.tex <==
\section{Proof of Lemmas and Propositions}\label{sec:proof_lemmas}
\subsection{Proof of Lemma \ref{lemma:concentration_sampled_theta}}
\begin{proof}
Throughout the proof, recall the fact that $\vthe$ is a fixed vector instead of a random vector, and we only adopt the Bayesian approach to adapt the TS framework. 
We first note that, 
according to the results on Bayesian LMM (page 361, \cite{wu2009mixed}), we have the following expression for the posterior of $\vthe$: 
\begin{equation}\label{eqn:theta_posterior}
    \vthe | \mH^e_{1:i} \sim \mathcal{N}\Big((\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\vPhi^T \mV^{-1}\vR, (\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\Big). 
\end{equation}
Recall that, when the context is clear, we may drop the subscript $1:i$ and superscript $e$. 
% We will first show that, with high probability, the sample task-specific prior is close to the true prior. 
% [as long as they are bounded. Introduce a condition. K and p will be naturally involved?]
Let $\hat{\vthe}^e_i = (\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\vPhi^T \mV^{-1}\vR$ be the maximum a posterior estimator of $\vthe$, which implies 
\begin{equation}\label{eqn:theta_hat_diff_distribution}
    \hat{\vthe}^e_i - \vthe | \vPhi \sim \mathcal{N}\Big( -[(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1} \vthe, [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1} - [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-2}
    \Big). 
\end{equation}




% \begin{lemma}\label{lemma:concentration_hat_theta}
% For any task $i \in [N]$, at the end of its alignment period, for any $\xi \in (0, 1)$, we have 
% \begin{align*}
%     \prob \big(||\hat{\vthe}^e_i - \vthe|| \ge 
%      [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(4 \sqrt{d} + 2 \sqrt{-log \xi}\big) + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
%     | \mH^e_{1:i}\big) \le \xi + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
% \end{align*}
% \end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Let $\vthe^e_i \sim \vthe|\mH^e_{1:i}$ be the sample from the posterior. 

\paragraph{Concentration of $\hat{\vthe}^e_i$ around $\vthe$.}
To derive the concentration of $\hat{\vthe}^e_i - \vthe$ around $\vzero$, 
we analyze the concentration of its mean around $\vzero$ and the magnitude of its variance separately. 
We begin by defining the event
\begin{equation*}
    \mJ_{\vPhi} \equiv  \big\{  \sigma_{\min}[\vPhi^T\vPhi] \ge 
    % [\frac{2||\vthe||}{\xi} - 1] (\sigma^2+1) 
    \frac{1}{2} i c_1K
    \big\}, 
\end{equation*}
% Define $$. 
% but C_1 can depend on d. 
According to Lemma \ref{lemma:fisher_lower}, based on  Assumption \ref{asmp:cov_x}, 
we have 
\begin{align}\label{eqn:prob_J_phi}
    \prob(\mJ_{\vPhi})
    % &= \prob \Big[  \sigma_{\min}[\frac{1}{i} \sum_{j=1}^i \vPhi_i^T\vPhi_i] \ge \frac{2||\vthe|| / \xi - 1}{i}(\sigma^2+1)\Big]\\
    &\ge 1 - d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
    % 1 - d\Big[ \frac{e^{-c}}{(1-c)^{1-c}} \Big]^{ic_1K}, 
\end{align}
% where $c = 1 -  \frac{2||\vthe|| / \xi - 1 }{ i c_1K}(\sigma^2 + 1)$. 

For the mean part of \eqref{eqn:theta_hat_diff_distribution}, based on the property of matrix  operator norm, we can derive 
\begin{align*}
    \mJ_{\vPhi} 
    &=  \big\{  \sigma_{\min}[\vPhi^T\vPhi] \ge \frac{1}{2} i c_1K \big\}\\
    % \{ (\sigma^2+1)^{-1} \sigma_{\min}[\vPhi^T\vPhi] + 1 \ge \frac{2||\vthe||}{\xi}\}\\
    &= \{ \sigma_{\min}[(\sigma^2+1)^{-1}\vPhi^T\vPhi + \vI] \ge \frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1 \}\\
    &= \{ \norm[\big]{[(\sigma^2+1)^{-1}\vPhi^T\vPhi + \vI]^{-1}} \le \frac{1}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1} 
    \}\\
    &\subseteq \{\norm[\big]{[(\sigma^2+1)^{-1}\vPhi^T\vPhi + \vI]^{-1}(-\vthe)} \le \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
    \}, 
    % \prob \Big[  \sigma_{\min}[\frac{1}{i} \sum_{j=1}^i \vPhi_i^T\vPhi_i] \ge \frac{2||\vthe|| / \xi - 1}{(\sigma^2+1)^{-1}i} \Big]
\end{align*}
where the third equality is due to $\sigma_{min} (\mathbf{A}) = ||\mathbf{A}^{-1}||$ for any invertible matrix $\mathbf{A}$. 
This relationship implies 
\begin{align*}
    \Mean [\hat{\vthe}^e_i - \vthe | \mJ_{\vPhi}] \le \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}. 
\end{align*}
% \begin{align*}
%     \prob \Big\{\Mean [\hat{\vthe}^e_i - \vthe | \mJ_{\vPhi}] \le \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1} \Big\} \ge 1 - d (\frac{e}{2})^{-\frac{c_1K}{2C_1}i}.     
% \end{align*}


For the variance part of \eqref{eqn:theta_hat_diff_distribution}, define a random vector $\vz \sim \normal(\vzero, [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1} - [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-2})$. 
According to the tail inequality for the Euclidean norm of Gaussian random vectors (see Lemma \ref{lemma:2_norm_Gaussian}), 
for any $\xi \in (0, 1)$, 
we have 
\begin{align}\label{eqn:normal_tail}
    \prob \Big[\norm{\vz} \le \sigma_{\vz} \sqrt{d} + \sigma_{\vz} \sqrt{2(-log \xi)} |\vPhi \Big]  \ge 1 - \xi, 
\end{align}
where $\sigma_{\vz} = \norm{[(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1} - [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-2}}^{1/2}$. 
% Set $4\sigma_{\vz} \sqrt{d} + 2\sigma_{\vz} \sqrt{-log \xi} = \xi / 2$, we have 
% $\xi = exp\{-[(\xi / 2 - 4\sigma_{\vz} \sqrt{d}) / (2\sigma_{\vz})]^2\}$. 
% Therefore, we obtained that 
% \begin{align}\label{eqn:normal_tail}
%     \prob \Big[\norm{\vz} \le \xi / 2 \Big]  \ge 1 - exp\{-\big[
%     \frac{\xi}{4\sigma_{\vz}} - 2 \sqrt{d} \big]^2\}. 
% \end{align}
% % monotone: []^2 >= xxx -> prob >= ...
We then focus on control $\sigma_{\vz}$:  
\begin{align*}
\sigma_{\vz}
&= \norm{
[(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1} \{ \vI - [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1}
\}}^{1/2} \\
&\le \Big\{ 
\norm{[(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1}} \times
\norm{\vI - [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1}}
\Big\}^{1/2}\\
&\le 
\norm{[(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1}}^{1/2}
% \\
% &= 
% [(\sigma^2+1)^{-1} \sigma_{\min}[\vPhi^T\vPhi] + 1]^{-1/2}
\end{align*}
where the first inequality follows from the sub-multiplicative property of the matrix operator norm, and the second  follows from the fact that $\norm{\vI - (\vI + \vA)^{-1}} \le 1$ for any symmetric matrix $\vA$. 


Therefore, conditional on $ \mJ_{\vPhi} $, we have 
$\sigma_{\vz} \le [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2}$, 
which together with \eqref{eqn:normal_tail} implies 
\begin{align*}
    \prob \Big[\norm{\vz} \le  [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big( \sqrt{d} + \sqrt{2} \sqrt{-log \xi}\big) | \mJ_{\vPhi} \Big] \ge 1 - \xi. 
\end{align*}

Note that, based on the triangle inequality, we have 
$||\hat{\vthe}^e_i - \vthe|| \le ||\Mean(\hat{\vthe}^e_i| \mJ_{\vPhi}) - \vthe|| + ||\hat{\vthe}^e_i - \Mean(\hat{\vthe}^e_i| \mJ_{\vPhi})|| $. 
Combining the two parts, we conclude with 
\begin{align}\label{eqn:concentration_mean}
    \prob \big(||\hat{\vthe}^e_i - \vthe|| \ge 
     [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(\sqrt{d} + \sqrt{2} \sqrt{-log \xi}\big) + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
    | \mJ_{\vPhi}\big) \le \xi. 
\end{align}

%  \mH^e_{1:i}
\paragraph{Concentration of $\vthe^e_i$ around $\hat{\vthe}^e_i$.}
Note that 
\begin{equation}
    \vthe^e_i - \hat{\vthe}^e_i |\vPhi \sim \mathcal{N}\Big(\vzero, (\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\Big). 
\end{equation}

% According to the tail inequality for the Euclidean norm of Gaussian random vectors \citep{hsu2012tail}, 
% for any $\delta \in (0, 1)$, 
% we have 
% \begin{align}
%             \prob \Big[\norm{\vz} \le 4\sigma_{\vz} \sqrt{d} + 2\sigma_{\vz} \sqrt{-log \delta} \Big]  \ge 1 - \delta,
% \end{align}
% where $\sigma_{\vz} = \norm{((\sigma^2 + 1)^{-1} \vPhi^T\vPhi + \vI)^{-1}}^{1/2}$. 

We begin by defining a random vector $\vz \sim \normal(\vzero, ((\sigma^2 + 1)^{-1} \vPhi^T\vPhi + \vI)^{-1})$. 
By similar arguments with that for the variance part in \eqref{eqn:theta_hat_diff_distribution}, we get
\begin{align*}
    \prob \Big[\norm{\vz} \le  [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(\sqrt{d} + \sqrt{2} \sqrt{-log \xi}\big) | \mJ_{\vPhi} \Big] \ge 1 - \xi, 
\end{align*}
which implies 
\begin{align}\label{eqn:res_sampled_mean_distance}
    \prob \Big[\norm{\vthe^e_i - \hat{\vthe}^e_i} \le  [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(\sqrt{d} + \sqrt{2} \sqrt{-log \xi}\big) | \mJ_{\vPhi} \Big] \ge 1 - \xi. 
    % \mH^e_{1:i}
\end{align}

Note that, based on the triangle inequality, we have $||\vthe^e_i - \vthe|| \le ||\vthe^e_i - \hat{\vthe}^e_i|| + ||\hat{\vthe}^e_i - \vthe||$. 
Therefore, applying an union bound to \eqref{eqn:concentration_mean} and \eqref{eqn:res_sampled_mean_distance} yields that
\begin{align*}
    \prob \Big[\norm{\vthe^e_i - \vthe} \le  [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(2 \sqrt{d} + 2\sqrt{2} \sqrt{-log \xi}\big)      + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1} | \mJ_{\vPhi} \Big] \ge 1 - 2\xi. 
    % \mH^e_{1:i}
\end{align*}
This result, together with \eqref{eqn:prob_J_phi}, implies that 
\begin{align*}
    \prob \big(||\vthe^e_i - \vthe|| \ge 
     [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(2 \sqrt{d} + 2\sqrt{2} \sqrt{-log \xi}\big) 
     + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
    \big) \le 2\xi + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
\end{align*}
    % | \mH^e_{1:i}
    
\end{proof}

\subsection{Proof of Lemma \ref{lemma:concentration_sampled_prior}}
\begin{proof}
% The second term is bounded w.h.p

The first term needs assumptions
\begin{align*}
    ||\vr^e_i - \vPhi_i\vthe ||
    &= ||\vPhi_i\vthe^e_i - \vPhi_i\vthe||\\
    &\le ||\vPhi_i|| \times ||\vthe^e_i - \vthe||\\
    &\le \sqrt{K} C_2 ||\vthe^e_i - \vthe||, 
\end{align*}
where the last inequality is based on  Assumption \ref{asmp:linear_magnitute}. 
Recall the results in Lemma \ref{lemma:concentration_sampled_theta} that
% based on the triangle inequality, we get that 
\begin{eqnarray}
\begin{split}
    \prob \Big(||\vr^e_i - \vPhi_i\vthe|| \ge 
    \sqrt{K} C_2 \big(
     [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} 
     &\big(2 \sqrt{d} + 2\sqrt{2} \sqrt{-log \xi}\big) \\
     &+ \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
     \big)
    \Big) 
    \le 2\xi + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
\end{split}
\end{eqnarray}

% It can be seen that, $c_4(i)$ will decays to $0$, roughly at a rate of $O(1 / \sqrt{i})$. 
% More precisely, 
% Recall that  $c_1K = c_1 K \log_{e/2}(NTd)$, 
Under Assumption \ref{asmp:linear_magnitute}, 
with $c_1' = c_1 \frac{(\sigma^2+1)^{-1}}{2}$, 
by setting $\xi = \frac{1}{NT}$, 
we can derive
\begin{eqnarray}
\begin{split}
    \prob \Big(||\vr^e_i - \vPhi_i\vthe|| \ge 
 2\sqrt{2} C_2 \sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-\frac{1}{2}} 
 + C_3[i c_1'K + 1]^{-1}
\Big) 
    \le \frac{2}{NT} + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
\end{split}
\end{eqnarray}

\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Lemma \ref{lemma:post_relationship}}
\begin{proof}
The relationship follows from the posterior updating rule for multivariate Gaussian. 
Specifically, we have 
\begin{align*}
    \Tilde{\vr}^e_i &= (\Cov^{-1} + \sigma^{-2} \vI)^{-1} (\Cov^{-1}\vr^e_i + \sigma^{-2} \vR^e_i);\\
    \Tilde{\Cov}^e_i &=  (\Cov^{-1} + \sigma^{-2} \vI)^{-1};\\
    \Tilde{\vr}^*_i &= (\Cov^{-1} + \sigma^{-2} \vI)^{-1} (\Cov^{-1}\vPhi_i\vthe + \sigma^{-2} \vR^*_i);\\
     \Tilde{\Cov}^*_i &=  (\Cov^{-1} + \sigma^{-2} \vI)^{-1}, 
\end{align*}
which implies
\begin{align*}
    \Tilde{\vr}^e_i - \Tilde{\vr}^*_i &= 
    (\Cov^{-1} + \sigma^{-2} \vI)^{-1} \big[\Cov^{-1} (\vr^e_i - \vPhi_i\vthe) + \sigma^{-2} (\veps^e_i - \veps^*_i) \big]\\
    % (\vI + \sigma^{-2} \Cov)^{-1}  
    % (\vr^e_i - \vPhi_i\vthe)\\
    \Tilde{\Cov}^e_i &= \Tilde{\Cov}^*_i. 
\end{align*}
\end{proof}


\subsection{Proof of Lemma \ref{lemma:regret_wrong_prior}}
\begin{proof}
Recall that 
\begin{align*}
    \Tilde{\vr}^e_i - \Tilde{\vr}^*_i &= (\Cov^{-1} + \sigma^{-2} \vI)^{-1} \big[\Cov^{-1} (\vr^e_i - \vPhi_i\vthe) + \sigma^{-2} (\veps^e_i - \veps^*_i) \big], 
\end{align*}
which implies $\Tilde{\vr}^e_i = \Tilde{\vr}^*_i$ when $\veps^*_i = \veps^e_i + \sigma^2 \Cov^{-1} (\vr^e_i - \vPhi_i\vthe)$. 
% With slight abuse of notations, w
We denote 
\begin{align}\label{eqn:one2one}
    h_i(\veps^e_i) \equiv \veps^e_i + \sigma^2 \Cov^{-1} (\vr^e_i - \vPhi_i\vthe), 
\end{align}
which will then allow us to apply a change-of-variable trick. 
We note this is an one-to-one mapping. 
Besides, due to the round robin nature, we have $\veps^*_i \sim \veps^e_i \sim \mathcal{N}(\vzero, \sigma^2 \vI)$. 

Define $\mJ_{\veps, \vr, i}$ as the event $\{|(\vr^e_i - \vPhi_i\vthe)^T \veps^e_{i}| \le \sigma\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)} \}$. 
We begin by expressing $BR_i(T-K; \Tilde{\vr}^e_i)$ as a function of $BR_i(T-K; \Tilde{\vr}^*_i)$ via a change of measure. 
% | \mJ_{\vr}
% We note that 
\begin{align*}
    % &BR_i(T-K; \Tilde{\vr}^e_i) \\
    % &= 
    % \vr_i, \Tilde{\vr}^e_i, #???
    &\Mean_{\veps^e_i}
    \Big[
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i)) \Big]\\
    &= \int_{\veps^e_i} \frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}} (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i) \\
    &= \int_{\veps^e_i} 
    \frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i)\\
    &= \int_{\veps^e_i} \I[\mJ_{\veps, \vr, i}]
    \frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i)\\
    &+ \int_{\veps^e_i} \I[\neg \mJ_{\veps, \vr, i}]
    \frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i) . \alignlable{eqn:two_terms}
\end{align*}
In what follows, we will control the two parts of \eqref{eqn:two_terms} separately. 


\paragraph{First part of \eqref{eqn:two_terms}.}
For the first part of \eqref{eqn:two_terms}, conditional on $\mJ_{\vr}$, we have 
\begin{align*}
    & \int_{\veps^e_i} \I[\mJ_{\veps, \vr, i}]
    \frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i)\\
    &\le 
    max \Big\{\I[\mJ_{\veps, \vr, i}]
        exp\Big(\frac{\norm{h_i(\veps^e_i)}^2- \norm{\veps^e_i}^2}{2\sigma^2}\Big)\Big\}
    \int_{\veps^e_i} \I[\mJ_{\veps, \vr, i}]
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i)\\
    &\le
    max \Big\{\I[\mJ_{\veps, \vr, i}]
        exp\Big(\frac{\norm{h_i(\veps^e_i)}^2- \norm{\veps^e_i}^2}{2\sigma^2}\Big)\Big\}
    \int_{\veps^e_i} 
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i)\\
    &=
    max \Big\{\I[\mJ_{\veps, \vr, i}]
        exp\Big(\frac{\norm{h_i(\veps^e_i)}^2- \norm{\veps^e_i}^2}{2\sigma^2}\Big)\Big\}
        BR_i(T-K; \Tilde{\vr}^*_i) \alignlable{eqn:first_part_full}, 
\end{align*}
where the second inequality follows from the fact that the integrand is non-negative. 
Recall that, without loss of generality, we have assumed $\Cov = \vI$. 
To control this term, we use the relationship \eqref{eqn:one2one} to yield
\begin{align*}
&max \Big\{\I[\mJ_{\veps, \vr, i}]
        exp\Big(\frac{\norm{h_i(\veps^e_i)}^2- \norm{\veps^e_i}^2}{2\sigma^2}\Big)\Big\}\\
&= max \Big\{\I[\mJ_{\veps, \vr, i}]
exp\Big(\frac{\norm{\veps^e_i + \sigma^2  (\vr^e_i - \vPhi_i\vthe)}^2- \norm{\veps^e_i}^2}{2\sigma^2})\Big\}\\
&= max \Big\{\I[\mJ_{\veps, \vr, i}]
exp\Big(
(\veps^e_i)^T (\vr^e_i - \vPhi_i\vthe)
+ \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
)\Big\}\\
% &\le
%  max \Big\{\I[\mJ_{\veps, \vr, i}]
% exp\Big(
% \norm{\veps^e_i} \norm{\vr^e_i - \vPhi_i\vthe}
% + \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
% )\Big\}\\
&\le 
exp\Big(
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
\sigma
\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}
+ \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
\Big),
\end{align*}
where the inequality is due to the definition of $\mJ_{\veps, \vr, i}$.

\paragraph{Second part of \eqref{eqn:two_terms}.}
For the second part of \eqref{eqn:two_terms}, we can bound it by 
\begin{align*}
&\int_{\veps^e_i} 
\I[\neg \mJ_{\veps, \vr, i}]
\frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
\frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i) \\
&\le \Mean \Big[
R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) , \neg \mJ_{\veps, \vr, i}
\Big] \times \prob[\neg \mJ_{\veps, \vr, i}] \alignlable{eqn:two_parts_of_part2}. 
\end{align*}

For the first term of \eqref{eqn:two_parts_of_part2}, 
we note the regret from $T - K$ interactions with task $i$ is always bounded by 
$(T-K) max(\vr_i)$, the expectation of which over the task distribution is bounded by $(T-K) C_2C_3$. 


For the second term of \eqref{eqn:two_parts_of_part2}, 
we recall the tail inequality of Gaussian distributions: 
for any random variable $z \sim \normal(0, \sigma^2)$, we have $\prob[|z| \ge c\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}] \le 2exp(-\norm{\vr^e_i - \vPhi_i\vthe}^2 c^2 log(NT)/\sigma^2)$, where $c$ is any constant. 
Notice that $(\vr^e_i - \vPhi_i\vthe)$ is independent with $\veps^e_{i}$, which implies that, for any fixed value of $\vr^e_i - \vPhi_i\vthe$, it holds that $(\vr^e_i - \vPhi_i\vthe)^T \veps^e_{i} \sim \normal\big(0, \sigma^2 \norm{\vr^e_i - \vPhi_i\vthe}^2 \big)$. 
Therefore, by setting $c = \sigma$, we have 
% we have $(\vr^e_i - \vPhi_i\vthe)^T \veps^e_{i} \sim \normal(0, \norm{\vr^e_i - \vPhi_i\vthe}^2)$, which implies 
\begin{align*}
\prob[\neg \mJ_{\veps, \vr, i}] 
&= \prob[|(\vr^e_i - \vPhi_i\vthe)^T \veps^e_{i}| \ge \sigma\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}] \\
&= \prob[|(\vr^e_i - \vPhi_i\vthe)^T \veps^e_{i}| \ge \sigma\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}|\vr^e_i - \vPhi_i\vthe] \\
&\le 2exp(-log(NT)) = \frac{2}{NT}
\end{align*}


% by similar arguments with the proof of Lemma \ref{lemma:concentration_sampled_theta} on the tail inequality for the Euclidean norm of a Gaussian random vector, 
% we can obtain that for any $\xi \in (0, 1)$, 
% \begin{align*}
%     \prob[\norm{\veps^e_i} > 4\sigma \sqrt{K} + 2\sigma \sqrt{-log \xi}] \le \xi. 
% \end{align*}
% By setting $4\sigma \sqrt{K} + 2\sigma \sqrt{-log \xi} = c_3$, which is equivalent to $\xi = exp\{-[(c_3 - 4\sigma \sqrt{K}) /  2\sigma]^2\}$, we get 
% \begin{align*}
%     \prob[\norm{\veps^e_i} > c_3] \le  exp\{-[(c_3 - 4\sigma \sqrt{K}) /  2\sigma]^2\}. 
% \end{align*}

Putting these two parts together, we obtain a bound for the second term of \eqref{eqn:two_terms} as 
\begin{align*}
&\int_{\veps^e_i} 
\I[\neg \mJ_{\veps, \vr, i}]
\frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
\frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i) \\
&\le \frac{2C_2C_3}{N}
% &\le (T-K) C_2C_3 exp\{-[(c_3 - 4\sigma \sqrt{K}) /  2\sigma]^2\}
\alignlable{eqn:bound_part2}. 
\end{align*}


Finally, 
combining \eqref{eqn:first_part_full} and \eqref{eqn:bound_part2}, 
we can obtain 
\begin{equation}
    \begin{split}
    &\Mean_{\veps^e_i}  
    \Big[
    R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \Big]\\
    &\le     
        exp\big(
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
\sigma
\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}
+ \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
\big)BR_i(T-K; \Tilde{\vr}^*_i)
+ \frac{2C_2C_3}{N}
        % + (T-K)C_2C_3  exp\{-(\frac{c_3 - 4\sigma \sqrt{K}}{ 2\sigma})^2\}
        % \Big]. 
    \end{split}
\end{equation}

\end{proof}


\input{regret_baselines}

\input{technical_lemmas}


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/computational_complexity.tex <==
\subsection{Computational complexity}\label{sec:Computational_complexity}
In this section, we analyze the computational complexity for {\name}. 
The specific complexity depends on: 
(i) the reward distribution, 
(ii) the hierarchical model one chooses, 
(iii) whether the vanilla version or some variant is used, 
and (iv) the order of interactions. 
Therefore, we will first present a general complexity bound and then discuss examples. 
For simplicity, we assume $T_1 = \dots = T_N = T$. 
Let $m(i,t)$ and $m'(i,t)$ be the number of data points for task $i$ alone and that for all tasks, until the $t$-th interaction with task $i$. 
The computation complexity is clearly dominated by one step: updating and sampling from the posterior. 
We denote its complexity at interaction $(i,t)$ by $c\big(m(i,t), m'(i,t)\big)$. 
Then, the total complexity is bounded by 
$O(\sum_{i=1}^N \sum_{t=1}^T c\big(m(i,t), m'(i,t)\big)$. 

For Gaussian bandits with LMM, 
recall that we can update $\vthe$ incrementally, and according to its posterior form \eqref{eqn:theta_posterior}, 
each time $O(d^3)$ flops are required to sample $\vthe$. 
Besides, $O(dK)$ flops are required to compute the prior mean, 
and $O(K^2)$ flops are required to compute the posterior of $\vr_i$. 
Therefore, with Algorithm 1, the total complexity is bounded by 
$O\big(NT(K^2 + d^3)\big)$. 
Under the sequential setting, with Algorithm 2, it can be reduced to 
$O\big(N(TK^2 + d^3)\big)$. 

For Bernoulli bandits with BBLM, suppose $M$ samples are taken in each round of MCMC sampling, and $c'\big(m(i,t), m'(i,t)\big)$ flops are needed to sample each, then under Algorithm \ref{alg:TS_faster_general} with $l = T$, we have that the total complexity is bounded by
$O(\sum_{t=1}^T Mc'\big(t, tN) + NTdK + NTK\big) = O(\sum_{t=1}^T Mc'\big(t, tN) + NTdK\big)$ under the concurrent setting, 
and $O\big(\sum_{i=1}^N Mc'\big(0, iT\big) + NdK + NTK\big) = 
O\big(\sum_{i=1}^N Mc'\big(0, iT\big) + NTK\big)$. 

% With the implementation in Appendix \ref{sec:appendix_implementation_gaussian}, 
% under the episodic setting, we have $m(i,t) = (t-1)$ and  $m'(i,t) = (i-1)*T + (t - 1)$, which together with our analysis in Appendix \ref{sec:appendix_implementation_gaussian}, imply that 
% $cost^1_{i,t} = O((n-1)T^3)$ and $cost^2_{i,t} = O(1)$. 
% Therefore, the total complexity is bounded by $O(n^2T^4)$. 
% Similarly, under the concurrent setting, we have 
% $cost^1_{i,t} = O(N(t-1)^3)$ and $cost^2_{i,t} = O(1)$, which 
% imply a total complexity bound $O(n^2T^4)$. 



\paragraph{Total amount of compute and the type of resources used.}
Our experiments are run on an c5d.24xlarge instance on the AWS EC2 platform, with 96 cores and 192GB RAM. 
It takes roughly 20 minutes to complete a setting in Figure \ref{fig:simu_Gaussian} and 3 hours for Figure \ref{fig:simu_Binary}. 

==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/incremental_LMM.tex <==
\subsection{Incremental implementation for LMM}
\begin{align*}
    &\vthe | \mH \sim \mathcal{N}\Big(\Tilde{\Cov}(\vPhi^T \mV^{-1}\vR + \Cov_{\vthe}^{-1}\vmu_{\vthe}), \Tilde{\Cov}\Big),\\
    &\Tilde{\Cov} = (\vPhi^T \mV^{-1} \vPhi + \Cov_{\vthe})^{-1}, \mV = \sigma^2 \vI_n + \Cov_{\delta}
\end{align*}

% We can actually replace this paragraph with the formula about theta in the appendix. 
% Then it could be more consistent. And more efficient. More intuitions. 
% And save space
% No need about this computation trick (the same for Susan's)
% \begin{equation}
%     \vthe | \mH^e_{1:i} \sim \mathcal{N}\Big((\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\vPhi^T \mV^{-1}\vR, (\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\Big), \mV = \sigma^2 \vI + \Cov_{\delta}
% \end{equation}


% theta contain task i
% then again to task i? things will become weird

(iii) $\prob(\vthe | \mH)$ permits incremental computation, which follows from the relationship
\begin{align*}
&\prob(\vthe|\mH \cup \{(a, r, \vx_{i}, i)\}) \\
&\propto \prob(\vthe) \prob(\mH \cup \{(a, r, \vx_{i}, i)\}|\vthe) \\
&\propto \prob(\vthe) \int_{\vr^-_i} \prob(\vr^-_i|\vthe) \prob(\mH^-_i|\vr^-_i)  d\vr^-_i
\int_{\vr_i}  \prob(\vr_i|\vthe) \prob(\mH_i |\vr_i) \prob(\{(a, r, \vx_{i}, i)\}|\vr_i) d\vr \\
&\propto \prob(\vthe) \int_{\vr} \prob(\vr|\vthe) \prob(\mH|\vr)  d\vr
\frac{\int_{\vr_i}  \prob(\vr_i|\vthe) \prob(\mH_i |\vr_i) \prob(\{(a, r, \vx_{i}, i)\}|\vr_i) d\vr_i
}{\int_{\vr_i}  \prob(\vr_i|\vthe) \prob(\mH_i |\vr_i)  d\vr_i}\\
&\propto \prob(\vthe|\mH) 
\frac{\int_{\vr_i}  \prob(\vr_i|\vthe) \prob(\mH_i |\vr_i) \prob(\{(a, r, \vx_{i}, i)\}|\vr_i) d\vr_i
}{\int_{\vr_i}  \prob(\vr_i|\vthe) \prob(\mH_i |\vr_i)  d\vr_i}\\
&\propto \prob(\vthe|\mH) \prob(\{(a, r, \vx_{i}, i)\}|\vr_i) \\
&= \prob(\vthe) \prob(\mH^-_i|\vthe) \prob(\mH_i \cup \{(a, r, \vx_{i}, i)\}|\vthe) \\
&\propto \prob(\vthe|\mH) \prob(\{(a, r, \vx_{i}, i)\}|\vthe)
\end{align*}
, where $\{(a, r, \vx_{i}, i)\}$ contains some new tuples. 

% Q: if incremental, how to Sigma_delta?
% Q: inverse trick? or incremental?
% \begin{equation}
% \end{equation}
% \Cov_{\delta}: diagnoal
% incremental
% if every time, then the same; just 1. incremental 2. approximate


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/regret_baselines.tex <==

\subsection{Regrets of the baseline TS algorithms}
In this section, we first recap the baseline TS algorithms discussed in Section \ref{sec:Theory}, and then provide formal statements about their regret bounds. 
OSFA applies a single $TS\big( Q(\vr_i) \big)$ algorithm to all tasks, where $Q(\vr_i)$ is the marginal distribution of $\vr_i$, while individual-TS applies a separate $TS\big( Q(\vr_i) \big)$ algorithm to each tasks. 
For meta-TS, under the sequential setting, following \cite{kveton2021meta}, we apply $TS\big( \normal(\vmu_i,\Cov) \big)$ to the $i$-th task, where $\vmu_i$ is sampled from the posterior of $\Mean[\vr_i]$ based on accumulated data from the finished $i-1$ tasks. 
Finally, linear-TS assumes $\vr_i = \vPhi_{i}\vthe$, requires a prior over $\vthe$ and maintains a posterior over it. We have the following results. 

\begin{proposition}\label{prop:rate_OSFA_linear}
Under Assumptions $1 - 3$, 
when $K < min(N,T)$, 
the multi-task regrets of OSFA and linear-TS under the LMM over $N$ tasks with $T$ interactions per task are both bounded by $O\big(NT \big)$. 
\end{proposition}

\begin{proposition}\label{prop:rate_ind_meta}
Under Assumptions $1 - 3$, 
when $K < min(N,T)$, 
the multi-task regret of individual-TS and meta-TS under the LMM over $N$ tasks with $T$ interactions per task are both bounded by $O\big(N\sqrt{KT}\big)$. 
\end{proposition}



These two propositions can be proved as follows. 

\begin{proof}[Proof of Proposition \ref{prop:rate_OSFA_linear}]
According to Assumption \ref{asmp:linear_magnitute}, 
we note the regret from one interaction with task $i$ is always bounded by
$K max(\vr_i)$, the expectation of which over the task distribution is bounded by $C_2C_3$. 
Therefore, the total regrets over $N$ tasks with $T$ interactions per task are both bounded by $O\big(NT \big)$.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:rate_ind_meta}]
The Bayes regret for each task can be derived from the prior-independent regret bound for Gaussian bandits in the literature (e.g., \citep{bubeck2014prior}) as $O(\sqrt{(T-K)KlogT})$. 
Therefore, the regret accumulated over $N$ tasks can be bounded by $O(N\sqrt{(T-K)KlogT})$. 
% agrawal2013further
\end{proof}

We note that, similar with results in \cite{metapricing} and \cite{kveton2021meta}, it is non-trivial to obtain lower bounds on the multi-task regrets for these baseline TS algorithms, due to the lack of understanding of the behaviour of a TS algorithm with mis-specified priors. 
To our knowledge, the above bounds are the tightest in the existing literature. 
In contrast, with information-sharing and thanks to the prior alignment technique, MTTS can be shown to yield a lower regret in rate. 

% To provide more insights, we next show that, for OSFA and linear-TS, the proportion of tasks whose highest reward is significantly higher than the assumed highest reward is bounded from zero, due to model misspecification; while for meta-TS and individual-TS, the proportion of tasks whose true prior is significantly different from the assumed prior is bounded from zero, due to the fact that they fail to learn $\prob(\vr_i|\vx_i)$. 


% % \begin{proposition}\label{prop:proportion_OSFA_linear}
% % Under Assumptions $1 - 3$, 
% % when $K < min(N,T)$, 
% % the multi-task regrets of OSFA and linear-TS under the LMM over $N$ tasks with $T$ interactions per task are both bounded by $O\big(NT \big)$. 
% % \end{proposition}

% \begin{proposition}\label{prop:proportion_ind_meta}
% Suppose for task $i$, the prior for either meta-TS or individual-TS is $Q(\vr_i)$ with expectation $\Mean[Q(\vr_i)]$. 
% For any constant $c_7$, the event  $\Big\{ \norm{\Mean(\vr_i|\vx_i) - \Mean[Q(\vr_i)]} \ge c_7\Big\}$ holds with probability larger than XX. 
% % Under Assumptions $1 - 3$, 
% % when $K < min(N,T)$, 
% % the multi-task regret of individual-TS and meta-TS under the LMM over $N$ tasks with $T$ interactions per task are both bounded by $O\big(N\sqrt{KT}\big)$. 
% \end{proposition}
% \begin{proof}[Proof of Proposition \ref{prop:proportion_ind_meta}]
% Under Assumption \ref{asmp:cov_x}, $\sigma_{min}\big( \Mean(\vPhi_i^T\vPhi_i) \big) \ge Kc_1$. 
% Recall $\Mean(\vr_i|\vx_i) = \vPhi_i \vthe$
% \end{proof}


% ASMP: E(r_i) != E(r_i|), or equivalently, there is heterogeneity caused by the metadata!
% for individual, there is heterogeneity! 
% [in the main text!]

==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/review_Hierachical.tex <==
\section{Review of Statistical Concepts}\label{sec:review-LMM}
% Mixed Effect Models
In this section, we first review several classic statistical concepts, including the hierarchical models, random effect model, fixed effect model, and mixed effect model. 
They are all general concepts in statistics and have been integrated with different models, and we may focus on their  most related forms for ease of exposition. 
See \cite{fitzmaurice2008primer,wu2009mixed} for more detailed discussions. 
Next, we discuss their connection with our model  and baselines mentioned in the main text. 

\subsection{Statistical concepts}\label{sec:review_stat_LMM}
Consider a supervised learning problem, where we have $N$ subjects. 
For each subject $i$, we have $M_i$ measurements, denoted as $\{Y_{i,t}\}_{t=1}^{M_i}$. 
% Assume the $i$th subject also has a feature vector $\vx_i$. 
In a classic example, each subject corresponds to a hospital and each measurement corresponds to the outcome of a patient treated in one of these hospitals. 


A random effect model assumes the data of subject $i$ is generated from some distributions $f_i(\cdot;\vthe_i)$ parameterized by $\vthe_i$, and these coefficients are sampled from an upper-level distribution as $\vthe_i \sim \mathcal{P}$. 
The coefficients and the corresponding distribution are hence  treated as random variables, which enables us to characterize the heterogeneity between subjects. 
Therefore, this class of models are referred to as random effect models. 

In contrast, in a fixed effect model, for each measurement $Y_{i,t}$, we additionally have some independent variables $X_{i,t}$, and they are related through a regression model $Y_{i,t} = f(X_{i,t}; \vthe) + \epsilon_{it}$, which is parameterized by an unknown parameter $\vthe$. Here, $\epsilon_{it}$ is the error term. 
The coefficient $\vthe$ is fixed across subjects, and hence this class of models are referred to as fixed effect models. 
It is mainly used to characterize the common structure across subjects. 

A mixed effect model is a combination of both: it includes both fixed effect terms and random effect terms. The random intercept model $Y_{i,j} = f(X_{i,j}; \vthe) + \delta_{i} + \epsilon_{it}$ with $\delta_{i} \sim \mathcal{P}$ and the random coefficient model $Y_{i,j} = f(X_{i,j}; \vthe + \vthe_i) + \epsilon_{i,t}$ with $\vthe_i \sim \mathcal{P}$ are two examples. 

Finally, these three models are all special case of the following  hierarchical model (a.k.a. multilevel models): 
\begin{align*}
    \vthe_i &\sim g(Z_i;\vthe),\\
    Y_{i,t} &\sim f(X_{i,t}, \vthe_i), 
\end{align*}
where $Z_i$ contains some (optional) static features for each task $i$, 
the first layer describes the relationship between subjects and the second layer describes the relationship between measurements for the same subject. 
% hospital

% $\{(X_{i,t}, Y_{i,t})\}_{j=1}^{M_i}$. 
\subsection{Relationship with bandits}
The aforementioned statistical concepts are typically introduced for supervised learning. 
We can naturally extend them to the decision-making setup, and connect them with the bandit problem.
We first recall the equivalent definition of the stochastic multi-armed bandit problem that, in the $t$th interaction with task $i$,  the rewards for all arms are  generated by $\mathbf{R}_{i,t} \sim \mathcal{N}(\vr_i, \sigma^2 \vI)$, and after taking an action $A_{i,t}$, the $A_{i,t}$-th entry of $\mathbf{R}_{i,t}$ will be observed as $R_{i,t}$. 



The meta bandit assumes that each task instance $
\vr_i$ is sampled from some task prior distribution $\mathcal{P}_{\vr}$, and then the rewards are generated from $\vr_i$. 
Therefore, at a high-level, the underlying model can be regarded as a random effect model. 
As a concrete example, we consider the Gaussian bandit case in \citet{kveton2021meta}. 
Let mean rewards of task $i$ be $\vr_i = (r_{i,1}, \dots, r_{i,K})^T$. 
At each time point $t$, the rewards are  generated by $\mathbf{R}_{i,t} \sim \mathcal{N}(\vr_i, \sigma^2 \vI)$. 
We assume the task instances are sampled by $\vr_i = \vthe_i \sim N(\vmu, \sigma^2_0 \vI)$.  
It is easy to see this model is a random effect model. 

For contextual MAB, 
the reward $R_{t}$ are often related with the context $S_{t}$ and the action $A_{t}$ by a  model $R_{t} \sim f(S_{t}, A_{t}; \vthe)  + \boldsymbol{\epsilon}_{i,t}$ parameterized by $\vthe$.
In our multi-task MAB setting, to adapt these algorithms, we can similarly assume $\mathbf{R}_{i, t} =  f(S_{i, t}; \vthe) + \boldsymbol{\epsilon}_{i,t}$, where $S_{i, t} \equiv X_i$ for all $t$. % , A_{i, t}
It is straightforward to check that these two models are both special cases of the fixed effect model. 

Finally, by setting $Z_i = \vx_i$, $\vthe_i = \vr_i$, $Y_{i,t} = R_{i,t}$ and $X_{i,t} = A_{i,t}$, it is easy to see our model \eqref{eqn:hierachical_model} is a hierarchical model, with the other two models as special cases. 
In particular, the LMM in Section \ref{sec:LMM} is  a mixed effect model. 
% Finally, as discussed, our model can be regarded as their combinations, and hence is

% The reward of arm for task $i$ $N(\vthe_i, \sigma)$. 
% $y_{it} = X_{it}\vthe + \epsilon_{it}$. 
% $S_{it}$ ignores the repeated measurement nature. 


% $N$ subjects and their coefficients are sampled according to $\vthe_i \sim \mathcal{P}$. 


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/table_rate.tex <==
\setlength{\tabcolsep}{5pt}
\begin{table}[t]
    \centering
    % for different methods
\caption{A summary of the multi-task regret bounds under the LMM. All logarithmic terms are hidden.}
\begin{tabular}{cccccc}
\toprule
% \multirow{2}{*}{Models} & \multicolumn{3}{c}{Metric 1} & Metric 2\\
% \cmidrule{2-4} \cmidrule{5-5} \\
{} & {\name} (the proposed)             & meta-TS    & individual-TS      & linear-TS & OSFA  \\
\midrule
Model & $\vr_i \sim f(\vr_i|\vx_i;\vthe) $  & $\vr_i \sim f(\vr|\vthe)$ & $\vr_i \sim \prob(\vr)$   & $\vr_i = f(\vx_i;\vthe)$  & $\vr_i \equiv \vr \sim \prob(\vr)$  \\
MTR   & $\sqrt{Nd}\sqrt{TK} + NK$ & $N\sqrt{TK}$ & $N\sqrt{TK}$   & $NT$ & $NT$    \\
\bottomrule
% \vspace{-0.5cm}
\end{tabular}
\end{table}\label{tab:regret}


==> Metadata-based Multi-Task Bandits with Bayesian Hierarchical Models/technical_lemmas.tex <==
\subsection{Additional technical lemmas}
In this section, we collect several additional technical lemmas. 
% and prove them when necessary. 
We first recap a mathematical result: 
\begin{lemma}[Lemma 20 in \cite{metapricing}]\label{lemma:e_1_2a}
    For any number $a \in [0,1]$, it holds that $exp(a) \le 1 + 2a$. 
\end{lemma}


The following lemma will give a lower bound for the smallest eigenvalue of our design matrix. 
\begin{lemma}[Theorem 3.1 in \cite{tropp2011user}]\label{lemma:fisher_lower}
For a series of independent, positive semidefinite matrices $\{\vA_k\}$ with dimension $d$,  suppose $||\vA_k|| \le R$ almost surely, 
then for any $\delta \in [0,1)$, we have
\begin{align*}
    \prob \big[\sigma_{min} (\sum_k \vA_k) \le (1-\delta) \mu_{min} \big] \le d [\frac{e^{-\delta}}{(1-\delta)^{1-\delta}}]^{\mu_{min} / R}, 
\end{align*}
where $\mu_{min} = \sigma_{min} (\sum_k \Mean \vA_k)$.
\end{lemma}

The following lemma states a tail inequality for the $2$-norm of a Gaussian vector. 
\begin{lemma}[Based on Lemma A.4 in \cite{hsu2012tail}]\label{lemma:2_norm_Gaussian}
For a $d$-dimensional random vector $\vz \sim \normal(0, \vI)$ and any $\xi \in (0,1)$, we have 
\begin{align*}
    \prob[||\vz||^2 \le d + 2\sqrt{d (-log\xi)} + 2  (-log\xi)] \ge 1 - \xi, 
\end{align*}
which implies, for any matrix $\vA$ with appropriate dimensions, we have 
\begin{align*}
&\prob\Big[||\vA\vz|| \le ||\vA|| (\sqrt{d} + \sqrt{2  (-log\xi)}\Big]\\
&=\prob\Big[||\vA\vz|| \le ||\vA||(d + 2\sqrt{2}\sqrt{d (-log\xi)} + 2  (-log\xi))^{1/2}\Big]\\
&\ge    \prob\Big[||\vA\vz|| \le ||\vA||(d + 2\sqrt{d (-log\xi)} + 2  (-log\xi))^{1/2}\Big] 
\ge 1 - \xi. 
\end{align*}
Notice that $\vA \vz \sim \normal(0, \vA^T \vA)$. 
\end{lemma}


==> Proof.tex <==
\section{Main Proof}\label{sec:main_proof}
For ease of notations, 
without loss of generality, 
we first consider the sequential setting, and we assume the tasks arrive according to their indexes, i.e., the $i$th task will arrive earlier than the $(i+1)$th. 
Otherwise, we can always re-index these tasks. 
Since in our proof, all analysis for the regret in task $i$ only uses the data generated by task $i$ itself and the data generated in the alignment periods of task $1, \dots, i - 1$, it is easy to verify that our proof continues to hold in other settings. 
% [more complex notations can be formalized after the proof is finished]. 

We first clarify some notations. 
We vertically stack the feature matrix for all tasks to define $\vPhi_{1:N} = (\vPhi_1; \dots; \vPhi_N)$, 
and we  can similarly define $\vdelta_{1:N} = (\vdelta_1^T, \dots, \vdelta_N^T)^T$. 
At the end of the alignment period of task $i$, we define the following notations: 
% the value of $\vPhi$  as
first, we define $\vPhi^e_{1:i} = (\vPhi_1; \dots; \vPhi_i)$, 
and we can similarly define $\vdelta^e_{1:i}$ and $\vR^e_{1:i}$; 
% Next, we define $\vvarphi^e_i$ as a matrix of dimension $(iT - T + K) \times (NK)$, where the $j$th row is an indicator vector with value $1$ at the entry $(i(j) - 1)T + A_j$; 
moreover, we denote $\mV^e_{1:i} = (\sigma^2 + 1) \vI$ of dimension $iK \times iK$. 
% $\Cov_{\vR}^{e,i} = \vPhi \vPhi^T + \vvarphi \vvarphi^T + \sigma^2 \vI$; 
finally, let $\mH^e_{1:i}$ be the history of all alignment periods so far. 
To simplify the notations, when the context is clear, we may drop the subscript $1:i$ and superscript   $e$. 
Recall that we use $\vI$ to denote identity matrix, the  dimension of which can be inferred from the context. 


The modified {\name} algorithm is summarized in Algorithm \ref{alg:modified_MTS}, and formally described as follows. 
For any $i \in [N]$, 
during our first $K$ interactions with task $i$, 
we pull the $K$ arms in a round robin. 
After this period, we sample a value $\vr^e_i$ from  the posterior $\vr | \mH^e_{1:i}$ , and then we use $\mathcal{N}(\vr^e_i, \Cov)$ as the prior of $\vr_i$ to continue interact with task $i$ as a standard single-task TS algorithm. 
In another word, we run $\TSnormal{\vr^e_i}$ with the following $T - K$ interactions. 
Note that this sampling is equivalent to first sample a value $\vthe^e_i \sim \vthe|\mH^e_{1:i}$, and then define $\vr^e_i = \vPhi_i\vthe^e_i$. 
Besides, as discussed in \eqref{alternative_form}, this procedure is equivalent to only use the data generated in the alignment periods to estimate the prior.  
Finally, we define a modified oracle-TS which also has the alignment period. The main part of our proof will focus on derive the regret to the modified oracle-TS, since its regret to the vanilla oracle-TS can be easily bounded. 

\input{Algorithm/alg_modified_MTS}


We begin by stating several lemmas, which will be used in our main proof. 
The proof of these lemmas are deferred to Appendix \ref{sec:proof_lemmas}. 
Without loss of generality, throughout the proof, we assume $\Cov_{\vthe} = \vI$, $\vmu_{\vthe} = \vzero$, and $\Cov = \vI$ to simplify the notations.  
It is easy to check that, under the boundedness assumption \ref{asmp:cov_others}, for general values of these terms, the regret bound still hold. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We first establish the concentration of $\vthe^e_i$ around $\vthe$. 
It mainly utilizes the property of Bayesian LMM.
%$\hat{\vthe}^e_i$. 
% at the end of its alignment period, 
\begin{lemma}[Concentration of $\vthe^e_i$]\label{lemma:concentration_sampled_theta}
For any task $i \in [N]$, 
% let $\vthe^e_i \sim \prob[\vthe|\mH^e_{1:i}]$. 
for any $\xi \in (0, 1)$, we have 
\begin{align*}
    \prob \Big(||\vthe^e_i - \vthe|| 
    \ge 
     [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(2 \sqrt{d} + 2\sqrt{2} \sqrt{-log \xi}\big) 
     + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}\Big) 
    \le 2\xi + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
\end{align*}
\end{lemma}
% \hat{\vthe}^e_i

% \subsection{Proof of Theorem \ref{thm:meta_ours}}
% \begin{proof}
% 1
% \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% , which together with Lemma \ref{lemma:concentration_hat_theta} can control the concentration of the sampled value of $\vthe$. 

Based on Lemma \ref{lemma:concentration_sampled_theta}, we are now ready to prove that the estimated task-specific prior mean will be close to the true prior mean with high probability. 
For any task $i \in [N]$, let $\vr^e_i = \vPhi_i\vthe^e_i$ be the sampled prior mean. 
Recall that $\Mean(\vr_i | \vx_i) = \vPhi_i\vthe$ is the true prior mean for a task with metadata $\vx_i$. We have the following result. 
\begin{lemma}[Concentration of $\vr^e_i$]\label{lemma:concentration_sampled_prior}
For any task $i \in [N]$, 
we have 
\begin{eqnarray}\label{eqn:concentration_sampled_prior}
\begin{split}
    \prob \Big(||\vr^e_i - \vPhi_i\vthe|| \ge 
 2\sqrt{2} C_2 \sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2} 
 + C_3[i c_1'K + 1]^{-1}\Big) 
    \le \frac{2}{NT} + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
\end{split}
\end{eqnarray}
where $c_1' = c_1 \frac{(\sigma^2+1)^{-1}}{2}$. 
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To derive the multi-task regret of the modified {\name}, 
we aim to use a "prior alignment" proof technique inspired by \cite{metapricing}. 
Specifically, one central challenge to the analysis is that, no existing method can well characterize the behaviour of a TS algorithm when the input prior is different with the true task distribution, even when the difference is negligible \cite{kveton2021meta, metapricing, liu2016prior}. 
Therefore, 
even though with Lemma \ref{eqn:concentration_sampled_prior}, we can establish that the learned prior will be more and more close to the ground truth as the number of tasks increases, 
and it is intuitive to believe that the multi-task regret per task will decay, 
it is challenging to formally prove such a regret bound following standard regret analysis approaches. 

The key idea of the "prior alignment" proof technique is that, 
suppose after some interactions with a task $i$, the posterior of $\vr_i$ for the modified {\name} is equal to the posterior for the modified oracle-TS, then their behaviour in the following interactions with this task will be exactly the same (in the probabilistic sense), and hence the multi-task regret in the following interactions with this task will be exactly zero. 
Suppose such an event happens with high probability, and this probability approaches $1$ as $i$ grows, we can then  derive a bound for the multi-task regret. 
This idea forms the skeleton of our proof. 



Towards this end, we begin by defining the realized random errors for the modified {\name} in the alignment period for the $i$th task as 
$\veps^e_i = (\epsilon_{i,1}, \dots, \epsilon_{i,K})^T$, where $\epsilon_{i,a}$ is the realized error when we pull arm $a$ in the $a$th interaction with task $i$. 
We can similarly define $\veps^*_i$ for the modified oracle-TS algorithm. 
Note that both algorithms take the same actions in the alignment period, and we also have $\veps^e_i \sim \veps^*_i \sim \mathcal{N}(\vzero, \sigma^2 \vI)$. 
We first note the following lemma, which establishes the difference between the posterior with $\mathcal{N}(\vr^e_i, \Cov)$ as the prior and the posterior with $\mathcal{N}( \vPhi_i\vthe, \Cov)$ as the prior, after observing $\vR^e_i$. 

\begin{lemma}[Posterior Difference]\label{lemma:post_relationship}
For any task $i \in [N]$, let  
$\mathcal{N}(\Tilde{\vr}^e_i, \Tilde{\Cov}^e_i)$ and $\mathcal{N}(\Tilde{\vr}^*_i, \Tilde{\Cov}^*_i)$ be the posterior after observing $\vR^e_i$, with $\mathcal{N}(\vr^e_i, \Cov)$  and $\mathcal{N}( \vPhi_i\vthe, \Cov)$ as the prior,  respectively. 
We have 
\begin{align*}
    \Tilde{\vr}^e_i - \Tilde{\vr}^*_i &= (\Cov^{-1} + \sigma^{-2} \vI)^{-1} \big[\Cov^{-1} (\vr^e_i - \vPhi_i\vthe) + \sigma^{-2} (\veps^e_i - \veps^*_i) \big]; \\
    \Tilde{\Cov}^e_i &= \Tilde{\Cov}^*_i. 
\end{align*}
\end{lemma}
A direct implication of this lemma is that, suppose when $\vr^e_i$ is close to $\vPhi_i\vthe$, 
the right-hand side of the first equation is equal to $0$ with high probability. 
Then, the multi-task regret of the modified {\name} in the following interactions with task $i$ will be exactly $0$, since the posterior after the alignment period is the same. 
% The multi-task regret when the condition does not hold can be simply bounded by 
% $(T - K) max(\vPhi_i\vthe) \le (T-K) C_2C_3$, 
% \hl{can introduce a condition to control as smaller. But needed?}
% while the probability of this event will approach $0$ when $i \rightarrow \infty$. 
% Specifically, for the first part, we have the following result. 

Given Lemma \ref{lemma:post_relationship}, we are now ready to apply the "prior alignment" technique to derive a regret bound for each task. 
For every $i \in [N]$, we denote the stochastic cumulative rewards in the last $T - K$ interactions starting from a posterior $\Tilde{\vr}$ as $R_i(T-K; \Tilde{\vr})$. Denote the cumulative rewards following the optimal action by $R^*_i(T-K)$. % of the modified oracle-TS
We denote the Bayes regret of $\TSnormal{\Tilde{\vr}^e_i}$ in the last $T - K$ interactions with task $i$ by
% a TS algorithm starting from the posterior $\Tilde{\vr}^e_i$
% _{\vr_i, \Tilde{\vr}^e_i, \veps^e_i}
% \sum_{t = K + 1}^{T} \big(  \big)
\begin{align*}
    BR_i(T-K; \Tilde{\vr}^e_i) = 
    \Mean \Big[R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \Big]. 
    % ( r_{i, a_i^*} - r_{i,A_{i,t}}). 
\end{align*}
We can similarly define $BR_i(T-K; \Tilde{\vr}^*_i)$. 
Our proof relies on the following bound, which controls the Bayes regret of a TS algorithm in the last $T - K$ interactions starting from a different prior. 
% let the posteriors be 
% $\mathcal{N}(\Tilde{\vr}^e_i, \Tilde{\Cov}^e_i)$ and $\mathcal{N}(\Tilde{\vr}^*_i, \Tilde{\Cov}^*_i)$, respectively. 
\begin{lemma}\label{lemma:regret_wrong_prior}
For any task $i \in [N]$
% , for $c_3 = 4\sigma \sqrt{K} + 2\sigma \sqrt{log(NT)}$, 
% with $C_6'$ as an universal constant, 
% |\mJ_{\vr}\Big
we have 
\begin{equation}\label{eqn:bound_J_r}
    \begin{split}
    &\Mean_{\veps^e_i}  
    \Big[
    R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \Big]\\
    &\le     
        exp\big(
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
\sigma
\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}
+ \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
\big)BR_i(T-K; \Tilde{\vr}^*_i)
+ \frac{2C_2C_3}{N}
        % + (T-K)C_2C_3  exp\{-(\frac{c_3 - 4\sigma \sqrt{K}}{ 2\sigma})^2\}
        % \Big]. 
%     &\Mean_{\veps^e_i|}  
%     \Big[
%     R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) | \mJ_{\vr} \Big]\\
%     &\le     
%         exp\big(
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
% + \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
% \big)BR_i(T-K; \Tilde{\vr}^*_i)
%         + (T-K)C_2C_3  exp\{-(\frac{c_3 - 4\sigma \sqrt{K}}{ 2\sigma})^2\}
%         % \Big]. 
    \end{split}
\end{equation}
\end{lemma}

% \begin{proposition}[Bayes regret of the oracle-TS]
% 1
% \end{proposition}
% We aim to establish that, 
% conditional on $\mJ_{\vr}$, 
% with high probability, for $\veps^e_i$, we can find the corresponding $\veps^*_i(\veps^e_i)$, and hence make sure the multi-task regret in the following steps is zero. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We are now ready to combine these results and present our main proof. 

\begin{proof}[Proof of Theorem \ref{thm:meta_ours}]
We first define the event that the estimated task-specific prior mean is close to the true one as 
\begin{align*}
    \mJ_{\vr} \equiv \Big\{||\vr^e_i - \vPhi_i\vthe|| \le 
 2\sqrt{2} C_2 \sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2} 
 + C_3[i c_1'K + 1]^{-1}
 , \forall i \in [N] \Big\}. 
    % | \mH^e_{1:i}
\end{align*}
For simplicity, 
we denote 
$c_4(i) \equiv  2\sqrt{2} C_2 \sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2} 
 + C_3[i c_1'K + 1]^{-1}$.
We note that $c_4(i)$ is a shorthand instead of a constant. 


% If not, we can bounded the regret by the maximum times $1 / \sqrt{i}$. 
% Recall our results in Lemma \ref{lemma:concentration_sampled_prior}: 
% \begin{eqnarray*}
% \begin{split}
%     \prob \Big(||\vr^e_i - \vPhi_i\vthe|| \ge 
%     \sqrt{K} c_1K \big(
%      [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} 
%      &\big(8 \sqrt{d} + 4 \sqrt{-log \xi}\big) \\
%      &+ \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
%      \big)
%     | \mH^e_{1:i}\Big) 
%     \le 2\xi + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
% \end{split}
% \end{eqnarray*}
% \hl{choose: the 2nd term can be control and the conclusion for the first part can hold.}


% \begin{equation}\label{def:BR}
%   BR(N, \{T_i\}) =  \mathbb{E}_{\vx, \vr, \epsilon} \sum_{i = 1}^N
%     \sum_{t = K + 1}^{T} ( r_{i, a_i^*} - r_{i,A_{i,t}}), 
% \end{equation}


% \begin{equation}
%       MTR(N, \{T_i\}; \mathcal{O}) =  \mathbb{E}_{\vx, \vr, \epsilon} \sum_{i = 1}^N 
%     \sum_{t = K + 1}^{T} ( r_{i, A^\mathcal{O}_{i,t}} - r_{i, A_{i,t}}), 
%     % \mathcal{O}(i)
% \end{equation}

% \textbf{Regret bound when $\mJ_{\vr}$ holds.}
We first focus on bounding the regret when $\mJ_{\vr}$ holds. 
% Recall that $c_3 = 4\sigma \sqrt{K} + 2\sigma \sqrt{log(NT)}$.
% Conditional on the event that the prior is close, 
% we can apply the prior alignment technique. 
Define
\begin{equation*}
    \mathcal{S} =  \Big\{i \in [N]: 
    2c_4(i)\sqrt{log(NT)} \le 1/2, \frac{\sigma}{2}c_4(i) \le 2\sqrt{log(NT)} \Big\}. 
    % , \;\;
    % \frac{\sigma^2}{2} c_4(i)^2 \le 1/2, \frac{\sigma^2}{2} c_4(i) \le c_3\}. 
\end{equation*}
% Since $d = o(N)$, $l$ is well defined and 
We first focus on the case that $\mathcal{S}$ is not empty. 
% The case that $\mathcal{S}$ is empty will be discussed at the end. 
Define $l = min(\mathcal{S})$. 
We have $l = O(d log(NT)  + log^2(NT))$ and $\mathcal{S} = \{i \in [N]: i \ge l\}$. 
It also implies $\frac{\sigma^2}{2}c_4(i)^2 \le 2\sigma c_4(i)\sqrt{log(NT)}$ for $i \ge l$. 

% agrawal2013further
% \norm{\vr^e_i - \vPhi_i\vthe}

% Besides, conditional on $\mJ_{\vr}$, we have $\norm{ (\vr^e_i - \vPhi_i\vthe)} \le c_4(i)$, which implies $\frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2 \le c_3 \norm{\vr^e_i - \vPhi_i\vthe}$. 
% \hl{some conditions required here. 2nd inequality}
    % &BR_i(T-K; \Tilde{\vr}^e_i) 
    % &\Mean_{\veps^e_i}  \sum_{t = K + 1}^{T} 
    % \Big[
    % (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i)) |\mJ_{\vr}\Big]\\

Therefore, 
for any $i \ge l$, % setting $\lambda = c_3$ in
by Lemma \ref{lemma:regret_wrong_prior}, we have
\begin{equation}\label{eqn:bound_J_r_large_i}
    \begin{split}
    &\Mean \Big[R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) | \Tilde{\vr}^e_i, \vPhi_i, \mathcal{J}_{\vr} \Big] \\
&\le     
exp\big(
\sigma
\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
+ \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
\big)BR_i(T-K; \Tilde{\vr}^*_i)
+ 2\frac{C_2 C_3}{N} \\
&\le     
exp\big(
% c_3 c_4(i)
c_4(i)\sigma\sqrt{2log(NT)}
+ \frac{\sigma^2}{2}c_4(i)^2
\big) BR_i(T-K; \Tilde{\vr}^*_i)
+ 2\frac{C_2 C_3}{N} \\
&\le 
\big(1 + 
8\sigma c_4(i)\sqrt{log(NT)}
\big)BR_i(T-K; \Tilde{\vr}^*_i)
        + 2\frac{C_2 C_3}{N} , 
\end{split}
\end{equation}
where the 
second inequality follows from the fact that $\norm{\vr^e_i - \vPhi_i\vthe} \le c_4(i)$ conditional on $\mJ_{\vr}$, and the last inequality is due to Lemma \ref{lemma:e_1_2a}. 
% (T-K)C_2C_3  exp\{-(\frac{c_3 - 4\sigma \sqrt{K}}{ 2\sigma})^2\}

% where the first term is due to $exp\big(
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
% + \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
% \big) \le exp\big(
% c_3 c_4(i)
% + \frac{\sigma^2}{2}c_4(i)^2
% \big)$

% better to refer to lemma 6, should be 
% $<=1+2(c3c4(i)+1/2)=2+2c3c4(i);
% c3c4(i)<=1/2 -> 1+4c3c4(i)<=2+2c3c4(i)$
% is it a problem?

% For any number $a \in [0,1]$, it holds that $exp(a) \le 1 + 2a$. 

% russo2014learning
For $i < l$, similar with Lemma 11 in \cite{metapricing}, we note that the Bayes regret for each task can be derived from the prior-independent regret bound for Gaussian bandits in the literature (e.g., \citep{bubeck2014prior}) as % agrawal2013further
\begin{align}\label{eqn:bound_J_r_small_i}
   \Mean \Big[R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) | \Tilde{\vr}^e_i, \vPhi_i, \mathcal{J}_{\vr} \Big] \le C_5 \sqrt{(T-K)KlogT}, 
\end{align}
where $C_5$ is a positive constant. 

% Recall the event 
% \begin{align*}
%     \mJ_{\vr} \equiv \{||\vr^e_i - \vPhi_i\vthe|| \ge 
%     \sqrt{K} c_1K \big(
%      [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} 
%      \big(8 \sqrt{d} + 4 \sqrt{-log \xi}\big) 
%      + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
%      \big) 
%      , \forall i \in [N]\}, 
%     % | \mH^e_{1:i}
% \end{align*}


% Combining \eqref{eqn:first_part_full}, \eqref{eqn:first_part_coef}, and \eqref{eqn:bound_part2}, we can obtain 
% \begin{equation}\label{eqn:bound_J_r}
%     \begin{split}
%     &\Mean_{\veps^e_i}  \sum_{t = K + 1}^{T} 
%     \Big[
%     (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i)) |\mJ_{\vr}\Big]\\
%     &\le     
%         (1 + 4c_3 c_4(i)) 
%         BR_i(T-K; \Tilde{\vr}^*_i) 
%         + (T-K) C_2C_3 exp\{-[(c_3 - 4\sigma \sqrt{K}) /  2\sigma]^2\}
%     \end{split}
% \end{equation}

% similar with the derivations for \eqref{eqn:bound_part2}, we can simply bound the multi-task regret for one task by 
% $(T-K) C_2C_3$. 
% Besides, 
% \textbf{Regret bound when $\neg \mJ_{\vr}$ holds.}
When $\neg \mJ_{\vr}$ holds, for $i \in [N]$, we define 
\begin{align*}
    \mJ_{\vr, i} \equiv \Big\{||\vr^e_i - \vPhi_i\vthe|| <
 2\sqrt{2} C_2 \sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2} 
 + C_3 [i c_1'K + 1]^{-1}\Big\}. 
    % | \mH^e_{1:i}
\end{align*}
From Lemma \ref{lemma:concentration_sampled_prior}, we know 
$\prob[\neg \mJ_{\vr, i}] \le 2\frac{1}{NT}+ d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}$. 
% we can apply a union bound over $i \in [N]$ to \eqref{eqn:concentration_sampled_prior} in to yield 
Then, by similar arguments with \eqref{eqn:bound_J_r_small_i}, we have 
\begin{equation}\label{eqn:bound_not_J_r}
    \begin{split}
    %     &\Mean \Big[\sum_{i=1}^N \big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \big) | \Tilde{\vr}^e_i, \vPhi_i, \neg \mathcal{J}_{\vr} \Big] \times
    % \prob[\mJ_{\vr}] \\
        &\sum_{i=1}^N \Mean \Big[ \big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \big) | \Tilde{\vr}^e_i, \vPhi_i, \neg \mathcal{J}_{\vr} \Big] \times
    \prob[\neg \mJ_{\vr}] \\
        &\le \sum_{i=1}^N \Mean \Big[ \big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \big) | \Tilde{\vr}^e_i, \vPhi_i, \neg \mathcal{J}_{\vr} \Big] \times
    \prob[\neg \mJ_{\vr, i}] \\
&\le \sum_{i=1}^N C_5 \sqrt{(T-K)KlogT} \times \prob[\neg \mJ_{\vr, i}]\\
&\le  C_5' d \sqrt{(T-K)KlogT}, 
    \end{split}
\end{equation}
where $C_5'$ is an universal constant. 


% \begin{align}
%     \Mean_{\veps^e_i}  \sum_{t = K + 1}^{T} 
%     \Big[
%     (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i)) |\neg \mJ_{\vr}\Big] \times
%     \prob[\neg \mJ_{\vr}] 
%         \le N(T-K) C_2C_3 [2\frac{1}{NT}+ d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}]. 
% \end{align}



% \textbf{Putting everything together.}
Finally, we note the following relationship
\begin{equation}\label{eqn:decomposition}
    \begin{split}
    &\Mean_{\veps^e_i}  
    \Big(R_i(T-K; \Tilde{\vr}^*_i) - R_i(T-K; \Tilde{\vr}^e_i)\Big)\\
    &=
    \Mean_{\veps^e_i}  
    \Big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i)\Big)
    - \Mean_{\veps^e_i}  
    \Big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^*_i)\Big)
    \\
    &=
    \Mean_{\veps^e_i}  
    \Big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) |\mJ_{\vr}\Big) \times
    \prob[\mJ_{\vr}] \\
    &+
    \Mean_{\veps^e_i}  
    \Big(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) |\neg \mJ_{\vr} \Big) \times
    \prob[\neg \mJ_{\vr}] 
    - BR_i(T-K; \Tilde{\vr}^*_i) %\\
    % &\le
    % 4c_3 c_4(i)
    % BR_i(T-K; \Tilde{\vr}^*_i) 
    % + (T-K) C_2C_3 exp\{-[(c_3 - 4\sigma \sqrt{K}) /  2\sigma]^2\}\\
    % &+
    % N(T-K) C_2C_3 [2\frac{1}{NT}+ d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}] \alignlable{eqn:bound_each_i}.
    \end{split}
\end{equation}



% \eqref{eqn:bound_J_r} and  \eqref{eqn:bound_not_J_r} together imply a bound on the multi-task regret as 
Denote the Bayes regret of the modified oracle-TS as $BR'(N, \{T_i\})$. 
Based on \eqref{eqn:bound_J_r_large_i}, \eqref{eqn:bound_J_r_small_i}, and \eqref{eqn:bound_not_J_r}, we sum \eqref{eqn:decomposition} from $i = 1$ to $N$ to yield the regret of the modified {\name} to the modified oracle-TS as 
\begin{align*}
    %&MTR(N, \{T_i\}; \mO')\\
    &BR(N, \{T_i\}) - BR'(N, \{T_i\})\\
    % =  \mathbb{E}_{\vx, \vr, \epsilon} \sum_{i = 1}^N 
    % \sum_{t = K + 1}^{T} ( r_{i, A^\mathcal{O}_{i,t}} - r_{i, A_{i,t}}), 
    &\le \sum_{i=l}^N \Big[
        8\sigma c_4(i)\sqrt{log(NT)}  BR_i(T-K; \Tilde{\vr}^*_i)
        + 2\frac{C_2 C_3}{N} 
    \Big]\\
    &\;\; + C_5 l \sqrt{(T-K)KlogT} + C_5'd \sqrt{(T-K)KlogT}\\
    &\le \sum_{i=l}^N C_4'\Big[
        \sqrt{log(NT)} (\sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2} 
        + C_3[i c_1'K + 1]^{-1}
        ) BR_i(T-K; \Tilde{\vr}^*_i)\\
    &\;\; 
    % (T-K)C_2C_3  exp\{-log(NT)\}
    \Big]+ O(1)
     + C_6 (l+d) \sqrt{(T-K)KlogT} \\
    &\le \sum_{i=l}^N C_4'\Big[
        \sqrt{log(NT)} (\sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-1/2}
        + C_3[i c_1'K + 1]^{-1}
        ) BR_i(T-K; \Tilde{\vr}^*_i)\Big] + O(1)\\
    &+ C'_6 (d log(NT) + log^2(NT)) \sqrt{(T-K)KlogT}  \\
    &= O(\sqrt{log(NT)} (\sqrt{d} + \sqrt{log(NT)} \big) \sqrt{N} \sqrt{(T-K)K logT}
    + (log(NT) d + log^2(NT)) \sqrt{(T-K)KlogT}), 
\end{align*}
where $C_4'$, $C_6$, and $C'_6$ some universal constants, 
the last inequality is due to $l = O(dlog(NT)  + log^2(NT))$, 
and the last equality is due to $BR_i(T-K; \Tilde{\vr}^*_i) = O(\sqrt{(T-K)K logT})$ according to Proposition 2 in \cite{russo2014learning}. 
In the last equality, we also utilize the fact that $\sum_{i=l}^{N}1/\sqrt{i} = O(\sqrt{N})$, and $\sum_{i=l}^{N}1/{i} = O(log(N))$. 
% results on 
% Gaussian bandits in the literature \cite{russo2014learning}. 
%  $l = O(N)$, 
Recall that, until now,  we consider the case that $\mathcal{S}$ is not empty. 
When $\mathcal{S}$ is empty, we have $N = O(log^2(NT))$, and then 
we can follow the arguments of \eqref{eqn:bound_J_r_small_i} to bound the regret when $\mJ_{\vr}$  holds as 
$O(log^2(NT)\sqrt{(T-K)KlogT})$, and we can similarly obtain the above bound. 


Finally, we bound the regret of the modified oracle-TS  to the vanilla oracle-TS. 
%  can be bounded by $O(NK)$
We denote the action that the modified oracle-TS takes at the $t$-th interaction with task $i$ as $A^{\Tilde{\mathcal{O}}}_{i,t}$. 
This multi-task regret of the modified oracle-TS is then equal to 
\begin{align*}
\mathbb{E}_{\vx, \vr, \epsilon} 
\sum_{t = 1}^{T} ( 
r_{i,A^{\mathcal{O}}_{i,t}} - 
r_{i, A^{\Tilde{\mathcal{O}}}_{i,t}}
)
&= \mathbb{E}_{\vx, \vr, \epsilon} 
\Big[
\big(
\sum_{t = 1}^{K} r_{i, A^{\mathcal{O}}_{i,t}} - 
\sum_{t = 1}^{K} r_{i, A^{\Tilde{\mathcal{O}}}_{i,t}}
\big)
+ 
\big(
\sum_{t = T - K + 1}^{T} r_{i, A^{\mathcal{O}}_{i,t}} - 
\sum_{t = T - K + 1}^{T} r_{i, A^{\Tilde{\mathcal{O}}}_{i,t}}
\big)
\Big]\\
&= O(K). 
\end{align*}
Here, for the first term, 
We note the regret from $K$ interactions with task $i$ is always bounded by 
$K max(\vr_i)$, the expectation of which over the task distribution is bounded by $KC_2C_3$. 
The second part is bounded by $0$, since the two algorithms share the same prior and the modified oracle-TS essentially have $K$ more data points with no confounding variables \cite{ye2020combining}. 

% For each $i$, the multi-task regret of the modified oracle-TS in the alignment period can be bounded by $KC_2C_3$. 
% For the remaining $T-K$ interactions, we note that $\vr_i | \vPhi_i \sim \normal(\vPhi_i\vthe, \Cov)$ and $\vR^e_i |\vr_i \sim \normal(\vr_i, \sigma^2 \vI)$. 
% Denote the corresponding density function as $h_1(\vr_i|\vPhi_i)$ and $h_2(\vR^e_i|\vr_i)$, respectively. 
% Write $h_3(\vr_i| \vR^e_i, \vPhi_i)$ as the posterior of $\vr_i$ after observing $\vR^e_i$. 
% Therefore, 
% conditional on $\vPhi_i$, 
% we can simply regard the behaviour of the modified oracle-TS in the remaining $T-K$ interactions as an vanilla oracle-TS algorithm with prior $\int h_3(\vr_i| \vR^e_i, \vPhi_i) h_2(\vR^e_i|\vr'_i) h_1(\vr'_i|\vPhi_i) d \vr'_i d \vR^e_i$, and hence bound 

Putting everything together, 
we conclude with  
\begin{align*}
    &MTR(N, \{T_i\})\\
    &= BR(N, \{T_i\}) - BR'(N, \{T_i\}) + N \times O(K)\\
    &= O(\sqrt{log(NT)} (\sqrt{d} + \sqrt{log(NT)} \big) \sqrt{N} \sqrt{(T-K)K logT}
    + (log(NT) d + log^2(NT)) \sqrt{(T-K)KlogT} + NK)\\
    &= O(\sqrt{log(NT)} (\sqrt{d} + \sqrt{log(NT)} \big) \sqrt{N} \sqrt{TK logT} 
    + log^2(NT) \sqrt{(T-K)KlogT}
    + NK)\\
    &= \TO(  \sqrt{N} \sqrt{dTK} + NK).
\end{align*}



\end{proof}



==> Proof_lemmas.tex <==
\section{Proof of Lemmas and Propositions}\label{sec:proof_lemmas}
\subsection{Proof of Lemma \ref{lemma:concentration_sampled_theta}}
\begin{proof}
Throughout the proof, recall the fact that $\vthe$ is a fixed vector instead of a random vector, and we only adopt the Bayesian approach to adapt the TS framework. 
We first note that, 
according to the results on Bayesian LMM (page 361, \cite{wu2009mixed}), we have the following expression for the posterior of $\vthe$: 
\begin{equation}\label{eqn:theta_posterior}
    \vthe | \mH^e_{1:i} \sim \mathcal{N}\Big((\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\vPhi^T \mV^{-1}\vR, (\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\Big). 
\end{equation}
Recall that, when the context is clear, we may drop the subscript $1:i$ and superscript $e$. 
% We will first show that, with high probability, the sample task-specific prior is close to the true prior. 
% [as long as they are bounded. Introduce a condition. K and p will be naturally involved?]
Let $\hat{\vthe}^e_i = (\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\vPhi^T \mV^{-1}\vR$ be the maximum a posterior estimator of $\vthe$, which implies 
\begin{equation}\label{eqn:theta_hat_diff_distribution}
    \hat{\vthe}^e_i - \vthe | \vPhi \sim \mathcal{N}\Big( -[(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1} \vthe, [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1} - [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-2}
    \Big). 
\end{equation}




% \begin{lemma}\label{lemma:concentration_hat_theta}
% For any task $i \in [N]$, at the end of its alignment period, for any $\xi \in (0, 1)$, we have 
% \begin{align*}
%     \prob \big(||\hat{\vthe}^e_i - \vthe|| \ge 
%      [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(4 \sqrt{d} + 2 \sqrt{-log \xi}\big) + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
%     | \mH^e_{1:i}\big) \le \xi + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
% \end{align*}
% \end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Let $\vthe^e_i \sim \vthe|\mH^e_{1:i}$ be the sample from the posterior. 

\paragraph{Concentration of $\hat{\vthe}^e_i$ around $\vthe$.}
To derive the concentration of $\hat{\vthe}^e_i - \vthe$ around $\vzero$, 
we analyze the concentration of its mean around $\vzero$ and the magnitude of its variance separately. 
We begin by defining the event
\begin{equation*}
    \mJ_{\vPhi} \equiv  \big\{  \sigma_{\min}[\vPhi^T\vPhi] \ge 
    % [\frac{2||\vthe||}{\xi} - 1] (\sigma^2+1) 
    \frac{1}{2} i c_1K
    \big\}, 
\end{equation*}
% Define $$. 
% but C_1 can depend on d. 
According to Lemma \ref{lemma:fisher_lower}, based on  Assumption \ref{asmp:cov_x}, 
we have 
\begin{align}\label{eqn:prob_J_phi}
    \prob(\mJ_{\vPhi})
    % &= \prob \Big[  \sigma_{\min}[\frac{1}{i} \sum_{j=1}^i \vPhi_i^T\vPhi_i] \ge \frac{2||\vthe|| / \xi - 1}{i}(\sigma^2+1)\Big]\\
    &\ge 1 - d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
    % 1 - d\Big[ \frac{e^{-c}}{(1-c)^{1-c}} \Big]^{ic_1K}, 
\end{align}
% where $c = 1 -  \frac{2||\vthe|| / \xi - 1 }{ i c_1K}(\sigma^2 + 1)$. 

For the mean part of \eqref{eqn:theta_hat_diff_distribution}, based on the property of matrix  operator norm, we can derive 
\begin{align*}
    \mJ_{\vPhi} 
    &=  \big\{  \sigma_{\min}[\vPhi^T\vPhi] \ge \frac{1}{2} i c_1K \big\}\\
    % \{ (\sigma^2+1)^{-1} \sigma_{\min}[\vPhi^T\vPhi] + 1 \ge \frac{2||\vthe||}{\xi}\}\\
    &= \{ \sigma_{\min}[(\sigma^2+1)^{-1}\vPhi^T\vPhi + \vI] \ge \frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1 \}\\
    &= \{ \norm[\big]{[(\sigma^2+1)^{-1}\vPhi^T\vPhi + \vI]^{-1}} \le \frac{1}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1} 
    \}\\
    &\subseteq \{\norm[\big]{[(\sigma^2+1)^{-1}\vPhi^T\vPhi + \vI]^{-1}(-\vthe)} \le \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
    \}, 
    % \prob \Big[  \sigma_{\min}[\frac{1}{i} \sum_{j=1}^i \vPhi_i^T\vPhi_i] \ge \frac{2||\vthe|| / \xi - 1}{(\sigma^2+1)^{-1}i} \Big]
\end{align*}
where the third equality is due to $\sigma_{min} (\mathbf{A}) = ||\mathbf{A}^{-1}||$ for any invertible matrix $\mathbf{A}$. 
This relationship implies 
\begin{align*}
    \Mean [\hat{\vthe}^e_i - \vthe | \mJ_{\vPhi}] \le \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}. 
\end{align*}
% \begin{align*}
%     \prob \Big\{\Mean [\hat{\vthe}^e_i - \vthe | \mJ_{\vPhi}] \le \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1} \Big\} \ge 1 - d (\frac{e}{2})^{-\frac{c_1K}{2C_1}i}.     
% \end{align*}


For the variance part of \eqref{eqn:theta_hat_diff_distribution}, define a random vector $\vz \sim \normal(\vzero, [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1} - [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-2})$. 
According to the tail inequality for the Euclidean norm of Gaussian random vectors (see Lemma \ref{lemma:2_norm_Gaussian}), 
for any $\xi \in (0, 1)$, 
we have 
\begin{align}\label{eqn:normal_tail}
    \prob \Big[\norm{\vz} \le \sigma_{\vz} \sqrt{d} + \sigma_{\vz} \sqrt{2(-log \xi)} |\vPhi \Big]  \ge 1 - \xi, 
\end{align}
where $\sigma_{\vz} = \norm{[(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1} - [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-2}}^{1/2}$. 
% Set $4\sigma_{\vz} \sqrt{d} + 2\sigma_{\vz} \sqrt{-log \xi} = \xi / 2$, we have 
% $\xi = exp\{-[(\xi / 2 - 4\sigma_{\vz} \sqrt{d}) / (2\sigma_{\vz})]^2\}$. 
% Therefore, we obtained that 
% \begin{align}\label{eqn:normal_tail}
%     \prob \Big[\norm{\vz} \le \xi / 2 \Big]  \ge 1 - exp\{-\big[
%     \frac{\xi}{4\sigma_{\vz}} - 2 \sqrt{d} \big]^2\}. 
% \end{align}
% % monotone: []^2 >= xxx -> prob >= ...
We then focus on control $\sigma_{\vz}$:  
\begin{align*}
\sigma_{\vz}
&= \norm{
[(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1} \{ \vI - [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1}
\}}^{1/2} \\
&\le \Big\{ 
\norm{[(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1}} \times
\norm{\vI - [(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1}}
\Big\}^{1/2}\\
&\le 
\norm{[(\sigma^2 + 1)^{-1}\vPhi^T\vPhi + \vI]^{-1}}^{1/2}
% \\
% &= 
% [(\sigma^2+1)^{-1} \sigma_{\min}[\vPhi^T\vPhi] + 1]^{-1/2}
\end{align*}
where the first inequality follows from the sub-multiplicative property of the matrix operator norm, and the second  follows from the fact that $\norm{\vI - (\vI + \vA)^{-1}} \le 1$ for any symmetric matrix $\vA$. 


Therefore, conditional on $ \mJ_{\vPhi} $, we have 
$\sigma_{\vz} \le [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2}$, 
which together with \eqref{eqn:normal_tail} implies 
\begin{align*}
    \prob \Big[\norm{\vz} \le  [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big( \sqrt{d} + \sqrt{2} \sqrt{-log \xi}\big) | \mJ_{\vPhi} \Big] \ge 1 - \xi. 
\end{align*}

Note that, based on the triangle inequality, we have 
$||\hat{\vthe}^e_i - \vthe|| \le ||\Mean(\hat{\vthe}^e_i| \mJ_{\vPhi}) - \vthe|| + ||\hat{\vthe}^e_i - \Mean(\hat{\vthe}^e_i| \mJ_{\vPhi})|| $. 
Combining the two parts, we conclude with 
\begin{align}\label{eqn:concentration_mean}
    \prob \big(||\hat{\vthe}^e_i - \vthe|| \ge 
     [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(\sqrt{d} + \sqrt{2} \sqrt{-log \xi}\big) + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
    | \mJ_{\vPhi}\big) \le \xi. 
\end{align}

%  \mH^e_{1:i}
\paragraph{Concentration of $\vthe^e_i$ around $\hat{\vthe}^e_i$.}
Note that 
\begin{equation}
    \vthe^e_i - \hat{\vthe}^e_i |\vPhi \sim \mathcal{N}\Big(\vzero, (\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\Big). 
\end{equation}

% According to the tail inequality for the Euclidean norm of Gaussian random vectors \citep{hsu2012tail}, 
% for any $\delta \in (0, 1)$, 
% we have 
% \begin{align}
%             \prob \Big[\norm{\vz} \le 4\sigma_{\vz} \sqrt{d} + 2\sigma_{\vz} \sqrt{-log \delta} \Big]  \ge 1 - \delta,
% \end{align}
% where $\sigma_{\vz} = \norm{((\sigma^2 + 1)^{-1} \vPhi^T\vPhi + \vI)^{-1}}^{1/2}$. 

We begin by defining a random vector $\vz \sim \normal(\vzero, ((\sigma^2 + 1)^{-1} \vPhi^T\vPhi + \vI)^{-1})$. 
By similar arguments with that for the variance part in \eqref{eqn:theta_hat_diff_distribution}, we get
\begin{align*}
    \prob \Big[\norm{\vz} \le  [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(\sqrt{d} + \sqrt{2} \sqrt{-log \xi}\big) | \mJ_{\vPhi} \Big] \ge 1 - \xi, 
\end{align*}
which implies 
\begin{align}\label{eqn:res_sampled_mean_distance}
    \prob \Big[\norm{\vthe^e_i - \hat{\vthe}^e_i} \le  [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(\sqrt{d} + \sqrt{2} \sqrt{-log \xi}\big) | \mJ_{\vPhi} \Big] \ge 1 - \xi. 
    % \mH^e_{1:i}
\end{align}

Note that, based on the triangle inequality, we have $||\vthe^e_i - \vthe|| \le ||\vthe^e_i - \hat{\vthe}^e_i|| + ||\hat{\vthe}^e_i - \vthe||$. 
Therefore, applying an union bound to \eqref{eqn:concentration_mean} and \eqref{eqn:res_sampled_mean_distance} yields that
\begin{align*}
    \prob \Big[\norm{\vthe^e_i - \vthe} \le  [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(2 \sqrt{d} + 2\sqrt{2} \sqrt{-log \xi}\big)      + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1} | \mJ_{\vPhi} \Big] \ge 1 - 2\xi. 
    % \mH^e_{1:i}
\end{align*}
This result, together with \eqref{eqn:prob_J_phi}, implies that 
\begin{align*}
    \prob \big(||\vthe^e_i - \vthe|| \ge 
     [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} \big(2 \sqrt{d} + 2\sqrt{2} \sqrt{-log \xi}\big) 
     + \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
    \big) \le 2\xi + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
\end{align*}
    % | \mH^e_{1:i}
    
\end{proof}

\subsection{Proof of Lemma \ref{lemma:concentration_sampled_prior}}
\begin{proof}
% The second term is bounded w.h.p

The first term needs assumptions
\begin{align*}
    ||\vr^e_i - \vPhi_i\vthe ||
    &= ||\vPhi_i\vthe^e_i - \vPhi_i\vthe||\\
    &\le ||\vPhi_i|| \times ||\vthe^e_i - \vthe||\\
    &\le \sqrt{K} C_2 ||\vthe^e_i - \vthe||, 
\end{align*}
where the last inequality is based on  Assumption \ref{asmp:linear_magnitute}. 
Recall the results in Lemma \ref{lemma:concentration_sampled_theta} that
% based on the triangle inequality, we get that 
\begin{eqnarray}
\begin{split}
    \prob \Big(||\vr^e_i - \vPhi_i\vthe|| \ge 
    \sqrt{K} C_2 \big(
     [\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1]^{-1/2} 
     &\big(2 \sqrt{d} + 2\sqrt{2} \sqrt{-log \xi}\big) \\
     &+ \frac{\norm{\vthe}}{\frac{(\sigma^2+1)^{-1}}{2} i c_1K + 1}
     \big)
    \Big) 
    \le 2\xi + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
\end{split}
\end{eqnarray}

% It can be seen that, $c_4(i)$ will decays to $0$, roughly at a rate of $O(1 / \sqrt{i})$. 
% More precisely, 
% Recall that  $c_1K = c_1 K \log_{e/2}(NTd)$, 
Under Assumption \ref{asmp:linear_magnitute}, 
with $c_1' = c_1 \frac{(\sigma^2+1)^{-1}}{2}$, 
by setting $\xi = \frac{1}{NT}$, 
we can derive
\begin{eqnarray}
\begin{split}
    \prob \Big(||\vr^e_i - \vPhi_i\vthe|| \ge 
 2\sqrt{2} C_2 \sqrt{K} \big(\sqrt{d} + \sqrt{log(NT)} \big) [i c_1'K + 1]^{-\frac{1}{2}} 
 + C_3[i c_1'K + 1]^{-1}
\Big) 
    \le \frac{2}{NT} + d (\frac{e}{2})^{-\frac{c_1}{2C_1}i}. 
\end{split}
\end{eqnarray}

\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Lemma \ref{lemma:post_relationship}}
\begin{proof}
The relationship follows from the posterior updating rule for multivariate Gaussian. 
Specifically, we have 
\begin{align*}
    \Tilde{\vr}^e_i &= (\Cov^{-1} + \sigma^{-2} \vI)^{-1} (\Cov^{-1}\vr^e_i + \sigma^{-2} \vR^e_i);\\
    \Tilde{\Cov}^e_i &=  (\Cov^{-1} + \sigma^{-2} \vI)^{-1};\\
    \Tilde{\vr}^*_i &= (\Cov^{-1} + \sigma^{-2} \vI)^{-1} (\Cov^{-1}\vPhi_i\vthe + \sigma^{-2} \vR^*_i);\\
     \Tilde{\Cov}^*_i &=  (\Cov^{-1} + \sigma^{-2} \vI)^{-1}, 
\end{align*}
which implies
\begin{align*}
    \Tilde{\vr}^e_i - \Tilde{\vr}^*_i &= 
    (\Cov^{-1} + \sigma^{-2} \vI)^{-1} \big[\Cov^{-1} (\vr^e_i - \vPhi_i\vthe) + \sigma^{-2} (\veps^e_i - \veps^*_i) \big]\\
    % (\vI + \sigma^{-2} \Cov)^{-1}  
    % (\vr^e_i - \vPhi_i\vthe)\\
    \Tilde{\Cov}^e_i &= \Tilde{\Cov}^*_i. 
\end{align*}
\end{proof}


\subsection{Proof of Lemma \ref{lemma:regret_wrong_prior}}
\begin{proof}
Recall that 
\begin{align*}
    \Tilde{\vr}^e_i - \Tilde{\vr}^*_i &= (\Cov^{-1} + \sigma^{-2} \vI)^{-1} \big[\Cov^{-1} (\vr^e_i - \vPhi_i\vthe) + \sigma^{-2} (\veps^e_i - \veps^*_i) \big], 
\end{align*}
which implies $\Tilde{\vr}^e_i = \Tilde{\vr}^*_i$ when $\veps^*_i = \veps^e_i + \sigma^2 \Cov^{-1} (\vr^e_i - \vPhi_i\vthe)$. 
% With slight abuse of notations, w
We denote 
\begin{align}\label{eqn:one2one}
    h_i(\veps^e_i) \equiv \veps^e_i + \sigma^2 \Cov^{-1} (\vr^e_i - \vPhi_i\vthe), 
\end{align}
which will then allow us to apply a change-of-variable trick. 
We note this is an one-to-one mapping. 
Besides, due to the round robin nature, we have $\veps^*_i \sim \veps^e_i \sim \mathcal{N}(\vzero, \sigma^2 \vI)$. 

Define $\mJ_{\veps, \vr, i}$ as the event $\{|(\vr^e_i - \vPhi_i\vthe)^T \veps^e_{i}| \le \sigma\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)} \}$. 
We begin by expressing $BR_i(T-K; \Tilde{\vr}^e_i)$ as a function of $BR_i(T-K; \Tilde{\vr}^*_i)$ via a change of measure. 
% | \mJ_{\vr}
% We note that 
\begin{align*}
    % &BR_i(T-K; \Tilde{\vr}^e_i) \\
    % &= 
    % \vr_i, \Tilde{\vr}^e_i, #???
    &\Mean_{\veps^e_i}
    \Big[
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i)) \Big]\\
    &= \int_{\veps^e_i} \frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}} (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i) \\
    &= \int_{\veps^e_i} 
    \frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i)\\
    &= \int_{\veps^e_i} \I[\mJ_{\veps, \vr, i}]
    \frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i)\\
    &+ \int_{\veps^e_i} \I[\neg \mJ_{\veps, \vr, i}]
    \frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i) . \alignlable{eqn:two_terms}
\end{align*}
In what follows, we will control the two parts of \eqref{eqn:two_terms} separately. 


\paragraph{First part of \eqref{eqn:two_terms}.}
For the first part of \eqref{eqn:two_terms}, conditional on $\mJ_{\vr}$, we have 
\begin{align*}
    & \int_{\veps^e_i} \I[\mJ_{\veps, \vr, i}]
    \frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i)\\
    &\le 
    max \Big\{\I[\mJ_{\veps, \vr, i}]
        exp\Big(\frac{\norm{h_i(\veps^e_i)}^2- \norm{\veps^e_i}^2}{2\sigma^2}\Big)\Big\}
    \int_{\veps^e_i} \I[\mJ_{\veps, \vr, i}]
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i)\\
    &\le
    max \Big\{\I[\mJ_{\veps, \vr, i}]
        exp\Big(\frac{\norm{h_i(\veps^e_i)}^2- \norm{\veps^e_i}^2}{2\sigma^2}\Big)\Big\}
    \int_{\veps^e_i} 
    \frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
    (R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i)\\
    &=
    max \Big\{\I[\mJ_{\veps, \vr, i}]
        exp\Big(\frac{\norm{h_i(\veps^e_i)}^2- \norm{\veps^e_i}^2}{2\sigma^2}\Big)\Big\}
        BR_i(T-K; \Tilde{\vr}^*_i) \alignlable{eqn:first_part_full}, 
\end{align*}
where the second inequality follows from the fact that the integrand is non-negative. 
Recall that, without loss of generality, we have assumed $\Cov = \vI$. 
To control this term, we use the relationship \eqref{eqn:one2one} to yield
\begin{align*}
&max \Big\{\I[\mJ_{\veps, \vr, i}]
        exp\Big(\frac{\norm{h_i(\veps^e_i)}^2- \norm{\veps^e_i}^2}{2\sigma^2}\Big)\Big\}\\
&= max \Big\{\I[\mJ_{\veps, \vr, i}]
exp\Big(\frac{\norm{\veps^e_i + \sigma^2  (\vr^e_i - \vPhi_i\vthe)}^2- \norm{\veps^e_i}^2}{2\sigma^2})\Big\}\\
&= max \Big\{\I[\mJ_{\veps, \vr, i}]
exp\Big(
(\veps^e_i)^T (\vr^e_i - \vPhi_i\vthe)
+ \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
)\Big\}\\
% &\le
%  max \Big\{\I[\mJ_{\veps, \vr, i}]
% exp\Big(
% \norm{\veps^e_i} \norm{\vr^e_i - \vPhi_i\vthe}
% + \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
% )\Big\}\\
&\le 
exp\Big(
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
\sigma
\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}
+ \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
\Big),
\end{align*}
where the inequality is due to the definition of $\mJ_{\veps, \vr, i}$.

\paragraph{Second part of \eqref{eqn:two_terms}.}
For the second part of \eqref{eqn:two_terms}, we can bound it by 
\begin{align*}
&\int_{\veps^e_i} 
\I[\neg \mJ_{\veps, \vr, i}]
\frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
\frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i) \\
&\le \Mean \Big[
R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) , \neg \mJ_{\veps, \vr, i}
\Big] \times \prob[\neg \mJ_{\veps, \vr, i}] \alignlable{eqn:two_parts_of_part2}. 
\end{align*}

For the first term of \eqref{eqn:two_parts_of_part2}, 
we note the regret from $T - K$ interactions with task $i$ is always bounded by 
$(T-K) max(\vr_i)$, the expectation of which over the task distribution is bounded by $(T-K) C_2C_3$. 


For the second term of \eqref{eqn:two_parts_of_part2}, 
we recall the tail inequality of Gaussian distributions: 
for any random variable $z \sim \normal(0, \sigma^2)$, we have $\prob[|z| \ge c\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}] \le 2exp(-\norm{\vr^e_i - \vPhi_i\vthe}^2 c^2 log(NT)/\sigma^2)$, where $c$ is any constant. 
Notice that $(\vr^e_i - \vPhi_i\vthe)$ is independent with $\veps^e_{i}$, which implies that, for any fixed value of $\vr^e_i - \vPhi_i\vthe$, it holds that $(\vr^e_i - \vPhi_i\vthe)^T \veps^e_{i} \sim \normal\big(0, \sigma^2 \norm{\vr^e_i - \vPhi_i\vthe}^2 \big)$. 
Therefore, by setting $c = \sigma$, we have 
% we have $(\vr^e_i - \vPhi_i\vthe)^T \veps^e_{i} \sim \normal(0, \norm{\vr^e_i - \vPhi_i\vthe}^2)$, which implies 
\begin{align*}
\prob[\neg \mJ_{\veps, \vr, i}] 
&= \prob[|(\vr^e_i - \vPhi_i\vthe)^T \veps^e_{i}| \ge \sigma\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}] \\
&= \prob[|(\vr^e_i - \vPhi_i\vthe)^T \veps^e_{i}| \ge \sigma\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}|\vr^e_i - \vPhi_i\vthe] \\
&\le 2exp(-log(NT)) = \frac{2}{NT}
\end{align*}


% by similar arguments with the proof of Lemma \ref{lemma:concentration_sampled_theta} on the tail inequality for the Euclidean norm of a Gaussian random vector, 
% we can obtain that for any $\xi \in (0, 1)$, 
% \begin{align*}
%     \prob[\norm{\veps^e_i} > 4\sigma \sqrt{K} + 2\sigma \sqrt{-log \xi}] \le \xi. 
% \end{align*}
% By setting $4\sigma \sqrt{K} + 2\sigma \sqrt{-log \xi} = c_3$, which is equivalent to $\xi = exp\{-[(c_3 - 4\sigma \sqrt{K}) /  2\sigma]^2\}$, we get 
% \begin{align*}
%     \prob[\norm{\veps^e_i} > c_3] \le  exp\{-[(c_3 - 4\sigma \sqrt{K}) /  2\sigma]^2\}. 
% \end{align*}

Putting these two parts together, we obtain a bound for the second term of \eqref{eqn:two_terms} as 
\begin{align*}
&\int_{\veps^e_i} 
\I[\neg \mJ_{\veps, \vr, i}]
\frac{exp(- \norm{\veps^e_i}^2 / 2\sigma^2)}{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)} 
\frac{exp(- \norm{h_i(\veps^e_i)}^2 / 2\sigma^2)}{(2\pi \sigma^2)^{K / 2}}
(R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) d\veps^e_i) \\
&\le \frac{2C_2C_3}{N}
% &\le (T-K) C_2C_3 exp\{-[(c_3 - 4\sigma \sqrt{K}) /  2\sigma]^2\}
\alignlable{eqn:bound_part2}. 
\end{align*}


Finally, 
combining \eqref{eqn:first_part_full} and \eqref{eqn:bound_part2}, 
we can obtain 
\begin{equation}
    \begin{split}
    &\Mean_{\veps^e_i}  
    \Big[
    R^*_i(T-K) - R_i(T-K; \Tilde{\vr}^e_i) \Big]\\
    &\le     
        exp\big(
% c_3 \norm{\vr^e_i - \vPhi_i\vthe}
\sigma
\norm{\vr^e_i - \vPhi_i\vthe}\sqrt{2log(NT)}
+ \frac{\sigma^2}{2}\norm{ (\vr^e_i - \vPhi_i\vthe)}^2
\big)BR_i(T-K; \Tilde{\vr}^*_i)
+ \frac{2C_2C_3}{N}
        % + (T-K)C_2C_3  exp\{-(\frac{c_3 - 4\sigma \sqrt{K}}{ 2\sigma})^2\}
        % \Big]. 
    \end{split}
\end{equation}

\end{proof}


\input{regret_baselines}

\input{technical_lemmas}


==> computational_complexity.tex <==
\subsection{Computational complexity}\label{sec:Computational_complexity}
In this section, we analyze the computational complexity for {\name}. 
The specific complexity depends on: 
(i) the reward distribution, 
(ii) the hierarchical model one chooses, 
(iii) whether the vanilla version or some variant is used, 
and (iv) the order of interactions. 
Therefore, we will first present a general complexity bound and then discuss examples. 
For simplicity, we assume $T_1 = \dots = T_N = T$. 
Let $m(i,t)$ and $m'(i,t)$ be the number of data points for task $i$ alone and that for all tasks, until the $t$-th interaction with task $i$. 
The computation complexity is clearly dominated by one step: updating and sampling from the posterior. 
We denote its complexity at interaction $(i,t)$ by $c\big(m(i,t), m'(i,t)\big)$. 
Then, the total complexity is bounded by 
$O(\sum_{i=1}^N \sum_{t=1}^T c\big(m(i,t), m'(i,t)\big)$. 

For Gaussian bandits with LMM, 
recall that we can update $\vthe$ incrementally, and according to its posterior form \eqref{eqn:theta_posterior}, 
each time $O(d^3)$ flops are required to sample $\vthe$. 
Besides, $O(dK)$ flops are required to compute the prior mean, 
and $O(K^2)$ flops are required to compute the posterior of $\vr_i$. 
Therefore, with Algorithm 1, the total complexity is bounded by 
$O\big(NT(K^2 + d^3)\big)$. 
Under the sequential setting, with Algorithm 2, it can be reduced to 
$O\big(N(TK^2 + d^3)\big)$. 

For Bernoulli bandits with BBLM, suppose $M$ samples are taken in each round of MCMC sampling, and $c'\big(m(i,t), m'(i,t)\big)$ flops are needed to sample each, then under Algorithm \ref{alg:TS_faster_general} with $l = T$, we have that the total complexity is bounded by
$O(\sum_{t=1}^T Mc'\big(t, tN) + NTdK + NTK\big) = O(\sum_{t=1}^T Mc'\big(t, tN) + NTdK\big)$ under the concurrent setting, 
and $O\big(\sum_{i=1}^N Mc'\big(0, iT\big) + NdK + NTK\big) = 
O\big(\sum_{i=1}^N Mc'\big(0, iT\big) + NTK\big)$. 

% With the implementation in Appendix \ref{sec:appendix_implementation_gaussian}, 
% under the episodic setting, we have $m(i,t) = (t-1)$ and  $m'(i,t) = (i-1)*T + (t - 1)$, which together with our analysis in Appendix \ref{sec:appendix_implementation_gaussian}, imply that 
% $cost^1_{i,t} = O((n-1)T^3)$ and $cost^2_{i,t} = O(1)$. 
% Therefore, the total complexity is bounded by $O(n^2T^4)$. 
% Similarly, under the concurrent setting, we have 
% $cost^1_{i,t} = O(N(t-1)^3)$ and $cost^2_{i,t} = O(1)$, which 
% imply a total complexity bound $O(n^2T^4)$. 



\paragraph{Total amount of compute and the type of resources used.}
Our experiments are run on an c5d.24xlarge instance on the AWS EC2 platform, with 96 cores and 192GB RAM. 
It takes roughly 20 minutes to complete a setting in Figure \ref{fig:simu_Gaussian} and 3 hours for Figure \ref{fig:simu_Binary}. 

==> incremental_LMM.tex <==
\subsection{Incremental implementation for LMM}
\begin{align*}
    &\vthe | \mH \sim \mathcal{N}\Big(\Tilde{\Cov}(\vPhi^T \mV^{-1}\vR + \Cov_{\vthe}^{-1}\vmu_{\vthe}), \Tilde{\Cov}\Big),\\
    &\Tilde{\Cov} = (\vPhi^T \mV^{-1} \vPhi + \Cov_{\vthe})^{-1}, \mV = \sigma^2 \vI_n + \Cov_{\delta}
\end{align*}

% We can actually replace this paragraph with the formula about theta in the appendix. 
% Then it could be more consistent. And more efficient. More intuitions. 
% And save space
% No need about this computation trick (the same for Susan's)
% \begin{equation}
%     \vthe | \mH^e_{1:i} \sim \mathcal{N}\Big((\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\vPhi^T \mV^{-1}\vR, (\vPhi^T \mV^{-1} \vPhi + \vI)^{-1}\Big), \mV = \sigma^2 \vI + \Cov_{\delta}
% \end{equation}


% theta contain task i
% then again to task i? things will become weird

(iii) $\prob(\vthe | \mH)$ permits incremental computation, which follows from the relationship
\begin{align*}
&\prob(\vthe|\mH \cup \{(a, r, \vx_{i}, i)\}) \\
&\propto \prob(\vthe) \prob(\mH \cup \{(a, r, \vx_{i}, i)\}|\vthe) \\
&\propto \prob(\vthe) \int_{\vr^-_i} \prob(\vr^-_i|\vthe) \prob(\mH^-_i|\vr^-_i)  d\vr^-_i
\int_{\vr_i}  \prob(\vr_i|\vthe) \prob(\mH_i |\vr_i) \prob(\{(a, r, \vx_{i}, i)\}|\vr_i) d\vr \\
&\propto \prob(\vthe) \int_{\vr} \prob(\vr|\vthe) \prob(\mH|\vr)  d\vr
\frac{\int_{\vr_i}  \prob(\vr_i|\vthe) \prob(\mH_i |\vr_i) \prob(\{(a, r, \vx_{i}, i)\}|\vr_i) d\vr_i
}{\int_{\vr_i}  \prob(\vr_i|\vthe) \prob(\mH_i |\vr_i)  d\vr_i}\\
&\propto \prob(\vthe|\mH) 
\frac{\int_{\vr_i}  \prob(\vr_i|\vthe) \prob(\mH_i |\vr_i) \prob(\{(a, r, \vx_{i}, i)\}|\vr_i) d\vr_i
}{\int_{\vr_i}  \prob(\vr_i|\vthe) \prob(\mH_i |\vr_i)  d\vr_i}\\
&\propto \prob(\vthe|\mH) \prob(\{(a, r, \vx_{i}, i)\}|\vr_i) \\
&= \prob(\vthe) \prob(\mH^-_i|\vthe) \prob(\mH_i \cup \{(a, r, \vx_{i}, i)\}|\vthe) \\
&\propto \prob(\vthe|\mH) \prob(\{(a, r, \vx_{i}, i)\}|\vthe)
\end{align*}
, where $\{(a, r, \vx_{i}, i)\}$ contains some new tuples. 

% Q: if incremental, how to Sigma_delta?
% Q: inverse trick? or incremental?
% \begin{equation}
% \end{equation}
% \Cov_{\delta}: diagnoal
% incremental
% if every time, then the same; just 1. incremental 2. approximate


==> regret_baselines.tex <==

\subsection{Regrets of the baseline TS algorithms}
In this section, we first recap the baseline TS algorithms discussed in Section \ref{sec:Theory}, and then provide formal statements about their regret bounds. 
OSFA applies a single $TS\big( Q(\vr_i) \big)$ algorithm to all tasks, where $Q(\vr_i)$ is the marginal distribution of $\vr_i$, while individual-TS applies a separate $TS\big( Q(\vr_i) \big)$ algorithm to each tasks. 
For meta-TS, under the sequential setting, following \cite{kveton2021meta}, we apply $TS\big( \normal(\vmu_i,\Cov) \big)$ to the $i$-th task, where $\vmu_i$ is sampled from the posterior of $\Mean[\vr_i]$ based on accumulated data from the finished $i-1$ tasks. 
Finally, linear-TS assumes $\vr_i = \vPhi_{i}\vthe$, requires a prior over $\vthe$ and maintains a posterior over it. We have the following results. 

\begin{proposition}\label{prop:rate_OSFA_linear}
Under Assumptions $1 - 3$, 
when $K < min(N,T)$, 
the multi-task regrets of OSFA and linear-TS under the LMM over $N$ tasks with $T$ interactions per task are both bounded by $O\big(NT \big)$. 
\end{proposition}

\begin{proposition}\label{prop:rate_ind_meta}
Under Assumptions $1 - 3$, 
when $K < min(N,T)$, 
the multi-task regret of individual-TS and meta-TS under the LMM over $N$ tasks with $T$ interactions per task are both bounded by $O\big(N\sqrt{KT}\big)$. 
\end{proposition}



These two propositions can be proved as follows. 

\begin{proof}[Proof of Proposition \ref{prop:rate_OSFA_linear}]
According to Assumption \ref{asmp:linear_magnitute}, 
we note the regret from one interaction with task $i$ is always bounded by
$K max(\vr_i)$, the expectation of which over the task distribution is bounded by $C_2C_3$. 
Therefore, the total regrets over $N$ tasks with $T$ interactions per task are both bounded by $O\big(NT \big)$.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:rate_ind_meta}]
The Bayes regret for each task can be derived from the prior-independent regret bound for Gaussian bandits in the literature (e.g., \citep{bubeck2014prior}) as $O(\sqrt{(T-K)KlogT})$. 
Therefore, the regret accumulated over $N$ tasks can be bounded by $O(N\sqrt{(T-K)KlogT})$. 
% agrawal2013further
\end{proof}

We note that, similar with results in \cite{metapricing} and \cite{kveton2021meta}, it is non-trivial to obtain lower bounds on the multi-task regrets for these baseline TS algorithms, due to the lack of understanding of the behaviour of a TS algorithm with mis-specified priors. 
To our knowledge, the above bounds are the tightest in the existing literature. 
In contrast, with information-sharing and thanks to the prior alignment technique, MTTS can be shown to yield a lower regret in rate. 

% To provide more insights, we next show that, for OSFA and linear-TS, the proportion of tasks whose highest reward is significantly higher than the assumed highest reward is bounded from zero, due to model misspecification; while for meta-TS and individual-TS, the proportion of tasks whose true prior is significantly different from the assumed prior is bounded from zero, due to the fact that they fail to learn $\prob(\vr_i|\vx_i)$. 


% % \begin{proposition}\label{prop:proportion_OSFA_linear}
% % Under Assumptions $1 - 3$, 
% % when $K < min(N,T)$, 
% % the multi-task regrets of OSFA and linear-TS under the LMM over $N$ tasks with $T$ interactions per task are both bounded by $O\big(NT \big)$. 
% % \end{proposition}

% \begin{proposition}\label{prop:proportion_ind_meta}
% Suppose for task $i$, the prior for either meta-TS or individual-TS is $Q(\vr_i)$ with expectation $\Mean[Q(\vr_i)]$. 
% For any constant $c_7$, the event  $\Big\{ \norm{\Mean(\vr_i|\vx_i) - \Mean[Q(\vr_i)]} \ge c_7\Big\}$ holds with probability larger than XX. 
% % Under Assumptions $1 - 3$, 
% % when $K < min(N,T)$, 
% % the multi-task regret of individual-TS and meta-TS under the LMM over $N$ tasks with $T$ interactions per task are both bounded by $O\big(N\sqrt{KT}\big)$. 
% \end{proposition}
% \begin{proof}[Proof of Proposition \ref{prop:proportion_ind_meta}]
% Under Assumption \ref{asmp:cov_x}, $\sigma_{min}\big( \Mean(\vPhi_i^T\vPhi_i) \big) \ge Kc_1$. 
% Recall $\Mean(\vr_i|\vx_i) = \vPhi_i \vthe$
% \end{proof}


% ASMP: E(r_i) != E(r_i|), or equivalently, there is heterogeneity caused by the metadata!
% for individual, there is heterogeneity! 
% [in the main text!]

==> review_Hierachical.tex <==
\section{Review of Statistical Concepts}\label{sec:review-LMM}
% Mixed Effect Models
In this section, we first review several classic statistical concepts, including the hierarchical models, random effect model, fixed effect model, and mixed effect model. 
They are all general concepts in statistics and have been integrated with different models, and we may focus on their  most related forms for ease of exposition. 
See \cite{fitzmaurice2008primer,wu2009mixed} for more detailed discussions. 
Next, we discuss their connection with our model  and baselines mentioned in the main text. 

\subsection{Statistical concepts}\label{sec:review_stat_LMM}
Consider a supervised learning problem, where we have $N$ subjects. 
For each subject $i$, we have $M_i$ measurements, denoted as $\{Y_{i,t}\}_{t=1}^{M_i}$. 
% Assume the $i$th subject also has a feature vector $\vx_i$. 
In a classic example, each subject corresponds to a hospital and each measurement corresponds to the outcome of a patient treated in one of these hospitals. 


A random effect model assumes the data of subject $i$ is generated from some distributions $f_i(\cdot;\vthe_i)$ parameterized by $\vthe_i$, and these coefficients are sampled from an upper-level distribution as $\vthe_i \sim \mathcal{P}$. 
The coefficients and the corresponding distribution are hence  treated as random variables, which enables us to characterize the heterogeneity between subjects. 
Therefore, this class of models are referred to as random effect models. 

In contrast, in a fixed effect model, for each measurement $Y_{i,t}$, we additionally have some independent variables $X_{i,t}$, and they are related through a regression model $Y_{i,t} = f(X_{i,t}; \vthe) + \epsilon_{it}$, which is parameterized by an unknown parameter $\vthe$. Here, $\epsilon_{it}$ is the error term. 
The coefficient $\vthe$ is fixed across subjects, and hence this class of models are referred to as fixed effect models. 
It is mainly used to characterize the common structure across subjects. 

A mixed effect model is a combination of both: it includes both fixed effect terms and random effect terms. The random intercept model $Y_{i,j} = f(X_{i,j}; \vthe) + \delta_{i} + \epsilon_{it}$ with $\delta_{i} \sim \mathcal{P}$ and the random coefficient model $Y_{i,j} = f(X_{i,j}; \vthe + \vthe_i) + \epsilon_{i,t}$ with $\vthe_i \sim \mathcal{P}$ are two examples. 

Finally, these three models are all special case of the following  hierarchical model (a.k.a. multilevel models): 
\begin{align*}
    \vthe_i &\sim g(Z_i;\vthe),\\
    Y_{i,t} &\sim f(X_{i,t}, \vthe_i), 
\end{align*}
where $Z_i$ contains some (optional) static features for each task $i$, 
the first layer describes the relationship between subjects and the second layer describes the relationship between measurements for the same subject. 
% hospital

% $\{(X_{i,t}, Y_{i,t})\}_{j=1}^{M_i}$. 
\subsection{Relationship with bandits}
The aforementioned statistical concepts are typically introduced for supervised learning. 
We can naturally extend them to the decision-making setup, and connect them with the bandit problem.
We first recall the equivalent definition of the stochastic multi-armed bandit problem that, in the $t$th interaction with task $i$,  the rewards for all arms are  generated by $\mathbf{R}_{i,t} \sim \mathcal{N}(\vr_i, \sigma^2 \vI)$, and after taking an action $A_{i,t}$, the $A_{i,t}$-th entry of $\mathbf{R}_{i,t}$ will be observed as $R_{i,t}$. 



The meta bandit assumes that each task instance $
\vr_i$ is sampled from some task prior distribution $\mathcal{P}_{\vr}$, and then the rewards are generated from $\vr_i$. 
Therefore, at a high-level, the underlying model can be regarded as a random effect model. 
As a concrete example, we consider the Gaussian bandit case in \citet{kveton2021meta}. 
Let mean rewards of task $i$ be $\vr_i = (r_{i,1}, \dots, r_{i,K})^T$. 
At each time point $t$, the rewards are  generated by $\mathbf{R}_{i,t} \sim \mathcal{N}(\vr_i, \sigma^2 \vI)$. 
We assume the task instances are sampled by $\vr_i = \vthe_i \sim N(\vmu, \sigma^2_0 \vI)$.  
It is easy to see this model is a random effect model. 

For contextual MAB, 
the reward $R_{t}$ are often related with the context $S_{t}$ and the action $A_{t}$ by a  model $R_{t} \sim f(S_{t}, A_{t}; \vthe)  + \boldsymbol{\epsilon}_{i,t}$ parameterized by $\vthe$.
In our multi-task MAB setting, to adapt these algorithms, we can similarly assume $\mathbf{R}_{i, t} =  f(S_{i, t}; \vthe) + \boldsymbol{\epsilon}_{i,t}$, where $S_{i, t} \equiv X_i$ for all $t$. % , A_{i, t}
It is straightforward to check that these two models are both special cases of the fixed effect model. 

Finally, by setting $Z_i = \vx_i$, $\vthe_i = \vr_i$, $Y_{i,t} = R_{i,t}$ and $X_{i,t} = A_{i,t}$, it is easy to see our model \eqref{eqn:hierachical_model} is a hierarchical model, with the other two models as special cases. 
In particular, the LMM in Section \ref{sec:LMM} is  a mixed effect model. 
% Finally, as discussed, our model can be regarded as their combinations, and hence is

% The reward of arm for task $i$ $N(\vthe_i, \sigma)$. 
% $y_{it} = X_{it}\vthe + \epsilon_{it}$. 
% $S_{it}$ ignores the repeated measurement nature. 


% $N$ subjects and their coefficients are sampled according to $\vthe_i \sim \mathcal{P}$. 


==> technical_lemmas.tex <==
\subsection{Additional technical lemmas}
In this section, we collect several additional technical lemmas. 
% and prove them when necessary. 
We first recap a mathematical result: 
\begin{lemma}[Lemma 20 in \cite{metapricing}]\label{lemma:e_1_2a}
    For any number $a \in [0,1]$, it holds that $exp(a) \le 1 + 2a$. 
\end{lemma}


The following lemma will give a lower bound for the smallest eigenvalue of our design matrix. 
\begin{lemma}[Theorem 3.1 in \cite{tropp2011user}]\label{lemma:fisher_lower}
For a series of independent, positive semidefinite matrices $\{\vA_k\}$ with dimension $d$,  suppose $||\vA_k|| \le R$ almost surely, 
then for any $\delta \in [0,1)$, we have
\begin{align*}
    \prob \big[\sigma_{min} (\sum_k \vA_k) \le (1-\delta) \mu_{min} \big] \le d [\frac{e^{-\delta}}{(1-\delta)^{1-\delta}}]^{\mu_{min} / R}, 
\end{align*}
where $\mu_{min} = \sigma_{min} (\sum_k \Mean \vA_k)$.
\end{lemma}

The following lemma states a tail inequality for the $2$-norm of a Gaussian vector. 
\begin{lemma}[Based on Lemma A.4 in \cite{hsu2012tail}]\label{lemma:2_norm_Gaussian}
For a $d$-dimensional random vector $\vz \sim \normal(0, \vI)$ and any $\xi \in (0,1)$, we have 
\begin{align*}
    \prob[||\vz||^2 \le d + 2\sqrt{d (-log\xi)} + 2  (-log\xi)] \ge 1 - \xi, 
\end{align*}
which implies, for any matrix $\vA$ with appropriate dimensions, we have 
\begin{align*}
&\prob\Big[||\vA\vz|| \le ||\vA|| (\sqrt{d} + \sqrt{2  (-log\xi)}\Big]\\
&=\prob\Big[||\vA\vz|| \le ||\vA||(d + 2\sqrt{2}\sqrt{d (-log\xi)} + 2  (-log\xi))^{1/2}\Big]\\
&\ge    \prob\Big[||\vA\vz|| \le ||\vA||(d + 2\sqrt{d (-log\xi)} + 2  (-log\xi))^{1/2}\Big] 
\ge 1 - \xi. 
\end{align*}
Notice that $\vA \vz \sim \normal(0, \vA^T \vA)$. 
\end{lemma}

